Expressivity of Neural Networks via Chaotic Itineraries beyond Sharkovsky's Theorem

Given a target function $f$, how large must a neural network be in order to approximate $f$? Recent works examine this basic question on neural network \textit{expressivity} from the lens of dynamical systems and provide novel ``depth-vs-width'' tradeoffs for a large family of functions $f$. They suggest that such tradeoffs are governed by the existence of \textit{periodic} points or \emph{cycles} in $f$. Our work, by further deploying dynamical systems concepts, illuminates a more subtle connection between periodicity and expressivity: we prove that periodic points alone lead to suboptimal depth-width tradeoffs and we improve upon them by demonstrating that certain ``chaotic itineraries'' give stronger exponential tradeoffs, even in regimes where previous analyses only imply polynomial gaps. Contrary to prior works, our bounds are nearly-optimal, tighten as the period increases, and handle strong notions of inapproximability (e.g., constant $L_1$ error). More broadly, we identify a phase transition to the \textit{chaotic regime} that exactly coincides with an abrupt shift in other notions of function complexity, including VC-dimension and topological entropy.

==> Beyond Sharkovsky Paper/abstract.tex <==
\begin{abstract}
    

%Given a target function $f$, how large does a neural network have to be before it can output $f$ approximately? This basic question in neural networks expressivity was recently examined from the lens of dynamical systems leading to novel ``depth vs width'' tradeoffs for a large family of functions $f$. %characterized by an oscillatory behavior.
%A key notion that was shown to govern such tradeoffs was the existence of higher-order fixed points in $f$'s trajectories (called \textit{periodic} points). In this paper, we further deploy dynamical systems ideas in the context of neural networks, proving that periodic points alone lead to far looser bounds on the depth-width tradeoffs; we improve upon them by analyzing stable and super-stable trajectories of $f$, demonstrating that certain ``chaotic itineraries'' can give stronger exponential tradeoffs, even in regimes where previous analyses would only imply polynomial gaps. Furthermore, our bounds are nearly-optimal and, contrary to prior works, they become tighter as the period increases, leading to a more refined understanding for why certain functions $f$ are hard-to-represent with low-depth networks. %As a byproduct, should we include RNN VC sentence?

Given a target function $f$, how large must a neural network be in order to approximate $f$?\\ 
Recent works examine this basic question on neural network \textit{expressivity} from the lens of dynamical systems and provide novel ``depth-vs-width'' tradeoffs for a large family of functions $f$. 
They suggest that such tradeoffs are governed by the existence of  \textit{periodic} points or \emph{cycles} in $f$. 
Our work, by further deploying dynamical systems concepts, illuminates a more subtle connection between periodicity and expressivity: we prove that periodic points alone lead to suboptimal depth-width tradeoffs and we improve upon them by demonstrating that certain ``chaotic itineraries'' give stronger exponential tradeoffs, even in regimes where previous analyses only imply polynomial gaps. 
Contrary to prior works, our bounds are nearly-optimal, tighten as the period increases, and handle strong notions of inapproximability (e.g., constant $L_1$ error). 
More broadly, we identify a phase transition to the \textit{chaotic regime} that exactly coincides with an abrupt shift in other notions of function complexity, including VC-dimension and topological entropy. 

%Finally, we develop strong relationships between periodicity in discrete dynamical systems and other notions of function complexity, 



%further dynamical systems ideas, stable and super-stable cycles analyzing specific chaotic itineraries that give sharper bounds on tradeoffs whereas just relying on periods we would get far looser bounds.



%byproduct VC dimension bounds based on our construction for iterated maps akin to recurrent neural networks.

%Whether a neural network will succeed or fail in representing (or even approximating) a given target function $f$ in its output depends on its depth and width. However, 

%Recent works have established such depth-width tradeoffs by relying on the oscillatory behavior of

%functions as depth-width property
%recent works
%dynamical systems deeper, twist
%1 technical sentence: stronger bounds, L1?, tradeoffs, existence of chaotic itineraries can lead to many more oscillations than what we would expect from Sharkovsky's theorem. 
%overall message
%  \todo{abstract here!}
  \end{abstract}


==> Beyond Sharkovsky Paper/abstract_arxiv.tex <==
Given a target function $f$, how large must a neural network be in order to approximate $f$?
Recent works examine this basic question on neural network \textit{expressivity} from the lens of dynamical systems and provide novel ``depth-vs-width'' tradeoffs for a large family of functions $f$. 
They suggest that such tradeoffs are governed by the existence of  \textit{periodic} points or \emph{cycles} in $f$. 
Our work, by further deploying dynamical systems concepts, illuminates a more subtle connection between periodicity and expressivity: we prove that periodic points alone lead to suboptimal depth-width tradeoffs and we improve upon them by demonstrating that certain ``chaotic itineraries'' give stronger exponential tradeoffs, even in regimes where previous analyses only imply polynomial gaps. 
Contrary to prior works, our bounds are nearly-optimal, tighten as the period increases, and handle strong notions of inapproximability (e.g., constant $L_1$ error). 
More broadly, we identify a phase transition to the \textit{chaotic regime} that exactly coincides with an abrupt shift in other notions of function complexity, including VC-dimension and topological entropy. 


==> Beyond Sharkovsky Paper/discussion.tex <==
\section{Conclusion}

%In the relatively young field of deep learning theory, researchers ask about the representational power of hierarchical networks, the behavior of iterates of the network parameters across steps of gradient descent, and how each layer of computation transfers the inputs that are passed into it.
%The much older field of dynamical systems offers a vast array of tools that machine learning researchers can draw on to formally pose and answer those questions.
In this work, we build new connections between deep learning theory and dynamical systems by applying results from discrete-time dynamical systems %that are well-known to applied mathematicians and foreign to most computer scientists
to obtain novel depth-width tradeoffs for the expressivity of neural networks. While prior works relied on Sharkovsky's theorem and periodicity to provide families of functions that are hard-to-approximate with shallow neural networks, we go beyond periodicity. Studying the chaotic itineraries of unimodal mappings, we reveal subtle connections between expressivity and different types of periods, and we use them to shed new light on the benefits of depth in the form of enhanced width lower bounds and stronger approximation errors. More broadly, we believe that it is an exciting direction for future research to exploit similar tools and concepts from the literature of dynamical systems in order to improve our understanding of neural networks, e.g., their dynamics, optimization and robustness properties.
%We believe that ideas about periodicity and chaos can be exploited broadly to improve our understanding of neural network dynamics and robustness, particularly those of recurrent neural networks.

%One of the limitations of our work is that we restrict ourselves to one-dimensional functions $f:[0,1] \to [0,1]$.
%The functions given here represent a broad array of ``hard'' functions that exhibit depth separation, but we believe that this work can be expanded by drawing from multi-dimensional discrete-time dynamical systems and incorporating other notions of function complexity.
%Notably, Sharkovsky's Theorem does not apply in two dimensions, so new tools must be found.\footnote{Consider the 2-dimensional mapping that rotates input $(x,y)$ by $120^\circ$. Any point will be a 3-cycle, but there is no 2-cycle.}
%However, given the depth and maturity of the field of dynamical systems, collaborations between ML and dynamical systems researchers are likely to yield these kinds of meaningful explanatory results about the powers and limitations of neural networks.

% \vaggos{say given the vast literature on dynamical systems there are many opportunities to use results from there. here we used discrete time dynamical systems and illuminate aspects for expressviity. we believe ideas developed here and chaos could be futher expoited for ROBUSTNESS etc....}

% \todo{tie-ins to RNNs}

% \todo{Connections to other recent papers about dynamical systems + ML\dots maybe some of them rely on Sharkovsky and have their results upgraded by looking instead at itineraries.}

%This paper improves the depth separation result of ReLU networks by connecting it to dynamical systems. It proves L1 error lower bound, extending previous classification error. 

%SEE ICML REVIEWS to get ideas for what to add how to phrase, what reviewers liked/didn/t like

==> Beyond Sharkovsky Paper/fig/fig-inc-cycle.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.45,xscale=0.45]
%uncomment if require: \path (0,768); %set diagram left start at 0, and has height of 768

%Straight Lines [id:da7068360793733492] 
\draw    (5.5,6.15) -- (5.5,603.61) ;
%Straight Lines [id:da5955719608763306] 
\draw    (654.5,603.61) -- (5.5,603.61) ;
%Curve Lines [id:da7052458170104179] 
\draw    (5.5,603.61) .. controls (422.51,-142.86) and (288.85,-125.93) .. (654.5,603.61) ;
%Flowchart: Connector [id:dp8705225816068709] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (342.84,52.66) .. controls (342.84,49.76) and (345.19,47.41) .. (348.09,47.41) .. controls (350.99,47.41) and (353.35,49.76) .. (353.35,52.66) .. controls (353.35,55.56) and (350.99,57.91) .. (348.09,57.91) .. controls (345.19,57.91) and (342.84,55.56) .. (342.84,52.66) -- cycle ;
%Straight Lines [id:da014058459506996357] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (346.34,55.58) -- (346.34,641.67) ;
%Flowchart: Connector [id:dp3874765474416759] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (576.88,454.78) .. controls (576.88,451.88) and (579.23,449.53) .. (582.13,449.53) .. controls (585.03,449.53) and (587.38,451.88) .. (587.38,454.78) .. controls (587.38,457.68) and (585.03,460.03) .. (582.13,460.03) .. controls (579.23,460.03) and (576.88,457.68) .. (576.88,454.78) -- cycle ;
%Straight Lines [id:da9114570296079929] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (582.13,460.03) -- (582.13,644.33) ;
%Curve Lines [id:da3619380243286747] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (253.54,149.54) .. controls (227.96,103.55) and (298.93,26.42) .. (345.96,51.44) ;
\draw [shift={(348.09,52.66)}, rotate = 211.32999999999998] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Connector [id:dp787327848414886] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (95.96,427.93) .. controls (95.96,425.03) and (98.31,422.68) .. (101.22,422.68) .. controls (104.12,422.68) and (106.47,425.03) .. (106.47,427.93) .. controls (106.47,430.84) and (104.12,433.19) .. (101.22,433.19) .. controls (98.31,433.19) and (95.96,430.84) .. (95.96,427.93) -- cycle ;
%Flowchart: Connector [id:dp10419292688954829] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (163.08,307.12) .. controls (163.08,304.22) and (165.43,301.87) .. (168.33,301.87) .. controls (171.23,301.87) and (173.59,304.22) .. (173.59,307.12) .. controls (173.59,310.02) and (171.23,312.37) .. (168.33,312.37) .. controls (165.43,312.37) and (163.08,310.02) .. (163.08,307.12) -- cycle ;
%Flowchart: Connector [id:dp16431490361405476] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (248.29,149.54) .. controls (248.29,146.64) and (250.64,144.29) .. (253.54,144.29) .. controls (256.45,144.29) and (258.8,146.64) .. (258.8,149.54) .. controls (258.8,152.44) and (256.45,154.79) .. (253.54,154.79) .. controls (250.64,154.79) and (248.29,152.44) .. (248.29,149.54) -- cycle ;
%Curve Lines [id:da3375031153111605] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (176.8,174.05) .. controls (180.82,164.28) and (205.8,122.23) .. (251.44,148.3) ;
\draw [shift={(253.54,149.54)}, rotate = 211.32999999999998] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da9324991459421863] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (168.33,307.12) .. controls (144.57,264.4) and (146.95,252.46) .. (151.55,243.14) ;
\draw [shift={(152.87,240.59)}, rotate = 477.9] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da733784180138128] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (101.22,427.93) .. controls (75.63,381.94) and (119.98,281.59) .. (166.22,305.92) ;
\draw [shift={(168.33,307.12)}, rotate = 211.32999999999998] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da12857623974330568] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (582.13,454.78) .. controls (531.32,509.95) and (132.37,531.6) .. (101.65,434.66) ;
\draw [shift={(101.22,433.19)}, rotate = 434.62] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da9212294086581905] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (100.71,425.93) -- (100.71,641.49) ;
%Straight Lines [id:da20223836106782112] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (168.33,307.12) -- (168.33,644.33) ;
%Straight Lines [id:da08019451344453787] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (252.38,149.54) -- (252.38,635) ;
%Flowchart: Connector [id:dp9431194313028666] 
\draw  [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] (617.15,534.74) .. controls (617.15,531.84) and (619.5,529.49) .. (622.4,529.49) .. controls (625.3,529.49) and (627.65,531.84) .. (627.65,534.74) .. controls (627.65,537.64) and (625.3,539.99) .. (622.4,539.99) .. controls (619.5,539.99) and (617.15,537.64) .. (617.15,534.74) -- cycle ;
%Straight Lines [id:da7987313429474685] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (622.98,537.66) -- (622.98,615.86) ;
%Curve Lines [id:da972320310686027] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ]   (348.09,52.66) .. controls (372.31,41.7) and (399.49,46.98) .. (427.24,63.64) .. controls (549.65,137.14) and (683.2,432.24) .. (623.32,533.23) ;
\draw [shift={(622.4,534.74)}, rotate = 301.98] [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Connector [id:dp067049996802649] 
\draw  [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] (63.86,486.88) .. controls (63.86,483.98) and (66.22,481.63) .. (69.12,481.63) .. controls (72.02,481.63) and (74.37,483.98) .. (74.37,486.88) .. controls (74.37,489.78) and (72.02,492.13) .. (69.12,492.13) .. controls (66.22,492.13) and (63.86,489.78) .. (63.86,486.88) -- cycle ;
%Straight Lines [id:da7368094553666249] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (69.7,489.8) -- (69.7,615.86) ;
%Flowchart: Connector [id:dp0364980716482306] 
\draw  [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] (128.65,368.4) .. controls (128.65,365.5) and (131,363.15) .. (133.9,363.15) .. controls (136.8,363.15) and (139.15,365.5) .. (139.15,368.4) .. controls (139.15,371.3) and (136.8,373.66) .. (133.9,373.66) .. controls (131,373.66) and (128.65,371.3) .. (128.65,368.4) -- cycle ;
%Straight Lines [id:da7147144830085386] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (133.9,368.4) -- (133.9,612.36) ;
%Flowchart: Connector [id:dp7596416045501773] 
\draw  [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] (291.48,85.93) .. controls (291.48,83.02) and (293.83,80.67) .. (296.73,80.67) .. controls (299.63,80.67) and (301.99,83.02) .. (301.99,85.93) .. controls (301.99,88.83) and (299.63,91.18) .. (296.73,91.18) .. controls (293.83,91.18) and (291.48,88.83) .. (291.48,85.93) -- cycle ;
%Straight Lines [id:da33994868835788283] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (296.73,85.93) -- (296.73,613.53) ;
%Curve Lines [id:da9876228817758563] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ]   (69.12,486.88) .. controls (19.71,446.44) and (61.55,366.52) .. (131.76,368.32) ;
\draw [shift={(133.9,368.4)}, rotate = 182.8] [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da09207233559028638] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ]   (131.56,366.07) .. controls (83.41,326.64) and (101.83,307.33) .. (115.77,287.14) ;
\draw [shift={(117.27,284.94)}, rotate = 483.69] [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da8511879364933572] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ]   (205.39,113.36) .. controls (206.54,103.63) and (253.08,90.55) .. (294.22,86.18) ;
\draw [shift={(296.73,85.93)}, rotate = 534.4100000000001] [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Connector [id:dp9202388124909902] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (597.89,494.47) .. controls (597.89,491.57) and (600.24,489.22) .. (603.14,489.22) .. controls (606.04,489.22) and (608.39,491.57) .. (608.39,494.47) .. controls (608.39,497.37) and (606.04,499.72) .. (603.14,499.72) .. controls (600.24,499.72) and (597.89,497.37) .. (597.89,494.47) -- cycle ;
%Straight Lines [id:da8100122274839643] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (603.14,499.72) -- (603.14,679.67) ;
%Flowchart: Connector [id:dp15826562494021634] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (81.96,459.45) .. controls (81.96,456.55) and (84.31,454.2) .. (87.21,454.2) .. controls (90.11,454.2) and (92.46,456.55) .. (92.46,459.45) .. controls (92.46,462.35) and (90.11,464.7) .. (87.21,464.7) .. controls (84.31,464.7) and (81.96,462.35) .. (81.96,459.45) -- cycle ;
%Straight Lines [id:da7703807186042282] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (88.44,460.7) -- (88.44,673.39) ;
%Curve Lines [id:da5096104847972356] 
\draw [color={rgb, 255:red, 114; green, 41; blue, 50 }  ,draw opacity=1 ]   (622.4,534.74) .. controls (564.04,621.85) and (124.61,592.81) .. (69.91,488.46) ;
\draw [shift={(69.12,486.88)}, rotate = 424.2] [fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da322303906191441] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (603.14,494.47) .. controls (544.78,581.58) and (142.33,565.25) .. (88,461.03) ;
\draw [shift={(87.21,459.45)}, rotate = 424.2] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Connector [id:dp04091200685998908] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (143.82,344.47) .. controls (143.82,341.57) and (146.17,339.22) .. (149.07,339.22) .. controls (151.97,339.22) and (154.33,341.57) .. (154.33,344.47) .. controls (154.33,347.38) and (151.97,349.73) .. (149.07,349.73) .. controls (146.17,349.73) and (143.82,347.38) .. (143.82,344.47) -- cycle ;
%Straight Lines [id:da04544020465093945] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (149.07,349.73) -- (149.07,673) ;
%Flowchart: Connector [id:dp914371670050395] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (224.36,188.17) .. controls (224.36,185.27) and (226.71,182.92) .. (229.62,182.92) .. controls (232.52,182.92) and (234.87,185.27) .. (234.87,188.17) .. controls (234.87,191.07) and (232.52,193.42) .. (229.62,193.42) .. controls (226.71,193.42) and (224.36,191.07) .. (224.36,188.17) -- cycle ;
%Straight Lines [id:da8380595860684885] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (229.62,193.42) -- (229.62,668.33) ;
%Flowchart: Connector [id:dp13104382005602555] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ] (315.41,62.11) .. controls (315.41,59.21) and (317.76,56.85) .. (320.66,56.85) .. controls (323.56,56.85) and (325.91,59.21) .. (325.91,62.11) .. controls (325.91,65.01) and (323.56,67.36) .. (320.66,67.36) .. controls (317.76,67.36) and (315.41,65.01) .. (315.41,62.11) -- cycle ;
%Straight Lines [id:da9155347081432625] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 114; green, 41; blue, 50 }  ,fill opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (320.46,67.36) -- (320.46,670.33) ;
%Curve Lines [id:da020204812654448068] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (84.58,457.7) .. controls (42.77,402.53) and (47.76,336.96) .. (147.56,344.36) ;
\draw [shift={(149.07,344.47)}, rotate = 184.61] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da6610310190419921] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (143.82,344.47) .. controls (117.93,308.63) and (119.5,299.41) .. (130.42,267.59) ;
\draw [shift={(131.27,265.1)}, rotate = 469.03] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da9699048107865567] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (161.04,218.41) .. controls (178.11,199.06) and (190.74,184.71) .. (226.8,187.89) ;
\draw [shift={(229.62,188.17)}, rotate = 186.26] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7645450980218567] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (229.62,188.17) .. controls (187.8,133) and (216.49,53.46) .. (316.52,60.71) ;
\draw [shift={(318.04,60.83)}, rotate = 184.61] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da23826649934354505] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (320.66,62.11) .. controls (403.25,-86.25) and (648.37,213.74) .. (603.14,494.47) ;
\draw [shift={(603.14,494.47)}, rotate = 279.15] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (332.01,642.19) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$1/2\ $};
% Text Node
\draw (575.21,644.1) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$x''$};
% Text Node
\draw (90.35,642.72) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$f( x'')$};
% Text Node
\draw (153.09,642.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$f^{2}( x'')$};
% Text Node
\draw (228.21,638.43) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$f^{p-2}( x'')$};
% Text Node
\draw (615.9,617.85) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 114; green, 41; blue, 50 }  ,opacity=1 ]  {$x'$};
% Text Node
\draw (53.45,613.18) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 114; green, 41; blue, 50 }  ,opacity=1 ]  {$f( x')$};
% Text Node
\draw (125.74,613.85) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 114; green, 41; blue, 50 }  ,opacity=1 ]  {$f^{2}( x')$};
% Text Node
\draw (285.41,615.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 114; green, 41; blue, 50 }  ,opacity=1 ]  {$f^{p-1}( x')$};
% Text Node
\draw (595.39,675.53) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$x^{*}$};
% Text Node
\draw (66.55,674.78) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$f\left( x^{*}\right)$};
% Text Node
\draw (127.91,675) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$f^{2}\left( x^{*}\right)$};
% Text Node
\draw (206.62,674.69) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$f^{p-2}\left( x^{*}\right)$};
% Text Node
\draw (298.79,673.93) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$f^{p-1}\left( x^{*}\right)$};
% Text Node
\draw (646.72,606.4) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x$};
% Text Node
\draw (41,34.4) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$f( x)$};


\end{tikzpicture}

==> Beyond Sharkovsky Paper/fig/fig-inc-intervals.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,337); %set diagram left start at 0, and has height of 337

%Straight Lines [id:da7068360793733492] 
\draw    (67.5,7.15) -- (67.5,265.14) ;
%Straight Lines [id:da5955719608763306] 
\draw    (347.74,265.14) -- (67.5,265.14) ;
%Curve Lines [id:da7052458170104179] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ]   (67.5,265.14) .. controls (247.57,-57.19) and (189.85,-49.89) .. (347.74,265.14) ;
%Flowchart: Connector [id:dp8705225816068709] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (213.17,27.23) .. controls (213.17,25.98) and (214.18,24.96) .. (215.43,24.96) .. controls (216.69,24.96) and (217.7,25.98) .. (217.7,27.23) .. controls (217.7,28.48) and (216.69,29.5) .. (215.43,29.5) .. controls (214.18,29.5) and (213.17,28.48) .. (213.17,27.23) -- cycle ;
%Flowchart: Connector [id:dp3874765474416759] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (332.13,236.97) .. controls (332.13,235.72) and (333.15,234.7) .. (334.4,234.7) .. controls (335.65,234.7) and (336.67,235.72) .. (336.67,236.97) .. controls (336.67,238.22) and (335.65,239.24) .. (334.4,239.24) .. controls (333.15,239.24) and (332.13,238.22) .. (332.13,236.97) -- cycle ;
%Straight Lines [id:da32414585374520755] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (215.11,26.52) -- (215.11,270.06) ;
%Straight Lines [id:da9982645121584954] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (334.4,236.97) -- (334.4,271.21) ;
%Flowchart: Connector [id:dp11337445005790259] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (100.53,201.56) .. controls (100.53,200.31) and (101.55,199.3) .. (102.8,199.3) .. controls (104.05,199.3) and (105.07,200.31) .. (105.07,201.56) .. controls (105.07,202.82) and (104.05,203.83) .. (102.8,203.83) .. controls (101.55,203.83) and (100.53,202.82) .. (100.53,201.56) -- cycle ;
%Straight Lines [id:da7803587502162856] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (102.8,201.56) -- (102.8,268.93) ;
%Straight Lines [id:da7071710334086063] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (121.8,165.29) -- (121.8,270.06) ;
%Flowchart: Connector [id:dp9130352141144631] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (119.53,165.29) .. controls (119.53,164.04) and (120.55,163.02) .. (121.8,163.02) .. controls (123.05,163.02) and (124.07,164.04) .. (124.07,165.29) .. controls (124.07,166.54) and (123.05,167.56) .. (121.8,167.56) .. controls (120.55,167.56) and (119.53,166.54) .. (119.53,165.29) -- cycle ;
%Flowchart: Connector [id:dp42374179605552276] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (135.65,135.35) .. controls (135.65,134.1) and (136.67,133.08) .. (137.92,133.08) .. controls (139.18,133.08) and (140.19,134.1) .. (140.19,135.35) .. controls (140.19,136.61) and (139.18,137.62) .. (137.92,137.62) .. controls (136.67,137.62) and (135.65,136.61) .. (135.65,135.35) -- cycle ;
%Flowchart: Connector [id:dp9656024065863953] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (171.06,71.73) .. controls (171.06,70.48) and (172.08,69.46) .. (173.33,69.46) .. controls (174.58,69.46) and (175.6,70.48) .. (175.6,71.73) .. controls (175.6,72.99) and (174.58,74) .. (173.33,74) .. controls (172.08,74) and (171.06,72.99) .. (171.06,71.73) -- cycle ;
%Straight Lines [id:da8538844459642152] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (137.92,135.35) -- (137.92,269.77) ;
%Straight Lines [id:da19740047838717412] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (173.33,71.73) -- (173.33,268.62) ;
%Curve Lines [id:da19712057513260794] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (121.8,163.02) .. controls (115.07,151.61) and (118.23,139.22) .. (132.74,135.88) ;
\draw [shift={(135.65,135.35)}, rotate = 532.35] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7096297633591004] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (102.8,201.56) .. controls (96.03,190.09) and (101.83,169.95) .. (116.82,165.84) ;
\draw [shift={(119.53,165.29)}, rotate = 532.35] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da45610957106349415] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (146.31,84.09) .. controls (148.47,78.41) and (155.44,74.51) .. (170.37,72.16) ;
\draw [shift={(173.33,71.73)}, rotate = 532.35] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da6739058041296793] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (137.92,135.35) .. controls (132.09,125.45) and (133.11,119.63) .. (135.25,115.63) ;
\draw [shift={(136.81,113.17)}, rotate = 485.54] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da6643359470366805] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (173.33,71.73) .. controls (163.03,56.08) and (187.91,10.64) .. (212.8,25.01) ;
\draw [shift={(215.11,26.52)}, rotate = 216.14] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da3500033372930782] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (215.43,27.23) .. controls (252.16,-9.39) and (370.75,177.03) .. (335.51,235.25) ;
\draw [shift={(334.4,236.97)}, rotate = 304.61] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da2586217224559795] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (334.4,236.97) .. controls (290.34,273.53) and (142.48,243.63) .. (104.46,203.41) ;
\draw [shift={(102.8,201.56)}, rotate = 409.49] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Brace [id:dp6748380319720335] 
\draw   (102.84,302.33) .. controls (102.84,304.9) and (104.12,306.18) .. (106.69,306.18) -- (106.69,306.18) .. controls (110.36,306.18) and (112.19,307.46) .. (112.19,310.03) .. controls (112.19,307.46) and (114.03,306.18) .. (117.7,306.18)(116.04,306.18) -- (117.7,306.18) .. controls (120.27,306.18) and (121.55,304.9) .. (121.55,302.33) ;
%Shape: Brace [id:dp9193244991486629] 
\draw   (121.84,302.9) .. controls (121.84,305.15) and (122.96,306.28) .. (125.21,306.28) -- (125.21,306.28) .. controls (128.43,306.28) and (130.04,307.41) .. (130.04,309.66) .. controls (130.04,307.41) and (131.65,306.28) .. (134.87,306.28)(133.42,306.28) -- (134.87,306.28) .. controls (137.12,306.28) and (138.24,305.15) .. (138.24,302.9) ;
%Shape: Brace [id:dp4188573395051751] 
\draw   (173.37,301.47) .. controls (173.37,306.14) and (175.7,308.47) .. (180.37,308.47) -- (184.67,308.47) .. controls (191.34,308.47) and (194.67,310.8) .. (194.67,315.47) .. controls (194.67,310.8) and (198,308.47) .. (204.67,308.47)(201.67,308.47) -- (208.97,308.47) .. controls (213.64,308.47) and (215.97,306.14) .. (215.97,301.47) ;
%Shape: Brace [id:dp9822509466026199] 
\draw   (216.55,301.18) .. controls (216.55,305.85) and (218.88,308.18) .. (223.55,308.18) -- (265.27,308.18) .. controls (271.94,308.18) and (275.27,310.51) .. (275.27,315.18) .. controls (275.27,310.51) and (278.6,308.18) .. (285.27,308.18)(282.27,308.18) -- (327,308.18) .. controls (331.67,308.18) and (334,305.85) .. (334,301.18) ;
%Shape: Ellipse [id:dp1754496405108379] 
\draw   (369.1,138.08) .. controls (369.1,131) and (374.84,125.27) .. (381.91,125.27) .. controls (388.99,125.27) and (394.72,131) .. (394.72,138.08) .. controls (394.72,145.15) and (388.99,150.89) .. (381.91,150.89) .. controls (374.84,150.89) and (369.1,145.15) .. (369.1,138.08) -- cycle ;
%Straight Lines [id:da7433685517183992] 
\draw    (394.72,138.08) -- (404.96,138.08) ;
\draw [shift={(407.96,138.08)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8687405359341835] 
\draw    (545.28,138.08) -- (556.1,138.08) ;
\draw [shift={(559.1,138.08)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da4670964616254172] 
\draw    (472.16,137.5) -- (482.26,137.5) ;
\draw [shift={(485.26,137.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da34462007636910985] 
\draw    (507.86,138.08) -- (517.09,138.08) ;
\draw [shift={(520.09,138.08)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da0057672384132689825] 
\draw    (573.06,151.18) .. controls (573.06,184.86) and (402.02,187.89) .. (383.06,153.6) ;
\draw [shift={(381.91,150.89)}, rotate = 433.18] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da8328222724858567] 
\draw    (573.06,151.18) .. controls (573.62,175.75) and (436.31,180.82) .. (421.76,153.52) ;
\draw [shift={(420.77,150.89)}, rotate = 437.12] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da2546474763984534] 
\draw    (573.06,151.18) .. controls (572.23,167.84) and (475.42,173.79) .. (460.63,152.71) ;
\draw [shift={(459.35,150.31)}, rotate = 429.52] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da27324303844843834] 
\draw    (573.06,151.18) .. controls (563.71,163) and (513.67,167.21) .. (499.91,153.02) ;
\draw [shift={(498.21,150.89)}, rotate = 417.46000000000004] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da06957144861741194] 
\draw    (573.06,151.18) .. controls (565.91,156.21) and (543.41,160.51) .. (534.47,153.1) ;
\draw [shift={(532.47,150.89)}, rotate = 416.31] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da0007563434331521179] 
\draw    (433.73,137.5) -- (443.54,137.5) ;
\draw [shift={(446.54,137.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Ellipse [id:dp6132232364297567] 
\draw   (407.96,138.08) .. controls (407.96,131) and (413.7,125.27) .. (420.77,125.27) .. controls (427.85,125.27) and (433.59,131) .. (433.59,138.08) .. controls (433.59,145.15) and (427.85,150.89) .. (420.77,150.89) .. controls (413.7,150.89) and (407.96,145.15) .. (407.96,138.08) -- cycle ;
%Shape: Ellipse [id:dp6025108421523422] 
\draw   (446.54,137.5) .. controls (446.54,130.43) and (452.27,124.69) .. (459.35,124.69) .. controls (466.42,124.69) and (472.16,130.43) .. (472.16,137.5) .. controls (472.16,144.58) and (466.42,150.31) .. (459.35,150.31) .. controls (452.27,150.31) and (446.54,144.58) .. (446.54,137.5) -- cycle ;
%Shape: Ellipse [id:dp8115642407167307] 
\draw   (519.66,138.08) .. controls (519.66,131) and (525.39,125.27) .. (532.47,125.27) .. controls (539.54,125.27) and (545.28,131) .. (545.28,138.08) .. controls (545.28,145.15) and (539.54,150.89) .. (532.47,150.89) .. controls (525.39,150.89) and (519.66,145.15) .. (519.66,138.08) -- cycle ;
%Shape: Ellipse [id:dp8997581185052426] 
\draw   (559.1,138.08) .. controls (559.1,131) and (564.83,125.27) .. (571.91,125.27) .. controls (578.98,125.27) and (584.72,131) .. (584.72,138.08) .. controls (584.72,145.15) and (578.98,150.89) .. (571.91,150.89) .. controls (564.83,150.89) and (559.1,145.15) .. (559.1,138.08) -- cycle ;
%Curve Lines [id:da7563362234499149] 
\draw    (581.7,129.59) .. controls (597.17,116.32) and (597.26,165.67) .. (582.79,150.28) ;
\draw [shift={(580.9,148.01)}, rotate = 413.25] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (340.98,262.02) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x$};
% Text Node
\draw (82.66,15.23) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$f( x)$};
% Text Node
\draw (200.98,272.57) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$x_{p-1}$};
% Text Node
\draw (325.87,272.28) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$x_{p}$};
% Text Node
\draw (94.27,271.63) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$x_{1}$};
% Text Node
\draw (112.98,271.91) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$x_{2}$};
% Text Node
\draw (129.39,272.49) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$x_{3}$};
% Text Node
\draw (161.39,272.78) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$x_{p-2}$};
% Text Node
\draw (102.61,312.39) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{1}$};
% Text Node
\draw (125.17,312.68) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{2}$};
% Text Node
\draw (182.52,313.82) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{p-2}$};
% Text Node
\draw (262.55,314.67) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{p-1}$};
% Text Node
\draw (375.17,132.32) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{1}$};
% Text Node
\draw (483.34,127.17) node [anchor=north west][inner sep=0.75pt]    {$\dotsc $};
% Text Node
\draw (414.46,132.32) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{2}$};
% Text Node
\draw (452.61,131.74) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{3}$};
% Text Node
\draw (523.28,131.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{p-2}$};
% Text Node
\draw (561.14,131.32) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$I_{p-1}$};


\end{tikzpicture}

==> Beyond Sharkovsky Paper/fig/fig-simple-fixed-point.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,238); %set diagram left start at 0, and has height of 238

%Straight Lines [id:da14021761165082447] 
\draw    (80.1,10) -- (80.1,155.3) ;
%Straight Lines [id:da5144503326290983] 
\draw    (386.59,155.3) -- (80.1,155.3) ;
%Straight Lines [id:da8555512162588199] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (147.77,93.52) -- (147.77,159.74) ;
%Shape: Brace [id:dp8448531191079238] 
\draw   (79.73,189.58) .. controls (79.73,194.25) and (82.06,196.58) .. (86.73,196.58) -- (103.33,196.58) .. controls (110,196.58) and (113.33,198.91) .. (113.33,203.58) .. controls (113.33,198.91) and (116.66,196.58) .. (123.33,196.58)(120.33,196.58) -- (139.92,196.58) .. controls (144.59,196.58) and (146.92,194.25) .. (146.92,189.58) ;
%Shape: Brace [id:dp0512529668630437] 
\draw   (147.17,190.21) .. controls (147.17,194.88) and (149.5,197.21) .. (154.17,197.21) -- (168.21,197.21) .. controls (174.88,197.21) and (178.21,199.54) .. (178.21,204.21) .. controls (178.21,199.54) and (181.54,197.21) .. (188.21,197.21)(185.21,197.21) -- (202.26,197.21) .. controls (206.93,197.21) and (209.26,194.88) .. (209.26,190.21) ;
%Shape: Ellipse [id:dp4642496548113897] 
\draw   (416.37,100.14) .. controls (416.37,92.4) and (422.65,86.13) .. (430.38,86.13) .. controls (438.12,86.13) and (444.39,92.4) .. (444.39,100.14) .. controls (444.39,107.87) and (438.12,114.15) .. (430.38,114.15) .. controls (422.65,114.15) and (416.37,107.87) .. (416.37,100.14) -- cycle ;
%Shape: Ellipse [id:dp41236657169946556] 
\draw   (458.88,100.14) .. controls (458.88,92.4) and (465.15,86.13) .. (472.89,86.13) .. controls (480.62,86.13) and (486.9,92.4) .. (486.9,100.14) .. controls (486.9,107.87) and (480.62,114.15) .. (472.89,114.15) .. controls (465.15,114.15) and (458.88,107.87) .. (458.88,100.14) -- cycle ;
%Shape: Ellipse [id:dp9802963778373845] 
\draw   (458.56,142.48) .. controls (458.56,134.74) and (464.83,128.47) .. (472.57,128.47) .. controls (480.31,128.47) and (486.58,134.74) .. (486.58,142.48) .. controls (486.58,150.22) and (480.31,156.49) .. (472.57,156.49) .. controls (464.83,156.49) and (458.56,150.22) .. (458.56,142.48) -- cycle ;
%Shape: Ellipse [id:dp6142958468523754] 
\draw   (415.9,142.48) .. controls (415.9,134.74) and (422.17,128.47) .. (429.91,128.47) .. controls (437.65,128.47) and (443.92,134.74) .. (443.92,142.48) .. controls (443.92,150.22) and (437.65,156.49) .. (429.91,156.49) .. controls (422.17,156.49) and (415.9,150.22) .. (415.9,142.48) -- cycle ;
%Shape: Ellipse [id:dp8207341400199923] 
\draw   (502.64,100.76) .. controls (502.64,93.03) and (508.91,86.75) .. (516.65,86.75) .. controls (524.39,86.75) and (530.66,93.03) .. (530.66,100.76) .. controls (530.66,108.5) and (524.39,114.78) .. (516.65,114.78) .. controls (508.91,114.78) and (502.64,108.5) .. (502.64,100.76) -- cycle ;
%Shape: Ellipse [id:dp42057095716500803] 
\draw   (502.64,143.11) .. controls (502.64,135.37) and (508.91,129.1) .. (516.65,129.1) .. controls (524.39,129.1) and (530.66,135.37) .. (530.66,143.11) .. controls (530.66,150.85) and (524.39,157.12) .. (516.65,157.12) .. controls (508.91,157.12) and (502.64,150.85) .. (502.64,143.11) -- cycle ;
%Straight Lines [id:da19972700290595147] 
\draw    (429.91,128.47) -- (429.91,117.15) ;
\draw [shift={(429.91,114.15)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da27175480154222953] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (80.1,155.3) -- (235,13) ;
%Curve Lines [id:da9195926618274903] 
\draw    (80.1,155.3) .. controls (149.28,122.9) and (156.36,66.7) .. (163.92,57.26) .. controls (171.48,47.81) and (216.34,29.39) .. (243.73,29.87) .. controls (271.12,30.34) and (300.4,45.45) .. (307.01,55.37) .. controls (313.63,65.29) and (317.88,123.37) .. (386.59,155.3) ;
%Flowchart: Connector [id:dp09307053659402897] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (145.29,93.52) .. controls (145.29,92.15) and (146.4,91.04) .. (147.77,91.04) .. controls (149.14,91.04) and (150.25,92.15) .. (150.25,93.52) .. controls (150.25,94.89) and (149.14,96) .. (147.77,96) .. controls (146.4,96) and (145.29,94.89) .. (145.29,93.52) -- cycle ;
%Flowchart: Connector [id:dp5263889732386211] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (207.37,36.62) .. controls (207.37,35.25) and (208.48,34.14) .. (209.85,34.14) .. controls (211.22,34.14) and (212.33,35.25) .. (212.33,36.62) .. controls (212.33,37.99) and (211.22,39.1) .. (209.85,39.1) .. controls (208.48,39.1) and (207.37,37.99) .. (207.37,36.62) -- cycle ;
%Straight Lines [id:da061507044563082314] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (209.85,36.62) -- (209.85,163.52) ;
%Straight Lines [id:da9148300551998201] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (243.73,29.87) -- (243.73,163.52) ;
%Straight Lines [id:da23253141529207633] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (275.96,36.15) -- (275.96,163.04) ;
%Straight Lines [id:da5163531059379349] 
\draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (322.5,95.41) -- (322.5,161.63) ;
%Shape: Brace [id:dp1749232641215519] 
\draw   (209.04,190.21) .. controls (209.04,194.84) and (211.36,197.16) .. (215.99,197.16) -- (215.99,197.16) .. controls (222.6,197.16) and (225.91,199.48) .. (225.91,204.11) .. controls (225.91,199.48) and (229.22,197.16) .. (235.84,197.16)(232.86,197.16) -- (235.84,197.16) .. controls (240.47,197.16) and (242.79,194.84) .. (242.79,190.21) ;
%Shape: Brace [id:dp8202624953612483] 
\draw   (243.51,190.21) .. controls (243.51,194.84) and (245.83,197.16) .. (250.46,197.16) -- (250.46,197.16) .. controls (257.08,197.16) and (260.39,199.48) .. (260.39,204.11) .. controls (260.39,199.48) and (263.7,197.16) .. (270.31,197.16)(267.33,197.16) -- (270.31,197.16) .. controls (274.94,197.16) and (277.26,194.84) .. (277.26,190.21) ;
%Shape: Brace [id:dp5584998733138133] 
\draw   (277.51,190.21) .. controls (277.51,194.88) and (279.84,197.21) .. (284.51,197.21) -- (290.53,197.21) .. controls (297.2,197.21) and (300.53,199.54) .. (300.53,204.21) .. controls (300.53,199.54) and (303.86,197.21) .. (310.53,197.21)(307.53,197.21) -- (316.54,197.21) .. controls (321.21,197.21) and (323.54,194.88) .. (323.54,190.21) ;
%Shape: Brace [id:dp32285617982822146] 
\draw   (323.89,190.06) .. controls (323.89,194.73) and (326.22,197.06) .. (330.89,197.06) -- (345.36,197.06) .. controls (352.03,197.06) and (355.36,199.39) .. (355.36,204.06) .. controls (355.36,199.39) and (358.69,197.06) .. (365.36,197.06)(362.36,197.06) -- (379.82,197.06) .. controls (384.49,197.06) and (386.82,194.73) .. (386.82,190.06) ;
%Straight Lines [id:da123366820748956] 
\draw    (472.89,128.47) -- (472.89,117.15) ;
\draw [shift={(472.89,114.15)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7339622353006783] 
\draw    (516.65,129.1) -- (516.65,117.78) ;
\draw [shift={(516.65,114.78)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da4373916001755509] 
\draw    (440.87,90.91) .. controls (454.61,60.22) and (411.03,60.19) .. (419.18,89.09) ;
\draw [shift={(420.09,91.86)}, rotate = 249.54000000000002] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da666736020225233] 
\draw    (526.35,89.97) .. controls (540.09,59.27) and (496.51,59.24) .. (504.66,88.15) ;
\draw [shift={(505.57,90.91)}, rotate = 249.54000000000002] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da42740492847580214] 
\draw    (482.9,90.44) .. controls (496.64,59.75) and (453.06,59.71) .. (461.21,88.62) ;
\draw [shift={(462.12,91.38)}, rotate = 249.54000000000002] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (379.22,154.08) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x$};
% Text Node
\draw (85.82,12.15) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$f( x)$};
% Text Node
\draw (139.53,155.53) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x_{1}$};
% Text Node
\draw (106.48,205.93) node [anchor=north west][inner sep=0.75pt]    {$I_{0}$};
% Text Node
\draw (171.25,205.83) node [anchor=north west][inner sep=0.75pt]    {$I_{1}$};
% Text Node
\draw (422.75,89.75) node [anchor=north west][inner sep=0.75pt]    {$I_{0}$};
% Text Node
\draw (465.25,89.75) node [anchor=north west][inner sep=0.75pt]    {$I_{1}$};
% Text Node
\draw (509.49,90.85) node [anchor=north west][inner sep=0.75pt]    {$I_{2}$};
% Text Node
\draw (201.4,156.95) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x_{2}$};
% Text Node
\draw (227.98,157.61) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$1/2$};
% Text Node
\draw (264.18,158.42) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$1-x_{2}$};
% Text Node
\draw (311.74,158.31) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$1-x_{1}$};
% Text Node
\draw (218.87,206.87) node [anchor=north west][inner sep=0.75pt]    {$I_{2}$};
% Text Node
\draw (252.97,205.93) node [anchor=north west][inner sep=0.75pt]    {$I_{2} '$};
% Text Node
\draw (292.17,205.46) node [anchor=north west][inner sep=0.75pt]    {$I_{1} '$};
% Text Node
\draw (345.53,206.4) node [anchor=north west][inner sep=0.75pt]    {$I_{0} '$};
% Text Node
\draw (420.01,132.72) node [anchor=north west][inner sep=0.75pt]    {$I_{0} '$};
% Text Node
\draw (462.52,132.72) node [anchor=north west][inner sep=0.75pt]    {$I_{1} '$};
% Text Node
\draw (506.75,133.83) node [anchor=north west][inner sep=0.75pt]    {$I_{2} '$};


\end{tikzpicture}

==> Beyond Sharkovsky Paper/intro.tex <==
\section{Introduction}

%depth inflation, architecture leads to expressivity, analogous to circuit for boolean functions
%simple XOR gate couldn't be represented and this was taken as evidence of weakness of neural networks leading the first AI winter.

%whether we want to deply a NN for image analysis or text or speech one of the first crucial decisions that will determine its success or failure is the architecture of the network

%bounded resources?
Whether a neural network (NN) succeeds or fails at a given task crucially depends on whether or not its architecture (depth, width, types of activation units etc.) is suitable for the task at hand. 
For example, a ``size-inflation'' phenomenon has occurred in recent years, in which NNs tend to be deeper and/or larger. 
Recall that in 2012, AlexNet had 8 layers.
In 2015, ResNet won the ImageNet competition with 152 layers~\citep{krizhevsky2012imagenet,he2016deep},
This trend still continues to date, with modern models using billions of parameters~\citep{brown2020language}. 
The empirical success of deep neural networks motivates researchers to ask: What are the theoretical benefits of depth, and what are the depth-vs-width tradeoffs?

This question gives rise to the study of neural network \textit{expressivity}, which characterizes the class of functions that are representable (or approximately representable) by a NN of certain depth, width, and activation. 
For instance, \cite{eldan2016COLT} propose a family of ``radial'' functions in $\mathbb{R}^d$ that are easily expressible with 3-layered feedforward neural nets of small width, but require any approximating 2-layer network to have exponentially (in $d$) many neurons. In other words, they formally show that depth---even if increased by 1---can be exponentially more valuable than width. 
%add Telgarsky, Schmitt here to illustrate and give a taste of the type of statements...some results: triagnle wave, polynomials. schmitt uses VC to give lower bounds for size of NN for polynomials of degree k, we deploy sharkovsky and get lower bounds for a wider array of periodic cycles...We illuminate the problem from different perspectives


Not surprisingly, understanding the expressivity of NNs was an early question asked in 1969, when Minsky and Papert showed that the Perceptron can only learn linearly separable data and fails on simple XOR functions~\citep{minsky2017perceptrons}. 
The natural question of which functions can multiple such Perceptrons (i.e., multilayer feedforward NN) express was addressed later by \cite{cybenko1989approximation,hornik1989multilayer} proving the so-called \textit{universal approximation} theorem. 
This states, roughly, that just one hidden layer of standard activation units (e.g., sigmoids, ReLUs etc.) suffices to approximate any continuous function arbitrarily well. 
Taken at face value, any continuous function is a 2-layer (i.e., 1-hidden-layer) network in disguise, and hence, there is no reason to consider deeper networks. 
However, the width required can grow arbitrarily, and many works in the following decades quantify those depth-vs-width tradeoffs.


%Numerous results in the literature have established variants of
%this universal approximation property by considering distinct function classes to be
%approximated by network archhitectures using different types of neural activation
%functions with respect to various approximation criteria, see for instance [1, 2, 3, 5,
%6, 11, 12, 14, 15]. (
%All these results and many others not referenced here, some of them being constructive, some being merely existence proofs, provide upper bounds for the network size
%asserting that good approximation is possible if there are sufficiently many network nodes available. This, however, is only a partial answer to the question that
%mainly arises in practical applications: "Given some function, how many network
%nodes are needed to approximate it?" Not much attention has been focused on
%establishing lower bounds on the network size and, in particular, for the approximation of functions over the reals. As far as the computation of binary-valued: GIVE CITATIONS FOR BOOLEAN FUNCTIONS AS WELL Koiran, Maass etc.....


Towards this direction, one typically identifies a function together with a ``measure of complexity'' to demonstrate benefits of depth. 
For example, the seminal work by \cite{telgarsky15,telgarsky16} relies on the number of oscillations of a simple triangular wave function. 
Other relevant notions of complexity to the expressivity of NNs include the VC dimension~\citep{warren1968lower,anthony1999neural,schmitt2000lower}, the number of linear regions~\citep{montufar2014number,arora2016understanding} or activation patterns~\citep{hanin2019deep}, the dimension of algebraic varieties~\citep{kileel2019expressive}, the Fourier spectrum~\citep{barron1993universal,eldan2016COLT,daniely2017depth,lee2017ability, bresler2020sharp}, fractals~\citep{malach2019deeper}, topological entropy~\citep{bzl20}, Lipschitzness~\citep{safran2019depth,hsu2021approximation}, global curvature and trajectory length~\citep{poole2016NIPS,raghu2017ICML} just to name a few. 



%should I put BZL here or above?
This work builds upon recent papers~\citep{cnpw19,cnp20}, which study expressivity from the lens of discrete-time dynamical systems and extend Telgarsky's results beyond triangle (tent) maps. 
At a high-level, their idea is the following: if the initial layers of a NN output a real-valued %\footnote{Lower bounds were proved for dimension 1. However similar statements hold in higher dimension.} 
function $f$, then concatenating the \textit{same} layers $k$ times one after the other outputs $ f^k  \vcentcolon = f\circ f\circ \ldots\circ f$, i.e., the composition of $f$ with itself $k$ times. 
By associating each discrete timestep $k$ to the output of the corresponding layer in the network, one can study expressivity via the underlying properties of $f$'s trajectories. 
Indeed, if $f$ contains higher-order fixed points, called \textit{periodic} points, then deeper NNs can efficiently approximate $f^k$, but shallower nets would require exponential width, governed by $f$'s periodicity.

Inspired by these novel connections to discrete dynamical systems, we pose the following natural question:
\begin{center}
\textit{Apart from periodicity, are there other properties of $f$'s trajectories governing the expressivity tradeoffs?}
\end{center}
%trajectory, periodicity, other properties, augment expressivity, tight bounds from periodicity, can we improve?

We indeed prove that $f$'s periodicity alone is not the end of the story, and we improve on the known depth-width tradeoffs from several perspectives. 
We exhibit functions of the same period with very different behaviors (see Sec.~\ref{ssec:warmup}) that can be distinguished by the concept of ``chaotic itineraries.'' 
We analyze these here in order to achieve nearly-optimal tradeoffs for NNs. 
Our work highlights why previous works that examine periodicity alone only obtain loose bounds. 
More specifically:
%SHOULD WE ADD BULLET POINTS? AND ROUGHLY STATE IN SIMPLE WORDS THE RESULTS?

\begin{itemize} 
\item We accurately quantify the oscillatory behavior of a large family of functions $f$. This leads to sharper and nearly-optimal lower bounds for the width of NNs that approximate $f^k$.
\item Our lower bounds cover a stronger notion of approximation error, i.e., \textit{constant} separations between NNs, instead of bounds that become small depending heavily on $f$ and its periodicity.
\item At a conceptual level, we introduce and study certain chaotic itineraries, which supersede Sharkovsky's theorem~(see Sec.~\ref{subsec:dds}). 
% Our contributions are powered by technical lower bounds on the eigenvalues of a discrete dynamical system arising from such itineraries and show how the resulting oscillations cannot shrink significantly.
\item We elucidate connections between periodicity and other function complexity measures like the VC-dimension and the topological entropy~\citep{alseda2000}. %, and the ease of neural network approximation.
We show that all of these measures undergo a phase transition that exactly coincides with the emergence of the chaotic regime based on periods.
\end{itemize}
%on a conceptual level: we identify that the itineraries are actually important and not only the length of the periodic cycles as prior works on the topic seems to suggest. this allows us to get more refined bounds.


To the best of our knowledge, we are the first to incorporate the notion of chaotic itineraries from discrete dynamical systems into the study of NN expressivity. Before stating and interpreting our results, we provide some basic definitions.


\subsection{Function Approximation and NNs}
%constant errors vs yx errors, L1 L\infty, classification, and history of increasingly better and better results in the litearture
This paper employs three notions of approximation to compare functions $f, g: [0,1] \to [0,1]$.
\begin{itemize}
    \item $L_1(f,g)= \norm[1]{f - g} = \int_{0}^1 \abs{f(x) - g(x)} dx.$
    \item $L_\infty(f,g)=\norm[\infty]{f - g} = \sup_{x \in [0, 1]} \abs{f(x) - g(x)}.$
    \item Classification error $\mathcal{R}_{S,t}$: For $t \in [0,1]$, let $\thres{t}{x} = \indicator{x \geq t}$. Let $S = \{x_1, \dots, x_n\} \subseteq [0,1]$. Then,
    $\errcls{S,t}{f,g}= \frac{1}{n} \sum_{i=1}^n \indicator{\thres{t}{f(x_i)} \neq \thres{t}{g(x_i)}}.$ 
\end{itemize}
For what follows, let $\mathcal{N}(u,\ell)$ be the family of feedforward NNs of depth $\ell$ and width at most $u$ per layer with ReLU activation functions.\footnote{Recall ReLU$(x)=\max(x,0)$.} All our results also hold for the more general family of semialgebraic activations~\citep{telgarsky16}.

%\clayton{Add a note that $L_1 > Cls, L_\infty$ in terms of LBs? I think it's ok to skip, since we will not only derive L_1 bounds. Maybe we can mention in the main body?}

%say about error f,g in classifictation: you choose y_i to be f(x_i) for example of g etc...  then say about comparing these types of errors... What is the best to approximate? and give historical progression with Schmitt

%ntioning that the telgarsky triangle has an increasing cycle of any length
% THIS MEANS WE IDENTIFY NOT ONLY PERIODS AS THE CULPRIT FOR NECESSITY OF DEPTH, BUT RATHER CHAOTIC ITINERARIES THAT GIVE MORE OSCILLATIONS AND SHARPER BOUNDS... so we still abstract away details from triangle wave, but give general certificates for functions that give us bounds...

%It is important to understand that when we prove lower bounds for the difference of two functions, then the most desirable result is to obtain an $L_1$ bound
%not sure if we should phrase classification error wrt to f,g not just f. but that's fine...

%, and in the context of depth-width tradeoffs, we have managed to obtain increasingly better and better separations.

 %and $\round(z) = \round_{1/2}(z)$.

%For some threshold $t \in [0,1]$, , and , we let the \textit{classification error} of $f$ be







\subsection{Discrete Dynamical Systems}
\label{subsec:dds}
%period, sharkovsky, hint that sharkovsky is not the whole story
%chaotic itinerary
To construct families of functions that yield depth-separation results, we rely on a standard notion of \textit{unimodal} functions from dynamical systems~\citep{mss73}.

\begin{definition}
     Let $f: [0,1]\to[0,1]$ be a continuous and piece-wise differentiable function. We say $f$ is a \emph{unimodal mapping} if:
    \begin{enumerate}
        \item $f(0) = f(1) = 0$, and $f(x) > 0$ for all $x \in (0,1)$.
        \item There exists a unique maximizer $x'\in (0,1)$ of $f$, i.e., $f$ is strictly increasing on the interval $[0, x')$ and strictly decreasing on $(x',1]$.
    \end{enumerate}
\end{definition}

Our constructions rely on unimodal functions that are concave and also symmetric (i.e., $f(x) = f(1-x)$ for all $x \in [0, 1]$). 
We note that the resulting function family is fairly general, already capturing the triangle waves of \cite{telgarsky15,telgarsky16} and the logistic map used in previous depth-separation results~\citep{schmitt2000lower}.
Moreover, the study of one-dimensional discrete dynamical systems by applied mathematicians explicitly identifies unimodal mappings as important objects of study~\citep{mss73, alseda2000}.

Recall that a fixed point $x^*$ of $f$ is a point where $f(x^*)=x^*$. A more general notion of higher-order fixed points is that of \textit{periodicity}.

% \begin{definition}
% Let $p\in \mathbb{N}$ with $p\ge1$. We say $f$ has \emph{periodicity} $p$ (or  has a point of period $p$), if there exists a point $x^* \in [0,1]$ such that:\footnote{Throughout the paper, $f^{p}$ means composition of $f$ with itself $p$ times.}
% $$
% 	f^{p}(x^*)=x^* {\text{ \ \ and\ \ \ }} f^{k}(x^*)\neq x^*, \ \forall k \in [p-1].
% $$
% The set $C \vcentcolon= \{x^*,f(x^*), f(f(x^*)),\dots, f^{p-1}(x^*)\}$ contains $p$ distinct elements and is called a \emph{$p$-cycle}. Fixed points correspond to $p=1$.
% %\clayton{Can we make $p$ a an ordered $p$-tuple rather than a set, since order matters? - I think for now this is simpler to grasp.}
 
% \end{definition}
\begin{definition}
For some $p \in \N$, we say that $x_1,\dots, x_p\in [0,1]$ is a \emph{$p$-cycle} if $f(x_j) = x_{j+1}$ for all $j \in [p-1]$ and $f(x_p) = x_1$.
We say that $f$ has \emph{periodicity} $p$ if such a cycle exists and that $x_1$ is a \emph{point of period $p$} if $x_1$ belongs to a $p$-cycle. 
Equivalently, $x_1$ is a point of period $p$ if $f^p(x_1) = x_1$ and $f^{k}(x_1) \neq x_1$\footnote{Throughout the paper, $f^{k}$ means composition of $f$ with itself $k$ times.} for all $k \in [p-1]$.\footnote{As is common, $[m] = \{1, 2, \dots, m\}$.}
\end{definition}

%chaos theory, period 3 implies chaos, 
Does the existence of some $p$-cycle in $f$ have any implications about the existence of other cycles?
% Are there constraints between the types of periods a mapping $f$ can possess? 
These relations between the periods of $f$ are of fundamental importance to the study of dynamical systems. 
In particular, \cite{li1975period} proved in 1975 that ``period 3 implies chaos'' in their celebrated work, which also introduced the term ``chaos'' to mathematics and later spurred the development of chaos theory. 
Interestingly, an even more general result was already obtained a decade earlier in Eastern Europe, by~\cite{sharkovsky1964coexistence,sharkovsky1965cycles}:


\begin{theorem}[Sharkovsky's Theorem]
\label{thm:sharkovsky}
Let $f: [0,1]\to[0,1]$ be continuous. If $f$ contains period $p$ and $p \triangleright p'$, then $f$ also contains period $p'$, where the symbol `` $\triangleright$'' is defined based on the following (decreasing) ordering: 
\[
3 \triangleright 5 \triangleright 7\triangleright \ldots \triangleright2\cdot3 \triangleright 2\cdot5 \triangleright 2\cdot7\triangleright\ldots
\]
\[
\ldots \triangleright 2^2\cdot3 \triangleright 2^2\cdot5 \triangleright 2^2\cdot7\triangleright\ldots\triangleright2^3\triangleright2^2\triangleright2\triangleright1.
\]
\end{theorem}

This ordering, called \textit{Sharkovsky's ordering}, is a total ordering on the natural numbers, where $l\triangleright r$ whenever $l$ is to the left of $r$. The maximum number in this ordering is 3; if $f$ contains period 3, then it also has all other periods, which is also known as \emph{Li-Yorke chaos}. 
\cite{cnpw19,cnp20} apply this theorem to obtain depth-width tradeoffs based on periods and obtain their most powerful results when $p = 3$. 
We go beyond Sharkovsky's theorem and prove that tradeoffs are determined by the ``itineraries'' of periods.\footnote{These are called ``patterns'' in~\cite{alseda2000}.}

%\begin{definition}[Chaotic Itineraries]
%    Let $C$ be some $p$-cycle $x_1, \dots, x_p$ of a unimodal $f$. 
%    The \emph{itinerary} of $C$ is a string $\textbf{a}=a_1a_2\ldots a_p \in \{L, C, R\}^p$ of length $p$, with:
%    \[a_i \vcentcolon = \begin{cases}
%        L & x_i < x_{\max} \\
%        C & x_i = x_{\max} \\
%        R & x_i > x_{\max}.
%    \end{cases}\]
%Furthermore, any itinerary consisting of $(p-1)$ consecutive $L$'s followed by a single $R$, i.e., $\textbf{a}= L^{p-1}R = LL\ldots LR$ is called a \emph{chaotic} itinerary.
%\end{definition}

\begin{definition}[Itineraries]
    For a $p$-cycle $x_1, \dots, x_p$, suppose that $x_{a_1} < \dots < x_{a_p}$ for $a_j \in [p]$.
    The \emph{itinerary} of the cycle is the cyclic permutation of $x_{a_1}, \dots, x_{a_p}$ induced by $f$, which we represent by the string $\ba= a_1\dots a_p$.
    Because cyclic permutations are invariant to rotation, we assume (wlog) that $a_1 = 1$.


    % The \textit{itinerary} of a $p$-cycle is a cyclic permutation of the $p$ sorted elements $x_1 < \dots < x_p$ that indicates in what order they are traversed.
    % We represent the permutation with a string $\ba=a_1a_2\ldots a_p \in [p]^p$ that encodes this ordering and implies that $f(x_{a_i}) = f(x_{a_{i+1}})$ for all $i \in [p-1]$ and $f(x_{a_p}) = f(x_{a_1})$.
    % Itineraries are invariant to rotation, so we can assume (wlog) $x_1$ to be the smallest element of $C$, i.e., $a_1 = 1$.
    
    % Let $C$ be a $p$-cycle $x_1, \dots, x_p$ of a mapping $f$. 
    % The \emph{itinerary} of $C$ is a string $\ba=a_1a_2\ldots a_p \in [p]^p$ of length $p$ representing a permutation of the points in $C$. That is, $a_ia_j$ is a substring of $\ba$ if $f(x_i) = x_j$. 
    % Itineraries are invariant to rotation, so we can assume (wlog) $x_1$ to be the smallest element of $C$, i.e., $a_1 = 1$.
\end{definition}  

\begin{definition} [Chaotic Itineraries]
%   Any itinerary whose cycle has $x_1 < x_2 < \dots < x_p$ is called a \emph{chaotic} itinerary and is identifiable by $12\dots p$. (Because of its form, it is often called an \emph{increasing} $p$-cycle as well.) 
    A $p$-cycle is a \emph{chaotic itinerary} or an \emph{increasing cycle} if its itinerary is $12\dots p$. That is, $x_1 < \dots < x_p$. 
\end{definition}
Examining chaotic itineraries circumvents the limitations of prior works based on periods and yields sharper exponential depth-width tradeoffs. 
Unlike other function complexity properties, the existence of a chaotic itinerary is easily verifiable (see App.~\ref{assec:identifying}).
To grasp clean examples of itineraries, see App.~\ref{assec:it-exs}.




%Observe that the number 3 is the largest according to this ordering. Sharkovsky showed a surprising and elegant result about his ordering: it describes which numbers can be periods for a
%continuous map on an interval; allowed periods must be a suffix of his ordering:


%According to Sharkovsky's Theorem, 3 is the maximum period, so one important and easy-to-remember corollary is that period 3 implies \textit{all} periods.\footnote{On a historical plot twist, this special case was proved a decade later by James Yorke and Tien-Yien Li, in their seminal paper called ``Period Three Implies Chaos''~\cite{li1975period}; this is a celebrated result that actually introduced the term ``chaos'' as used in Mathematics (chaos theory).}



% $x^*$ is a \textit{fixed point} if $f(x^*) = x^*$.
%    For any $p > 1$, $x^*$ is a \textit{$p$-cyclic} point if $f^p(x^*) = x^*$ and $f^q(x^*) \neq x^*$ for all $q < p$.
%    We say that $f$ has a \textit{$p$-cycle} if there exists $p$ points $x_1, \dots, x_p$ such that $f(x_i) = x_{i+1}$ for $i \in [p-1]$ and $f(x_p) = x_1$.


\subsection{Our Main Contributions}

Our principal goal is to use knowledge about $f$'s itineraries to more accurately quantify the ``oscillations'' of $f^k$ as a measure of complexity and draw connections to other complexity measures. 
Section~\ref{sec:lb} produces sharper and more robust NN approximability tradeoffs than prior works by leveraging chaotic itineraries and unimodality.
Section~\ref{sec:phase} shows how a phase transition in VC-dimension and topological entropy of $f$ occurs exactly when the growth rate of oscillations shifts from polynomial to exponential. 


While previous works count oscillations too, they either construct too narrow a range of functions\footnote{e.g.,~\cite{telgarsky15,telgarsky16} only analyzes triangles.}, obtain loose depth-width tradeoffs\footnote{e.g.,~\cite{cnpw19,cnp20} have a suboptimal dependence on $p$ under stringent Lipschitz assumptions.}, or have unsatisfactory approximation error. \footnote{e.g.,~\cite{cnpw19,cnp20,bzl20} do not obtain constant error rates.} 
In Section~\ref{sec:lb}, we improve along these three directions by taking advantage of the unimodality and itineraries of $f$. 
% Roughly speaking, we compose $k$ times a unimodal function $f$ with itself to obtain $f^k$. 
The \textit{unimodality} of $f$ allows us to quantify both the number of piecewise monotone pieces of $f^k$ (i.e., oscillations) and the corresponding height between the highest and lowest values of $f^k$'s oscillations. 
This improvement on the height enables stronger notions of function approximation (e.g., constant error rates with no dependence on $f$ or its period $p$). 
\textit{Chaotic itineraries} allow an improved analysis of the number of oscillations in $f^k$ and grant sharper exponential lower bounds on the width of any shallow net $g$ approximating $f^k$. 

We say that our results are \textit{nearly-optimal} because we exhibit a broad family of functions $f$ that are inapproximable by shallow networks of width $O(\rho^k)$ for $\rho$ arbitrarily close to 2.
Because no unimodal function $f$ can induce more than $2^k$ oscillations in $f^k$, we cannot aspire to tighter exponent bases in this setting.\footnote{Our results also transfer to non-unimodal functions via the observation that for bimodal $g$, there is some unimodal $f$ such that the number of oscillations of $g$ is at most twice those of $f$.}
On the other hand, none of the bounds from previous works (except the narrow bounds of Telgarsky) produce width bounds of more than $\Omega(\phi^k)$, where $\phi \approx 1.618$ is the Golden Ratio.
To demonstrate our sharper tradeoffs, we state a special case of our results for the $L_\infty$ error.

\begin{theorem}\label{thm:motivation-lb-inc} 
% Let $g\in \mathcal{N}(u,\ell)$. For $p\ge 3$, let $\rho$ be the largest root of the polynomial equation $\lambda^{p} - 2\lambda^{p-1} + 1 = 0$.\footnote{Notice that $\rho \geq \max({2 - \frac4{2^{p}},{\tfrac{1+\sqrt 5}{2}}})$~(see Fact~\ref{fact:root-lb}) and is much stronger than previous bounds~\citep{cnpw19,cnp20}.} Moreover, let $f$ be any symmetric, concave unimodal mapping with a increasing $p$-cycle. For all $k\in\N$, if $g$ has $L_\infty(f^k,g) \le \tfrac{1}{36}$, then it must have large width:\todo{swap polynomial with bound}
% \[
% u  > \frac{1}{8} \rho^{k/\ell}
% \]
For $p \geq 3$ and $k \in \N$, consider any symmetric, concave unimodal mapping $f$ with an increasing $p$-cycle and any $g \in \mathcal{N}(u, \ell)$ with width \[u \leq \frac18 \left(\max\paren{2-\frac4{2^p}, \phi}\right)^{k/\ell}\]
Then, $L_\infty(f^k, g) = \Omega(1)$, independent of $f,p,k$.
\end{theorem}  
%\clayton{How about we instead say ``there exists a $\rho \geq 2 - \frac4{2^{\rho}}$'' to avoid introducing the polynomial? I like this polynomial to be there just so that they wonder how did it appear ? :P}
    
\begin{remark} When $g$ is shallow with depth $\ell=O(k^{1-\eps})$ (e.g., $\ell=k^{0.99}$), then its width must be exponentially large in order to well-approximate $f^k$.
% This shows how depth can be exponentially more valuable than width. 
% Moreover, $\rho \geq \max({2 - \frac4{2^{p}},{\tfrac{1+\sqrt 5}{2}}})$~(see Fact~\ref{fact:root-lb}). 
This exponential separation is sharper than prior works~\citep{cnpw19,cnp20}, and quickly becomes even sharper (tending to 2) with larger values of $p$. 
This is counterintuitive as Sharkovsky's ordering implies that period 3 is the most chaotic and prior works recover a suboptimal rate of at most $\phi\approx 1.618$ (see Table~\ref{table:rho_inc}). 
% Since $\rho\le 2$ for unimodal $f$, our bound quickly converges to the optimal tradeoff (see Fig.~\ref{fig:toy-intro}). 
\end{remark}
\begin{remark}
Our approximation error is constant independent of all other parameters $f, k, p$. 
Previous results~\citep{cnpw19,cnp20,bzl20} obtain a gap that depends on $f,p$ and may be arbitrarily small.
Moreover, we have required nothing of the Lipschitz constant of $f$, unlike the strict assumptions on the Lipschitz constant $L$ of $f$ by~\cite{cnp20} (e.g., they require $L=\phi$ for period $p=3$).
Indeed, Propositions~\ref{prop:need-symmetry} and \ref{prop:need-concavity} in the Appendix~\ref{assec:sym-conc} illustrate how their lower bounds break down for large $L$ and how their $L_\infty$ bounds can shrink, becoming arbitrarily weak for certain 3-periodic $f$.
\end{remark}

We also present analogous results for the classification error and the $L_1$ errors. Please see the full statements in Theorems~\ref{thm:main-linf} and \ref{thm:main-l1}. Furthermore, Theorems~\ref{thm:odd-linf} and \ref{thm:odd-l1} offer an improvement on the results of \cite{cnp20} by giving constant-accuracy $L_\infty$ lower bounds without needing a chaotic itinerary.

In addition, Section~\ref{sec:phase} relates our chaotic itineraries to standard notions of function complexity like the VC dimension and the topological entropy (for precise definitions, see Sec.~\ref{sec:phase}). The types of periodic itineraries of $f$ give rise to two regimes: the \textit{doubling} regime and the \textit{chaotic} regime. In the former, we have a polynomial number of oscillations, while the latter is characterized by an exponential number of oscillations. Here we show the following correspondence:

\begin{theorem}[Informal]\label{thm:informal-phase}
The transition between these two regimes exactly coincides with a sharp transition in the VC-dimension of the iterated mappings $f^k$ for fixed $f$ (from bounded to infinite) and in the topological entropy (from zero to positive).
\end{theorem}


%challenge? technical side? more broadly VC...
\paragraph{Our Techniques} To quantify the oscillations of $f^k$, we use its chaotic itineraries to decompose the $[0,1]$ interval into several subintervals $\{I_j\}_{j=1}^{j=p-1}$. We count the number of times $f^k$ ``visits'' each $I_j$, by identifying a suitable matrix $A$ whose spectral radius is a lower bound on the growth rate of oscillations. The associated characteristic polynomial of $A$ is $\lambda^{p} - 2\lambda^{p-1} + 1$ and has larger spectral radius that that of prior works for \textit{all} periods. 
Moreover, the corresponding oscillations of at least one of the subintervals $I_j$ do not shrink in size, giving a bound on the total number of oscillations of a \textit{sufficient} size. 
This provides a lower bound on the height between the peak and the bottom of these oscillations that later provides \textit{constant} approximation errors for small shallow NNs.

More broadly, our work builds on the efforts to characterize large families of functions that give depth separations and addresses questions raised by~\cite{eldan2016COLT,telgarsky16,poole2016NIPS, malach2019deeper} about the properties of hard-to-represent functions. Similar to periods, the concept of chaotic itineraries can serve as a certificate of complexity, which is also easy to verify for unimodal $f$ (see Proposition~\ref{prop:half-inc-cycle} in Appendix).

%and relying on shallow nets few oscillations, 




%high-level: shallow nets few oscillations, deep nets large number of oscillations, following prior works we use oscillations as notion of complexity. We present refined bounds based on our unimodal funtions and f^k. This boosted oscillations numbers allow to get our improved bounds alongside the VC and topological entropy phase shift.



%on a technical level: eigenvalue analysis based on chaotic itineraries provide us with more oscillations. Furthermore, they provide us with constat-separated oscillations sth which was not known if it can be done before where the gap was shrinking based on y-x which we could not control. Now we change the quantifiers saying that for there is a gap such that for any period p .... whereas before they said for every period p function there is a constant that depends on f and p and y-x such that... this boosting on the number of oscillations allow us to get sharper tradeoffs that become sharper and sharper as p increases, sth that was not known before and are nearly optimal approaching the best 2^n dependence of unimodal functions.

%more broadly, we also provide evidence that the shift in regimes from doubling to chaotic coincides exactly with VC bounds change and also topological entropy of related function family based on iterated maps.

%say that throughout the paper we provide experiments or simulations to demonstrate our resutls.

%briefly we summarize our contributions bellow: give 3 bullet points: 1) sharkovsky and periods not the end of story. using chaotic itineraries we get boosted number of oscillations. 2) these translate to larger and constant gaps in errors, better dependence on p, more subtle connection with expressivity and depth-width tradeoffs. Informally, state two main theorems. 3) state informally results for VC and topological entropy.


%some of our results are incomparable to prior works: on the one hand, in ICML they have very stringent assumptions on the lipschitz constant in order to prove bounds which we destroy by the two counterexamples. On the other hand, we do require symmetry and concavity and altough natural these can't compare with the lipschitz assumption. We get stronger separations compared to ICLR, we completely generalize Telgarsky, and we get better bounds than Harvard paper.


\section{Warm-up Examples}\label{ssec:warmup}

This section presents illustrative examples and instantiates our results for some simple cases. 
These highlight the limitations of exclusively considering periodicity of cycles alone---and not itineraries---when developing accurate oscillation/crossing bounds~(see also Def.~\ref{def:osc},~\ref{def:cross}) and sharp expressivity tradeoffs.

%To demonstrate the strength of our bounds and the centrality of itineraries to the connections between dynamical systems and neural network expressivity, we consider a simple case where itineraries supersede periodicity in number of oscillations and hardness of approximation.

Consider the three unimodal mappings in Figure~\ref{fig:toy-ex-compare-map}, $f_{\ba}$ with itineraries $\ba \in \{1324, 1234, 123\}$. 
Observe that $f_{1234}$ has the cycle $(\frac{1}{5}, \frac{2}{5}, \frac{3}{5}, \frac{4}{5})$, $f_{1324}$ has $(\frac{1}{5}, \frac{3}{5}, \frac{2}{5}, \frac{4}{5})$, and $f_{123}$ has $(\frac{1}{4}, \frac{1}{2}, \frac{3}{4})$. Despite their similarities, they give rise to significantly different behaviours in $f_{\ba}^k$.

What do prior works based on NN approximation with respect to periods and Sharkovsky's theorem alone tell us?  
\cite{cnpw19,cnp20} show that the 3-cycle of $f_{123}$ ensures that $f^k$ has $\Omega(\phi^k)$ oscillations, where $\phi \approx 1.618$ is the golden ratio. However, their theorems do not imply anything for $f_{1324}$ and $f_{1234}$, since 4 is a power of 2, and they require odd periods.  
%One might expect a ``chaos hierarchy'' that ranks $f_{123}$ above $f_{1324}$ and %$f_{1234}$.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-compare_map.png}
    \caption{Plots of unimodal mappings with different itineraries $f_{1234}$, $f_{1324}$, and $f_{123}$. Despite their similarities, $f_{1234}$ leads to the most oscillations and sharpest depth-width tradeoffs (see Fig.~\ref{fig:toy-intro}).}
    \label{fig:toy-ex-compare-map}
\end{figure}
As it turns out, $f_{1234}$ leads to exponential oscillations and $f_{1324}$ leads only to polynomial oscillations:
\begin{itemize}
    \item A mapping with a 1324-itinerary is guaranteed no other cycles except the 2-cycle and a fixed point~\citep{mss73}. 
    Sharkovsky's theorem and \cite{cnpw19} predict this outcome, since 4 is the third-right-most element of the Sharkovsky ordering, and its existence alone promises nothing more.
    The ordering of itineraries introduced by~\citep{mss73} (see Table~\ref{table:itineraries} in Appendix) indicates that the particular 1324-itinerary only implies the periods 2 and 1, and confirms this intuition.
    % \vaggos{what is 12 itinerary?}
    We classify this itinerary as part of the \emph{doubling regime} and prove in Theorem~\ref{thm:properties-doubling} that any $f^k$ with a \textit{maximal} 1324-itinerary (that is, there is no 8-cycle) cannot exhibit sharp depth-width tradeoffs: for any $\eps>0$, there exists a 2-layer ReLU neural network $g$ of width $O(\frac{k^3}{\eps})$ such that 
    $L_\infty(f_{1324}^k, g) \leq \eps.$
    

    \item Going beyond Sharkovsky's theorem, a mapping with a 1234-itinerary---even though it is of period 4---it is guaranteed to contain a 3-cycle as well (see Table~\ref{table:itineraries} in Appendix). Hence, ``itinerary-1234 implies period-3, implies chaos,'' and $f_{1234}^k$ has at least $\Omega(\phi^k)$ oscillations and is hard to approximate by small shallow NNs. Moreover, Theorem~\ref{thm:main-linf} and Table~\ref{table:rho_inc} show that $f_{1234}^k$ actually has $\Omega(\rho^k)$ oscillations for $\rho \approx 1.839 > \phi$. A corollary is that any NN $g$ of depth $\sqrt{k}$ and width $O(1.839^{\sqrt{k}})$ has $L_{\infty}(f_{1234}^k, g) = \Omega(1)$, which is a stronger separation (\textit{constant} error) than the ones given by~\cite{cnpw19, cnp20}.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-osc.png}
    \caption{The chaotic itinerary $f_{1234}$ has more oscillations than $f_{123}$ even though $3 \triangleright 4$ by Sharkovsky's Theorem. Itineraries $f_{1234}$ and $f_{1324}$ (both of period 4) differ dramatically in oscillation count, showing why periodicity alone fails to capture the optimal tradeoffs.}
    \label{fig:toy-intro}
\end{figure}
%\vspace{-0.4cm}
The reverse is not true: Sharkovsky's Theorem guarantees that period-3 implies period-4, but the only 4-cycle guaranteed by the theorem is actually the non-chaotic 1324-itinerary, already shown to lead to minimal function complexity. 


Furthermore, as $p$ increases, the existence of a chaotic itinerary $12\dots p$ on $f$ ensures that $f^k$ has $\Omega(\rho^k)$ oscillations for $\rho \to 2$.\footnote{Similarly to~\cite{telgarsky16}, the optimal achievable rate is $\rho\le 2$ if we start with a unimodal $f$ (e.g., tent map). If one used multimodal functions as a building block (e.g., starting with $f'=f^2$ or $f'=f^3$), we could achieve larger rates (e.g., 4 or 8 respectively).} Figure~\ref{fig:toy-intro} demonstrates these differences in oscillations (by counting the number of monotone pieces of functions $f^k_{\mathbf{a}}$ with a maximal itinerary-$\mathbf{a}$). As indicated theoretically, the number of oscillations of $f_{1324}$ is polynomially-bounded, while the others grow exponentially fast, with $f_{1234}$ being closer to $2^k$. Please see Appendix~\ref{asec:warmup} for more such examples. 

%As a result, the true chaos hierarchy of these functions orders them as $f_{1234} > f_{123} >  f_{1324}$.
Generally, prior constructions where the oscillation count of $f^k$ increase at a rate faster than $\phi^k$ were too narrow (including only the triangle map). 
Because $f_{1234}$ breaks the barrier, we abstract away the details and point to chaotic itineraries as the main source of complexity, leading to sharper depth-width tradeoffs. 

While periodicity tells a compelling story about why $f_{123}^k$ is difficult to approximate, it fails to explain why $f_{1234}^k$ is even more complex.
The exponential-vs-polynomial gap in the function complexity of $f_{1234}$ and $f_{1324}$ depends solely on the order of the elements of the cycle and distinguishes functions that NNs can easily approximate from those they cannot.

The remainder of the paper addresses the question introduced here---when does the itinerary tell us much more than the length of the period---in a general context that explores a ``hierarchy'' of such chaotic itineraries, strengthens a host of NN inapproximability bounds (Sec.~\ref{sec:lb}), and reveals tight connections with other complexity notions, like the VC-dimension and topological entropy~(Sec.~\ref{sec:phase}).




%however in the study of DS it is known that orbits specifically can govern the oscillations rather than just the orbit length. Can we further deploy this idea to give better bounds on the tradeoffs?
\iffalse
\newpage
\vaggos{check two recent papers neurips related? Exact expressibility of functions vs approximate...}

\vaggos{bounded width also limits the NN so benefits of width?}

%cite Minsk Papert Perceptron multilayerThis led to s which state
%unbounded width
%works try to quantify the tradeoffs
%using various techniques all over math
%more broadly, analogous questions are fundamental in complexity, circuit and other models of computation


%a basic, yet challenging question in deep learning theory with rich connections to many other areas of mathematics and computer science. One of the earliest results


%parity function in boolean functions is difficult unless we have logn depth...

%AI Winter due to misunderstanding about XOR and expressivity. so we need to figure out the class of functions representable. 
%2 vs 3 layers 

%Why aren’t AIs running around solving all the world’s problems? In brief, the problem is that neural networks are hard to train. Just because you know there should be a set of parameters that approximates your function well with your given network architecture, doesn’t mean there is any good way of finding those parameters.


\vaggos{our bounds: they tighten as the period increases contrary to prior works.}
\vaggos{important to clarify that we quantify the xy gap. for every function that had odd period there exist xy... exists xy gap such that every function with odd period has gap at least some 0.1 or sth...}

-DNNs remarkable performance last few years, but why do deeper nets perform better than shallow? Expressivity questions studies types of functions that are representable or approximately representable by the output of a NN. e.g. can we find functions that are easily represented as 3 layers but not as two? Cite Eldan/Shamir. What about deeper regimes? However early results show depth 2 suffices. Bounded resources lead to depth vs width separations. An example is Telgarsky's result which gives a specific function that deep nets represent easily but shallow nets need to be exponentially wide. A main question in Telgarsky's and other papers (cite Malach/SSS) is to find larger families or what are the properties of such hard-to-represent functions?

-List of complexity measures to distinguish depth separations. Note that the question of expressivity makes sense in other computational models like boolean circuits where analogous depth separation results are fundamental in complexity theory etc. (cite Hastad).

-Most recently papers rely on dynamical systems ideas eg ICLR ICML and Harvard paper. Nice thing about these is that they point out to exciting new connections with DS literature and be able to prove much stronger bounds and larger families of functions that yield depth separations.

-Crucial connecting thread is higher order notion of fixed points and oscillations that was made explicit in ICLR/ICML via Sharkovsky's theorem.

-Pose 1 main motivating question: Can we go beyond Sharkovsky's theorem and exploit further properties of chaotic maps derive sharper depth separation results further proving benefits of depth for certain classes of functions?

-explain the main surprise, state informal theorem, explain bounds, and how we improve.

-motivating warm-up example: idea of ``chaotic itineraries'' and connection to eigenvalue and characteristic polynomial governing the oscillations.

-show two period 3 functions one with LLLR other with RRRL so we get different bounds. Trajectory matters cause if we only had RRRL then we could even get only prime period 4 and hence polynomially many oscillations.




%expressivity, standard old results, newer approach Telgarsky with dynamical systems, notions of copmlexity

%motivating example: not tent map, not periodic analysis, but LLLR gives tight bounds



\vaggos{chaotic itineraries lead to better characteristic polynomial}

\vaggos{Title: may be good to include somehow the words "chaotic itineraries" or "benefits of depth" or "depth-width tradeoffs" ...}



\vaggos{regarding high level: it's good to formulate 1 or 2 questions in the introduction that are very natural and intuitive. Examples: "Can we characterize benefits of depth in neural networks via larger families of functions?" or "Can we exploit dynamical systems constructions to obtain sharper tradeoffs for the benefits of depth?"...}

\vaggos{It's nice for our story to have a "surprise" element. This can be for example: Based on prior works, from the Sharkovsky ordering one expects fewer and fewer oscillations as the period increases and especially if it's a power of 2. However we show the opposite can happen. The crucial observation is that types of itineraries matter.}

\vaggos{When we phrase our main result, I think the community is more interested in hearing about Neural Networks tradeoffs or NN limitations or NN benefits of depth vs width. We should phrase our result as such I think i.e. the application of all the theory is that shallow nets cannot approximate certain large families of functions.}

\vaggos{Periods serve as certificate of difficulty or of necessity of depth. Here we give another type of certificate that can point to very sharp separations or important benefits of depth"...}

\vaggos{Motivation: we can still include sth about Recurrent Neural Nets since our functions come from iterated applications of the "same network" in some sense. (understanding limitations and types of functions RNNs can represent is important)}

\vaggos{Potential Remarks we should add: what about semialgebraic gates in NN? or we talk only about ReLU? I guess this should be easy since we only use the upper bound on monotone pieces. What about higher dimensions? Telgarsky and in ICLR/ICML dealt with it simply by saying about a projection on a direction that contains lots of oscillations. Can we get away with a simple remark on that?}

\vaggos{Examples: Can we have examples where lipschitz $L >> \rho$ and then ICML fails i.e. L1 error is still 0 instead of >0? Maybe like a convex steep function or sth? Also, we should add maybe pathological example with topological entropy $\pm\infty$ so to point out the weakness in Harvard paper about their notion of separation... (doubly weak since they have potentially shrinking separation)}

\vaggos{For background story: Telgarsky shows triangle (very specific function) but gets sharp $2^t$ separations. Natural question: What if we don't have a triangle exactly? Can we relax tent-map-assumption and give larger families? Telgarsky's result won't tell us anything. ICLR/ICML: Yes even if only odd periods are present we get separations but less sharp e.g. $sqrt{2}^t$ instead of $2^t$. But can we exploit further structure to get sharper bounds? Here: Yes, trajectory or chaotic itineraries are important and give almost $2^t$ separations.}

\vaggos{"We are first to find that periods don't tell the whole story and that types of itineraries matter"
Vaggelis
(e.g., since 4 appears almost last in Sharkovsky's ordering one might expect not strong separations, YET we get very sharp due to itinerary LLLR --> counterintuitive based on prior works)}

\todo{Start off by focusing on motivation of LLLR super-stable tent map cycle. Shows sub-optimality of ICLR, allows us to instantiate ICML bounds, Lipschitz, constant size (chaotic itinerary)\dots motivate extension to longer cycles with more LLLLLLLLLLLR. Increasing period can actually help when you care about making it harder to learn, unlike Sharkovsky!! Give an informal theorem statement.}

\todo{Show limitations of these methods with any curve with LRRR cycle and no 8-cycles that can be polynomially approximated. What's the difference? Number of oscillations. Ask question: is this the end of the cycle? No!}

Motivating question in ML theory: depth separation/powers of depth. Introduced by \cite{telgarsky16} to capture what deep networks can compute but shallow networks cannot. Telgarsky took gave an $L_1$ lower bound by applying iterated triangle maps to show that they create highly oscillatory functions that can't be approximated NNs that aren't sufficiently deep or exponentially wide.

Question was built upon by \cite{cnpw19} (by Sharkovsky, $L_\infty$ depth-separation bounds can be created whenever there's an non-power-of-two cycle), \cite{cnp20} (tighter lower bounds by periodicity, $L_1$ bounds under a Lipschitzness assumption), and \cite{bzl20} (lower bounds tied to topological entropy rather than periodicity).


A broader story about periodicity can be told by incorporating more dynamical systems theory from papers like \cite{mss73}. Namely, it's not just the length of the cycle of $f$ but also the itinerary of the cycle that determines how many oscillations that $f^k$ has and how difficult $f^k$ is to approximate. For instance, a LLLR 4-cycle will produce $\rho^k$ oscillations, while a ``maximal'' LRLR 4-cycle will produce $k^2$ oscillations.


To tell this story, we consider a broad class of scaling concave unimodal maps and examine how their behavior changes as the scaling parameter $r$ increases. We can divide functions in the family into two regimes based on the size of $r$: the \textit{doubling regime} and the \textit{chaos regime}.
Awareness of these regimes can give us more specific and powerful bounds than the preceding papers.
    
In the doubling regime, the largest period is a power of two that strictly increases as $r$ increases. There is always a stable cycle. All PO2 periods have the same kind of itinerary. If the maximal period is $2^q$, then the number of oscillations of $f^k$ is $O(k^q)$, the topological entropy is zero, and the VC dimension is $O(2^q)$. (We're thinking of VC dimension mostly as a general measure of function class complexity rather than in its more specific learning theory context. This is because the hypothesis class of $\{f^k: k \in \mathbb{N}\}$ is not terribly natural for ML.)


In the chaos regime, there are tons of types of cycles of different itineraries. These cycles obey Sharkovsky's theorem, but there's more than that. For instance, the ``maximal'' itinerary $L^{p-1} R$ occurs for every $p$ in increasing order of $p$, and the number of oscillations strictly increases with increasing $r$. We can then show that the number of oscillations gets increasingly close to $2^k$ as $p$ increases (irrespective of Sharkovsky). Thus, you can have exponentially many oscillations even when the stable cycle has length a power of two. The topological entropy is nonzero, and the VC dimension is infinite.

We can also produce stronger bounds than \cite{cnpw19} and \cite{cnp20} because we can show that an interval of width $0.1$ is crossed a large number of times; this gives immediate $L_\infty$ bounds without needing more assumptions.

\vaggos{"Also the aforementioned phase transition is also quantifiable via the VC dimension which is another standard way of characterizing the complexity of functions, and hence also of NN capabilities" -- sth along these lines just to include VC

(e.g., I guess there are NN bounds based on depth, width for their VC dimension, so if the functions we try to represent have infinite VC dimension then we can't approximate them basically.)}


\subsection{Related Work}

\vaggos{search most recent related works: ie Shamir recent paper, Chelsea Finn on Reinforcement Learning, MIT for graph neural nets, Loukas etc.}
\todo{Dynamical systems papers like \cite{mss73}}

\todo{Depth separation results by \cite{telgarsky16}, \cite{cnpw19}, \cite{bzl20}. 
Be clear about their limitations.}
\begin{itemize}
    \item \cite{telgarsky16} considers only a single type of function that is difficult to approximate; unclear from that paper alone whether that's a single hard instance or one of a more general class.
    \item \cite{cnpw19} extends this to a broader family of iterated functions, showing that a function with a non-power-of-two period is hard to approximate in a weaker sense than \cite{telgarsky16} (not $\L_1$ error). Based on Sharkovsky's theorem (period-3 implies any period).
    \item \cite{cnp20} builds on its predecessor by giving tighter bounds based on periods and showing limited conditions where $L_1$ bounds can be obtained. However, these bounds are still not the full story, and they give few settings where the $L_1$ bounds apply and are strong.
    \item \cite{bzl20} connects these concepts to topological entropy and proves bounds related to that. However, those bounds are also weaker than $L_1$.
\end{itemize}


\subsection{Our Results}

\begin{enumerate}
    \item We point out an incompleteness in the past theory. Namely, Sharkovsky's theorem doesn't tell the whole story, and much tighter bounds can be obtained if one assumes that certain ``itineraries'' of cycles exist.
    \item We give stronger $L_\infty$ lower bounds on approximating functions with neural networks. Unlike previous work, these are at least constant-size for large networks whenever there is any non-power-of-two cycle.
    \item We give several instances of strong $L_1$ bounds by applying the methodology of \cite{cnp20} for ``superstable'' cycles of certain itineraries on the tent map.
    \item More from a dynamical systems perspective, we note that these and the preceding results are characterized by a phase transition at between a ``doubling regime'' and a ``chaotic regime.'' We note that these regimes correspond to sharp cutoffs in the periodicity, the number of oscillations, the topological entropy, and the VC dimension of a corresponding function class. Our connections to the VC dimension are novel and demonstrate a sharp change in function complexity.
\end{enumerate}

\vaggos{Definition 1: can we include simple examples where if we didn't have assumption 1 or ass. 2 or ass. 3 then we will fail? Just to point out why we make these fairly natural assumptions. For example condition 2 seems to be there for purely technical reasons; do we mind if f is all 0 in the beginning for some interval?}
\fi

==> Beyond Sharkovsky Paper/intro_arxiv.tex <==
\section{Introduction}

%depth inflation, architecture leads to expressivity, analogous to circuit for boolean functions
%simple XOR gate couldn't be represented and this was taken as evidence of weakness of neural networks leading the first AI winter.

%whether we want to deply a NN for image analysis or text or speech one of the first crucial decisions that will determine its success or failure is the architecture of the network

%bounded resources?
Whether a neural network (NN) succeeds or fails at a given task crucially depends on whether or not its architecture (depth, width, types of activation units etc.) is suitable for the task at hand. 
For example, a ``size-inflation'' phenomenon has occurred in recent years, in which NNs tend to be deeper and/or larger. 
Recall that in 2012, AlexNet had 8 layers.
In 2015, ResNet won the ImageNet competition with 152 layers~\citep{krizhevsky2012imagenet,he2016deep},
This trend still continues to date, with modern models using billions of parameters~\citep{brown2020language}. 
The empirical success of deep neural networks motivates researchers to ask: What are the theoretical benefits of depth, and what are the depth-vs-width tradeoffs?

This question gives rise to the study of neural network \textit{expressivity}, which characterizes the class of functions that are representable (or approximately representable) by a NN of certain depth, width, and activation. 
For instance, \cite{eldan2016COLT} propose a family of ``radial'' functions in $\mathbb{R}^d$ that are easily expressible with 3-layered feedforward neural nets of small width, but require any approximating 2-layer network to have exponentially (in $d$) many neurons. In other words, they formally show that depth---even if increased by 1---can be exponentially more valuable than width. 
%add Telgarsky, Schmitt here to illustrate and give a taste of the type of statements...some results: triagnle wave, polynomials. schmitt uses VC to give lower bounds for size of NN for polynomials of degree k, we deploy sharkovsky and get lower bounds for a wider array of periodic cycles...We illuminate the problem from different perspectives


Not surprisingly, understanding the expressivity of NNs was an early question asked in 1969, when Minsky and Papert showed that the Perceptron can only learn linearly separable data and fails on simple XOR functions~\citep{minsky2017perceptrons}. 
The natural question of which functions can multiple such Perceptrons (i.e., multilayer feedforward NN) express was addressed later by \cite{cybenko1989approximation,hornik1989multilayer} proving the so-called \textit{universal approximation} theorem. 
This states, roughly, that just one hidden layer of standard activation units (e.g., sigmoids, ReLUs etc.) suffices to approximate any continuous function arbitrarily well. 
Taken at face value, any continuous function is a 2-layer (i.e., 1-hidden-layer) network in disguise, and hence, there is no reason to consider deeper networks. 
However, the width required can grow arbitrarily, and many works in the following decades quantify those depth-vs-width tradeoffs.


%Numerous results in the literature have established variants of
%this universal approximation property by considering distinct function classes to be
%approximated by network archhitectures using different types of neural activation
%functions with respect to various approximation criteria, see for instance [1, 2, 3, 5,
%6, 11, 12, 14, 15]. (
%All these results and many others not referenced here, some of them being constructive, some being merely existence proofs, provide upper bounds for the network size
%asserting that good approximation is possible if there are sufficiently many network nodes available. This, however, is only a partial answer to the question that
%mainly arises in practical applications: "Given some function, how many network
%nodes are needed to approximate it?" Not much attention has been focused on
%establishing lower bounds on the network size and, in particular, for the approximation of functions over the reals. As far as the computation of binary-valued: GIVE CITATIONS FOR BOOLEAN FUNCTIONS AS WELL Koiran, Maass etc.....


Towards this direction, one typically identifies a function together with a ``measure of complexity'' to demonstrate benefits of depth. 
For example, the seminal work by \cite{telgarsky15,telgarsky16} relies on the number of oscillations of a simple triangular wave function. 
Other relevant notions of complexity to the expressivity of NNs include the VC dimension~\citep{warren1968lower,anthony1999neural,schmitt2000lower}, the number of linear regions~\citep{montufar2014number,arora2016understanding} or activation patterns~\citep{hanin2019deep}, the dimension of algebraic varieties~\citep{kileel2019expressive}, the Fourier spectrum~\citep{barron1993universal,eldan2016COLT,daniely2017depth,lee2017ability, bresler2020sharp}, fractals~\citep{malach2019deeper}, topological entropy~\citep{bzl20}, Lipschitzness~\citep{safran2019depth,hsu2021approximation}, global curvature and trajectory length~\citep{poole2016NIPS,raghu2017ICML} just to name a few. 



%should I put BZL here or above?
This work builds upon recent papers~\citep{cnpw19,cnp20}, which study expressivity from the lens of discrete-time dynamical systems and extend Telgarsky's results beyond triangle (tent) maps. 
At a high-level, their idea is the following: if the initial layers of a NN output a real-valued %\footnote{Lower bounds were proved for dimension 1. However similar statements hold in higher dimension.} 
function $f$, then concatenating the \textit{same} layers $k$ times one after the other outputs $ f^k  \vcentcolon = f\circ f\circ \ldots\circ f$, i.e., the composition of $f$ with itself $k$ times. 
By associating each discrete timestep $k$ to the output of the corresponding layer in the network, one can study expressivity via the underlying properties of $f$'s trajectories. 
Indeed, if $f$ contains higher-order fixed points, called \textit{periodic} points, then deeper NNs can efficiently approximate $f^k$, but shallower nets would require exponential width, governed by $f$'s periodicity.

Inspired by these novel connections to discrete dynamical systems, we pose the following natural question:
\begin{center}
\textit{Apart from periodicity, are there other properties of $f$'s trajectories governing the expressivity tradeoffs?}
\end{center}
%trajectory, periodicity, other properties, augment expressivity, tight bounds from periodicity, can we improve?

We indeed prove that $f$'s periodicity alone is not the end of the story, and we improve on the known depth-width tradeoffs from several perspectives. 
We exhibit functions of the same period with very different behaviors (see Sec.~\ref{ssec:warmup}) that can be distinguished by the concept of ``chaotic itineraries.'' 
We analyze these here in order to achieve nearly-optimal tradeoffs for NNs. 
Our work highlights why previous works that examine periodicity alone only obtain loose bounds. 
More specifically:
%SHOULD WE ADD BULLET POINTS? AND ROUGHLY STATE IN SIMPLE WORDS THE RESULTS?

\begin{itemize} 
\item We accurately quantify the oscillatory behavior of a large family of functions $f$. This leads to sharper and nearly-optimal lower bounds for the width of NNs that approximate $f^k$.
\item Our lower bounds cover a stronger notion of approximation error, i.e., \textit{constant} separations between NNs, instead of bounds that become small depending heavily on $f$ and its periodicity.
\item At a conceptual level, we introduce and study certain chaotic itineraries, which supersede Sharkovsky's theorem~(see Sec.~\ref{subsec:dds}). 
% Our contributions are powered by technical lower bounds on the eigenvalues of a discrete dynamical system arising from such itineraries and show how the resulting oscillations cannot shrink significantly.
\item We elucidate connections between periodicity and other function complexity measures like the VC-dimension and the topological entropy~\citep{alseda2000}. %, and the ease of neural network approximation.
We show that all of these measures undergo a phase transition that exactly coincides with the emergence of the chaotic regime based on periods.
\end{itemize}
%on a conceptual level: we identify that the itineraries are actually important and not only the length of the periodic cycles as prior works on the topic seems to suggest. this allows us to get more refined bounds.


To the best of our knowledge, we are the first to incorporate the notion of chaotic itineraries from discrete dynamical systems into the study of NN expressivity. Other related works that have previously used ideas from chaotic dynamical systems (e.g., Li-Yorke chaos) to show the convergence (or not) of standard optimization methods, e.g., gradient descent, multiplicative weights update algorithm, include~\cite{lee2019first,palaiopanos2017multiplicative}. Before stating and interpreting our results, we provide some basic definitions.


\subsection{Function Approximation and NNs}
%constant errors vs yx errors, L1 L\infty, classification, and history of increasingly better and better results in the litearture
This paper employs three notions of approximation to compare functions $f, g: [0,1] \to [0,1]$.
\begin{itemize}
    \item $L_1(f,g)= \norm[1]{f - g} = \int_{0}^1 \abs{f(x) - g(x)} dx.$
    \item $L_\infty(f,g)=\norm[\infty]{f - g} = \sup_{x \in [0, 1]} \abs{f(x) - g(x)}.$
    \item Classification error $\mathcal{R}_{S,t}$: For $t \in [0,1]$, let $\thres{t}{x} = \indicator{x \geq t}$. Let $S = \{x_1, \dots, x_n\} \subseteq [0,1]$. Then,
    $\errcls{S,t}{f,g}= \frac{1}{n} \sum_{i=1}^n \indicator{\thres{t}{f(x_i)} \neq \thres{t}{g(x_i)}}.$ 
\end{itemize}
For what follows, let $\mathcal{N}(u,\ell)$ be the family of feedforward NNs of depth $\ell$ and width at most $u$ per layer with ReLU activation functions.\footnote{Recall ReLU$(x)=\max(x,0)$.} All our results also hold for the more general family of semialgebraic activations~\citep{telgarsky16}.

%\clayton{Add a note that $L_1 > Cls, L_\infty$ in terms of LBs? I think it's ok to skip, since we will not only derive L_1 bounds. Maybe we can mention in the main body?}

%say about error f,g in classifictation: you choose y_i to be f(x_i) for example of g etc...  then say about comparing these types of errors... What is the best to approximate? and give historical progression with Schmitt

%ntioning that the telgarsky triangle has an increasing cycle of any length
% THIS MEANS WE IDENTIFY NOT ONLY PERIODS AS THE CULPRIT FOR NECESSITY OF DEPTH, BUT RATHER CHAOTIC ITINERARIES THAT GIVE MORE OSCILLATIONS AND SHARPER BOUNDS... so we still abstract away details from triangle wave, but give general certificates for functions that give us bounds...

%It is important to understand that when we prove lower bounds for the difference of two functions, then the most desirable result is to obtain an $L_1$ bound
%not sure if we should phrase classification error wrt to f,g not just f. but that's fine...

%, and in the context of depth-width tradeoffs, we have managed to obtain increasingly better and better separations.

 %and $\round(z) = \round_{1/2}(z)$.

%For some threshold $t \in [0,1]$, , and , we let the \textit{classification error} of $f$ be







\subsection{Discrete Dynamical Systems}
\label{subsec:dds}
%period, sharkovsky, hint that sharkovsky is not the whole story
%chaotic itinerary
To construct families of functions that yield depth-separation results, we rely on a standard notion of \textit{unimodal} functions from dynamical systems~\citep{mss73}.

\begin{definition}
     Let $f: [0,1]\to[0,1]$ be a continuous and piece-wise differentiable function. We say $f$ is a \emph{unimodal mapping} if:
    \begin{enumerate}
        \item $f(0) = f(1) = 0$, and $f(x) > 0$ for all $x \in (0,1)$.
        \item There exists a unique maximizer $x'\in (0,1)$ of $f$, i.e., $f$ is strictly increasing on the interval $[0, x')$ and strictly decreasing on $(x',1]$.
    \end{enumerate}
\end{definition}

Our constructions rely on unimodal functions that are concave and also symmetric (i.e., $f(x) = f(1-x)$ for all $x \in [0, 1]$). 
We note that the resulting function family is fairly general, already capturing the triangle waves of \cite{telgarsky15,telgarsky16} and the logistic map used in previous depth-separation results~\citep{schmitt2000lower}.
Moreover, the study of one-dimensional discrete dynamical systems by applied mathematicians explicitly identifies unimodal mappings as important objects of study~\citep{mss73, alseda2000}.

Recall that a fixed point $x^*$ of $f$ is a point where $f(x^*)=x^*$. A more general notion of higher-order fixed points is that of \textit{periodicity}.

% \begin{definition}
% Let $p\in \mathbb{N}$ with $p\ge1$. We say $f$ has \emph{periodicity} $p$ (or  has a point of period $p$), if there exists a point $x^* \in [0,1]$ such that:\footnote{Throughout the paper, $f^{p}$ means composition of $f$ with itself $p$ times.}
% $$
% 	f^{p}(x^*)=x^* {\text{ \ \ and\ \ \ }} f^{k}(x^*)\neq x^*, \ \forall k \in [p-1].
% $$
% The set $C \vcentcolon= \{x^*,f(x^*), f(f(x^*)),\dots, f^{p-1}(x^*)\}$ contains $p$ distinct elements and is called a \emph{$p$-cycle}. Fixed points correspond to $p=1$.
% %\clayton{Can we make $p$ a an ordered $p$-tuple rather than a set, since order matters? - I think for now this is simpler to grasp.}
 
% \end{definition}
\begin{definition}
For some $p \in \N$, we say that $x_1,\dots, x_p\in [0,1]$ is a \emph{$p$-cycle} if $f(x_j) = x_{j+1}$ for all $j \in [p-1]$ and $f(x_p) = x_1$.
We say that $f$ has \emph{periodicity} $p$ if such a cycle exists and that $x_1$ is a \emph{point of period $p$} if $x_1$ belongs to a $p$-cycle. 
Equivalently, $x_1$ is a point of period $p$ if $f^p(x_1) = x_1$ and $f^{k}(x_1) \neq x_1$\footnote{Throughout the paper, $f^{k}$ means composition of $f$ with itself $k$ times.} for all $k \in [p-1]$.\footnote{As is common, $[m] = \{1, 2, \dots, m\}$.}
\end{definition}

%chaos theory, period 3 implies chaos, 
Does the existence of some $p$-cycle in $f$ have any implications about the existence of other cycles?
% Are there constraints between the types of periods a mapping $f$ can possess? 
These relations between the periods of $f$ are of fundamental importance to the study of dynamical systems. 
In particular, \cite{li1975period} proved in 1975 that ``period 3 implies chaos'' in their celebrated work, which also introduced the term ``chaos'' to mathematics and later spurred the development of chaos theory. 
Interestingly, an even more general result was already obtained a decade earlier in Eastern Europe, by~\cite{sharkovsky1964coexistence,sharkovsky1965cycles}:


\begin{theorem}[Sharkovsky's Theorem]
\label{thm:sharkovsky}
Let $f: [0,1]\to[0,1]$ be continuous. If $f$ contains period $p$ and $p \triangleright p'$, then $f$ also contains period $p'$, where the symbol `` $\triangleright$'' is defined based on the following (decreasing) ordering: 
\[
3 \triangleright 5 \triangleright 7\triangleright \ldots \triangleright2\cdot3 \triangleright 2\cdot5 \triangleright 2\cdot7\triangleright\ldots
\]
\[
\ldots \triangleright 2^2\cdot3 \triangleright 2^2\cdot5 \triangleright 2^2\cdot7\triangleright\ldots\triangleright2^3\triangleright2^2\triangleright2\triangleright1.
\]
\end{theorem}

This ordering, called \textit{Sharkovsky's ordering}, is a total ordering on the natural numbers, where $l\triangleright r$ whenever $l$ is to the left of $r$. The maximum number in this ordering is 3; if $f$ contains period 3, then it also has all other periods, which is also known as \emph{Li-Yorke chaos}. 
\cite{cnpw19,cnp20} apply this theorem to obtain depth-width tradeoffs based on periods and obtain their most powerful results when $p = 3$. 
We go beyond Sharkovsky's theorem and prove that tradeoffs are determined by the ``itineraries'' of periods.\footnote{These are called ``patterns'' in~\cite{alseda2000}.}

%\begin{definition}[Chaotic Itineraries]
%    Let $C$ be some $p$-cycle $x_1, \dots, x_p$ of a unimodal $f$. 
%    The \emph{itinerary} of $C$ is a string $\textbf{a}=a_1a_2\ldots a_p \in \{L, C, R\}^p$ of length $p$, with:
%    \[a_i \vcentcolon = \begin{cases}
%        L & x_i < x_{\max} \\
%        C & x_i = x_{\max} \\
%        R & x_i > x_{\max}.
%    \end{cases}\]
%Furthermore, any itinerary consisting of $(p-1)$ consecutive $L$'s followed by a single $R$, i.e., $\textbf{a}= L^{p-1}R = LL\ldots LR$ is called a \emph{chaotic} itinerary.
%\end{definition}

\begin{definition}[Itineraries]
    For a $p$-cycle $x_1, \dots, x_p$, suppose that $x_{a_1} < \dots < x_{a_p}$ for $a_j \in [p]$.
    The \emph{itinerary} of the cycle is the cyclic permutation of $x_{a_1}, \dots, x_{a_p}$ induced by $f$, which we represent by the string $\ba= a_1\dots a_p$.
    Because cyclic permutations are invariant to rotation, we assume (wlog) that $a_1 = 1$.


    % The \textit{itinerary} of a $p$-cycle is a cyclic permutation of the $p$ sorted elements $x_1 < \dots < x_p$ that indicates in what order they are traversed.
    % We represent the permutation with a string $\ba=a_1a_2\ldots a_p \in [p]^p$ that encodes this ordering and implies that $f(x_{a_i}) = f(x_{a_{i+1}})$ for all $i \in [p-1]$ and $f(x_{a_p}) = f(x_{a_1})$.
    % Itineraries are invariant to rotation, so we can assume (wlog) $x_1$ to be the smallest element of $C$, i.e., $a_1 = 1$.
    
    % Let $C$ be a $p$-cycle $x_1, \dots, x_p$ of a mapping $f$. 
    % The \emph{itinerary} of $C$ is a string $\ba=a_1a_2\ldots a_p \in [p]^p$ of length $p$ representing a permutation of the points in $C$. That is, $a_ia_j$ is a substring of $\ba$ if $f(x_i) = x_j$. 
    % Itineraries are invariant to rotation, so we can assume (wlog) $x_1$ to be the smallest element of $C$, i.e., $a_1 = 1$.
\end{definition}  

\begin{definition} [Chaotic Itineraries]
%   Any itinerary whose cycle has $x_1 < x_2 < \dots < x_p$ is called a \emph{chaotic} itinerary and is identifiable by $12\dots p$. (Because of its form, it is often called an \emph{increasing} $p$-cycle as well.) 
    A $p$-cycle is a \emph{chaotic itinerary} or an \emph{increasing cycle} if its itinerary is $12\dots p$. That is, $x_1 < \dots < x_p$. 
\end{definition}
Examining chaotic itineraries circumvents the limitations of prior works based on periods and yields sharper exponential depth-width tradeoffs. 
Unlike other function complexity properties, the existence of a chaotic itinerary is easily verifiable (see App.~\ref{assec:identifying}).
To grasp clean examples of itineraries, see App.~\ref{assec:it-exs}.




%Observe that the number 3 is the largest according to this ordering. Sharkovsky showed a surprising and elegant result about his ordering: it describes which numbers can be periods for a
%continuous map on an interval; allowed periods must be a suffix of his ordering:


%According to Sharkovsky's Theorem, 3 is the maximum period, so one important and easy-to-remember corollary is that period 3 implies \textit{all} periods.\footnote{On a historical plot twist, this special case was proved a decade later by James Yorke and Tien-Yien Li, in their seminal paper called ``Period Three Implies Chaos''~\cite{li1975period}; this is a celebrated result that actually introduced the term ``chaos'' as used in Mathematics (chaos theory).}



% $x^*$ is a \textit{fixed point} if $f(x^*) = x^*$.
%    For any $p > 1$, $x^*$ is a \textit{$p$-cyclic} point if $f^p(x^*) = x^*$ and $f^q(x^*) \neq x^*$ for all $q < p$.
%    We say that $f$ has a \textit{$p$-cycle} if there exists $p$ points $x_1, \dots, x_p$ such that $f(x_i) = x_{i+1}$ for $i \in [p-1]$ and $f(x_p) = x_1$.


\subsection{Our Main Contributions}

Our principal goal is to use knowledge about $f$'s itineraries to more accurately quantify the ``oscillations'' of $f^k$ as a measure of complexity and draw connections to other complexity measures. 
Section~\ref{sec:lb} produces sharper and more robust NN approximability tradeoffs than prior works by leveraging chaotic itineraries and unimodality.
Section~\ref{sec:phase} shows how a phase transition in VC-dimension and topological entropy of $f$ occurs exactly when the growth rate of oscillations shifts from polynomial to exponential. 


While previous works count oscillations too, they either construct too narrow a range of functions\footnote{e.g.,~\cite{telgarsky15,telgarsky16} only analyzes triangles.}, obtain loose depth-width tradeoffs\footnote{e.g.,~\cite{cnpw19,cnp20} have a suboptimal dependence on $p$ under stringent Lipschitz assumptions.}, or have unsatisfactory approximation error. \footnote{e.g.,~\cite{cnpw19,cnp20,bzl20} do not obtain constant error rates.} 
In Section~\ref{sec:lb}, we improve along these three directions by taking advantage of the unimodality and itineraries of $f$. 
% Roughly speaking, we compose $k$ times a unimodal function $f$ with itself to obtain $f^k$. 
The \textit{unimodality} of $f$ allows us to quantify both the number of piecewise monotone pieces of $f^k$ (i.e., oscillations) and the corresponding height between the highest and lowest values of $f^k$'s oscillations. 
This improvement on the height enables stronger notions of function approximation (e.g., constant error rates with no dependence on $f$ or its period $p$). 
\textit{Chaotic itineraries} allow an improved analysis of the number of oscillations in $f^k$ and grant sharper exponential lower bounds on the width of any shallow net $g$ approximating $f^k$. 

We say that our results are \textit{nearly-optimal} because we exhibit a broad family of functions $f$ that are inapproximable by shallow networks of width $O(\rho^k)$ for $\rho$ arbitrarily close to 2.
Because no unimodal function $f$ can induce more than $2^k$ oscillations in $f^k$, we cannot aspire to tighter exponent bases in this setting.\footnote{Our results also transfer to non-unimodal functions via the observation that for bimodal $g$, there is some unimodal $f$ such that the number of oscillations of $g$ is at most twice those of $f$.}
On the other hand, none of the bounds from previous works (except the narrow bounds of Telgarsky) produce width bounds of more than $\Omega(\phi^k)$, where $\phi \approx 1.618$ is the Golden Ratio.
To demonstrate our sharper tradeoffs, we state a special case of our results for the $L_\infty$ error.

\begin{theorem}\label{thm:motivation-lb-inc} 
% Let $g\in \mathcal{N}(u,\ell)$. For $p\ge 3$, let $\rho$ be the largest root of the polynomial equation $\lambda^{p} - 2\lambda^{p-1} + 1 = 0$.\footnote{Notice that $\rho \geq \max({2 - \frac4{2^{p}},{\tfrac{1+\sqrt 5}{2}}})$~(see Fact~\ref{fact:root-lb}) and is much stronger than previous bounds~\citep{cnpw19,cnp20}.} Moreover, let $f$ be any symmetric, concave unimodal mapping with a increasing $p$-cycle. For all $k\in\N$, if $g$ has $L_\infty(f^k,g) \le \tfrac{1}{36}$, then it must have large width:\todo{swap polynomial with bound}
% \[
% u  > \frac{1}{8} \rho^{k/\ell}
% \]
For $p \geq 3$ and $k \in \N$, consider any symmetric, concave unimodal mapping $f$ with an increasing $p$-cycle and any $g \in \mathcal{N}(u, \ell)$ with width \[u \leq \frac18 \left(\max\paren{2-\frac4{2^p}, \phi}\right)^{k/\ell}\]
Then, $L_\infty(f^k, g) = \Omega(1)$, independent of $f,p,k$.
\end{theorem}  
%\clayton{How about we instead say ``there exists a $\rho \geq 2 - \frac4{2^{\rho}}$'' to avoid introducing the polynomial? I like this polynomial to be there just so that they wonder how did it appear ? :P}
    
\begin{remark} When $g$ is shallow with depth $\ell=O(k^{1-\eps})$ (e.g., $\ell=k^{0.99}$), then its width must be exponentially large in order to well-approximate $f^k$.
% This shows how depth can be exponentially more valuable than width. 
% Moreover, $\rho \geq \max({2 - \frac4{2^{p}},{\tfrac{1+\sqrt 5}{2}}})$~(see Fact~\ref{fact:root-lb}). 
This exponential separation is sharper than prior works~\citep{cnpw19,cnp20}, and quickly becomes even sharper (tending to 2) with larger values of $p$. 
This is counterintuitive as Sharkovsky's ordering implies that period 3 is the most chaotic and prior works recover a suboptimal rate of at most $\phi\approx 1.618$ (see Table~\ref{table:rho_inc}). 
% Since $\rho\le 2$ for unimodal $f$, our bound quickly converges to the optimal tradeoff (see Fig.~\ref{fig:toy-intro}). 
\end{remark}
\begin{remark}
Our approximation error is constant independent of all other parameters $f, k, p$. 
Previous results~\citep{cnpw19,cnp20,bzl20} obtain a gap that depends on $f,p$ and may be arbitrarily small.
Moreover, we have required nothing of the Lipschitz constant of $f$, unlike the strict assumptions on the Lipschitz constant $L$ of $f$ by~\cite{cnp20} (e.g., they require $L=\phi$ for period $p=3$).
Indeed, Propositions~\ref{prop:need-symmetry} and \ref{prop:need-concavity} in the Appendix~\ref{assec:sym-conc} (see also Fig.~\ref{fig:asymmetric}, Fig.~\ref{fig:non-concave}), and Figure~\ref{fig:non-concave-intro} illustrate how their lower bounds break down for large $L$ and how their $L_\infty$ bounds can shrink, becoming arbitrarily weak for certain 3-periodic $f$.
\end{remark}

    
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/fig-non-concave1.png}
         \includegraphics[width=0.45\textwidth]{fig/fig-non-concave10.png}
        \caption{To illustrate the limitations of prior work \citep{cnpw19, cnp20, bzl20}, we visualize a unimodal mapping $f$ on the left and $f^{10}$ on the right where $f$ has a 3-cycle without $f^{10}$ having large oscillations.
        As guaranteed by the previous results, the total number of oscillations of $f^{k}$ is $\Omega(\phi^k)$; however, each is of magnitude at most $\eps$ for this construction and $f^k$ can be $\eps$-approximated by a two-layer constant-width neural network, by Proposition~\ref{prop:need-concavity}. Here, $\eps = 0.1$, but it may be arbitrarily small. Hence, to obtain non-trivial constant-accuracy lower bounds on the size of neural network needed to approximate $f^k$, it is insufficient to require only that $f$ has a 3-cycle.}
        \label{fig:non-concave-intro}
    \end{figure}

We also present analogous results for the classification error and the $L_1$ errors. Please see the full statements in Theorems~\ref{thm:main-linf} and \ref{thm:main-l1}. Furthermore, Theorems~\ref{thm:odd-linf} and \ref{thm:odd-l1} offer an improvement on the results of \cite{cnp20} by giving constant-accuracy $L_\infty$ lower bounds without needing a chaotic itinerary.

In addition, Section~\ref{sec:phase} relates our chaotic itineraries to standard notions of function complexity like the VC dimension and the topological entropy (for precise definitions, see Sec.~\ref{sec:phase}). The types of periodic itineraries of $f$ give rise to two regimes: the \textit{doubling} regime and the \textit{chaotic} regime. In the former, we have a polynomial number of oscillations, while the latter is characterized by an exponential number of oscillations. Here we show the following correspondence:

\begin{theorem}[Informal]\label{thm:informal-phase}
The transition between these two regimes exactly coincides with a sharp transition in the VC-dimension of the iterated mappings $f^k$ for fixed $f$ (from bounded to infinite) and in the topological entropy (from zero to positive).
\end{theorem}


%challenge? technical side? more broadly VC...
\paragraph{Our Techniques} To quantify the oscillations of $f^k$, we use its chaotic itineraries to decompose the $[0,1]$ interval into several subintervals $\{I_j\}_{j=1}^{j=p-1}$. We count the number of times $f^k$ ``visits'' each $I_j$, by identifying a suitable matrix $A$ whose spectral radius is a lower bound on the growth rate of oscillations. The associated characteristic polynomial of $A$ is $\lambda^{p} - 2\lambda^{p-1} + 1$ and has larger spectral radius that that of prior works for \textit{all} periods. 
Moreover, the corresponding oscillations of at least one of the subintervals $I_j$ do not shrink in size, giving a bound on the total number of oscillations of a \textit{sufficient} size. 
This provides a lower bound on the height between the peak and the bottom of these oscillations that later provides \textit{constant} approximation errors for small shallow NNs.

More broadly, our work builds on the efforts to characterize large families of functions that give depth separations and addresses questions raised by~\cite{eldan2016COLT,telgarsky16,poole2016NIPS, malach2019deeper} about the properties of hard-to-represent functions. Similar to periods, the concept of chaotic itineraries can serve as a certificate of complexity, which is also easy to verify for unimodal $f$ (see Proposition~\ref{prop:half-inc-cycle} in Appendix).

%and relying on shallow nets few oscillations, 




%high-level: shallow nets few oscillations, deep nets large number of oscillations, following prior works we use oscillations as notion of complexity. We present refined bounds based on our unimodal funtions and f^k. This boosted oscillations numbers allow to get our improved bounds alongside the VC and topological entropy phase shift.



%on a technical level: eigenvalue analysis based on chaotic itineraries provide us with more oscillations. Furthermore, they provide us with constat-separated oscillations sth which was not known if it can be done before where the gap was shrinking based on y-x which we could not control. Now we change the quantifiers saying that for there is a gap such that for any period p .... whereas before they said for every period p function there is a constant that depends on f and p and y-x such that... this boosting on the number of oscillations allow us to get sharper tradeoffs that become sharper and sharper as p increases, sth that was not known before and are nearly optimal approaching the best 2^n dependence of unimodal functions.

%more broadly, we also provide evidence that the shift in regimes from doubling to chaotic coincides exactly with VC bounds change and also topological entropy of related function family based on iterated maps.

%say that throughout the paper we provide experiments or simulations to demonstrate our resutls.

%briefly we summarize our contributions bellow: give 3 bullet points: 1) sharkovsky and periods not the end of story. using chaotic itineraries we get boosted number of oscillations. 2) these translate to larger and constant gaps in errors, better dependence on p, more subtle connection with expressivity and depth-width tradeoffs. Informally, state two main theorems. 3) state informally results for VC and topological entropy.


%some of our results are incomparable to prior works: on the one hand, in ICML they have very stringent assumptions on the lipschitz constant in order to prove bounds which we destroy by the two counterexamples. On the other hand, we do require symmetry and concavity and altough natural these can't compare with the lipschitz assumption. We get stronger separations compared to ICLR, we completely generalize Telgarsky, and we get better bounds than Harvard paper.


\section{Warm-up Examples}\label{ssec:warmup}

This section presents illustrative examples and instantiates our results for some simple cases. 
These highlight the limitations of exclusively considering periodicity of cycles alone---and not itineraries---when developing accurate oscillation/crossing bounds~(see also Def.~\ref{def:osc},~\ref{def:cross}) and sharp expressivity tradeoffs.

%To demonstrate the strength of our bounds and the centrality of itineraries to the connections between dynamical systems and neural network expressivity, we consider a simple case where itineraries supersede periodicity in number of oscillations and hardness of approximation.

Consider the three unimodal mappings in Figure~\ref{fig:toy-ex-compare-map}, $f_{\ba}$ with itineraries $\ba \in \{1324, 1234, 123\}$. 
Observe that $f_{1234}$ has the cycle $(\frac{1}{5}, \frac{2}{5}, \frac{3}{5}, \frac{4}{5})$, $f_{1324}$ has $(\frac{1}{5}, \frac{3}{5}, \frac{2}{5}, \frac{4}{5})$, and $f_{123}$ has $(\frac{1}{4}, \frac{1}{2}, \frac{3}{4})$. Despite their similarities, they give rise to significantly different behaviours in $f_{\ba}^k$.

What do prior works based on NN approximation with respect to periods and Sharkovsky's theorem alone tell us?  
\cite{cnpw19,cnp20} show that the 3-cycle of $f_{123}$ ensures that $f^k$ has $\Omega(\phi^k)$ oscillations, where $\phi \approx 1.618$ is the golden ratio. However, their theorems do not imply anything for $f_{1324}$ and $f_{1234}$, since 4 is a power of 2, and they require odd periods.  
%One might expect a ``chaos hierarchy'' that ranks $f_{123}$ above $f_{1324}$ and %$f_{1234}$.


\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{fig/fig-toy-ex-compare_map.png}
    \caption{Plots of unimodal mappings with different itineraries $f_{1234}$, $f_{1324}$, and $f_{123}$. Despite their similarities, $f_{1234}$ leads to the most oscillations and sharpest depth-width tradeoffs (see Fig.~\ref{fig:toy-intro}).}
    \label{fig:toy-ex-compare-map}
\end{figure}
As it turns out, $f_{1234}$ leads to exponential oscillations and $f_{1324}$ leads only to polynomial oscillations:
\begin{itemize}
    \item A mapping with a 1324-itinerary is guaranteed no other cycles except the 2-cycle and a fixed point~\citep{mss73}. 
    Sharkovsky's theorem and \cite{cnpw19} predict this outcome, since 4 is the third-right-most element of the Sharkovsky ordering, and its existence alone promises nothing more.
    The ordering of itineraries introduced by~\citep{mss73} (see Table~\ref{table:itineraries} in Appendix) indicates that the particular 1324-itinerary only implies the periods 2 and 1, and confirms this intuition.
    % \vaggos{what is 12 itinerary?}
    We classify this itinerary as part of the \emph{doubling regime} and prove in Theorem~\ref{thm:properties-doubling} that any $f^k$ with a \textit{maximal} 1324-itinerary (that is, there is no 8-cycle) cannot exhibit sharp depth-width tradeoffs: for any $\eps>0$, there exists a 2-layer ReLU neural network $g$ of width $O(\frac{k^3}{\eps})$ such that 
    $L_\infty(f_{1324}^k, g) \leq \eps.$
    

    \item Going beyond Sharkovsky's theorem, a mapping with a 1234-itinerary---even though it is of period 4---it is guaranteed to contain a 3-cycle as well (see Table~\ref{table:itineraries} in Appendix). Hence, ``itinerary-1234 implies period-3, implies chaos,'' and $f_{1234}^k$ has at least $\Omega(\phi^k)$ oscillations and is hard to approximate by small shallow NNs. Moreover, Theorem~\ref{thm:main-linf} and Table~\ref{table:rho_inc} show that $f_{1234}^k$ actually has $\Omega(\rho^k)$ oscillations for $\rho \approx 1.839 > \phi$. A corollary is that any NN $g$ of depth $\sqrt{k}$ and width $O(1.839^{\sqrt{k}})$ has $L_{\infty}(f_{1234}^k, g) = \Omega(1)$, which is a stronger separation (\textit{constant} error) than the ones given by~\cite{cnpw19, cnp20}.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{fig/fig-toy-ex-osc.png}
    \caption{The chaotic itinerary $f_{1234}$ has more oscillations than $f_{123}$ even though $3 \triangleright 4$ by Sharkovsky's Theorem. Itineraries $f_{1234}$ and $f_{1324}$ (both of period 4) differ dramatically in oscillation count, showing why periodicity alone fails to capture the optimal tradeoffs.}
    \label{fig:toy-intro}
\end{figure}
%\vspace{-0.4cm}
The reverse is not true: Sharkovsky's Theorem guarantees that period-3 implies period-4, but the only 4-cycle guaranteed by the theorem is actually the non-chaotic 1324-itinerary, already shown to lead to minimal function complexity. 


Furthermore, as $p$ increases, the existence of a chaotic itinerary $12\dots p$ on $f$ ensures that $f^k$ has $\Omega(\rho^k)$ oscillations for $\rho \to 2$.\footnote{Similarly to~\cite{telgarsky16}, the optimal achievable rate is $\rho\le 2$ if we start with a unimodal $f$ (e.g., tent map). If one used multimodal functions as a building block (e.g., starting with $f'=f^2$ or $f'=f^3$), we could achieve larger rates (e.g., 4 or 8 respectively).} Figure~\ref{fig:toy-intro} demonstrates these differences in oscillations (by counting the number of monotone pieces of functions $f^k_{\mathbf{a}}$ with a maximal itinerary-$\mathbf{a}$). As indicated theoretically, the number of oscillations of $f_{1324}$ is polynomially-bounded, while the others grow exponentially fast, with $f_{1234}$ being closer to $2^k$. Please see Appendix~\ref{asec:warmup} for more such examples. 

%As a result, the true chaos hierarchy of these functions orders them as $f_{1234} > f_{123} >  f_{1324}$.
Generally, prior constructions where the oscillation count of $f^k$ increase at a rate faster than $\phi^k$ were too narrow (including only the triangle map). 
Because $f_{1234}$ breaks the barrier, we abstract away the details and point to chaotic itineraries as the main source of complexity, leading to sharper depth-width tradeoffs. 

While periodicity tells a compelling story about why $f_{123}^k$ is difficult to approximate, it fails to explain why $f_{1234}^k$ is even more complex.
The exponential-vs-polynomial gap in the function complexity of $f_{1234}$ and $f_{1324}$ depends solely on the order of the elements of the cycle and distinguishes functions that NNs can easily approximate from those they cannot.

The remainder of the paper addresses the question introduced here---when does the itinerary tell us much more than the length of the period---in a general context that explores a ``hierarchy'' of such chaotic itineraries, strengthens a host of NN inapproximability bounds (Sec.~\ref{sec:lb}), and reveals tight connections with other complexity notions, like the VC-dimension and topological entropy~(Sec.~\ref{sec:phase}).




%however in the study of DS it is known that orbits specifically can govern the oscillations rather than just the orbit length. Can we further deploy this idea to give better bounds on the tradeoffs?
\iffalse
\newpage
\vaggos{check two recent papers neurips related? Exact expressibility of functions vs approximate...}

\vaggos{bounded width also limits the NN so benefits of width?}

%cite Minsk Papert Perceptron multilayerThis led to s which state
%unbounded width
%works try to quantify the tradeoffs
%using various techniques all over math
%more broadly, analogous questions are fundamental in complexity, circuit and other models of computation


%a basic, yet challenging question in deep learning theory with rich connections to many other areas of mathematics and computer science. One of the earliest results


%parity function in boolean functions is difficult unless we have logn depth...

%AI Winter due to misunderstanding about XOR and expressivity. so we need to figure out the class of functions representable. 
%2 vs 3 layers 

%Why aren’t AIs running around solving all the world’s problems? In brief, the problem is that neural networks are hard to train. Just because you know there should be a set of parameters that approximates your function well with your given network architecture, doesn’t mean there is any good way of finding those parameters.


\vaggos{our bounds: they tighten as the period increases contrary to prior works.}
\vaggos{important to clarify that we quantify the xy gap. for every function that had odd period there exist xy... exists xy gap such that every function with odd period has gap at least some 0.1 or sth...}

-DNNs remarkable performance last few years, but why do deeper nets perform better than shallow? Expressivity questions studies types of functions that are representable or approximately representable by the output of a NN. e.g. can we find functions that are easily represented as 3 layers but not as two? Cite Eldan/Shamir. What about deeper regimes? However early results show depth 2 suffices. Bounded resources lead to depth vs width separations. An example is Telgarsky's result which gives a specific function that deep nets represent easily but shallow nets need to be exponentially wide. A main question in Telgarsky's and other papers (cite Malach/SSS) is to find larger families or what are the properties of such hard-to-represent functions?

-List of complexity measures to distinguish depth separations. Note that the question of expressivity makes sense in other computational models like boolean circuits where analogous depth separation results are fundamental in complexity theory etc. (cite Hastad).

-Most recently papers rely on dynamical systems ideas eg ICLR ICML and Harvard paper. Nice thing about these is that they point out to exciting new connections with DS literature and be able to prove much stronger bounds and larger families of functions that yield depth separations.

-Crucial connecting thread is higher order notion of fixed points and oscillations that was made explicit in ICLR/ICML via Sharkovsky's theorem.

-Pose 1 main motivating question: Can we go beyond Sharkovsky's theorem and exploit further properties of chaotic maps derive sharper depth separation results further proving benefits of depth for certain classes of functions?

-explain the main surprise, state informal theorem, explain bounds, and how we improve.

-motivating warm-up example: idea of ``chaotic itineraries'' and connection to eigenvalue and characteristic polynomial governing the oscillations.

-show two period 3 functions one with LLLR other with RRRL so we get different bounds. Trajectory matters cause if we only had RRRL then we could even get only prime period 4 and hence polynomially many oscillations.




%expressivity, standard old results, newer approach Telgarsky with dynamical systems, notions of copmlexity

%motivating example: not tent map, not periodic analysis, but LLLR gives tight bounds



\vaggos{chaotic itineraries lead to better characteristic polynomial}

\vaggos{Title: may be good to include somehow the words "chaotic itineraries" or "benefits of depth" or "depth-width tradeoffs" ...}



\vaggos{regarding high level: it's good to formulate 1 or 2 questions in the introduction that are very natural and intuitive. Examples: "Can we characterize benefits of depth in neural networks via larger families of functions?" or "Can we exploit dynamical systems constructions to obtain sharper tradeoffs for the benefits of depth?"...}

\vaggos{It's nice for our story to have a "surprise" element. This can be for example: Based on prior works, from the Sharkovsky ordering one expects fewer and fewer oscillations as the period increases and especially if it's a power of 2. However we show the opposite can happen. The crucial observation is that types of itineraries matter.}

\vaggos{When we phrase our main result, I think the community is more interested in hearing about Neural Networks tradeoffs or NN limitations or NN benefits of depth vs width. We should phrase our result as such I think i.e. the application of all the theory is that shallow nets cannot approximate certain large families of functions.}

\vaggos{Periods serve as certificate of difficulty or of necessity of depth. Here we give another type of certificate that can point to very sharp separations or important benefits of depth"...}

\vaggos{Motivation: we can still include sth about Recurrent Neural Nets since our functions come from iterated applications of the "same network" in some sense. (understanding limitations and types of functions RNNs can represent is important)}

\vaggos{Potential Remarks we should add: what about semialgebraic gates in NN? or we talk only about ReLU? I guess this should be easy since we only use the upper bound on monotone pieces. What about higher dimensions? Telgarsky and in ICLR/ICML dealt with it simply by saying about a projection on a direction that contains lots of oscillations. Can we get away with a simple remark on that?}

\vaggos{Examples: Can we have examples where lipschitz $L >> \rho$ and then ICML fails i.e. L1 error is still 0 instead of >0? Maybe like a convex steep function or sth? Also, we should add maybe pathological example with topological entropy $\pm\infty$ so to point out the weakness in Harvard paper about their notion of separation... (doubly weak since they have potentially shrinking separation)}

\vaggos{For background story: Telgarsky shows triangle (very specific function) but gets sharp $2^t$ separations. Natural question: What if we don't have a triangle exactly? Can we relax tent-map-assumption and give larger families? Telgarsky's result won't tell us anything. ICLR/ICML: Yes even if only odd periods are present we get separations but less sharp e.g. $sqrt{2}^t$ instead of $2^t$. But can we exploit further structure to get sharper bounds? Here: Yes, trajectory or chaotic itineraries are important and give almost $2^t$ separations.}

\vaggos{"We are first to find that periods don't tell the whole story and that types of itineraries matter"
Vaggelis
(e.g., since 4 appears almost last in Sharkovsky's ordering one might expect not strong separations, YET we get very sharp due to itinerary LLLR --> counterintuitive based on prior works)}

\todo{Start off by focusing on motivation of LLLR super-stable tent map cycle. Shows sub-optimality of ICLR, allows us to instantiate ICML bounds, Lipschitz, constant size (chaotic itinerary)\dots motivate extension to longer cycles with more LLLLLLLLLLLR. Increasing period can actually help when you care about making it harder to learn, unlike Sharkovsky!! Give an informal theorem statement.}

\todo{Show limitations of these methods with any curve with LRRR cycle and no 8-cycles that can be polynomially approximated. What's the difference? Number of oscillations. Ask question: is this the end of the cycle? No!}

Motivating question in ML theory: depth separation/powers of depth. Introduced by \cite{telgarsky16} to capture what deep networks can compute but shallow networks cannot. Telgarsky took gave an $L_1$ lower bound by applying iterated triangle maps to show that they create highly oscillatory functions that can't be approximated NNs that aren't sufficiently deep or exponentially wide.

Question was built upon by \cite{cnpw19} (by Sharkovsky, $L_\infty$ depth-separation bounds can be created whenever there's an non-power-of-two cycle), \cite{cnp20} (tighter lower bounds by periodicity, $L_1$ bounds under a Lipschitzness assumption), and \cite{bzl20} (lower bounds tied to topological entropy rather than periodicity).


A broader story about periodicity can be told by incorporating more dynamical systems theory from papers like \cite{mss73}. Namely, it's not just the length of the cycle of $f$ but also the itinerary of the cycle that determines how many oscillations that $f^k$ has and how difficult $f^k$ is to approximate. For instance, a LLLR 4-cycle will produce $\rho^k$ oscillations, while a ``maximal'' LRLR 4-cycle will produce $k^2$ oscillations.


To tell this story, we consider a broad class of scaling concave unimodal maps and examine how their behavior changes as the scaling parameter $r$ increases. We can divide functions in the family into two regimes based on the size of $r$: the \textit{doubling regime} and the \textit{chaos regime}.
Awareness of these regimes can give us more specific and powerful bounds than the preceding papers.
    
In the doubling regime, the largest period is a power of two that strictly increases as $r$ increases. There is always a stable cycle. All PO2 periods have the same kind of itinerary. If the maximal period is $2^q$, then the number of oscillations of $f^k$ is $O(k^q)$, the topological entropy is zero, and the VC dimension is $O(2^q)$. (We're thinking of VC dimension mostly as a general measure of function class complexity rather than in its more specific learning theory context. This is because the hypothesis class of $\{f^k: k \in \mathbb{N}\}$ is not terribly natural for ML.)


In the chaos regime, there are tons of types of cycles of different itineraries. These cycles obey Sharkovsky's theorem, but there's more than that. For instance, the ``maximal'' itinerary $L^{p-1} R$ occurs for every $p$ in increasing order of $p$, and the number of oscillations strictly increases with increasing $r$. We can then show that the number of oscillations gets increasingly close to $2^k$ as $p$ increases (irrespective of Sharkovsky). Thus, you can have exponentially many oscillations even when the stable cycle has length a power of two. The topological entropy is nonzero, and the VC dimension is infinite.

We can also produce stronger bounds than \cite{cnpw19} and \cite{cnp20} because we can show that an interval of width $0.1$ is crossed a large number of times; this gives immediate $L_\infty$ bounds without needing more assumptions.

\vaggos{"Also the aforementioned phase transition is also quantifiable via the VC dimension which is another standard way of characterizing the complexity of functions, and hence also of NN capabilities" -- sth along these lines just to include VC

(e.g., I guess there are NN bounds based on depth, width for their VC dimension, so if the functions we try to represent have infinite VC dimension then we can't approximate them basically.)}




\subsection{Related Work}

\vaggos{search most recent related works: ie Shamir recent paper, Chelsea Finn on Reinforcement Learning, MIT for graph neural nets, Loukas etc.}
\todo{Dynamical systems papers like \cite{mss73}}

\todo{Depth separation results by \cite{telgarsky16}, \cite{cnpw19}, \cite{bzl20}. 
Be clear about their limitations.}
\begin{itemize}
    \item \cite{telgarsky16} considers only a single type of function that is difficult to approximate; unclear from that paper alone whether that's a single hard instance or one of a more general class.
    \item \cite{cnpw19} extends this to a broader family of iterated functions, showing that a function with a non-power-of-two period is hard to approximate in a weaker sense than \cite{telgarsky16} (not $\L_1$ error). Based on Sharkovsky's theorem (period-3 implies any period).
    \item \cite{cnp20} builds on its predecessor by giving tighter bounds based on periods and showing limited conditions where $L_1$ bounds can be obtained. However, these bounds are still not the full story, and they give few settings where the $L_1$ bounds apply and are strong.
    \item \cite{bzl20} connects these concepts to topological entropy and proves bounds related to that. However, those bounds are also weaker than $L_1$.
\end{itemize}


\subsection{Our Results}

\begin{enumerate}
    \item We point out an incompleteness in the past theory. Namely, Sharkovsky's theorem doesn't tell the whole story, and much tighter bounds can be obtained if one assumes that certain ``itineraries'' of cycles exist.
    \item We give stronger $L_\infty$ lower bounds on approximating functions with neural networks. Unlike previous work, these are at least constant-size for large networks whenever there is any non-power-of-two cycle.
    \item We give several instances of strong $L_1$ bounds by applying the methodology of \cite{cnp20} for ``superstable'' cycles of certain itineraries on the tent map.
    \item More from a dynamical systems perspective, we note that these and the preceding results are characterized by a phase transition at between a ``doubling regime'' and a ``chaotic regime.'' We note that these regimes correspond to sharp cutoffs in the periodicity, the number of oscillations, the topological entropy, and the VC dimension of a corresponding function class. Our connections to the VC dimension are novel and demonstrate a sharp change in function complexity.
\end{enumerate}

\vaggos{Definition 1: can we include simple examples where if we didn't have assumption 1 or ass. 2 or ass. 3 then we will fail? Just to point out why we make these fairly natural assumptions. For example condition 2 seems to be there for purely technical reasons; do we mind if f is all 0 in the beginning for some interval?}
\fi

==> Beyond Sharkovsky Paper/lb.tex <==
\section{Depth-Width Tradeoffs via Chaotic Itineraries}\label{sec:lb}

% \vaggos{Section 3 to include briefly: What is the main technical contribution or our work? do we recover Telgarsky or ICLR/ICML? maybe only for classification error bounds? Maybe even for L1 in the special case of $L=\rho$?}


We give our main hardness results on the inapproximability of functions generated by repeated compositions of $f$ to itself when $f$ has certain cyclic behavior.
Section~\ref{ssec:lb-increasing} applies insights about chaotic itineraries to prove constant $L_\infty$ and $L_1$ lower bounds on the accuracy of approximating $f^k$ when $f$ has an increasing cycle.
Section~\ref{ssec:lb-odd} strengthens previous bounds on the number of oscillations when $f$ has an odd cycle, which is not necessarily increasing.
Appendix~\ref{asec:compare} presents Table~\ref{table:compare} that illustrates the key differences between results.


\subsection{Notation}
% Our plan is to use properties of the $p$-cycles of mappings $f$ in order to derive properties of $f^k$ and to establish the difficulty of approximating $f^k$ with neural networks. 
To measure the function complexity of $f^k$, we count the number of times $f^k$ oscillates. 
% To quantify the tendency of $f^k$ to oscillate, we develop ways to accurately count the number of monotone pieces $f^k$ has. 
%\cite{telgarsky16, cnpw19, cnp20, bzl20} show that counting the number of oscillations of $f^k$ is key to proving that it cannot be approximated by any polynomial-size shallow neural network.
We employ two notions of oscillation counts.
The first is relatively weak and counts every interval on which $f$ is either increasing or decreasing, regardless of its size.

\begin{definition}\label{def:osc}
    Let $f: [0, 1] \to [0, 1]$. $\oscm(f)$ represents the \emph{number of monotone pieces} of $f$. That is, it is the minimum $m$ such that there exists $x_0 = 0 < x_1 < \dots < x_{m-1} < x_m = 1$ where $f$ is monotone on $[x_{j-1}, x_{j}]$ for all $j\in [m]$.
\end{definition}

The second instead counts the number of times a fixed interval of size $b-a$ is crossed:

\begin{definition}\label{def:cross}
    Let $f: [0, 1] \to [0, 1]$ and $[a, b] \in [0,1]$. 
    $\osci{a,b}(f)$ represents the \emph{number of crossings} of $f$ on the interval $[a,b]$. 
    That is, it is the maximum $c$ such that there exist \[0 \leq x_1 < x'_1 \leq x_2 < x'_2 \leq \dots \leq x_c < x_c' \leq 1\] where for all $j \in [c]$, $f([x_j, x'_j]) \subset [a,b]$ and either $f(x_j) = a$ and $f(x'_j) = b$ or vice versa.
\end{definition}

\newcommand{\rhoinc}[1]{\rho_{\mathrm{inc}, #1}}
\newcommand{\rhoodd}[1]{\rho_{\mathrm{odd}, #1}}

\paragraph{Characteristic Polynomials} The base of the exponent of our width bounds is shown to equal the largest root of one of two polynomials:
\begin{align*}
    P_{\mathrm{inc}, p}(\lambda) &= \lambda^p - 2\lambda^{p-1} + 1, \\
    P_{\mathrm{odd}, p}(\lambda) &= \lambda^p - 2\lambda^{p-2} - 1.
\end{align*}
Let $\rhoinc{p}$ and $\rhoodd{p}$ be the largest roots of $P_{\mathrm{inc}, p}$ and $P_{\mathrm{odd}, p}$ respectively.
Table~\ref{table:rho_inc} illustrates that as $p$ grows, $\rhoinc{p}$ increases to 2, while $\rhoodd{p}$ drops to $\sqrt{2}$.
Note that $\rhoodd{p} \in (\sqrt{2}, \sqrt{2 + 2/2^{p/2}})$ \citep{alseda2000}.
We bound the growth rate of $\rhoinc{p}$ with the following: 

\begin{restatable}{fact}{factrootlb}\label{fact:root-lb}
    $\rhoinc{p} \in [\max(2 - \frac{4}{2^p}, \phi), 2)$, where $\phi = \frac{1+ \sqrt{5}}{2}$ is the Golden Ratio.
\end{restatable}

We prove Fact~\ref{fact:root-lb} in Appendix~\ref{assec:fact}.

% {\renewcommand{\arraystretch}{1.5}
\begin{table}[]
    \centering
     \caption{
     Approximate values of $\rhoinc{p}$, the lower bound on $\rhoinc{p}$ in Fact~\ref{fact:root-lb}, and $\rhoodd{p}$ (for odd $p$).\\}
    %  Explicit values of $\rho$ exponents that lower-bound the width needed for $f^k$ to be approximated by a shallow neural network when $f$ has an increasing $p$-cycle. By Lemma~\ref{lemma:increasing-constant-osc}, $\rho$ is the largest root of $\lambda^p - 2 \lambda^{p-1} + 1 = 0$ (approximately solved by WolframAlpha). We also include the lower bounds on $\rho$ given by Fact~\ref{fact:root-lb} and \cite{cnp20} (for any odd cycles), which is the largest root of $\lambda^p - 2\lambda^{p-2} -1 = 0$.\\}
    \begin{tabular}{|l|l|l|l|}
    \hline
    $p$  & $\rhoinc{p}$                              & Fact~\ref{fact:root-lb}   & $\rhoodd{p}$     \\ \hline\hline
    $3$  & $1.618$ & $1.618$ &  $1.618$  \\ \hline
    $4$  & $1.839$                        & $1.75$  & n/a \\ \hline
    $5$  & $1.928$                        & $1.875$ & $1.513$  \\ \hline
    $6$  & $1.966$                        & $1.938$ & n/a\\ \hline
    $7$  & $1.984$                        & $1.969$ & $1.466$\\ \hline
    $8$  & $1.992$                        & $1.984$ & n/a\\ \hline
    $9$  & $1.996$                        & $1.992$ & $1.441$\\ \hline
    $10$ & $1.999$                        & $1.996$ & n/a                 \\ \hline
    \end{tabular}
    \label{table:rho_inc}
\end{table}
% }

\subsection{Inapproximability of Iterated Functions with Increasing Cycles}\label{ssec:lb-increasing}

Our inapproximability results that govern the size of neural network $g$ necessary to adequately approximate $f^k$ when $f$ has an increasing cycle (like Theorem~\ref{thm:motivation-lb-inc}) rely on a key lemma that bounds the number of constant-size oscillations of $f^k$.

\begin{restatable}[Oscillation Bound for Increasing Cycles]{lemma}{lemmaincreasingconstantosc}\label{lemma:increasing-constant-osc}
    Suppose $f$ is a symmetric, concave unimodal mapping with an increasing $p$-cycle for some $p \geq 3$.
    % Let $\rho$ be the largest root of the polynomial equation $\lambda^{p} - 2\lambda^{p-1} + 1 = 0$.
    Then, there exists $[a,b] \subset [0, 1]$ with $b - a \geq \frac{1}{18}$ such that $\osci{a,b}(f^k) \geq \tfrac12\rhoinc{p}^k$ for all $k \in \N$.
\end{restatable}

We prove Lemma~\ref{lemma:increasing-constant-osc} in Appendix~\ref{assec:inc-constant-osc-proof}.
For an increasing $p$-cycle $x_1, \dots, x_p$, we lower-bound $\oscm(f^k)$ (the total number of monotone pieces, regardless of size) by relating the number of times $f^k$ crosses each interval $[x_j, x_{j+1}]$ to the number of crossings of $f^{k-1}$.
Doing so entails analyzing the largest eigenvalues of a transition matrix, which gives rise to the polynomial $P_{\mathrm{inc}, p}$.
We prove that the intervals crossed must be sufficiently large due to the symmetry, concavity, and unimodality of $f$.

\begin{remark}\label{remark:inc-close}
    If one does not wish to assume that $f$ is unimodal, symmetric, or concave, then the proof can be modified to show that $\osci{a,b}(f^k) = \Omega(\rho^k)$ for the same $\rho$, but for $a$ and $b$ dependent on $f$.
    These results are similar in flavor to those of \cite{cnpw19, cnp20, bzl20}, and they suffer from the same drawback: potentially vacuous approximation bounds when $a$ and $b$ are close.
    Appendix~\ref{assec:sym-conc} shows natural functions that are either not symmetric or not concave, whose oscillations shrink in size arbitrarily.
\end{remark}

%Our inapproximability results are consequences of this lemma and previous works' connections between the number of oscillations and the inapproximability of a neural network.

% \begin{restatable}{fact}{factrootlb}\label{fact:root-lb}
%     Let $\rho$ be the largest root of the polynomial equation $\lambda^{p} - 2\lambda^{p-1} + 1 = 0$.
%     Then, $\rho \in [\max(2 - \frac{4}{2^p}, \phi), 2)$, where $\phi = \frac{1+ \sqrt{5}}{2}$ is the Golden Ratio.
% \end{restatable}

\subsubsection{$L_\infty$ Approximation and Classification}
Our first result is a restatement of Theorem~\ref{thm:motivation-lb-inc} that quantifies inapproximability in terms of both $L_\infty$ and classification error, which are comparable to the respective results of \cite{bzl20} and \cite{cnpw19}.

\begin{theorem}\label{thm:main-linf}
    Suppose $f$ is a symmetric concave unimodal mapping with an increasing $p$-cycle for some $p \geq 3$.
    Then, any $k \in \N$ and $g\in \mathcal{N}(u, \ell)$ with $u \leq \frac{1}{8} \rhoinc{p}^{k/\ell}$ have
    $\norml[\infty]{f^k - g} = \Omega(1)$.
    
    Moreover, there exists $S$ with $\abs{S} = \frac{1}{2} \floorl{\rhoinc{p}^{k/\ell}}$ and $t \in (0,1)$ such that $\errcls{S,t}{f^k, g} \geq \frac{1}{4}.$
\end{theorem}
    The proof follows from our main Lemma~\ref{lemma:increasing-constant-osc} above and Theorem~\ref{thm:general-lb-cls}/Corollary~\ref{cor:general-lb-linf} in the Appendix (two previous inapproximability bounds based on oscillations).

Despite relying on unimodality assumptions and the existence of increasing cycles, Theorem~\ref{thm:main-linf} obtains much stronger bounds than its previous counterparts:
\begin{itemize}
    \item The assumption that $f$ has an increasing cycle causes a much larger exponent base for the width bound. 
    \cite{cnpw19, cnp20} only prove that the existence of 3-cycle mandates a width of $\Omega(\phi^{k/\ell})$.
    We exactly match that bound for $p=3$, and improve upon it when $p > 3$.
    As illustrated by Table~\ref{table:rho_inc}, increasing $p$ pushes the base $\rhoinc{p}$ rapidly to 2, which is the maximum exponent base for the increase of oscillations of any unimodal map. (And the maximal topological entropy of a unimodal map.)
    This also approximately matches the bases from \cite{bzl20}, which scale with the topological entropy of $f$.
    \item As illustrated in Appendix~\ref{assec:sym-conc}, the inaccuracy of neural networks with respect to the $L_\infty$ approximation in~\cite{cnpw19, cnp20,bzl20} may be arbitrarily small for certain choices of $f$. 
    Our unimodality assumptions ensure that the oscillations of $f^k$ are large and hence, that the inaccuracy of $g$ is constant.
\end{itemize}

% This result differs from and builds upon the two analogous results in multiple ways, despite requiring stronger assumptions of increasing periods.
% \begin{enumerate}
%     \item The result by \cite{bzl20} only shows that there exists some $\epsilon > 0$ that depends on $f$ such that 
%     \[\max_{x \in [0,1]} \abs{f(x) - g(x)} \geq \epsilon.\]
%     This means that there's no guarantee that the $L_\infty$ error---already a weak way of measuring error---is non-trivially large.
%     To contrast, we give a constant lower bound that does not depend on $f$ or $p$.
%     \item The classification error bounds from \cite{cnpw19} suffer from the same issue, because they permit the gaps between $f$ and $g$ to be infinitesimally small. Broadly, $L_\infty$ bounds improve upon these.
%     \item The results of \cite{cnpw19} correspond to the largest root $\rho'$ of another polynomial, $\lambda^{p-1} - \lambda^{p-2} - 1 = 0$. In the case $p = 3$, $\rho = \rho'$, and the terms perfectly match. However, their $\rho'$ strictly decreases as $p$ increases, while ours increases. We bound the rate of increase in \todo{lemma here}. Therefore, we are able to effectively incorporate the additional information about the itinerary of the cycles to obtain tighter bounds, which converge to $2$ as $p$ becomes large.
% \end{enumerate}

% We build on the inapproximability results of \cite{cnpw19, cnp20, bzl20} with a pair of theorems, each of which shows that the existence of an increasing $p$-cycle for any $p \geq 3$ in $f$ implies that any polynomial-width neural network cannot approximate $f^k$ when its depth is much smaller than $k$.


% \vaggos{x,y used to depend on f, period p but not number of iterations: this is a uniform bound: any function will lead to that separation}

% \vaggos{can we rephrase th.18 wrt to topological entropy? saying that we beat Harvard paper since our separation is constant?}

\subsubsection{$L_1$ Approximation}
We also strengthen the bound on $L_1$-inapproximability given by \cite{cnp20} by again introducing a stronger exponent and applying unimodality to yield a constant-accuracy bound.

\begin{theorem}\label{thm:main-l1}
    Consider any $L$-Lipschitz $f: [0,1] \to [0,1]$ with an increasing $p$-cycle for some $p \geq 3$.
    % Let $\rho$ be the largest root of the polynomial equation $\lambda^{p} - 2\lambda^{p-1} + 1 = 0$ and suppose $L = \rho$.
    If $L = \rhoinc{p}$, then for any $k \in \N$, any $g \in \mathcal{N}(u,\ell)$ with $u \leq \frac{1}{16} \rhoinc{p}^{k/\ell}$ has $\norml[1]{f^k - g} = \Omega(1).$
\end{theorem}

    The proof follows again using our main Lemma~\ref{lemma:increasing-constant-osc} and using Theorem~\ref{thm:general-lb-l1} in the Appendix.

% The analogous result in~\cite{cnp20} is somewhat diminished by the fact that \vaggos{they exhibit only one function -- stronger polynomial here} where the Lipschitzness constraint is met.
We make Theorem~\ref{thm:main-l1} more explicit by showing that many tent maps meet the Lipschitzness condition.
Let $\ftent{r} = 2r\min(x, 1-x)$ be the tent map, parameterized by $r \in (0,1)$
Our result improves upon~\cite{cnp20}, by obtaining constant approximation error and using the larger $\rhoinc{p}$ rather than $\rhoodd{p}$.

\begin{restatable}{corollary}{cormainl}\label{cor:main-l1}
    % For some $p \geq 3$, let $\rho_p$ be the largest root of the polynomial equation $\lambda^p - 2\lambda^{p-1} + 1 = 0$
    For any $p \geq 3$ and $k \in \N$, any $g \in \mathcal{N}(u,\ell)$ with $u \leq \frac{1}{16} \rhoinc{p}^{k/\ell}$ has $\norml[1]{\ftent{\rhoinc{p}}^k - g} = \Omega(1).$
\end{restatable}

We prove Corollary~\ref{cor:main-l1} in Appendix~\ref{assec:cor-main-proof}. The only non-trivial part of the proof involves proving the existence of an increasing $p$-cycle that causes $f^k$ to have $\Omega(\rhoinc{p}^k)$ oscillations.


% This bound is comparable to the $L_1$ bounds from \cite{cnp20}, with a few key caveats and improvements.
% The right-hand-size of the \cite{cnp20} lower bounds depend on the function $f$, so it may be arbitrarily small, rather than constant-valued as we have here.
% Their results only remain constant with the number of applications $k$ if the Lipschitz constant of the function equals $\rho$. 
% However, they only show that this holds when there is a super-stable 3-cycle; our results fulfill that condition for a broader range of cycles and the exponent approaches $2$ as $p$ becomes large, hence matching \cite{telgarsky16}.



\subsection{Improved Bounds for Odd Periods}\label{ssec:lb-odd}

While Theorems~\ref{thm:main-linf} and \ref{thm:main-l1} give stricter bounds on the width of neural networks needed to approximate iterated functions $f^k$ than \cite{cnpw19, cnp20}, they also require extra assumptions about the cycles---namely, that the cycles are increasing.
However, more powerful inapproximability results with constant error are still possible even without additional assumptions.
Specifically, we leverage unimodality to improve the desired inaccuracy to a constant without compromising width.
% That is, the degree of inapproximability is a constant, rather than a term that may depend on $f$ and $p$.

As before, the results hinge on a key technical lemma that bounds the number of interval crossings.

\begin{restatable}{lemma}{lemmaoddconstantosc}\label{lemma:odd-constant-osc}
    For some odd $p \geq 3$, suppose $f$  is a symmetric concave unimodal mapping with an odd $p$-cycle.
    % Let $\rho$ be the largest root of the polynomial equation \[\lambda^p - 2\lambda^{p-2} - 1 = 0.\]
    Then, there exists $[a,b] \subset [0, 1]$ with $b - a \geq 0.07$ such that $\osci{a,b}(f^k) = \rhoodd{p}^{k-p}$ for any $k \in \N$.
\end{restatable}

We prove Lemma~\ref{lemma:odd-constant-osc} in Appendix~\ref{assec:lemma-odd-proof}. The challenging part is to find a lower bound on the length of the intervals crossed.


Like before, we provide lower-bounds on approximation up to a constant degree.

\begin{theorem}\label{thm:odd-linf}
    For some odd $p \geq 3$, suppose $f$ is a symmetric, concave unimodal mapping with any $p$-cycle.
    % Let $\rho$ be the largest root of the polynomial equation $\lambda^p - 2\lambda^{p-2} - 1 = 0.$
    Then, any $k \in \N$ and any $g \in \mathcal{N}(u,\ell)$ with $u \leq \frac{1}{8} \rhoodd{p}^{(k-p)/\ell}$ have
    $\norml[\infty]{f^k - g} = \Omega(1).$
    
    Moreover, there exists $S$ with $\abs{S} = \frac{1}{2} \floorl{\rhoodd{p}^k}$ and $t \in (0,1)$ such that 
    $\errcls{S,t}{f^k, g} \geq \frac{1}{4}.$
    % \clayton{do we need classification part?}
\end{theorem}
    The proof is immediate from Lemma~\ref{lemma:odd-constant-osc}, Theorem~\ref{thm:general-lb-cls}, and Corollary~\ref{cor:general-lb-linf} in the Appendix.

We also get the analogous result but for the $L_1$ error:

\begin{theorem}\label{thm:odd-l1}
    Consider any $L$-Lipschitz $f: [0,1] \to [0,1]$ with a $p$-cycle for some odd $p \geq 3$.
    % Let $\rho$ be the largest root of the polynomial equation \[\lambda^p - 2\lambda^{p-2} - 1 = 0\] and suppose $L \leq \rho$.
    If $L = \rhoodd{p}$, then, any $k \in \N$ and $g \in \mathcal{N}(u,\ell)$ with $u \leq \frac{1}{16} \rhoodd{p}^{(k-p)/\ell}$ have $\norml[1]{f^k - g} = \Omega(1).$
\end{theorem}

    The proof is immediate from Lemma~\ref{lemma:increasing-constant-osc} and Theorem~\ref{thm:general-lb-l1} in the Appendix.

% \begin{remark}
% Corollary~4.4.22 of~\cite{alseda2000} implies that for any odd $p$, $\rho$ defined above satisfies 
% \[\rho \in \paren{\sqrt{2}, \sqrt{2 + \frac{2}{2^{p/2}}}}.\]
% \end{remark}

% \todo{maybe also give $L_1$ lower bounds for super-stable tent map odd periods}
%\vaggos{add comment for high dimensions and semialgebraic gates? - quickly}

==> Beyond Sharkovsky Paper/phase.tex <==
\section{Periods, Phase Transitions and Function Complexity}\label{sec:phase}

We formalize the correspondence between different notions of function complexity in dynamical systems and learning theory: neural network approximation, oscillation count, cycle itinerary, topological entropy, and VC-dimension.
We make Theorem~\ref{thm:informal-phase} rigorous by presenting two regimes into which unimodal mappings can be classified---the \emph{doubling regime} and the \emph{chaotic regime}---and show that all of these measurements of complexity hinge on which regime a function belongs to.\footnote{These two regimes correspond to different settings of the parameters $r$ in the bifurcation diagram of Figure~\ref{fig:bifurcation} in the Appendix. The doubling regime is the left-hand-side, where the stable periods routinely split in two before the first chaos is encountered. The chaotic regime is to the right-hand-side, which is characterized by chaos punctuated by intermittent stability.}



% \subsection{Phase Transition for Unimodal Mappings}
% Based on the connections drawn by \cite{bzl20} and the previous theorems, these can be shown to correspond to inapproximability results for neural networks.
% We prove two theorems, each corresponding to the two regimes that $f$ may belong to: the \textit{doubling regime} and the \textit{chaotic regime}.
Some components of the claims regarding the topological entropy are the immediate consequences of other results; however, we include them to give a complete picture of the gap between the two regimes.
To the best of our knowledge, we believe the bound on monotone pieces of $f^k$ in the doubling regime and both VC-dimension bounds below to be novel.

We define VC-dimension and introduce topological entropy in Appendix~\ref{asec:phase}, along with the proofs of both theorems.
For VC-dimension, we consider the hypothesis class $\hyp{f,t} := \{\thres{t}{f^k}: k \in \mathbb{N}\}$, which corresponds to the class of iterated fixed maps.
%\vaggos{top. entropy result may not come as a surprise for someone in Dyn. Sys. but prior results BZL give shrinking bounds nevertherless...}
% \todo{Note that the width of the doubling interval is zero for the tent mapping\dots first theorem is more interesting to maps like logistic}

\begin{restatable}{theorem}{thmpropertiesdoubling}[Doubling Regime]\label{thm:properties-doubling}
    Suppose $f$ is a symmetric unimodal mapping whose maximal cycle is a primary cycle of length $p = 2^q$. That is, there exists a $p$-cycle but no $2p$-cycles (and thus, no cycles with lengths non-powers-of-two). Then, the following are true:
    \begin{enumerate}
        \item For any $k \in \N$, $\oscm(f^k) = O((4k)^{q+1})$.
        \item For any $k \in \N$, there exists $g \in \mathcal{N}(u,2)$ with $u= O((4k)^{q+1}/\eps)$ such that $\norm[\infty]{g - f^k} \leq \epsilon$. 
        Moreover, if $f = \ftent{r}$, then there exists $g \in \mathcal{N}(u,2)$ with $u = O((4k)^{q+1})$ and $g = f^k$.
        \item $\htop(f) = 0$.
        \item For any $t \in (0, 1)$, $\vc(\hyp{f, t}) \leq 18p^2$.
    \end{enumerate}
\end{restatable}


\begin{restatable}{theorem}{thmpropertieschaotic}[Chaotic Regime]\label{thm:properties-chaotic}
    Suppose $f$ is a unimodal mapping that has a $p$-cycle where $p$ is not a power-of-two. Then, the following are true:
    \begin{enumerate}
        \item There exists some $\rho \in (1, 2]$ such that for any $k \in \N$, $\oscm(f^k) = \Omega(\rho^k)$.
        \item For any $k \in \N$ and any $g \in \mathcal{N}(u,\ell)$ with $\ell \leq k$ and $u \leq \frac{1}{8} \rho^{k/\ell}$, there exist samples $S$ with $\abs{S}= \frac12 \floor{\rho^k}$ such that $\errcls{S, 1/2}{f^k, g} \geq \frac14$.
        \item $\htop(f) \geq \rho > 0$.
        \item There exists a $t \in (0,1)$ such that $\vc(\hyp{f, t}) = \infty$.
    \end{enumerate}
\end{restatable}

\begin{remark}\label{remark:non-primary}
    As discussed in Appendix~\ref{asec:itineraries}, any non-primary cycle implies the existence of a cycle whose length is not a power of two. Thus, these results also apply if there exists any non-primary power-of-two cycle, such as the 1234-itinerary 4-cycle.
\end{remark}

%\begin{remark}
 %   Bullet point 2 of Theorem~\ref{thm:properties-chaotic} is far from the strongest claim in this paper about neural network inapproximability of chaotic mappings.
  %  Theorems~\ref{thm:main-linf}, \ref{thm:main-l1}, \ref{thm:odd-linf}, and \ref{thm:odd-l1} enhance the study of the chaotic regime by providing more powerful lower bounds on the numbers of oscillations of $f^k$ and stricter hardness results for neural networks approximation, but they require more assumptions. 
%\end{remark}

% \vaggos{it's cool that oscillations and VC bounds they correlate. finite-PO2 vs infinite-odd: massive phase transitions happening in both complexity measure: interesting for future work, draw from Dynamical Systems literature.}

==> Beyond Sharkovsky Paper/prelims.tex <==
% \section{Preliminaries}

% \subsection{Notation}
% For $f, g: [0,1] \to [0,1]$, let
% \[\norm[1]{f - g} = \int_{0}^1 \abs{f(x) - g(x)} dx\]
% and
% \[\norm[\infty]{f - g} = \sup_{x \in [0, 1]} \abs{f(x) - g(x)}.\]

% For $x \in [0,1]$, let $\round_t(z) = \indicator{z \geq t}$ and $\round(z) = \round_{1/2}(z)$.

% For some threshold $t \in [0,1]$, $n \in \N$, and sample $S = \{(x_i, y_i) \in [0,1] \times \bit: i \in [n]\}$, we let the \textit{classification error} of $f$ be
% \[\errcls{S,t}{f} = \frac{1}{n} \sum_{i=1}^n \indicator{y_i = \round_t(f(x))}.\]

% Let $[m] = \{1, 2, \dots, m\}$.

% \subsection{Discrete Dynamical Systems}
% We construct hard functions for neural networks to approximate and investigate the function complexity properties of a family of iterated one-dimensional maps, $f^k$, for some function $f:[0,1]\to[0,1]$.
% Borrowing from the literature on discrete dynamical systems \cite{mss73}, we limit ourselves to a certain class of mappings---which we refer to as \textit{unimodal mappings}---that yield nice dynamical systems properties.

% \begin{definition}
%     $f: [0,1]\to[0,1]$ is a \textit{unimodal mapping} if it fulfills the following characteristics:
%     \begin{enumerate}
%         \item $f$ is continuous and piece-wise differentiable on $[0,1]$.
%         \item $f(x) > 0$ for all $x \in (0,1)$ and $f(0) = f(1) = 0$.
%         \item There exists some $x_{\max}$ that uniquely maximizes $f$. $f$ is strictly increasing on the interval $[0, x_{\max})$ and decreasing on $(x_{\max},1]$.
%     \end{enumerate}
%     Periodically, we will need to make additional assumptions about $f$ for our results to hold. We say that $f$ is a \textit{concave} unimodal mapping if $f$ is also concave on $[0,1]$, and that $f$ is a \textit{symmetric} unimodal mapping if $f(x) = f(1-x)$ for all $x \in [0, 1]$.
% \end{definition}

% Two very standard unimodal mappings that are symmetric and concave are the \textit{logistic mapping} and the \textit{tent mapping} defined respectively as:
%  \[\flog{r}(x) = 4r x(1 - x)\] and  \[\ftent{r}(x) = \begin{cases}2rx & x \leq \frac{1}{2} \\ 2r(1 - x) & x \geq \frac{1}{2} \end{cases},\] 
%  Though trivial, they will serve as guiding examples for building intuition throughout the paper. They are both  parameterized by $r \in (0, 1]$ and studying their phase transitions as the parameter $r$ changes will be illuminating for understanding the chaotic itineraries.


% As shown in recent papers on the intersection of machine learning and discrete dynamical systems \cite{cnpw19, cnp20}, the periodicity of a unimodal mapping corresponds to key properties such as the number of monotone pieces of $f^k$.
% We define those concepts.

% \begin{definition}
%     $x^*$ is a \textit{fixed point} if $f(x^*) = x^*$.
%     For any $p > 1$, $x^*$ is a \textit{$p$-cyclic} point if $f^p(x^*) = x^*$ and $f^q(x^*) \neq x^*$ for all $q < p$.
%     We say that $f$ has a \textit{$p$-cycle} if there exists $p$ points $x_1, \dots, x_p$ such that $f(x_i) = x_{i+1}$ for $i \in [p-1]$ and $f(x_p) = x_1$.
% \end{definition}

% Sharkovsky's Theorem proves a clear relationship between the various periodicities of some mapping $f$. 
% It provides an ordering on the natural numbers such that if $p$ precedes $q$ in the ordering, then the existence of a $q$-cycle implies the existence of a $p$-cycle

% \begin{theorem}
%     \todo{Sharkovksy's goes here!}
%     \vaggos{I will write Sharkovsky and explain in intro.}
% \end{theorem}

% Past results \cite{cnpw19, cnp20} apply Sharkovsky's Theorem to show that the existence of a certain cycle in a mapping $f$ implies that $f^k$ will be difficult to approximate.
% Our key results are to show that more information than just the length of the cycle is relevant to determining the complexity of $f$ (and hence, the hardness of approximation). 
% We define a notion of \textit{cycle itinerary}, which we rely on heavily when proving our bounds.

% \clayton{Let's call these ``patterns'' instead and write them as permutations rather than L/Rs. e.g. $(1,2,3,4,5)$ instead of $L^4R$.}

% \begin{definition}
%     Consider some $p$-cycle $x_1, \dots, x_p$. 
%     The \textit{itinerary} of this cycle is some string of length $a \in \{L, C, R\}^p$, where 
%     \[a_i := \begin{cases}
%         L & x_i < x_{\max} \\
%         C & x_i = x_{\max} \\
%         R & x_i > x_{\max}.
%     \end{cases}\]
% \end{definition}

% \begin{remark}
%     This is slightly different notation than the notion used in Table~1 of \cite{mss73}, which focuses on only the itineraries of cycles that contain a $C$ and represents a $p$-cycle with a string of length $p-1$.
% \end{remark}



% The story of cycles in discrete dynamical systems can be shown to be more complex than just what is indicated in Sharkovsky's theorem.
% The application of Sharkovsky's Theorem in \cite{cnpw19, cnp20} non-power-of-two cycles are in $f$ are key to showing that $f^k$ is hard to approximate by neural networks.
% In this work, we illustrate that this is only a small piece of the puzzle and that the trajectory of the cycles matter too.
% Certain power-of-two cycles are more indicative of $f^k$ being hard to approximate than $f$; for instance, the existence of an $L^3R$ 4-cycle gives more powerful approximation bounds than the existence of a 3-cycle.

% Since cycles of the form $L^{p-1}R$ and $L^{p-2}CR$ will be frequently considered in this work, we give them a name.

% \begin{definition}
%     $f$ has an \textit{increasing $p$-cycle} if it has a $p$-cycle with $x_1 < x_2 < \dots < x_p$.
% \end{definition}
% If $f$ is unimodal, we can show that a cycle is an increasing $p$-cycle if and only if its itinerary is $L^{p-1}R$, $L^{p-2}CR$, or $L^{p-2}R^2$. \todo{prove this/refer to appendix}





% \begin{itemize}
%     \item Cycle itineraries and order from \cite{mss73}. Note that it's first a bunch of PO2 cycles (doubling regime) and then a bunch of others (chaotic regime). First cycles appear in order of Sharkovsky's thoerem. Cycles never go away as scaling parameter increases. Final stable cycle of period $p$ is $L^{p-1}R$. (Lemma 3 of OC, ideally with less notation involved)
% \end{itemize}

% \clayton{Idea: one of the things we'll have trouble with here is that the proofs are more cumbersome than the ideas. For instance, the MSS73 chart implies on inspection that a cycle of the form $RL^{p-1}$ implies the existence of one of the form $RL^{p-2}$. But it's somewhat cumbersome to prove. 

% Maybe we can define a list of heuristic rules in a section that hold and motivate them, which can encapsulate concepts that are a pain to prove but easy to observe via MSS or visuals. When describing the proof we can refer back to these kinds of heuristics to make it easier to understand, while still including all of the rigor in other areas.}

% \subsection{Number and Size of Oscillations}
% Our plan is to use properties of the $p$-cycles of mappings $f$ in order to derive properties of $f^k$ and to establish the difficulty of approximating $f^k$ with neural networks. 
% To measure the function complexity of $f^k$, we primarily rely on the number of times $f^k$ oscillates. To quantify the tendency of $f^k$ to oscillate, we develop ways to accurately count the number of monotone pieces $f^k$ has. 

% %\cite{telgarsky16, cnpw19, cnp20, bzl20} show that counting the number of oscillations of $f^k$ is key to proving that it cannot be approximated by any polynomial-size shallow neural network.

% We employ two notions of oscillation counts.
% The first is a weak notion, which counts every interval on which $f$ is either increasing or decreasing, regardless of how large this interval is.

% \begin{definition}\label{def:osc}
%     Let $f: [0, 1] \to [0, 1]$. We let $\oscm(f)$ represent the \emph{number of monotone pieces} of $f$. That is, it is the minimum $m$ such that there exists $x_0 = 0 < x_1 < \dots < x_{m-1} < x_m = 1$ such that $f$ is monotone on $[x_j, x_{j+1}]$ for all $j\in \{0\}\cup[m-1]$.
% \end{definition}

% The second instead counts the number of times a certain interval of size $b-a$ is crossed:

% \begin{definition}\label{def:cross}
%     Let $f: [0, 1] \to [0, 1]$ and $[a, b] \in [0,1]$. We let $\osci{a,b}(f)$ represent the \emph{number of crossings} of $f$ on the interval $[a,b]$. 
%     That is, it is the maximum $c$ such that there exist \[0 \leq x_1 < x'_1 \leq x_2 < x'_2 \leq \dots \leq x_c < x_c' \leq 1\] such that for all $j \in [c]$, $f([x_j, x'_j]) \subset [a,b]$ and either $f(x_j) = a$ and $f(x'_j) = b$ or vice versa.
% \end{definition}

%\subsection{Neural Networks}

%\todo{brief definition of ReLU neural network of some width and depth}

%\vaggos{We should add a small paragraph to compare L1, classification, $L_\infty$ and constant-gap-$L_\infty$ just to clarify the different regimes. It's nice here to include a "historical" review of how recent papers (Telgarsky's, ours, Harvard, others, current) tried to obtain bounds for these different problems...}



==> Beyond Sharkovsky Paper/supp_compare.tex <==
\section{Comparison with Prior Works}\label{asec:compare}

Given the large number of results presented in this paper and the many axes of comparison one can draw between these results and their predecessors in \cite{telgarsky16, cnpw19, cnp20}, we provide Table~\ref{table:compare} to illuminate these comparisons.
It reinforces our key contributions, namely that (1) the presence of increasing cycles makes a function more difficult to approximate than a 3-cycle alone; (2) requiring that $f$ satisfy unimodality constraints gives lower-bounds to constant accuracy that cannot be made vacuous by adversarial choices of $f$; and (3) the key distinction between ``hard'' and ``easy'' functions is the existence of non-primary power-of-two cycles.




\begin{table}[]
{\renewcommand{\arraystretch}{1.25}
\scalebox{0.72}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|p{3.8cm}|}
\cline{2-11}
                                  & \textbf{Condition}                        & \textbf{Approx.}    & \textbf{Unimodal?} & \textbf{Concave?} & \textbf{Symmetric?} & \textbf{$L\leq\rho$?} & \textbf{Acc.}          & \textbf{Exp.}               & \textbf{Hard?} & \textbf{Source}                                                                      \\ \hline
\multicolumn{1}{|l|}{\textbf{1}}  & \textbf{Maximal PO2}                      & \textbf{$L_\infty$} & \textbf{Yes}       & \textbf{No}       & \textbf{Yes}        & \textbf{No}        & \textbf{$\Omega(1)$}   & \textbf{Any}                & \textbf{No}    & \textbf{Thm~\ref{thm:properties-doubling}}                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{2}}  & $\htop(f) \geq \rho$                      & $L_\infty$          & No                 & No                & No                  & No                 & $\epsilon(f)$          & $\rho$                      & Yes            &BZL~Thm~16                                                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{3}}  & \textbf{Non-primary}                      & \textbf{Cls.}       & \textbf{No}        & \textbf{No}       & \textbf{No}         & \textbf{No}        & \textbf{$\frac{1}{4}$} & \textbf{$(1, \phi]$}        & \textbf{Yes}   & \textbf{CNPW~Thm~1.6, Remark~\ref{remark:non-primary}}                      \\ \hline
\multicolumn{1}{|l|}{\textbf{4}}  & \textbf{Non-primary}                      & \textbf{$L_\infty$} & \textbf{No}        & \textbf{No}       & \textbf{No}         & \textbf{No}        & \textbf{$\epsilon(f)$} & \textbf{$(1, \phi]$}        & \textbf{Yes}   & \textbf{CNPW~Thm~1.6, Remark~\ref{remark:non-primary}, BZL~Thm~16} \\ \hline
\multicolumn{1}{|l|}{\textbf{5}}  & Non-PO2                                   & Cls.                & No                 & No                & No                  & No                 & $\frac{1}{4}$          & $(1, \phi]$                 & Yes            & CNPW~Thm~1.6                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{6}}  & Non-PO2                                   & $L_\infty$          & No                 & No                & No                  & No                 & $\epsilon(f)$          & $(1, \phi]$                 & Yes            & CNPW~Thm~1.6, BZL~Thm~16                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{7}}  & Odd cycle                                 & Cls.                & No                 & No                & No                  & No                 & $\frac{1}{4}$          & $(\sqrt{2}, \phi]$          & Yes            & CNP~Thm~1.1                                                                 \\ \hline
\multicolumn{1}{|l|}{\textbf{8}}  & Odd cycle                                 & $L_\infty$          & No                 & No                & No                  & No                 & $\epsilon(f)$          & $(\sqrt{2}, \phi]$          & Yes            & CNP~Thm~1.1, BZL~Thm~16                                            \\ \hline
\multicolumn{1}{|l|}{\textbf{9}}  & \textbf{Odd cycle}                        & \textbf{$L_\infty$} & \textbf{Yes}       & \textbf{Yes}      & \textbf{Yes}        & \textbf{No}        & \textbf{$\Omega(1)$}   & \textbf{$(\sqrt{1}, \phi]$} & \textbf{Yes}   & \textbf{Thm~\ref{thm:odd-linf}}                                                      \\ \hline
\multicolumn{1}{|l|}{\textbf{10}} & Odd cycle                                 & $L_1$               & No                 & No                & No                  & Yes                & $\epsilon(f)$          & $(\sqrt{2}, \phi]$          & Yes            & CNP~Thm~1.2                                                                 \\ \hline
\multicolumn{1}{|l|}{\textbf{11}} & {$\ftent{\rho_p/2}$} & {$L_1$}      & {Implied}   & {Implied}  & {Implied}    & {Implied}   & {$\Omega(1)$}   & {$(\sqrt{2}, \phi]$}        & {Yes}   & {CNP~Lemma~3.6}                                                       \\ \hline

\multicolumn{1}{|l|}{\textbf{12}} & \textbf{Odd cycle}                        & \textbf{$L_1$}      & \textbf{Yes}       & \textbf{Yes}      & \textbf{Yes}        & \textbf{Yes}       & \textbf{$\Omega(1)$}   & \textbf{$(\sqrt{2}, \phi]$} & \textbf{Yes}   & \textbf{Thm~\ref{thm:odd-l1}}                                                        \\ \hline
\multicolumn{1}{|l|}{\textbf{13}} & \textbf{Inc. Cycle}                       & \textbf{Cls.}       & \textbf{No}        & \textbf{No}       & \textbf{No}         & \textbf{No}        & \textbf{$\frac{1}{4}$} & \textbf{$[\phi,2)$}         & \textbf{Yes}   & \textbf{Thm~\ref{thm:main-linf}, Remark~\ref{remark:inc-close}}                      \\ \hline
\multicolumn{1}{|l|}{\textbf{14}} & \textbf{Inc. Cycle}                       & \textbf{$L_\infty$} & \textbf{No}        & \textbf{No}       & \textbf{No}         & \textbf{No}        & \textbf{$\epsilon(f)$} & \textbf{$[\phi,2)$}         & \textbf{Yes}   & \textbf{Thm~\ref{thm:main-linf}, Remark~\ref{remark:inc-close}}                      \\ \hline
\multicolumn{1}{|l|}{\textbf{15}} & \textbf{Inc. Cycle}                       & \textbf{$L_\infty$} & \textbf{Yes}       & \textbf{Yes}      & \textbf{No}         & \textbf{No}        & \textbf{$\Omega(1)$}   & \textbf{$[\phi,2)$}         & \textbf{No}    & \textbf{Prop~\ref{prop:need-symmetry}}                                               \\ \hline
\multicolumn{1}{|l|}{\textbf{16}} & \textbf{Inc. Cycle}                       & \textbf{$L_\infty$} & \textbf{Yes}       & \textbf{No}       & \textbf{Yes}        & \textbf{No}        & \textbf{$\Omega(1)$}   & \textbf{$[\phi,2)$}         & \textbf{No}    & \textbf{Prop~\ref{prop:need-concavity}}                                              \\ \hline
\multicolumn{1}{|l|}{\textbf{17}} & \textbf{Inc. Cycle}                       & \textbf{$L_\infty$} & \textbf{Yes}       & \textbf{Yes}      & \textbf{Yes}        & \textbf{No}        & \textbf{$\Omega(1)$}   & \textbf{$[\phi,2)$}         & \textbf{Yes}   & \textbf{Thm~\ref{thm:main-linf}}                                                     \\ \hline
\multicolumn{1}{|l|}{\textbf{18}} & \textbf{Inc. Cycle}                       & \textbf{$L_1$}      & \textbf{No}        & \textbf{No}       & \textbf{No}         & \textbf{Yes}       & \textbf{$\epsilon(f)$} & \textbf{$[\phi,2)$}         & \textbf{Yes}   & \textbf{Thm~\ref{thm:main-l1}, CNP~Thm~1.2}                                 \\ \hline
\multicolumn{1}{|l|}{\textbf{19}} & \textbf{Inc. Cycle}                       & \textbf{$L_1$}      & \textbf{Yes}       & \textbf{Yes}      & \textbf{Yes}        & \textbf{Yes}       & \textbf{$\Omega(1)$}   & \textbf{$[\phi,2)$}         & \textbf{Yes}   & \textbf{Thm~\ref{thm:main-l1}}                                                       \\ \hline
\multicolumn{1}{|l|}{\textbf{20}} & \textbf{$\ftent{\rho_p/2}$} & \textbf{$L_1$}      & \textbf{Implied}   & \textbf{Implied}  & \textbf{Implied}    & \textbf{Implied}   & \textbf{$\Omega(1)$}   & \textbf{$[\phi, 2)$}        & \textbf{Yes}   & \textbf{Cor~\ref{cor:main-l1}}                                                       \\ \hline
\multicolumn{1}{|l|}{\textbf{21}} & $\ftent{1}$                               & $L_1$               & Implied            & Implied           & Implied             & Implied            & $\Omega(1)$            & 2                           & Yes            & Telgarsky                                                                  \\ \hline
\end{tabular}}}
\caption{Compares the conditions and limitations of the theoretical results presented in this paper and its predecessors. New results are bolded.}
\label{table:compare}
\end{table}

We provide context for each column to clarify what its cells mean and how to compare their values.

\begin{itemize}
    \item ``\textbf{Condition}'' specifies what must be true of the complexity of $f$ in order for the relevant bounds to occur. All but the latter two conditions describe a very broad array of functions, while the last two focus only on a restricted subset of tent mappings.
    \begin{itemize}
        \item ``Maximal PO2'' means that the maximal cycle of $f$ is a primary\footnote{See Appendix~\ref{assec:order}.} $p$-cycle where $p$ is a power of two. This means that $f$ lies in the doubling regime described in Theorem~\ref{thm:properties-doubling}.
        \item ``$\htop(f) \geq \rho$'' considers any $f$ with a lower-bound on its topological entropy for some $\rho > 1$. Notably, all conditions other than ``Maximal PO2'' satisfy this for some $\rho$.
        \item ``Non-primary'' means that any non-primary cycle exists in $f$. That is, if $f$ is known to have a non-primary power-of-two cycle, then the results apply. 
        \item ``Non-PO2'' refers to any $f$ that has a $p$-cycle where $p$ is not a power of two.
        \item ``Odd cycle'' includes any $f$ that has a $p$-cycle where $p$ is odd.
        \item ``Inc. cycle'' means that $f$ has an increasing $p$-cycle for some $p$, i.e. a cycle with itinerary $12\dots p$.
        \item $\ftent{\rho_p/2}$ refers to families of tent maps scaled by $\rho_p$ solving the polynomials from \cite{cnp20} Lemma~3.6 (for odd periods) and Corollary~\ref{cor:main-l1} (for increasing cycles).
        \item The last row refers exclusively to the tent map of height 1 and slope 2.
    \end{itemize}

    \item ``\textbf{Approx.}'' refers to how difference between neural network $g$ and iterated map $f^k$ is measured. 
    The options are $L_1$, $L_\infty$, and classification error.
    It's easier to show that $g$ can $L_1$-approximate $f^k$ than it is to show that $g$ can $L_\infty$-approximate $f$; conversely, it's most impressive to show lower bound results with respect to the $L_1$ error than it is for the $L_\infty$ error.
    
    \cite{cnpw19, cnp20} consider classification error, \cite{bzl20} focus on $L_\infty$ approximation, and \cite{cnp20} also consider $L_1$ approximation. We routinely translate classification errors to $L_\infty$ errors using Corollary~\ref{cor:general-lb-linf}, which draws on Theorem~16 of \cite{bzl20}.
    
    \item ``\textbf{Unimodal?},'' ``\textbf{Concave?},'' and ``\textbf{Symmetric?},'' have ``Yes'' if and only if $f$ must meet the respective property for the proof to hold. 
    They have ``Implied'' if the value of ``Condition'' already ensures that the property is satisfied and the requirement need not be enforced.
    
    \item ``$L \leq \rho$?'' is ``Yes'' if the results only hold if $f$ is chosen with a Lipschitz constant less than the rate of growth of its oscillations. This is a very restrictive condition met by very few functions (including no logistic maps with cycles).
    
    \item ``\textbf{Acc.}'' specifies the desired accuracy of the hardness result. ``$\Omega(1)$'' means that there exists some constant $\epsilon$ such that for any choice of $f$ in the category, any neural network $g$ will be unable to approximate $f$ up to accuracy $\epsilon$.
    ``$\eps(f)$'' means that the degree of approximation may depend on the chosen function $f$ (and the period $p$) that belongs to the category; these bounds may be vacuous by an adversarial choice of $f$.
    As a result, hardness results with ``$\Omega(1)$'' are more impressive.
    
    \item ``\textbf{Exp.}'' refers to the base of the exponent of the lower-bound on the width necessary to approximate $f^k$ using a shallow network $g$.
    Larger values indicate stronger bounds.
    
    \item ``\textbf{Hard?}'' is ``Yes'' if for every $f$ satisfying the conditions to the left, $f$ cannot be approximated up to the specified accuracy by any neural network $g$.
    It is ``No'' if there exists some $f$ satisfying the conditions that can be approximated to a stronger degree of accuracy.
    
    \item ``\textbf{Source}'' denotes where to find the result. Some of the less interesting results are not given their own theorems and rather are immediate implications of several theorems across this body of literature. For the sake of space, we use ``CNPW'' to refer to \citep{cnpw19}; ``CNP'' for \citep{cnpw19}; ``BZL'' for \citep{bzl20}; and ``Telgarsky'' for \citep{telgarsky16}.
\end{itemize}

==> Beyond Sharkovsky Paper/supp_doubling.tex <==
\section{Additional Proofs for Section~\ref{sec:phase}}\label{asec:phase}

\subsection{Preliminaries}

Before reintroducing and proving the theorems about the doubling and chaotic regime, we introduce topological entropy and define VC-dimension.

\subsubsection{Topological Entropy}
Topological entropy is a well-known measure of function complexity in dynamical systems that measures the ``bumpiness'' of a mapping. 
Like we do with chaotic itineraries, \cite{bzl20}~draw analogies between the neural network approximability of $f^k$ and the topological entropy of $f$.
We do not give a rigorous definition of topological entropy, but we include a well known result connecting topological entropy to the number of monotone pieces (not constant-sized crossings), which is stated as Lemma~3 of the aforementioned work.

\begin{lemma}\label{lemma:htop}[\cite{mw80, young81}]
    If $f:[0,1]\to[0,1]$ is continuous and piece-wise monotone, then the topological entropy of $f$ satisfies the following:
    \[\htop(f) = \lim_{k \to \infty} \frac{1}{k} \log \oscm(f^k).\]
\end{lemma}

\subsubsection{VC-Dimension}
We capture the complexity of the mappings produced by repeated application of $f$, by measuring the capability of a family of iterates to fit arbitrarily-labeled samples with the VC-dimension. 
For some threshold parameter $t \in (0, 1)$, we first define a hypothesis class  that we use to cast this family of iterated functions as Boolean-valued.

\begin{definition}
    For some unimodal $f: [0,1]\to[0,1]$ and threshold $t \in (0,1)$, let \[\hyp{f,t} := \{\thres{t}{f^k}: k \in \mathbb{N}\}\]
    be the Boolean-valued hypothesis class of classifiers of composed functions.
\end{definition}

The following is the standard definition of the VC-dimension:

\begin{definition}[\cite{vc13}]
    For some hypothesis class $\mathcal{H}$ containing functions $[0,1] \to \{0,1\}$, we say that $\mathcal{H}$ \emph{shatters} samples $x_1, \dots, x_d \in [0,1]$ if for every labeling of the samples $\sigma_1, \dots, \sigma_d \in \bit$, there exists some $h\in \mathcal{H}$ such that $h(x_i) = \sigma_i$ for all $i \in [d]$. 
    The \emph{VC-dimension} of $\mathcal{H}$, $\vc(\mathcal{H})$ is the maximum $d$ such that there exists $x_1, \dots, x_d \in [0,1]$ that $\mathcal{H}$ shatters.
\end{definition}

$\vc(\hyp{f,t})$ will be a useful measurement of complexity of the mapping $f$, which as we show is tighly connected with the notion of periodicity and oscillations. 
Notably, this is a measurement of the complexity of iterated maps and is \textit{not} a typical formulation of VC-dimension for neural networks, since those typically would consider a fixed depth and a fixed width, but variable values for the weights, rather than fixed $f$ and variable $k$.


% \vaggos{check with prior work on topological entropy and VC dimension: maybe different classes?}

% \section{SUPPLEMENT TO PROOF OF THEOREM~\ref{thm:properties-doubling}}

\subsection{Proof for Theorem~\ref{thm:properties-doubling} and \ref{thm:properties-chaotic}}

\thmpropertiesdoubling*
\begin{proof}
    Claim 1 follows from a somewhat involved argument in Appendix~\ref{assec:doubling-monotone} that uses an inductive argument to compare the behavior of a mapping with a maximal $p$-cycle to one with a maximal $\frac{p}{2}$-cycle.
    By categorizing intervals of $[0,1]$ based on how $f^k$ behaves on that interval, we analyze how $f^{k+1}$ in turn behaves, which leads to a bound on the monotone pieces $\oscm(f^k)$.
    
    Claim 2 is a simple consequence of Claim 1, by using the fact that a ReLU network can piecewise approximate each monotone piece of $f^k$.
    This argument appears in Appendix~\ref{assec:doubling-nn}.
    
    Claim 3 follows easily from Claim 1 and Lemma~\ref{lemma:htop}. We note that this derivation about the topological entropy and the periodicity of $f$ is a known fact in the dynamical systems community.
    
    Claim 4 relies on another recursive argument that frames VC-dimension in terms of the possible trajectories of $f^k(x)$ for fixed $x$ and changing $k$. 
    We characterize these trajectories by making use of Regular Expressions and by bounding the corresponding VC dimension in Appendix~\ref{assec:doubling-vc}.
\end{proof}

\thmpropertieschaotic*
\begin{proof}
    Claims 1 and 2 are immediate implications Theorems~1.5 and 1.6 of~\cite{cnpw19}.
    Claim 3 follows by applying Lemma~\ref{lemma:htop} to Claim 1 (again this derivation about the topological entropy is basic in the literature on dynamical systems).
    
    The most interesting part of the theorem is the last claim. We prove Claim 4 in Appendix~\ref{asec:chaotic} by showing that the VC-dimension of the class is at least $d$ for all $d \in \N$.
    The argument relies on the existence of an infinite number of cycles of other lengths, as guaranteed by Sharkovsky's Theorem.
\end{proof}


\subsection{Proof of Theorem~\ref{thm:properties-doubling}, Claim 1}\label{assec:doubling-monotone}

We restate Claim~1 of the theorem as the following proposition and prove it.

\begin{proposition}[Claim 1 of Theorem~\ref{thm:properties-doubling}]\label{prop:properties-doubling-osc}
    Suppose $f$ is a symmetric unimodal mapping whose maximal cycle is of length $p = 2^q$. Then, for any $k \in \N$, $M(f^k) = O((4k)^{q+1})$.
\end{proposition}

In order to bound the number of times $f$ oscillates based on its power-of-two periods, we categorize $f$ by its cyclic behavior and the bound the number of local maxima and minima $f$ has based on its characterization.

\begin{definition}[Category]
    For $q \geq 0$ and $z \in \bit$, let $\category{q,z}$ contain the set of all symmetric unimodal functions $f$ such that (1) $f$ has a $2^q$-cycle, (2) $f$ does not have a $2^{q+1}$-cycle, and (3) $\thres{1/2}{f^{2^q}(\frac{1}{2})} = z$.
    % In addition, let $\category{-1, z}$ contain all such functions that do not have a fixed point. 
\end{definition}

% Note that $\category{-1, 1} = \emptyset$ because the any $f$ with $f(\frac{1}{2}) \geq \frac{1}{2}$ and $f(1) = 0$ must contain a fixed point on the interval $[\frac{1}{2}, 1]$.

We abuse notation to let $\oscm(\category{q,z}^k) = \max_{f \in \category{q,z}} \oscm(f^k)$.
Thus, for $f$ given in the theorem statement with a $2^q$-cycle, but not a $2^{q+1}$-cycle, our final bound is obtained by 
\[\oscm(f^m) \leq \max\{\oscm(\category{q,0}^m), \oscm(\category{q,1}^m)\}.\]
We let $\oscm(f, a, b)$ represent the number of monotone pieces of $f$ on the sub-interval $[a, b] \subset [0, 1]$. 

We build a large-scale inductive argument by first bounding base cases $\oscm(\category{0,0}^k)$ and $\oscm(\category{0, 1}^k)$. 
Then, we relate $\oscm(\category{q, z}^k)$ to $\oscm(\category{q-1, 1-z}^k)$ to get the desired outcome. 

Before beginning the proof, we state a slight refinement of the part of the theorem, which takes into account the newly-introduced categories, from which the claim follows.
\begin{proposition}\label{prop:osc-category-bound}
For any $k \in \N$, $q\geq 0$, and $z \in \bit$, 
\[\oscm(\category{q, z}^k) \leq \begin{cases}
   2(3q)^k & \text{$q$ is even, $z = 0$, or $q$ is odd, $z = 1$}\\
   2(3q)^{k+1} & \text{$q$ is even, $z = 1$, or $q$ is odd, $z = 0$}.
\end{cases}\]
\end{proposition}

Thus, proving Proposition~\ref{prop:osc-category-bound} is sufficient to prove Proposition~\ref{prop:properties-doubling-osc}.
The remainder of the section proves Proposition~\ref{prop:osc-category-bound}.

\subsubsection{Special Case Proof for $q =1$}\label{sec:ub-special-case}
We show that $\oscm(\category{0,0}^k) = 2$ and $\oscm(\category{0,1}^k) = 2k$.

For $f_r$ as defined above, we characterize the number of oscillations that are added by increasing $r$ past $\frac{1}{2}$, where super-stability of a fixed point exists.
Figure \ref{fig:ub-specific} illustrates those results.

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{fig/fig-ub-specific-0.png}
    \includegraphics[width=0.49\textwidth]{fig/fig-ub-specific-1.png}
    \caption{The base case results of  Proposition~\ref{prop:osc-category-bound} demonstrate the number of oscillations of $f^k$ increases when $f$ moves from $\category{0, 0}$ to $\category{0, 1}$.
    The plots show $f$ and $f^5$ for $f \in \category{0, 0}$ ($f = \flog{0.45}$) on the left and $f \in \category{0,1}$ ($f =\flog{0.775}$) on the right.}
    \label{fig:ub-specific}
\end{figure}

To analyze the oscillation patterns of $f^k$, we define several ``building blocks,'' which  represent disjoint pieces of $f^k$.
That is, the interval $[0,1]$ can be partitioned into several sub-intervals, each of which has $f^k$ follow certain simple behavior that we categorize.
We argue that any iterate can be decomposed into those pieces and then show how applying $f$ to $f^{k}$ modifies the pieces in order to analyze $f^{k+1}$. 
Here are the function pieces that we analyze, which map interval $[a, b] \subseteq [0, 1]$ to $[0, 1]$:
\begin{definition}
    For any $f: [0, 1] \rightarrow [0, 1]$ and for any $[a, b] \subseteq [0, 1]$, $f$ is referred to on interval $[a, b]$ as:
    \begin{itemize}
        \item a \textbf{increasing crossing piece} $\ic$ if $f$ is strictly increasing on $[a, b]$ and has $f(a) = 0$, $f(b) > \frac{1}{2}$, and $f'(b) > 0$;
        \item a \textbf{decreasing crossing piece} $\dc$ if $f$ is strictly decreasing on $[a,b]$ and has $f(a) > \frac{1}{2}$, $f(b) = 0$, and $f(a) < 0$;
        \item a \textbf{up peak} $\up$ if there exists some $c \in (a, b)$ that maximizes $f$ on $[a,b]$, $f$ is strictly increasing on $[a, c)$, $f$ is strictly decreasing on $(c, b]$, and $f(x) > \frac{1}{2}$ for all $x \in [a, b]$;
        \item a \textbf{up valley} $\uv$ if there exists some $c \in (a, b)$ that minimizes $f$ on $[a,b]$, $f$ is strictly decreasing on $[a, c)$, $f$ is strictly increasing on $(c, b]$, and $f(x) > \frac{1}{2}$ for all $x \in [a, b]$; and
        \item a \textbf{down peak} $\dpk$ if there exists some $c \in (a, b)$ that maximizes $f$ on $[a,b]$, $f$ is strictly increasing on $[a, c)$, $f$ is strictly decreasing on $(c, b]$, and $f(x) \leq \frac{1}{2}$ for all $x \in [a, b]$.
    \end{itemize}
    If there exists a sequence of intervals $J_1, \dots, J_m$ such that $f$ is piece $\eta_i$ on $J_i$, then we represented $f$ with the string $\eta_1 \dots \eta_m$.
\end{definition}

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{fig/fig-ub-specific-classifications.png}
    \caption{For $f\in\category{0,1}$ ($f = \flog{0.775}$), visualizes the decomposition of $f$, $f^2$, and $f^3$ into $\ic\up\dc$, $\ic\up\uv\up\dc$, and $\ic(\up\uv)^2\up\dc$ respectively.}
    \label{fig:ub-specific-classification}
\end{figure}

We specify an invariant for each part of the theorem, such that proving the invariant is sufficient to prove the proposition:
\begin{enumerate}
    \item If $f \in \category{0, 0}$, then $f^k$ is a down peak on $[0,1]$ for all $k$, and $f^k$ has two monotone pieces.
    \item If $f \in \category{0, 1}$, $f$ is represented by $\ic(\up\uv)^{k-1}\up\dc$. That is, $[0, 1]$ can be partitioned into $2k + 1$ subsequent intervals $J_1, \dots J_{2k+1}$ such that $f^k$ is an increasing crossing piece on $J_1$, a decreasing crossing piece on $J_{2k+1}$ (if $k \neq 0$), an up peak on $J_{2j}$ for $j \in \{1, \dots, k\}$, and a up valley on $J_{2j + 1}$ for $j \in \{1, \dots, k-1\}$.
    Hence, $f^k$ has $k$ distinct maxima and $2k$ monotone pieces.
    Figure \ref{fig:ub-specific-classification} illustrates this invariant.
\end{enumerate}

% Because $f$ is continuous, it follows that $f^k$ is continuous. %Then, we can find that local maxima correspond exactly with high peak and low peak segments in the above constructions.\footnote{There may need to be a more rigorous argument made here.}

\textbf{Base Case:}
\begin{enumerate}
    \item For $f\in\category{0,0}$, $f^1 = f$ is trivially a down peak on $[0, 1]$ by the definition of $\category{0,0}$, since $\frac{1}{2}$ maximizes $f$.
    \item For $f\in\category{0,1}$, $f$ can be represented by $\ic\up\dc$. That is, $[0, 1]$ can be decomposed into intervals $I_1$, $I_2$, and $I_3$, on which $f_r$ is an increasing crossing piece, an up peak, and a decreasing crossing piece respectively.
\end{enumerate}

\textbf{Inductive Step:}

We examine what happens to each function piece when $f$ is applied to it. We can use the following analysis, along with the inductive hypothesis to show that $f^{k+1}$ can be decomposed as we expect it to be.
\begin{enumerate}
    \item Examining the \textbf{down peak} proves first invariant for the case when $f\in \category{0,0}$. Because $f$ strictly increases on $[0, \frac{1}{2}]$ and because $f([0, 1]) \subseteq [0, \frac{1}{2}]$ if $f^k$ is a down peak, $f \circ f^k$ also supports a down peak on $[0, 1]$.
    
    Because we inductively assume that $f^k$ is a low peak on $[0, 1]$, it then follows that $f^{k+1}$ is also a down peak on $[0, 1]$.

    \item 
    We first prove a claim, which implies that $f$ has no down peaks for $f \in \category{0,1}$. Let $\xmax = f(\frac{1}{2})$,
    \begin{claim}
    If $f \in \category{0,1}$, then $f((\frac{1}{2}, \xmax]) \subseteq (\frac{1}{2}, \xmax]$.
    \end{claim}
    \begin{proof}
    Because $\frac{1}{2}$ maximizes $f$, $f(x) \leq \xmax$ for all $x \in [\frac{1}{2}, \xmax]$.
    Since $f$ monotonically decreases, on $[\frac{1}{2}, \xmax]$, the claim can only be false if $f(\xmax) < \frac{1}{2}$.
    We show by contradiction that this is impossible.
    
    Because $f$ is continuous and monotonically increases on $[0, \frac{1}{2}]$ and ranges from $0$ to $\xmax \geq \frac{1}{2}$, there exists some $x' \leq \frac{1}{2}$ such that $f(x') = \frac{1}{2}$ and $f^2(x') = \xmax$.
    
    Let $g(x) = f^2(x) - x$.
    By assumption, $g(\frac{1}{2}) = f(\xmax) - \frac{1}{2} < 0$. 
    By definition of $x'$, $g(x') = \frac{1}{2} - x' \geq 0$.
    Because $g$ is continuous, the Intermediate Value Theorem implies the existence of $x'' \in [x', \frac{1}{2})$ such that $g(x'') = 0$ and $f^2(x'') = x''$.
    Since $f$ has no two-cycles, it must be the cause that $f(x'') = x''$ and $x'' = \frac{1}{2}$.
    However, this contradicts our finding that $x'' < \frac{1}{2}$, which means that $f(\xmax) \geq \frac{1}{2}$ and the claim holds.
    \end{proof}
    
    Now, we proceed with analyzing each of the function pieces on some interval $[a, b] \subseteq [0, 1]$ when $f \in \category{0,1}$. The transformations are visualized in Figure \ref{fig:ub-specific-classification}. 
    
    \begin{itemize}
        \item \textbf{Increasing crossing piece}: If $f^k$ has an $\ic$ on $[a,b]$, then $f^{k+1}$ can be represented by $\ic\up$ on $[a,b]$. 
        
        There exist $c$ and $d$ such that $a < d < c < \frac{1}{2} < b$, $f^k(c) = \frac{1}{2}$, and $f^k(d) = c $. Then, $[a, \frac{1}{2}(c + d)]$ supports an increasing crossing piece on $f \circ f^k$---because $f(f^k(a)) = 0$, $f(f^k(\frac{1}{2}(c + d))) > \frac{1}{2}$, and $f \circ f^k$ is strictly increasing on that interval since $f$ is increasing before reaching $\frac{1}{2}$. $[0.5(c + d), b]$ supports a high peak---because $c$ is a local maxima on $f \circ f^k$, and $f \circ f^k$ is strictly increasing before $c$ and strictly decreasing after $c$.
        \item \textbf{Decreasing crossing piece}: For the same arguments, $f^{k+1}$ can represented by $\up\dc$ on $[a,b]$ if $f^k$ is represented by $\dc$ on $[a,b]$.
        \item \textbf{Up peak}: Because $f$ strictly decreases for $x > \frac{1}{2}$ and because $f^k([a, b]) \subseteq (\frac{1}{2}, \xmax]$ if $\up$ represents $f^k$ on $[a, b]$, $c$ becomes a local minimum for $f \circ f^k$, and $f^{k+1}$ is a high valley $\uv$ on $[a,b]$.
        \item \textbf{Up valley}:  Because $f$ strictly decreases for $x > \frac{1}{2}$ and because $f^k([a, b]) \subseteq (\frac{1}{2}, \xmax]$ if $\uv$ represents $f^k$ on $[a, b]$, $c$ becomes a local maximum for $f \circ f^k$, and $f^{k+1}$ is a high peak $\up$ on $[a,b]$.
    \end{itemize}
    
    Now, consider the inductive hypothesis. Because $f^k$ can be represented by $\ic(\up\uv)^{k-1}\up\dc$, applying the above transformations to each piece implies that $f^{k+1}$ can be represented by $\ic(\up\uv)^{k}\up\dc$. Hence, the inductive argument goes through.
\end{enumerate}


\subsubsection{General Case Proof}\label{sec:ub-general-case}
The argument proceeds inductively.
We show that if we have some $f \in \category{q,k}$, then we can find some other function $h \in \category{q-1,1-k}$ and characterize the behavior of $f$ in terms of the behavior of $h$.

Since we assume that $q \geq 1$, there will always exist some $x^* > \frac{1}{2}$ that is a fixed point of $f$.\footnote{Sharkovsky's Theorem yields this by showing that the existence of a $2^q$-cycle implies the existence of any $2^j$-cycle, for all $j \in \{0, \dots, q-1\}$. $x^* > \frac12$ by our assumption that a 2-cycle $x_1 < x_2$ exists. It must be true that $x_2 > \frac{1}{2}$; otherwise, $f(x_2) > x_2 > x_1$, which breaks the cycle. Because $f(\frac{1}{2}) > \frac{1}{2}$ and $f(x_2) < x_2$, there exists $x^* \in (\frac{1}{2}, x_2)$ such that $f(x^*) = x^*$ by the Intermediate Value Theorem.}
By symmetry, $f(1- x^*) = x^*$.
Let $\phi:[0,1] \to [1-x^*, x^*]$ be a decreasing isomorphism with $\phi(x) = x^* - x(2x^* - 1)$, and let
\[h = \phi^{-1} \circ f^2 \circ \phi.\]
$h$ is a useful construct, because its behavior resembles simpler versions of $f$, with fewer cycles and oscillations. We use properties of $h$ to relate pieces of $f^k$ to those of $h^{k/2}$. 
We illustrate this recursive and fractal-like behavior in Figure \ref{fig:ub-general-hr}.

Note that $h^k = \phi^{-1} \circ f^{2k} \circ \phi$.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{fig/fig-ub-general-hr.png}
    \caption{Visualizes the analogy between mappings in $\category{q, z}$ and $\category{q-1,1-z}$. The left plots the first 4 iterates of $f= \flog{0.9} \in \category{4, 1}$ (has a maximal 4-cycle with $f^4(\frac{1}{2}) > \frac{1}{2}$), while the right plots those of $f = \flog{0.85} \in \category{2,0}$ (has a maximal 2-cycle with $f^2(\frac{1}{2}) < \frac{1}{2}$. The purple highlighted regions on the left behave qualitatively similar to $\flog{0.85}$, while the green regions are similar to $\flog{0.85}^2$.}
    \label{fig:ub-general-hr}
\end{figure}

\begin{lemma}\label{lemma:doubling-h}
    $h$ is a symmetric unimodal mapping with $h \in \category{q-1, 1-z}$.
\end{lemma}
\begin{proof}
We verify the conditions for $f$ to be unimodal mapping.
\begin{enumerate}
    \item $h$ is continuous and piece-wise differentiable on $[0, 1]$ because $f^2$ is, and $h$ is merely a linear transformation of $f^2$.
    
    \item $h(0) = h(1) = 0$. $h((0, 1))$ is strictly positive because $f((1- x^*, x^*)) = (x^*, \xmax)$, $f^2((1- x^*, x^*)) = (f(\xmax), x^*)$, and $f(\xmax) < f(x^*) = x^*$ by $f$ being decreasing on $[\frac{1}{2}, 1]$.
    
    \item $h$ is uniquely maximized by $\frac{1}{2}$ because $\frac{1}{2}$ minimizes $f^2$ on the interval $[1 - x^*, x^*]$. 
    $f$ maps both $[1-x^*, \frac{1}{2}]$ and $[\frac{1}{2}, x^*]$ onto $[x^*, \xmax]$ and is increasing and decreasing on the respective intervals.
    Because $f$ maps $[x^*, \xmax]$ onto $[f(\xmax), x^*]$ and $f(\xmax) < x^*$ and is decreasing on $[x^*, \xmax]$, $f^2$ is increasing on $[1-x^*, \frac{1}{2}]$ and decreasing on $[\frac{1}{2}, x^*]$.
    
    Thus, $h$ is maximized by $\frac{1}{2}$, increases before $\frac{1}{2}$, and decreases after $\frac{1}{2}$.
        
    \item We must also show that $h$ is well-defined, which entails proving that $h(x) \leq 1$ for all $x \in [0, 1]$. 
    Suppose that were not the case. 
    Then, $h(\frac{1}{2}) > 1$, and there exists some $x' \leq \frac{1}{2}$ with $h(x') = 1$.
    There also exists some $x^{**} \in [1-x', 1]$ with $h(x^{**}) = x^{**}$ by the Intermediate Value Theorem.

    Let $g(x) = h^3(x) - x$ and note that $g$ is continuous on $[0, x']$. 
    Observe that $g(1-x^{**}) = 2x^{**} - 1 > 0$ and $g(x') = -x' < 0$.
    Thus, there exists $x'' \in [1 - x^{**}, x']$ with $g(x'') = 0$.
    Because $h$ is increasing on $[0, x']$ and $x' > 1 - x^{**}$, it must be the case that $h(x') > x^{**} > x'$.
    Thus, $x^{**}$ is not a fixed point and must be on a 3-cycle in $h$.
    
    However, if $x^{**}$ is on a 3-cycle in $h$, then $\phi(x^{**})$ must be part of a 6-cycle in $f$.
    This contradicts the assumption that $f$ cannot have a $2^{q+1}$-cycle, because Sharkovsky's Theorem states that a 6-cycle implies a $2^{q+1}$-cycle.

\end{enumerate}

We show that $h$ is symmetric.
    \begin{align*}
        h(x)
        &= \phi^{-1}(f^2(\phi(x))) 
        = \phi^{-1}( f^2(1 - \phi(x)))
        = \phi^{-1}(f^2(1 - x^* + x(2x^* - 1))) \\
        &= \phi^{-1}(f^2(x^* - (1-x)(2x^* - 1)))
        = \phi^{-1}(f^2(\phi(1-x))) = h(1-x).
    \end{align*}
    
If $f^{2^{q}}(\frac{1}{2}) \geq \frac{1}{2}$, then $h^{2^{q-1}}(\frac{1}{2}) \leq \frac{1}{2}$, and if $f^{2^{q}}(\frac{1}{2}) \leq \frac{1}{2}$, then $h^{2^{q-1}}(\frac{1}{2}) \geq \frac{1}{2}$. Thus, $\thres{1/2}{h^{2^{q-1}}(\frac{1}{2})} = \thres{1/2}{f^{2^q}(\frac{1}{2})}$.
By Lemma~\ref{lemma:hr-super-stable}, $h$ has a $2^{q-1}$-cycle and does not have a $2^{q}$-cycle. Thus, $h \in \category{q-1, 1-z}$.
\end{proof}

\begin{lemma}\label{lemma:hr-super-stable}
    For $p \in \mathbb{Z}_{+}$, $h$ has a $p$-cycle if and only if $f$ has a $2p$-cycle.
\end{lemma}
\begin{proof}
    Suppose $x_1, \dots, x_p$ is a $p$-cycle for $h$. Then,
    $\phi(x_1), \dots ,\phi(x_p)$
    is a $p$-cycle for $f^2$. 
    If $x_1, \dots, x_p$ are distinct, then so must be $\phi(x_1), \dots ,\phi(x_p)$, since $\phi$ is an isomorphism.
    Thus, 
    \[\phi(x_1), f(\phi(x_1)), \dots, \phi(x_p), f(\phi(x_p))\]
    is a $2p$-cycle for $f$.
    
    Conversely, if $x_1, \dots, x_{2p}$ is a $2p$-cycle for $f$, then $x_1, x_3, \dots, x_{2p-1}$ is a $p$-cycle for $f^2$ and 
    \[\phi^{-1}(x_1), \dots, \phi^{-1}(x_{2p})\]
    is a $p$-cycle for $h$.
\end{proof}

We proceed with a proof similar in structure to the one in the last section, where we divide each $f^{k}$ into intervals and monitor the evolution of each as $k$ increases. We define the classes of the pieces of some 1-dimensional map $f^{k}$ on interval $[a, b]$ below. We visualize these classes in Figure \ref{fig:ub-general-classification}.
\begin{itemize}
    \item $f^{k}$ is an \textbf{approach} $\app$ on $[a, b]$ if $f$ is strictly increasing, $f^{k}(a) = 0$, and $f^{k}(b) = 1-x^*$.
    \item Similarly, $f^{k}$ is a \textbf{departure} $\dep$ on $[a, b]$ if $f^k$ is strictly decreasing, $f^k(a) = 1-x^*$, and $f^k(b) = 0$.
    \item $f^{k}$ is an \textbf{$i$-Left Valley} $\lv_i$ on $[a, b]$ if $f^{k}:[a, b] \rightarrow [f(\xmax), x^*]$ and if there exists some strictly increasing and bijective $\sigma: [a, b] \rightarrow [1 - x^*, x^*]$ such that $f^{k} = \phi \circ h^i \circ \phi^{-1} \circ \sigma$ on $[a, b]$. Note that $f^{k}(a) = f^{k}(b) = x^*$---unless $i = 0$, in which case $f^k(a) = 1-x^*$ and $f_r^k(b) = x^*$.
    \item $f^{k}$ is analogously a \textbf{$i$-Right Valley} $\rv_i$ if the same condition holds, except that $\sigma$ is strictly decreasing.
    \item $f^{k}$ is an \textbf{$i$-Left Peak} $\lp_i$ on $[a, b]$ if $f^{k-1}$ is $\lv_{i-1}$ on $[a, b]$. It follows that $f^{k}:[a, b] \rightarrow [x^*, \xmax]$, that there exists some $c \in [a, b]$ such that $f^{k}(c) = \xmax$ (because $\frac{1}{2} \in [f(\xmax), x^*]$), and that $f^{k}(a) = f^{k}(b) = x^*$.
    \item $f^{k}$ is an \textbf{$i$-Right Peak} $\rp_i$ on $[a, b]$ if $f^{k-1}$ is $\rv_{i-1}$ on $[a, b]$. The same claims hold as $\lp_i$.
 \end{itemize}
 
 \begin{figure}
     \centering
     \includegraphics[width=0.6\textwidth]{fig/fig-ub-general-classifications.png}
     \caption{Similar to Figure~\ref{fig:ub-specific-classification}, visualizes the classifications of $f, f^2, f^3, f^4$ for $f=\flog{0.9} \in \category{4,1}$, and demonstrates that the decompositions are $\app\lv_0\lp_0\rv_0\dep$, $\app\lv_0\lp_1\lv_1\rp_1\rv_0\dep$, $\app\lv_0\lp_1\lv_1\lp_2\rv_1\rp_1\rv_0\dep$, and $\app\lv_0\lp_1\lv_1\lp_2\lv_2\rp_2\rv_1\rp_1\rv_0\dep$ respectively.}
     \label{fig:ub-general-classification}
 \end{figure}
 
 Now, the proof of the number of oscillations proceeds in two steps. (1) We analyze how each of the above pieces evolves with each application of $f$. (2) We show how many maxima and minima each translates to.
 
\begin{lemma}\label{lemma-piece-decomposition}
     When $f \in \category{q,z}$ for $q \geq 1$ and for all $k \in \mathbb{Z}_{+}$, $f^k$ can be decomposed into $2k + 3$ pieces $\eta_1, \dots, \eta_{2k + 3}$ such that
     \[\text{$\eta_i$ is }
     \begin{cases}
        \text{$\app$ if $i = 1$} \\
        \text{$\lv_j$ if $i = 2j + 2$ for $j \in \{0, 1, \dots, \floor{k / 2}\}$} \\
        \text{$\lp_j$ if $i = 2j + 1$ for $j \in \{1, \dots, \floor{(k+1)/2}\}$} \\
        \text{$\rv_j$ if $i = 2k - 2j + 2$ for $j \in \{0, 1, \dots, \floor{(k-1)/ 2}\}$} \\
        \text{$\rp_j$ if $i = 2k - 2j + 3$ for $j \in \{1, \dots, \floor{k/2}\}$} \\
        \text{$\dep$ if $i = 2k + 3$} \\
     \end{cases}\]
     
     That is, if $k$ is even, then $f$ can be represented by \[\app \lv_0 \lp_1 \lv_1 \dots \lv_{k/2 - 1} \lp_{k/2} \lv_{k/2} \rp_{k/2} \rv_{k/2 - 1} \dots \rv_1 \rp_2 \rv_0\dep.\]
     If $k$ is odd, then $f$ is represented by
     \[\app \lv_0 \lp_1 \lv_1 \dots \lp_{(k-1)/2} \lv_{(k-1)/2}\lp_{(k+1)/2} \rv_{(k-1)/2} \rp_{(k - 1)/2} \dots \rv_1 \rp_2 \rv_0\dep.\]
\end{lemma}
\begin{proof}
    This lemma is proved inductively. $f$ can be decomposed into the pieces $\app\lv_0 \lp_1\rv_0 \dep$.
    \begin{itemize}
        \item 
        By unimodality and symmetry, $f$ is strictly increasing on $[0, \frac{1}{2})$ and strictly decreasing on $(\frac{1}{2}, 1]$. 
        There exists some $x_1$ such that $[0, x_1]$ is strictly increasing and $f(x_1) = 1 - x^*$ (because $1 - x^* < x^* < \xmax$). Thus, $f$ is $\app$ on $[0, x_1]$.
        Similarly, $[1-x_1, 1]$ is strictly decreasing and $f(1- x_1) = 1 - x^*$, which implies that $f$ is $\dep$ on $[1-x_1, 1]$.
        
        \item Note that $x_1 < 1 - x^* < x^* < 1-x_1$, and $f$ is increasing on $[x_1, 1 - x^*]$ and decreasing on $[x^*, 1-x_1]$. 
        
        Because $[x_1, 1 - x^*]$ is monotone, there exists continuous and increasing $\sigma: [x_1, 1 - x^*] \rightarrow [1 - x^*, x^*]$ such that $f(x) = \sigma(x)$. Since $h^0$ is the identity map, it trivially also holds that $f(x) = \phi(h^0(\phi^{-1}(\sigma(x))))$. Because $f(x_1) = 1 - x^*$ and $f(x^*) = x^*$, it follows that $f$ is $\lv_0$ on $[x_1, 1- x^*]$.
        
        By a similar argument, $f$ is $\rv_0$ on $[x^*, 1-x_1]$, with the only difference being that $\sigma$ needs to be strictly decreasing for it to hold.
        \item $[1-x^*, x^*]$ is $\lp_1$ because $[1-x^*, x^*]$ is $\lv_0$ on the identity map $f^0$. This trivially holds using the identity $\sigma$ map.
    \end{itemize}
    
    Now, we prove the inductive step, which can be summed up by the following line:
    \[\app \rightarrow \app \lv_0; \dep \rightarrow \rv_0\dep; \lv_j \rightarrow \lp_{j+1}; \lp_j \rightarrow \lv_j; \rv_j \rightarrow \rp_{j+1}; \rp_j \rightarrow \rv_j.\]
    We show each part of the relationship as follows:
    \begin{itemize}
        \item If $f^k$ is $\app$ on $[0, b]$, then there exists some $c \in (0, b)$ such that $f^{k+1}(c) = 1 - x^*$ because $f^k$ is an isomorphism between $[0, b]$ and $[0, x^*]$.
        
        It follows that $f^{k+1}$ is $\app$ on $[0, c]$ because $f^{k+1}$ is strictly increasing on the interval from $0$ to $1 - x^*$.
        
        $[c, b]$ is $\lv_0$ because there must exist some increasing $\sigma$ such that $f^{k+1}(x) = \sigma(x)$ on that interval. Thus, it follows that $f^{k+1} = \phi\circ h^0 \circ \phi^{-1}\circ \sigma$ on $[0,b]$.
        
        \item The same argument holds for $\dep$. If $f^k$ is $\dep$ on $[a, 1]$, then there exists $c \in (a, 1)$ such that $[a, c]$ is $\rv_0$ and $[c, 1]$ is $\dep$.
        
        \item If $f^k$ is $\lv_j$ on $[a, b]$, then $f^{k+1}$ is $\lp_{j+1}$ on the same interval by the definition of $\lp_{j+1}$.
        
        \item Similarly, if $f^k$ is $\rv_j$ on $[a, b]$, then $f^{k+1}$ is $\rp_{j+1}$ on the same interval by the definition of $\rp_{j+1}$.
        
        \item If $f^k$ is $\lp_j$ on $[a, b]$, then $f^{k-1}$ is $\lv_{j-1}$ and hence $f^{k-1}$ maps to $[f(\xmax), x^*]$ on the interval. Therefore, there exists $\sigma$ such that $f^{k-1} = \phi \circ h^{j-1} \circ \phi^{-1} \circ\sigma$ on the interval. We use the properties of $h$ to show that $f^{k+1}$ is $\lv_{j}$ on $[a, b]$. Note that $f^2 = \phi \circ h \circ \phi^{-1}$ on $[f(\xmax), x^*]$.
        % \begin{align*}
        %     f^{k+1}(x)
        %     &= f^2(f_r^{k-1}(x)) 
        %     = \phi(h(\phi^{-1}(\phi(h^{j-1}(\phi^{-1}(\sigma(x)))))))
        %     = \phi(h^{j}(\phi^{-1}(\sigma(x))))
        % \end{align*}
        \begin{align*}
            f^{k+1}
            &= f^2 \circ f^{k-1}
            = \phi \circ h\circ \phi^{-1} \circ \phi \circ h^{j-1}\circ\phi^{-1}\circ\sigma
            = \phi\circ h^{j}\circ\phi^{-1}\circ\sigma
        \end{align*}
        Thus, $f^{k+1}$ satisfies the condition to be $\lv_j$.
        \item By a identical argument, if $f^k$ is $\rp_j$ on $[a, b]$, then $f^{k+1}$ is $\rv_{j}$.
    \end{itemize}
    The remainder of this argument follows by applying the above transition rules for each piece to the inductive hypothesis about the ordering of pieces in $f^k$ to obtain the ordering for $f^{k+1}$.
\end{proof}

Now, we determine how many local maxima and minima are contained in each type of piece. Let $\maxima(f)$ and $\minima(f)$ represent the number of local maxima and minima respectively on mapping $f$ on interval $[0,1]$. We bound the total number of monotone pieces with these bounds by using $\oscm(f) = 2 \maxima(f)$. We similarly abuse notation to bound the number of maxima and minima in a category with $\maxima(\category{q,z}^k)$ and $\minima(\category{q,z}^k)$, and in the interval $[a,b]$ with $\maxima(f, a,b)$ and $\minima(f, a,b)$. 

By the base case in the previous section $\maxima(\category{0,0}^k) = 1$, $\minima(\category{0,0}^k) = 2$, $\maxima(\category{0,1}^k) = k,$ and $\minima(\category{0,1}^k) = k+1$. We obtain recurrences to represent $\maxima(\category{q,z}^k)$ and $\minima(\category{q,z}^k)$.

For each part, we rely on the following facts: If $\sigma$ is a strictly increasing bijection, then $\maxima(f \circ \sigma, a, b) = \maxima(f,a ,b)$. If $\sigma$ is strictly decreasing, then $\minima(f \circ \sigma, a, b) = \maxima(f,a ,b)$. (The reverse are true for minima of $f$.)

We analyze each type of piece individually, considering what happens when $f$ has some kind of piece on interval $[a, b]$.

\begin{itemize}
    \item Because $\app$ and $\dep$ segments are strictly increasing or decreasing, $\maxima(f, a, b) = 0$ when $f$ has either piece on $[a,b]$. $\minima(f, a,b) = 1$ because segments that support $\app$ contain $0$ and segments with $\dep$ have $1$, each of which $f$ maps to 0.
    \item Because each $\lv_i$ segment of $f^k$ on $[a,b]$ can be represented as $\phi \circ h^{i} \circ \phi^{-1} \circ \sigma$, and because $\phi$ is strictly decreasing, $\maxima(f_r^k, a, b) = \minima(h^i)$ and $\minima(f_r^k, a, b) = \maxima(h^i)$.
    By Lemma~\ref{lemma:doubling-h}, $h \in \category{q-1, 1-z}$, $\maxima(f_r^k, a, b) \leq \minima(\category{q-1, 1-z}^i)$ and $\minima(f_r^k, a, b) \leq \maxima(\category{q-1, 1-z}^i)$.
    
    The same analysis holds for each $\rv_i$ segment. 
    
    \item 
    Consider an $\lp_i$ segment of $f^k$ on $[a, b]$, which has output spanning the interval $[x^*, \xmax]$. Because $x^* > \frac{1}{2}$, $f$ is strictly decreasing on the domain $[x^*, \xmax]$. Thus, $f^{k+1}$ must satisfy $\maxima(f_r^{k+1},a, b) = \minima(f_r^{k},a, b)$ and $\minima(f_r^{k+1},a, b) = \maxima(f_r^{k},a, b)$.
    
    Note by the definition of $\lp_i$ that $[a,b]$ must also support an $\lv_{i-1}$ segment on $f^{k-1}$ and an $\lv_{i}$ segment on $f^{k+1}$. 
    From the previous bullet, the $\lv_i$ segment must have at most $\minima(\category{q-1, 1-z}^i)$ maxima and $\maxima(\category{q-1, 1-z}^i)$ minima. 
    Because there must be a one-to-one correspondence between minima of $f^{k+1}$ and maxima of $f^{k}$ on the interval and vice versa, the $\lp_i$ segment has $\maxima(f_r^k, a, b) \leq \maxima(\category{q-1, 1-z}^i)$ and $\minima(f_r^k, a, b) \leq \minima(\category{q-1, 1-z}^i)$.
    
    The same analysis hold for each $\rp_i$ segment.
\end{itemize}

Therefore, we can construct a recurrence relationship for the number of maxima and minima for $f_r^k$ based on the sequences found in Lemma \ref{lemma-piece-decomposition}.

\begin{align*}
   \maxima(\category{q,z}^k)
    &\leq \underbrace{\sum_{i=0}^{\floor{k/2}} \minima(\category{q-1, 1-z}^k)}_{\lv_i} 
    + \underbrace{\sum_{i=0}^{\floor{(k-1)/2}} \minima(\category{q-1, 1-z}^k)}_{\rv_i} 
    \\&\quad+ \underbrace{\sum_{i=1}^{\floor{(k+1)/2}} \maxima(\category{q-1, 1-z}^k)}_{\lp_i} 
    + \underbrace{\sum_{i=1}^{\floor{k/2}} \maxima(\category{q-1, 1-z}^k)}_{\rp_i} \\
    \minima(\category{q,z}^k)
    &= \underbrace{2}_{\app \& \dep} 
    + \underbrace{\sum_{i=0}^{\floor{k/2}} \maxima(\category{q-1, 1-z}^k)}_{\lv_i} 
    + \underbrace{\sum_{i=0}^{\floor{(k-1)/2}} \maxima(\category{q-1, 1-z}^k)}_{\rv_i} 
    \\&\quad+ \underbrace{\sum_{i=1}^{\floor{(k+1)/2}} \minima(\category{q-1, 1-z}^k)}_{\lp_i} 
    + \underbrace{\sum_{i=1}^{\floor{k/2}} \minima(\category{q-1, 1-z}^k)}_{\rp_i} 
\end{align*}

We bound $\maxima(\category{q,z}^k)$ and $\minima(\category{q,z}^k)$ by induction to prove Proposition~\ref{prop:osc-category-bound}.
We use the following inductive assumption over all $k$, $q$, and $z$, which suffices to prove the claim:
\[\maxima(\category{q, z}^k), \minima(\category{q, z}^k) \leq \begin{cases}
   (4q)^k & \text{$q$ is even, $z = 0$, or $q$ is odd, $z = 1$}\\
   (4q)^{k+1} & \text{$q$ is even, $z = 1$, or $q$ is odd, $z = 0$}.
\end{cases}\]

By the previous section, the claim holds for $q = 0$ and all $k$ and $z$, which gives the base case.

Moving forward, we assume that the claim holds for all values of $q'$ with $q' \leq q$ and any $k$ and $z$. 
We prove that it holds for $q+1$ with any choices of $k$ and $z$.

We show that the bound holds for $\minima(\category{q+1, z}^k)$ when $q+1$ is even and $z = 1$, or $q+1$ is odd and $z = 0$. The other cases are nearly identical. Since the bounds are trivial for $k = 1$, we prove them below for $k \geq 2$.

\begin{align*}
    \minima(\category{q+1, z}^k)
    &\leq 2 + \sum_{i=0}^{\floor{k/2}} (4i)^{q+1} + \sum_{i=0}^{\floor{(k-1)/2}} (4i)^{q+1} + \sum_{i=0}^{\floor{(k+1)/2}} (4i)^{q+1} + \sum_{i=0}^{\floor{k/2}} (4i)^{q+1} \\
    &\leq 4 \cdot \frac{k}{2} \cdot (2k)^{q+1} + (2(k+1))^{q+1} \leq (2k)^{q+2} + (3k)^{q+1} \leq (4k)^{q+2}.
    % &\leq 2 + 8 \cdot C^q \int_{0}^{k} x^q dx \\
    % &= 2 + \frac{8 C^q k^{q+1}}{q + 1} \\
    % &\leq 2(1 + 2C^q k^{q + 1}) \\
    % &\leq 2(Ck)^{q+1},
    % &\leq 2 + 2 \left(\frac{k+1}{2}\right)^q +  8 \sum_{i=1}^{k/2} i^q \\
    % &\leq 2 + 2 \left(\frac{k+1}{2}\right)^q + 8 \sum_{i=1}^{k/2} \left(\frac{k}{2}\right)^{q-1} i \\
    % &= 2 + \frac{(k+1)^q}{2^{q-1}} +  8 \left(\frac{k}{2}\right)^{q-1} \cdot \frac{\left(\frac{k}{2} + 1\right)\left(\frac{k}{2}\right)}{2} \\
    % &\leq 2 + \frac{(k+1)^q}{2^{q-1}} + \frac{k^{q+1}}{2^{q-2}}\\
    % &\leq 2 k^{q + 1}
\end{align*}

\subsection{Proof of Theorem~\ref{thm:properties-doubling}, Claim 2}\label{assec:doubling-nn}


We restate the claim:
\begin{proposition}[Claim 2 of Theorem~\ref{thm:properties-doubling}]\label{prop:properties-doubling-approx}
    Suppose $f$ is a symmetric unimodal mapping whose maximal cycle is of length $p = 2^q$. 
    For any $k \in \N$, there exists $g\in\mathcal{N}(u, 2)$ with width $u = O((4k)^{q+1}/\eps)$ such that $L_\infty{f^k,g} \leq \epsilon$. Moreover, if $f = \ftent{r}$, then there exists $g$ of width $O((4k)^{q+1})$ with $g = f^k$.
\end{proposition}

\begin{proof}
    
This part follows the bound on monotone pieces of $f^k$ given in Proposition~\ref{prop:properties-doubling-osc} and a simple neural network approximation bound.

\begin{lemma}
    Consider some continuous $f: [0,1] \to [0,1]$ with $\oscm(f) \leq m$.
    For any $\eps \in (0, 1)$, there exists $g \in \mathcal{N}(u,2)$ of width $u =O(\frac{m}{\eps})$ such that $L_\infty(f, g) \leq \eps.$
\end{lemma}

\begin{proof}
    A monotone function mapping to $[0,1]$ can be $\eps$-approximated by a piecewise-linear function with $O(\frac{1}{\eps})$ pieces, and hence, a 2-layer ReLU network of width $O(\frac{1}{\eps})$.
    
    Every monotone piece can be approximated as such, which means that $g$ has width $O(\frac{m}{\eps})$.
\end{proof}

For the case where $f = \ftent{r}$ for some $r$, it is always true that $\abs{\frac{d}{dx} \ftent{r}^k(x)} = (2r)^k$, except when $x$ is a local maximum or minimum. 
Thus, every monotone piece of $f^k$ is linear, and $f$ can be exactly expressed with a piecewise linear function with $O((4q)^{k+1})$ pieces, and also a ReLU neural network of width $((4q)^{k+1})$.
\end{proof}


\subsection{Proof of Theorem~\ref{thm:properties-doubling}, Claim 4}\label{assec:doubling-vc}

Recall that for unimodal $f: [0,1]\to[0,1]$ and threshold $t \in (0,1)$, \[\hyp{f,t} := \{\thres{t}{ f^k}: k \in \mathbb{N}\}\]
is the hypothesis class under consideration.

\begin{proposition}[Claim 4 of Theorem~\ref{thm:properties-doubling}]\label{prop:properties-doubling-vc}
    Suppose $f$ is a symmetric unimodal mapping whose maximal cycle is of length $p = 2^q$. 
    For any $t \in (0, 1)$, $\vc(\hyp{f, t}) \leq 18p^2$.
\end{proposition}

This proof is involved and requires some setup and new definitions. 

\subsubsection{Notation}
Let $\boolseq$ represent all countable infinite sequences of Boolean values, and let $\boolstr$ represent all finite sequences (including the empty sequence).

For $y \in \boolseq$, let $y_{i:j} = (y_i, \dots, y_{j}) \in \bit^{j-i+1}$ and $y_{i:} = (y_i, y_{i+1}, \dots) \in \boolseq$.
For $w \in \bit^n, w' \in \bit^{n'}$, let $ww' = w \circ w' \in \bit^{n+n'}$ be their concatenation.
Let $w^j = w \circ w \circ \dots \circ w \in \bit^{jn}$.

\subsubsection{Iterated Boolean-Valued Functions, Regular Expressions, and VC-Dimension}
Before we give the main result, we give a way to upper-bound the VC-dimension of countably infinite hypothesis classes $\hc = \{h_1, h_2, \dots, \} \subseteq ([0,1] \to \{0, 1\})$. 
For some $x \in \mathcal{X}$, define $\seq{\hc}: [0,1] \to \boolseq$ as $\seq{\hc}(x) = (h_i(x))_{i \in \N}$. We by $\hc$ over all choices of $x \in [0,1]$:
\[\Seq{\hc} = \{\seq{\hc}(x): \ x \in [0,1]\} \subset \boolseq.\]

With this notation, $\hc$ shatters $d$ points if and only if there exist $\ys1,\dots,\ys{d} \in \Seq{\hc}$ such that $\absl{\{(\ys1_j, \dots, \ys{n}_j): j \in \N\}} = 2^d$.
% for all $\sigma \in \{0, 1\}^d$, there exists $j$ such that $(\ys1_j, \dots, \ys{n}_j) = \sigma$. 
We equivalently say that $\ys1,\dots,\ys{d}$ are shattered.

Here's where the idea of Regular Expressions (Regexes) comes in. If we can show all elements in $\Seq{\hc}$ are represented by some infinite-length Regex, then we can upper-bound the number of points $\hc$ can shatter, which is necessary to bound the expressive capacity of unimodal functions with recursive properties. 

To that end, we first introduce a different notion of shattering. Then, we'll give an upper-bound for the VC-dimension of $\hc$ when we have a Regex for $\Seq{\mathcal{H}}$. 

\begin{definition}
    We say that $\hc$ (or $\Seq{\hc}$) \textbf{weakly shatters} $d$ points if there exist $\ws{1}\circ \ys1, \dots , \ws{d}\circ \ys{d} \in \Seq{\mathcal{H}}$ for $\ws1,\dots, \ws{d} \in \boolstr$ such  that $\ys1,\dots, \ys{d}$ are shattered.
    Let the \textbf{weak VC-dimension} of $\hc$ represent the maximum number of points $\hc$ can weakly shatter and denote it $\vcw(\hc) = \vcw(\Seq{\hc})$.
\end{definition}

Using this notation, we can extend our notion of weak VC-dimension to any subset of $\boolseq$, whether or not it corresponds to a hypothesis class. If $\hc \subset S \subset \boolseq$, then $\vcw(\hc) \leq \vcw(S)$.

Note that if $\hc$ shatters $d$ points, then it also trivially weakly shatters $d$ points. We can get this by taking $w_1 = \dots, w_d$ to be the empty strings. Thus, the $\vc(\hc) \leq \vcw(\hc)$.

A Regex is a recursively defined subset of $\boolseq$ that can be represented by a string. We describe how a Regex $R \subseteq \boolseq$ can be defined below.

\begin{itemize}
    \item One way to define a Regex is with a repeating sequence $w^{\infty}$ for $w \in \bit^n$. That is, \[w^{\infty} = \{y \in \boolseq: y_{in+1: (i+1)n} = w, \forall i \in \N\}.\] For instance, $(011)^{\infty} = \{(0,1,1,0,1,1,0,1,1,\dots)\}$.
    \item For $w \in \bit^n$, if $R$ is a Regex, then $w R$ is also a Regex. This means satisfying sequences must start with $w$ and then the remainder of the bits must satisfy $R$. 
    \[wR = \{y \in \boolseq: y_{1:n} = w, y_{n+1:} \in R\}.\]
    \item $w^* R$ is also a Regex, where $w^*$ represents any number of recurrences of the finite sequence $s$. That is,
    \[w^* R =\cup_{j=0}^\infty w^j R.\]
    \item If $R'$ is also a Regex, then so is $R \cup R'$.
    % \item As an extension for the previous property, $w^{?} R := wR \cup R$ is also a Regex.
    \item If $R'$ is also a Regex, then so is $R \oplus R'$, where the odd entries of sequences in $R \oplus R'$ concatenated together must be in $R$ and the even entries must be in $R'$.
    \[R \oplus R' = \{y \in \boolseq: y_{1,3,5, \dots} \in R, y_{2,4,6,\dots} \in R'\}.\]
\end{itemize}

Now, we can create a recursive upper-bound on the number of points $\hc$ can weakly shatter. 
To do so, we assume that $\hc \subseteq R$ for some Regex $R$ and bound the weak VC dimension of $R$.

\begin{lemma}\label{lemma-regex}
 Consider infinite-length Regexes $R, R', R''$ and $w \in \bit^n$.
 \begin{enumerate}
     \item If $R = w^{\infty}$, then $\vcw(R) \leq \log_2 n$.
     \item If $R = wR'$, then $\vcw(R) \leq \vcw(R') + \log_2 n + 1$.
     \item If $R = w^* R'$, then $\vcw(R) \leq \vcw(R') + \log_2 n + 1$.
     \item If $R = R' \cup R''$, then $\vcw(R) \leq \vcw(R') + \vcw(R'')$.
    %  \item If $R = w^? R'$, then $\vcw(R) \leq \vcw(R') + \log_2 n + 1$.
     \item If $R = R' \oplus R''$, then $\vcw(R) \leq 4 \max(\vcw(R'), \vcw(R''))+2$.
 \end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}
    \item If $R = w^{\infty}$, then the set $Y = \{y: w\circ y \in w^\infty, w \in \boolstr\}$ contains at most $n$ elements. 
    Hence, 
    \[\abs{\{(\ys1_j,\dots,\ys{d}_j): j\in\N\}} \leq n\]
    for any fixed $\ys1,\dots,\ys{d}\in Y$, and
    no more than $d= \log_2 n$ points can be weakly shattered.
    
    \item Suppose $R$ weakly shatters $d$ points, so $\ys1,\dots, \ys{d}$ are shattered for some $\ws1\circ\ys1,\dots,\ws{d}\circ \ys{d} \in R$.
    If $Y = \{(\ys1_j, \dots, \ys{d}_j): j \in \N\}$ and $Y_n = \{(\ys1_j, \dots, \ys{d}_j): j \leq n\}$, then $\absl{Y} = 2^d$ and $\absl{Y_n} \leq n$.
    There exists some $v \in \bit^{1+ \log_2 n}$ such that $v \circ \sigma \in Y \setminus Y_n$ for all $\sigma \in \bit^{d -1- \log_2 n}$. 
    Therefore, \[\absl{\{(\ys{2+\log_2 n}_j, \dots, \ys{d}_j): j > n\}} = 2^{d - 1 - \log_2n},\] and there exist $d -1- \log_2 n$ points that can be weakly shattered by $R'$, since none of the labelings with $w$ are necessary.
    
    % \item Suppose $R$ weakly shatters $d$ points. $\ys1,\dots, \ys{d}$ are shattered for some $\ws1\circ\ys1,\dots,\ws{d}\circ \ys{d} \in R$, which means that for all $\sigma \in \bit^d$, there exists $j_\sigma$ such that $\sigma = (\ys1_{j_\sigma},\dots, \ys{d}_{j_\sigma})$.
    % Let $\sigma_1, \dots, \sigma_n$ be the labelings with the smallest respective indices $j_\sigma$.
    % Then, there exists some $v \in \bit^{1+ \log_2 n}$ such that $v$ is not a prefix of $\sigma_1, \dots, \sigma_n$. 
    % Therefore, all assignments of the form $\sigma = v \circ \sigma'$ for $\sigma' \in \bit^{d -1- \log_2 n}$ are fit by some $\sigma_j > n$.
    % Therefore, there exist $d - 1-\log_2 n$ points that can be shattered without needing the first $n$ characters of $\ys{j}$. Hence, there exist $d - \log_2 n$ points that can be weakly shattered by $R'$, since $s$ is redundant.
    % \footnote{
    % We assume for simplicity here that $n$ is a power of two. We add 1 to the final weak VC-dimension bound to account for the possibility otherwise, which will require the addition of ceilings.}
    
    \item Once again, suppose $R$ weakly shatters $d$ points, $\ys1,\dots, \ys{d}$ for $\ws1\circ\ys1,\dots,\ws{d}\circ \ys{d} \in R$.
    Because each $\ws{i} \circ \ys{i} \in w^*R'$, there exists an index $\ell_i$ such that $(\ws{i} \circ \ys{i})_{1:\ell_i} = w^{\ell_i / n}$ and $(\ws{i} \circ \ys{i})_{\ell_i+1:} \in R'$. 
    Without loss of generality, assume $\ys1,\dots, \ys{d}$ are ordered such that $\ell_i - \abs{\ws{i}}$ decreases.
    That is, the first $1+\log_2 n$ sequences are the ones that ``leave $w^*$ last.''
    Let $\ell^* := \ell_{1+\log_2 n} - \abs{\ws{1+\log_2 n}}$.
    Define $Y$ and $Y_{\ell^*}$ analogously to the previous part and note that $\absl{Y} = 2^d$. Because $Y_{\ell^*}$ corresponds only to labelings where the first $1 + \log_2 n$ elements come from subsets of $w^\infty$, there exists some $v \in \bit^{1+ \log_2 n}$ such that $v \circ \sigma \in Y \setminus Y_{\ell^*}$ for all $\sigma \in \bit^{d - 1  -\log_2 n}$.
    As before, there exist $d -1- \log_2 n$ points that can be weakly shattered by $R'$
    
    \item There is no set of $\vcw(R')+1$ and $\vcw(R'') +1$ points that can be weakly shattered by $R'$ and $R''$ respectively. 
    Any $\vcw(R')+\vcw(R'')+1$ points in $R$ must have at either $\vcw(R')+1$ points in $R'$ or $\vcw(R'')+1$ points in $R''$.
    Thus, at least one subset cannot be shattered.
    
    % \item Because $s^?R' \subset s^*R'$, part 3 gives the claim.
    
    \item 
    Suppose without loss of generality that $d := \vcw(R') \geq \vcw(R'')$.
    Consider any $\ws{1}\circ\ys1,\dots, \ws{d}\circ\ys{4d+3} \in R$.
    WLOG, assume that $\abs{\ws{1}}, \dots, \abs{\ws{2d+2}}$ are even, which implies that $\ws{1}_{\text{odd}}\circ \ys{1}_{\text{odd}}, \dots \ws{2d+2}_{\text{odd}}\circ \ys{2d+2}_{\text{odd}} \in R'$ and $\ws{1}_{\text{even}}\circ \ys{1}_{\text{even}}, \dots \ws{2d+2}_{\text{even}}\circ \ys{2d+2}_{\text{even}} \in R''$. 
    Therefore,
    \begin{align*}
        \abs{\{(\ys1_j, \dots, \ys{4d+3}_j): j \in \N\}} 
        &\leq 2^{2d+1}\abs{\{(\ys1_j, \dots, \ys{2d+2}_j): j \in \N\}} \\
        &\leq 2^{2d+1}\paren{\abs{\{(\ys1_j, \dots, \ys{2d+2}_j): j \in \N_{\text{odd}}\}} + \abs{\{(\ys1_j, \dots, \ys{2d+1}_j): j \in \N_{\text{even}}\}}} \\
        &\leq 2^{2d+1}\cdot 2 \sum_{i=0}^{d} {2d+2 \choose i} 
        < 2^{2d+2}\cdot 2^{2d+1} 
        = 2^{4d+3}.
    \end{align*}
    The last line follows by the Sauer Lemma. 
    Thus, $R$ cannot shatter $4d+3$ points if $R'$ and $R''$ cannot shatter $d$ points.
    
    % \item We consider the proposition in terms of the hypothesis classes corresponding to $R'$ and $R''$, $\hc'$ and $\hc''$ respectively. Then, $\hc = \hc' \cup \hc'$, and we use the \todo{cite?} fact that $\vc(\hc) \leq 1 + 2 \max(\vc(\hc'), \vc(\hc''))$.
\end{enumerate}
\end{proof}

Here's an example of how to apply our regex rules:
\begin{align*}
    \vcw(1^* 0(01)^{\infty} \cup 10^{\infty})
    &\leq \vcw(1^* 0(01)^{\infty}) + \vcw(10^{\infty}) \\
    &\leq 1 + \vcw(0(01)^{\infty}) + 1 + \vcw(0^\infty) \\
    &\leq 2 + 1 + \vcw((01)^\infty) \\
    &\leq 3 + 1 = 4.
\end{align*}

\subsubsection{Proof of the Proposition~\ref{prop:properties-doubling-vc}}
Recall that we consider the hypothesis class \[\hc_{f,t} := \{\thres{t}{  f^k}: k \in \N\}\]
for symmetric unimodal $f$ and $t \in (0,1)$.

To build up the argument, we first bound the VC-dimension for two simple cases. 
\begin{itemize}
    \item 
    First, we consider the case when $f$ has no fixed point. 
    Thus, for all $x \in (0, 1]$, $f(x) < x$, which means that the sequence $f(x), f^2(x), \dots$ is decreasing. 

    If the threshold $t$ is $0$ or is greater than $f(\frac{1}{2})$, then the sequence will be all 0's or 1's, which will imply that $\vc(\hc_{f, t}) = 0$. Thus, the only interesting thresholds are $t \in (0, f(\frac{1}{2})]$. Because the sequence is decreasing, $\Seq{\hc_{f,t}} = 1^* 0^{\infty}$. From Lemma \ref{lemma-regex}, $\vc(\hc_{f,t}) \leq \vcw(\hc_{f, t})  \leq 1$.
    
    \item 
    Let $x_1 < \dots < x_m$ be all the fixed points of $f$. Suppose $x_m \leq \frac{1}{2}$. By symmetry, for all $j \in [m]$, $f(1-x_j) = x_j$.
    
    To analyze this function, we partition $[0, 1]$ into $2m + 2$ intervals: $I_0 = [0, x_1), I_0' = (1-x_1, 1]$, $I_m = [x_m, \frac12]$, $I_m' = (\frac12, 1-x_m]$, $I_j = [x_j, x_{j+1})$, and $I_j' = (1-x_{j+1},1- x_j]$ for all $j \in \{1, \dots, m-1\}$ (visualized in Figure \ref{fig:simple-fixed-point}).
    
    \begin{figure}
        \centering
        \input{fig/fig-simple-fixed-point}
        \caption{A plot of $f$ with fixed point $m=2$ fixed points---both less than $\frac{1}{2}$---subdivided into intervals. The relationships of which intervals $f$ maps onto one another are also visualized.}
        \label{fig:simple-fixed-point}
    \end{figure}
    Because $f$ is unimodal and because the edges of all intervals map to fixed points, for all $j \in \{0, \dots, m\}$, $f(I_j') = f(I_j) = I_j$. In this case, it must be the case that $q = 0$ because $f$ cannot have a 2-cycle. Such a cycle is impossible because it would have to be contained entirely in some $I_j$. In those intervals, it must be the case that either $\forall x \in I_j$, $f(x) \geq x$, or $\forall x \in I_j$, $f(x) \leq x$ (if this were not the case, then this would imply the existence of a fixed point other than $x_j$ in $I_j$). Thus, cyclic behavior within an interval is impossible.
    
    Thus, we can construct a Regex to represent the itinerary of any $x \in [0, 1]$: $ \bigcup_{j=0}^{m} I_j^{\infty}$.\footnote{
    This is a massive abuse of notation, but we use the same Regex notation to denote the intervals that are traversed as we use to denote the values of Boolean sequence.} 
    Now, we consider all possible locations of threshold $t$:
    \begin{itemize}
        \item If $t \in I_j$, such that $f(x) \geq x$ for $x \in I_j$, then $\Seq{\hc_{f,t}} \subseteq 0^* 1^{\infty} \cup 0^{\infty} \cup 1^{\infty}$. By Lemma \ref{lemma-regex}, $\vcw(\hc_{f,t}) \leq 1$.
        \item If $t \in I_j$, such that $f(x) \leq x$ for $x \in I_j$, then $\Seq{\hc_{f,t}} \subseteq 1^* 0^{\infty} \cup 0^{\infty} \cup 1^{\infty}$. By Lemma~\ref{lemma-regex}, $\vcw(\hc_{f,t}) \leq 1$.
        \item If $t \in \bigcup_{j=0}^m I_j'$, then $\Seq{\hc_{f,t}} = 0^{\infty}$, and $\vcw(\hc_{f,t}) = 0$.
    \end{itemize}

\end{itemize}

Now, we give a lemma, which relates the VC-dimension of complex functions to that of simpler ones.
Let $\category{q}$ refer to the family of symmetric unimodal functions that have a $2^q$-cycle but not a $2^{q+1}$-cycle.

\begin{lemma}\label{lemma:vc-recursive}
    For any $f \in \category{q}$ with fixed point $x^* > \frac12$ and any $t \in [0,1]$, \[\vcw(\hc_{f,t}) \leq 4 \max_{g \in \category{q-1}, t'\in [0,1]}\vcw(\hc_{g, t'})+10.\]
\end{lemma}
\begin{proof}
    
Consider some such $f$. Let $x_1< \dots< x_m$ be the fixed points of $f$ where $ x_m=x^* > \frac12$. Because $\frac12$ maximizes $f$, $f(\frac12) \geq x_m > \frac12$. This fixed point must the only fixed point no smaller than $\frac12$; the existence of another such fixed point would contradict the fact that $f$ is decreasing on $(\frac12, 1]$. Thus, $x_1, \dots, x_{m-1} < \frac12$.

We build a recursive relationship by considering $f^2$ and relating some its output on some segments of $[0, 1]$ to other maps with smaller $q$. For now, we instead attempt to upper-bound the VC-dimension of $\mathcal{H}_{f^2, t}$.

For all $j \in [m]$, unimodality implies that $x_j$ and $1-x_j$ are the only points that map to $x_j$ and that the following ordering holds.
\[0 < x_1 < \dots, < x_{m-1} < 1-x_m < \frac12 < x_m < 1-x_{m-1} < \dots, 1-x_1 < 1.\]

By the Intermediate Value Theorem, there exists some $x_m' \in (x_m, 1-x_{m-1})$ such that $f(x_m') = f(1-x_m') = 1-x_m$ and $f^2(x_m') =f^2(1-x_m')= x_m$.

We define intervals as follows:
\begin{itemize}
    \item $I_0 = [0, x_1)$ and $I_0' = (1-x_1, 1]$.
    \item For all $j \in [m-2]$, $I_j = [x_j, x_{j+1})$ and $I_{j}' = (1-x_{j+1}, 1-x_j]$.
    \item $I_{m-1} = [x_{m-1}, 1-x_{m}')$ and $I_{m-1}' = (x_{m}', 1-x_{m-1}]$.
    \item $I_{m} = [1-x_m', 1-x_m)$ and $I_m' = (x_m, x_m']$.
    \item $I_{m+1} = [1-x_m, \frac12)$, and $I_{m+1}' = [\frac12, x_{m}]$.
\end{itemize}

For any $j \in \{0, \dots, m+1\}$, $f$ is increasing on all intervals $I_j$ and decreasing on $I_j'$. 
By symmetry, $f(I_j) = f(I_j')$.
For all $j \in \{0, \dots, m-2\}$, $f(I_j) = I_j$. $f(I_{m-1}) = I_{m-1} \cup I_m$, $f(I_m) = I_{m+1} \cup I_{m+1}'$, and $f(I_{m+1}) \subseteq I_{m}'$, because $f(\frac12) \in [x_m, x_m')$.\footnote{
This must be the case for the assumptions to be met. If $f(\frac12) < x_m$, then $x_m$ cannot be a fixed point because $\frac12$ maximizes $f$. If $f(\frac12) > x_m'$, then there exists a 3-cycle with points in $I_{m+1}, I_{m-1}', I_m$, which contradicts the assumption that we only have power-of-two cycles.}

From there, we obtain additional properties for $f^2$: $f^2(I_{m-1}) = I_{m-1} \cup I_{m} \cup I_{m+1} \cup I_{m+1}'$, $f^2(I_m) \subseteq I_{m}'$, and $f^2(I_{m+1}) \subset I_{m+1} \cup I_{m+1}'$. This suggests that there is recurrent structure that we can take advantage of to count all of the patterns.

Let $J_{m+1} := I_{m+1} \cup I_{m+1}'$. We create a Regex to track the behavior of iterates $f^2$, which we visualize in Figure~\ref{fig:inductive-fixed-point}:
\[\bigcup_{j=0}^{m-2} I_j^{\infty}\ \cup\  I_{m-1}^* I_m I_m^{\prime \infty}\ \cup\ I_m^{\prime \infty} \ \cup\  I_{m-1}^* J_{m+1}^{\infty}.\]

When an iterate of $f^2$ gets ``stuck'' in one of $I_0, I_1, \dots, I_{m-1}$, it must either be at a fixed point, be strictly increasing, or be strictly decreasing. To suggest otherwise would imply the existence of another fixed point in those intervals, because $f^2$ is monotonically increasing or decreasing in all of those and either all $x$ yield $f^2(x) \geq x$ or $f^2(x) \leq x$.

For the remaining intervals, one might notice in Figure \ref{fig:inductive-fixed-point} that zooming in on the intervals $I_{m}$, $J_{m+1}$, and $I_{m}'$ for $f^2$ gives what looks like unimodal maps.\footnote{We use similar techniques here to those used in Section \ref{sec:ub-general-case}.} We take advantage of that structure to bound the complexity of the 0/1 Regexes for those intervals. We can formalize this by defining symmetric unimodal mappings $h_m$ and $h_{m+1}$ and bijective monotonic mappings $\phi_m: I_{m}' \to (0,1]$ (increasing) and $\phi_{m+1}: J_{m+1} \to [0,1]$ (decreasing) such that:
\begin{itemize}
    \item For $x \in I_m$, $f^2(x) = \phi_m^{-1} \circ h_m \circ \phi_m(1-x).$
    \item For $x \in I_m'$, $f^2(x) = \phi_m^{-1} \circ h_m \circ \phi_m(x).$
    \item For $x \in J_{m+1}$, $f^2(x) = \phi_{m+1}^{-1} \circ h_{m+1} \circ \phi_{m+1}(x).$
\end{itemize}

\begin{figure}
    \centering
    \include{fig/fig-inductive-fixed-point}
    \caption{Like Figure~\ref{fig:simple-fixed-point}, plot of $f$ and $f^2$ with $m = 3$ fixed points with $x_m > \frac{1}{2}$ and visualizes the mappings between intervals.}
    \label{fig:inductive-fixed-point}
\end{figure}

Because $f$ cannot have a cycle of length $2^{q+1}$, $h_m$ and $h_{m+1}$ may not have cycles of length $2^q$. 
Thus, we can reason inductively about how iterates behave when they're trapped in those intervals.

We do another case analysis of the 0/1 Regexes induced by different choices of $t$.
\begin{itemize}
    \item If $t \in I_j$ for $j \in \{0, \dots, m-1\}$, then $\Seq{\mathcal{H}_{f^2, t}} \subseteq 0^\infty \cup 1^{\infty} \cup 0^* 1^{\infty} \cup 1^* 0^{\infty}$ because a sequence of iterates only crosses $t$ if it enters the correct interval $I_j$, where the iterate then will be stuck and must monotonically increase or decrease. By Lemma \ref{lemma-regex}, $\vcw(\hc_{f^2, t}) \leq 2$.
    
    \item If $t \in I_j'$ for $j \in \{0, \dots, m-1\}$, then $\Seq{\mathcal{H}_{f^2, t}} = 0^{\infty}$, and $\vcw(\hc_{f^2, t}) = 0$.
    
    \item If $t \in I_{m}$, then $\Seq{\mathcal{H}_{f^2, t}} = 0^{\infty} \cup 1^{\infty} \cup 0^* 1^{\infty}$. Then, $\vcw(\hc_{f^2, t}) \leq 1$.
    
    \item If $t \in J_{m+1}$, then $\Seq{\hc_{f^2, t}} = 0^{\infty} \cup 0^* 1^{\infty} \cup 0^* J_{m+1}^{\infty}$. Because $h_{m+1}$ has at most a cycle of length $2^{q-1}$, we have that \[\vcw(\hc_{f^2, t}) \leq 2 + \max_{t'}\vcw(\hc_{h_{m+1}, t'}).\]
    
    \item If $t \in I_{m}'$, then $\Seq{{\hc}_{f^2, t}} = 0^{\infty} \cup 0^* I_m^{\prime \infty}$. 
    This gives us that \[\vcw(\hc_{f^2, t}) \leq 1 + \max_{t'} \vcw(\hc_{h_m, t'}).\]
\end{itemize}

To get $\vcw(\hc_{f, t})$, notice that $\Seq{\hc_{f, t}} = \Seq{\hc_{f^2, t}} \oplus \Seq{\hc_{f^2, t}'}$, where $\hc_{f^2, t}'$ refers to the outcome of all odd iterates of $f$. 
We show that $\Seq{\hc_{f^2, t}'} \subseteq \Seq{\hc_{f^2, t}}$ because the latter could induce all sequences produced by the former by starting with some $x'$ such that $f^2(x') = f(x)$. 
Thus, by Lemma \ref{lemma-regex}, 
\begin{align*}
    \vcw(\hc_{f, t}) 
    & \leq  4\max_{t'}\vcw(\hc_{f^2,t'}) + 2  \\
    & \leq 4 \max(2 + \max_{t'}\vcw(\hc_{h_{m+1}, t'}),1 + \max_{t'} \vcw(\hc_{h_m, t'})) + 2 \\
    &\leq 4\max_{g \in \category{q-1}, t'} \vcw(\hc_{g,t'}) + 10.\qedhere
\end{align*}
\end{proof}

Now, we prove a bound on the VC-dimension for arbitrary $q$ by induction with Lemma \ref{lemma:vc-recursive} to show that for $\vc(\mathcal{H}_{f, t}) \leq 18 \cdot 4^q$.

This holds when $q = 0$. There are two possible cases for the fixed point of such an $f$. If the the largest fixed point is smaller than $\frac12$, then, by the simple cases explored at the beginning, $\vcw(\mathcal{H}_{f, t}) \leq 1$. 
Otherwise, we apply Lemma \ref{lemma:vc-recursive} along with the the other simple case---which tells us what happens when there are no fixed point---to get that $\vcw(\hc_{f, t}) \leq 4 (1) + 10 = 14$. This trivially satisfies the proposition.

For the inductive step for arbitrary $q$, we iteratively apply Lemma~\ref{lemma:vc-recursive} to obtain the final bound.
\begin{align*}
    \vc(\mathcal{H}_{f, t})
    &\leq 4\max_{g \in \category{q-1}, t'} \vcw(\hc_{g,t'}) + 10 \\
    &\leq 4^q \max_{g \in \category{0}, t'} \vcw(\hc_{g,t'}) + 10 \sum_{i=0}^{q-1}4^i \\
    &\leq 14 \cdot 4^q + \frac{10}{3} 4^q \leq 18 \cdot 4^q.
\end{align*}

% \subsubsection{Upper-Bound on VC-Dimension for Variable Intervals}

% Here, we obtain an upper-bound similar to Theorem \ref{thm:vc-fixed-ub-po2}, except that we now allow the threshold $t$ to vary within the hypothesis class, rather than be a fixed parameter. We consider the following modified hypothesis class for concave $\beta$-unimodal $f$:
% \[\mathcal{H}_{f} = \left\{x \mapsto \indicator{f^k(x) \geq t}: k \in \mathbb{Z}_{+}, t \in [0, 1]\right\}.\]

% Unlike the previous section, we're now considering an uncountably infinite hypothesis class. Because $\HH_{f, t} \subset \HH_f$, we expect the VC-dimension of $\HH_f$ to be larger than that of $\HH_{f, t}$; indeed, it's not obvious from the outset that the VC-dimension $\HH_f$ will even be finite when the maximal cycle in $f$ has length a power of two. Nonetheless, we show the following result with the help of similar concepts from the Theorem \ref{thm:vc-fixed-ub-po2}.

% \begin{theorem}\label{thm:vc-var-ub-po2}
%     If for some $q \in \mathbb{Z}_{\geq 0}$, the longest cycle in $f$ has length $2^q$, then $\mathcal{H}_{f}$ has VC-dimension at most $24 \cdot 2^q$.
% \end{theorem}
% \begin{proof}
%     In the proof of Theorem \ref{thm:vc-fixed-ub-po2}, we took advantage of the fact that we could express the possible outputs of each hypothesis class $\HH_{f,t}$ as an infinite-length Regex of 0's and 1's. Here, we use a similar technique, except that we instead regard each $\HH_f$ as a Regex of intervals on $[0, 1]$ such that iterates in those intervals are either non-increasing or non-decreasing.
    
%     Suppose we partition $[0, 1]$ into such intervals $I_1 < I_2 < \dots < I_m$. Then, for some $x \in [0, 1]$ and some $f$, we can obtain a sequence $s_{f}(x) = I(f(x)), I(f^2(x)), \dots$, where $I$ is a function that gives the interval that contains the point. We once again consider a set
%     \[S_{f} = \{s_{f}(x): x \in \mathcal{X}\},\]
%     which can be represented by a Regex with alphabet $I_1, \dots, I_m$.
    
%     From these Regexes, we find techniques that allow us to bound the VC-dimension of $\HH_f$. The properties found here are not complete like those for the fixed-threshold case, but they're sufficient for this proof. 
    
%     \begin{lemma}\label{lemma:regex-interval}
%         Suppose $f: [0,1] \to [0, 1]$ is a continuous function. Let intervals $I_1 < \dots < I_m$ partition $[0, 1]$ such that in each $I_j$, either $f$ is increasing on $I_j$ or $f$ is decreasing. Suppose that the hypothesis classes corresponding to Regexes $R_1$ and $R_2$ that shatter at most $n_1$ and $n_2$ points respectively. The following are true:
%         \begin{enumerate}
%             \item If $S_f = I_j^{\infty}$ and $f$ is increasing on $I_j$, then $VC(\HH_f) \leq 1$.
%             \item If $S_f = I_j^{\infty}$ and $f$ is decreasing on $I_j$, then $VC(\HH_f) \leq 2$.
%             \item If $S_f = I_j R_1$, then $VC(\HH_f) \leq n_1 + 1$.
%             \item If $S_f = I_j^{*} R_1$ and $f$ is increasing on $I_j$, and $I_j$ precedes all intervals in $R_1$, then $VC(\HH_f) \leq n_1 + 1$.
%             \item If $S_f = R_1 \cup R_2$, then $VC(\HH_f) \leq n_1 + n_2$.
%             \item If $S_f = R_1 \oplus R_2$, then $VC(\HH_f) \leq 1 + 2\max(n_1, n_2)$.
%         \end{enumerate}
%     \end{lemma}
%     \begin{proof}
%         \begin{enumerate}
%             \item Consider any $x_1, x_2 \in [0, 1]$ with $f(x_1) < f(x_2)$. Then, for all $k \geq 1$, $f^k(x_1) < f^k(x_2)$. We cannot shatter the points because there is no $h \in \HH_f$ with $h(x_1)= 1$ and $h(x_2) = 0$.
%             \item Consider any $x_1, x_2, x_3 \in [0, 1]$ with $f(x_1) < f(x_2) < f(x_3)$. Then, for all odd $k$, $f(x_1) < f(x_2) < f(x_3)$, and for all even $k \geq 2$, $f(x_1) > f(x_2) > f(x_3)$. They cannot be shattered because there is no $h \in \HH_f$ with $h(x_1) = 0, h(x_2) = 1 h(x_3) = 0$.
%             \item Suppose that $S_f$ could shatter $n_1+2$ points $x_1, \dots, x_{n_1 + 2}$. WLOG assume that $f(x_1) \leq f(x_2) \leq \dots \leq f(x_{n_1+2})$. Consider all $2^{n_1 + 1}-1$ non-trivial labelings $h$ with $h(x_1) = 1$. None of those can be met when $k = 1$; thus, they must all be able to be represented by $R_1$. Thus, $R_1$ is able to shatter $n_1 + 1$ points, a contradiction. 
%             \item Suppose that $S_f$ could shatter $n_1+2$ points $x_1, \dots, x_{n_1 + 2}$. WLOG assume that $f(x_1) \leq f(x_2) \leq \dots \leq f(x_{n_1+2})$. We must have $f(x_1) \in I_j$; otherwise, $R_1$ would be able to shatter $n_1 + 2$ points. Because $f$ is increasing on $I_j$ , and $I_j$ is ``less than'' all intervals in $R_1$, if $f^k(x_1) \in I_j$, then $f^k(x_1) \leq f^k(x_j)$ for all other $j$.
            
%             Consider all $2^{n_1 + 1}-1$ non-trivial labelings $h$ with $h(x_1) = 1$. None of those can be met while $f^k(x_1) \in I_j$; thus, they must all be able to be represented by $R_1$. Thus, $R_1$ is able to shatter $n_1 + 1$ points, a contradiction. 
            
%             \item Suppose that $S_f$ could shatter $n_1+n_2 +1$ points. Then, $n_1+1$ of those points will obey $R_1$ or $n_2+1$ will obey $R_2$. WLOG assume the former holds. Shattering these $n_1+n_2 +1$ will thus require that the $n_1+1$ following $R_1$ will be shattered by $R_1$, which is a contradiction.
            
%             \item We have that $\HH_f = \HH_1 \cup \HH_2$, where $\HH_1$ and $\HH_2$ are a hypothesis classes respecting $R_1$ and $R_2$ respectively. By the basic fact about VC-dimension of unions of sets, $VC(\HH_f) \leq 1 + 2\max(VC(\HH_1), VC(\HH_2))$.
%         \end{enumerate}
%     \end{proof}
    
%     Armed with these facts, we prove the bound from on $VC(\HH_f)$ using what we already know about the orders of intervals of $f$ from the proof of Theorem \ref{thm:vc-fixed-ub-po2}.
    
%     We again start by considering two simple cases:
%     \begin{itemize}
%         \item If $f$ is $\beta$-unimodal without a fixed point, consider the partition $I_1 = [0, \beta], I_1'= [\beta, 1]$. For all $x \in [0,1]$, $f(x) \in I_1$ and $f(x) < x$. Thus, $S_f = I_1^{\infty}$. Because $f$ is increasing on $I_1$, $VC(\HH_f) \leq 1$.
        
%         \item If $f$ has fixed points $x_1 < \dots < x_m \leq \beta$. As described in the proof of Theorem \ref{thm:vc-fixed-ub-po2}, $[0, 1]$ can be partitioned into $2m+2$ intervals $I_0 < \dots < I_{m}< I_{m}'< \dots< I_{0}'$ such that $S_f = \bigcup_{j=0}^m I_j^{\infty}$. Because $f$ is increasing on each $I_j$ and because of the union property for Regexes, $VC(\HH_f) \leq 1$.
%     \end{itemize}
    
%     Now, we create an analogue to Lemma \ref{lemma:vc-recursive}. 
%     \begin{lemma}
%         Suppose asymmetric unimodal function $f$ has a maximal cycle of length $2^q$ for $q \geq 0$, and suppose the for maximal fixed point $x^*$ of $f$, $x^* > \beta$ where $\beta$ maximizes $f$. Then, $VC(\HH_{f}) \leq 2 d + 11$, where $d$ is the maximum VC-dimension of any $\HH_g$ for any asymmetric unimodal $g$ \textit{without} a cycle of length $2^q$. 
%     \end{lemma}
%     \begin{proof}
%         We shamelessly rip off the proof of Lemma \ref{lemma:vc-recursive}, down the same partitioning of intervals $I_0 < \dots < I_{m} < J_{m+1} < I_m' < \dots I_0'$. We also steal their Regex for intervals of $[0,1]$ for $f^2$:
%         \[\bigcup_{j=0}^{m-2} I_j^{\infty}\ \cup\ I_{m-1}^* I_m I_m^{\prime \infty}\ \cup\ I_m^{\prime \infty} \ \cup\ I_{m-1}^* J_{m+1}^{\infty}.\footnote{This looks slightly different than the one on the other section for now because we're not counting iterates for $k = 0$ here. This is the way it should be; I just haven't updated the text in the other section to match here yet.}\]
        
%         Because $J_{m+1}$ corresponds to $g$, the $J_{m+1}^{\infty}$ can shatter no more than $d$ points. We can now assemble an upper-bound on $VC(\HH_{f^2})$ by applying Lemma \ref{lemma:regex-interval} and decomposing the Regex term-by-term. The number under each under-brace corresponds to the maximum number of points the indicated Regex could shatter. Note that $f$ is increasing on all $I_j$ and decreasing on all $I_j'$.
%         \[\underbrace{\underbrace{\bigcup_{j=0}^{m-2} \underbrace{I_j^{\infty}}_1}_1\ \cup\ \underbrace{I_{m-1}^* \underbrace{I_m \underbrace{I_m^{\prime \infty}}_2}_3}_4 \ \cup\ \underbrace{I_m^{\prime \infty}}_2 \ \cup\ \underbrace{I_{m-1}^* \underbrace{J_{m+1}^{\infty}}_d}_{d+1}}_{d+5}\]
        
%         As before, this similarly holds for $\HH_{f^2}'$.
        
%         Because $S_f = S_{f^2} \oplus S_{f^2}'$, it follows that $VC(\HH_f) \leq 2d + 11$.
%     \end{proof}
    
%     As before, it now suffices to show the main claim by inductively proving a slightly stronger: $VC(\HH_f) \leq 24 \cdot 2^q - 11$. 
    
%     For the base case of $q = 0$, $f$ must either satisfy the second simple case (in which case, $VC(\HH_f) \leq 1$) or it is obtained by applying Lemma \ref{lemma:regex-interval} for $q = 0$ and invoking the first simple case ($VC(\HH_f) \leq 2(1) + 11 = 13$). This trivially satisfies the proposition.
    
%     The inductive step involves applying Lemma \ref{lemma:vc-recursive} for an arbitrary $q$:
%     \[VC(\HH_{f}) \leq 2(24 \cdot 2^{q-1} - 11) + 11 = 24 \cdot 2^q + 11 - 22 = 24 \cdot 2^q - 11 \]
    
%     Thus, the claim holds. 
    
% \end{proof}


\subsection{Proof of Theorem~\ref{thm:properties-chaotic}, Claim 4}\label{asec:chaotic}

\begin{proposition}\label{proposition:odd-vc-dim}
    Suppose $f$ is a symmetric unimodal function with a $2^q m$-cycle for odd $m$. 
    Then for 
    % \[K = \Omega\left(2^q\left[\left(\frac{m}{\ln m} + d\right)\ln\left(\frac{m}{\ln m} + d\right)\right]^d\right),\]
    \[K = \exp\paren{O\paren{q + d\log(d+m)}},\]
    $\vc(\hc_{f,K})\geq d$ for
    $\hc_{f,K} = \left\{\thres{1/2}{ f^k}: k \in [K]\right\}.$
\end{proposition}
The claim holds by this proposition, since the VC-dimension of $\hc_f$ is larger than every $d$ and hence must be infinite.
\begin{proof}
    The proof of this claim relies on the existence of a lemma that describes a characteristic of odd-period cycles of unimodal functions.
    
    \begin{lemma}\label{lemma:odd-cycle-left}
         Let $f$ be a symmetric unimodal function with some odd cycle $ x_1, x_2, \dots, x_{m}$ of length $m > 1$ such that $f(x_i) = x_{i+1}$ and $f(x_{m}) = x_1$. Then, there exists some $i$ such that $x_i < \frac{1}{2}$ and $f(x_i) \geq \frac{1}{2}$.
    \end{lemma}
    \begin{proof}
        To prove the claim, it suffices to show that the following two cases are impossible: (1) $x_1, \dots, x_{m} < \frac{1}{2}$ and (2) $x_1, \dots, x_{m} \geq \frac{1}{2}$.
        
        \begin{enumerate}
            \item Suppose $x_1, \dots, x_{m} < \frac{1}{2}$. 
            By unimodality $x_j < x_{j'}$ implies that $f(x_j) < f(x_{j'})$.
            If $x_1$ is the smallest element of the cycle, then $f(x_1) > x_1$.
            For any other $x_j$, $f(x_j) > x_1$, which means that $x_1$ cannot be part of a cycle, which contradicts the odd cycle.
            
            \item Suppose instead that $x_1, \dots, x_{m} \geq \frac{1}{2}$. 
            
            For this to be the case, $f(\frac12) > \frac12$ by unimodality. This fact paired with $f(1) < 1$ implies the existence of some $x^* \in (\frac12, 1)$ with $f(x^*) = x^*$. Because $f$ is decreasing on $[1/2, 1]$, $f([1/2, x^*)) \subseteq (x^*, 1]$ and $f((x^*, 1]) = [0, x^*)$. 
            
            If $x_1 \in [\frac12, x^*)$, then $x_2 \in (x^*, 1]$, and $x_3 \in [\frac12, x^*)$. 
            If apply this fact repeatedly, the oddness of $m$ implies that $x_{m} \in [\frac12, x^*)$ and $x_1 \in (x^*, 1]$, a contradiction.\qedhere
        \end{enumerate}
    \end{proof}
    
    We show that $\vc(\hc_{f^{2^q}, K/2^q}) > d$.
    If $f$ has a cycle of length $2^q \cdot m$, then $f^{2^q}$ has a cycle of length $m$. By Sharkovskii's Theorem, for all odd $m' > m$, $f^{2^q}$ also has a cycle of length $m'$. Let $p_1 < \dots < p_d$ be the smallest prime numbers greater than $m$. According to Lemma \ref{lemma:primes-in-interval}, $p_d \leq \left(\frac{K}{2^q}\right)^{1/d}$ for 
    \[K =2^q \paren{O(\max(d\log d, m)}^d = \exp\paren{O\paren{q + d\log(d+m)}}.\]
    
    For $j \in [m]$, let $x^{(j)}$ be the point guaranteed by Lemma~\ref{lemma:odd-cycle-left} with $f^{2^q \cdot p_j}(x^{(j)}) = x^{(j)}$, $x^{(j)} < \frac{1}{2}$, and $f^{2^q}(x^{(j)}) \geq \frac{1}{2}$. Therefore, it follows that $f^{2^q \cdot \ell p_j}(x^{(j)}) < \frac{1}{2}$ and $f^{2^q (\ell p_j + 1)}(x^{(j)}) \geq \frac{1}{2}$ for all $\ell \in \mathbb{Z}_{\geq 0}$.
    
    To show that $\hc_{f^{2^q}}$ shatters $x^{(1)}, \dots, x^{(d)}$, we show that for any labeling $\sigma \in \bit^d$, there exists $h \in \hc_{f^{2^q},K/2^q}$ such that $h(x^{(j)}) = \sigma_j$.
    \begin{itemize}
        \item If $\sigma = (0, \dots, 0)$, then consider $f^{2^q \cdot k}$, where $k = \prod_{j=1}^n p_j$. 
        Then, for all $j$, $f^{2^q \cdot k}(x^{(j)}) < \frac{1}{2}$. 
        Because $k \leq p_d^d \leq \frac{K}{2^q}$, there exists some $h \in \hc_{f^{2^q}, K/2^q}$ that assigns zero to every $x^{(j)}$.
        
        \item Similarly, if $\sigma = (1, \dots, 1)$, we instead consider $f^{2^q \cdot k}$ for $k = 1 + \prod_{j=1}^n p_j$. 
        Now, for all $j$, $f^{2^q \cdot k}(x^{(j)}) \geq \frac{1}{2}$, and $k \leq p_d^d \leq \frac{K}{2^q}$, which means there exists satisfactory $h \in \hc_{f^{2^q}, K/2^q}$.
        
        \item Otherwise, assume WLOG that $(\sigma_1, \dots, \sigma_{\ell}) = (0, \dots, 0)$ and $(\sigma_{\ell+1}, \dots, \sigma_d) = (1, \dots, 1)$ for $\ell \in (1, d)$. 
        We satisfy the claim for $f^{2^q \cdot k}$ if we choose some $k$ with $k = q_1 \prod_{i=1}^{\ell} p_i = 1 + q_2 \prod_{i=\ell+1}^d p_i$, for some $q_1, q_2 \in \mathbb{Z}_+$. 
        
        We find $q_1 \in [\prod_{i=\ell+1}^d p_i]$ and $q_2 \in [ \prod_{i=1}^{\ell} p_i ]$ by choosing them such that:
        \begin{align*}
            q_1 \prod_{i=1}^{\ell} p_i &\equiv 1 \pmod{\prod_{i=\ell+1}^d p_i} \\
            q_2  \prod_{i=\ell+1}^d p_i &\equiv -1 \pmod{\prod_{i=1}^{\ell} p_i} .
        \end{align*}
        
        % We can find such $q_1$ and $q_2$ by using Euclidean algorithm to solve
        % \[q_1 \prod_{i=1}^{\ell} p_i - q_2\prod_{i=\ell+1}^n p_i = 1 .\]
        This is possible because $p_1, \dots, p_d$ are prime, and $\gcd\left(\prod_{i=1}^{\ell} p_i, \prod_{i=\ell+1}^d p_i\right) = 1$.
        
        Because $k \leq \prod_{i=1}^d p_i \leq p_d^d \leq \frac{K}{2^q}$, there must exist some satisfactory $h \in \mathcal{H}_{f^{2^q}, K/2^q}$.\qedhere
    \end{itemize}
\end{proof}


\begin{lemma}\label{lemma:primes-in-interval}
    For $m \geq 3$ and any $d \geq 0$, there exist $d$ primes such that $m \leq p_1 < \dots < p_d$ for \[p_d = O(\max(d\log d, m)).\]
\end{lemma}
\begin{proof}
    Let $\pi(x) = \abs{\{y \in [x]: y \text{ is prime}\}}$ be the number of primes no larger than $x$.
    By the Prime Number Theorem, 
    \[\frac{x}{\log(x) + 2} \leq \pi(x) \leq \frac{x}{\log(x) - 4},\]
    for all $x \geq 55$ \citep{rosser41}.
    Thus, for some $m' = O(\max(d\log d, m))$,
    the number of prime numbers smaller than $m'$ is
    \[\Omega\paren{\frac{d\log d}{\log(d\log d)} + \frac{m}{\log m}} = \Omega\paren{d +\frac{m}{\log m}}, \]
    and the number between $m$ and $m'$ is $\Omega(d).$
    Thus, $p_d \leq m'$.
\end{proof}


% \begin{lemma}\label{lemma:primes-in-interval-old}
%         For any $m \in \mathbb{Z}_+$, there exist $n$ primes $p_1 < \dots < p_n$ with $p_1 > m$ such that
%         \[p_n \leq \left(\frac{10\max(m,150)}{\ln(\max(m,150))} + 2n\right) \ln \left(\frac{40\max(m,150)}{\ln(\max(m,150))} + 8n\right).\]
%     \end{lemma}
%     \begin{proof}
%         Let $\pi(x) = \abs{\{y \in [x]: y \text{ is prime}\}}$ be the number of primes no larger than $x$. We have the following bound for $x \geq 55$ (\href{https://en.wikipedia.org/wiki/Prime_number_theorem#Non-asymptotic_bounds_on_the_prime-counting_function}{reference}):
%         \[\frac{x}{\ln(x) + 2} \leq \pi(x) \leq \frac{x}{\ln(x) - 4}.\]
        
%         We can prove this lemma by finding some $z$ such that $\pi(z) - \pi(m) \geq n$. We use the above bounds to find such a $z$. Let $a = \max(m, 150)$. We apply Fact \ref{fact:ln-asymp} by assuming that $z \geq 2A(\ln A + C)$ with $A = n + \frac{a}{\ln(a) - 4}$ and $C = 2$.
%         \begin{align*}
%             \pi(z) - \pi(m)
%             &\geq \pi(z) - \pi(a) \\
%             &\geq \frac{z}{\ln(z) + 2} - \frac{a}{\ln(a) - 4} \\
%             &\geq \frac{\left(n + \frac{a}{\ln (a) - 4}\right)(\ln z + 2)}{\ln(z) + 2} - \frac{a}{\ln(a) - 4} \\
%             &= n
%         \end{align*}
        
%         Now, it only remains to show that choosing $z = (\frac{10a}{\ln a} + 2n)\ln(\frac{40a}{\ln a} +8n))$ satisfies $z \geq 2A(\ln A + C)$. Note that $a \geq 150$, $\ln(a) \geq 5$, and $e^2 \leq 8$.
%         \begin{align*}
%             2A(\ln A + C)
%             &= 2\left(n + \frac{a}{\ln(a) - 4}\right)\left(2 + \ln\left(n + \frac{a}{\ln(a) - 4}\right)\right) \\
%             &\leq 2\left(n + \frac{a}{\ln(a) - \frac{4}{5} \ln(a)}\right)\left(\ln 8 + \ln\left(n + \frac{a}{\ln(a) - \frac{4}{5}\ln(a)}\right)\right) \\
%             &= \left(2n + \frac{10a}{\ln(a)}\right) \ln\left(8n + \frac{40a}{\ln(a)}\right)
%         \end{align*}
%     \end{proof}
    
%     \begin{fact}\label{fact:ln-asymp}
%         For all $A, C \geq 0$, if $x \geq 2A(\ln A + C)$, then $x \geq A(\ln x + C)$.
%     \end{fact}
%     \begin{proof}
%         Let $g(x) = x - A(\ln x + C)$. It suffices to show that $g(x) \geq 0$ when $x \geq 2A(\ln A + C)$.
        
%         Consider the derivative of $g$: $g'(x) = 1 - \frac{A}{x}$. Note that $g'$ is increasing with $x$ and $g'(x) \geq \frac{1}{2}$ when $x \geq 2A$.
        
%         Therefore, for $x \geq 2A$, we have
%         \begin{align*}
%             g(x) 
%             &\geq \frac{1}{2}(x - 2A) + g(2A) \\
%             &= \frac{x}{2} - A + 2A - A(\ln(2A) + C) \\
%             &= \frac{x}{2} + A(1 - \ln 2 - \ln A - C) \\
%             &\leq \frac{x}{2} - A(\ln A + C).
%         \end{align*}
        
%         Thus, we get $g(x) > 0$ if $x \geq 2A(\ln A + C)$.
%     \end{proof}

% \todo{better incorporate in}

==> Beyond Sharkovsky Paper/supp_itineraries.tex <==
\section{More Examples for Itineraries}\label{asec:itineraries}

\subsection{Examples of Itineraries}\label{assec:it-exs}

Let the tent map and logistic map be defined by $\ftent{r}(x) = 2r\max(x, 1-x)$ and $\flog{r}(x) = 4rx(1-x)$ respectively, for parameter $r \in (0,1)$.

\begin{example}\label{ex:two-cycle}
    For all $r \in (\frac{1}{2}, 1]$, there is a two-cycle $C$ of itinerary 12 (which is the only itinerary for a 2-cycle) in $\ftent{r}$ with
    \[C = \paren{\frac{2r}{1 + 4r^2}, \frac{4r^2}{1 + 4r^2}}.\]
\end{example}

\begin{example}
    When $r = \frac{1+ \sqrt{5}}{4}$, there is a two-cycle $C$ of $\flog{r}$ with 
    \[C = \paren{ \frac{1}{2}, \frac{1+ \sqrt{5}}{4}}.\]
\end{example}

\begin{example}
    When $r \in [\frac{1+ \sqrt{5}}{4}, 1]$, $\ftent{r}$ has a three-cycle $C$ of itinerary 123 with 
    \[C= \paren{\frac{2r}{1 + 8r^3}, \frac{4r^2}{1 + 8r^3}, \frac{8r^3}{1 + 8r^3}}.\] 
    Note that this and Example~\ref{ex:two-cycle} are consistent with Sharkovsky's Theorem; whenever there exists a three-cycle, there also exists a two-cycle.
\end{example}

\begin{example}
    When $r \in [\frac{1}{2}, 1]$, there also exists a four-cycle $C$ of itinerary $1324$ for $\ftent{r}$ with 
    \[C = \paren{ \frac{8r^3 - 4r^2 + 2r}{16r^2 + 1},\frac{16r^4 - 8r^3 + 4r^2}{16r^2 + 1},\frac{16r^4 - 8r^3 + 2r}{16r^2 + 1}, \frac{16r^4 - 4r^2 + 2r}{16r^2 + 1}}.\]
    Again, this reaffirms Sharkovsky's Theorem, since this cycle always exists when the above three-cycle exists.
\end{example}

\begin{example}
    However, when $r \in (0.9196\dots, 1]$, there also exists a four-cycle $C$ of itinerary $1234$ for $\ftent{r}$ with 
    \[C= \paren{\frac{2r}{16r^2 + 1}, \frac{4r^2}{16r^2 + 1}, \frac{8r^3 }{16r^2 + 1}, \frac{16r^4}{16r^2 + 1}}.\] 
    This demonstrates a relationship \textit{beyond} Sharkovsky's theorem: whenever a $1234$ four-cycle exists, a $123$ three-cycle also exists. This will be integral to the bounds we show.
\end{example}

\begin{example}
    The triangle map from~\cite{telgarsky16}, $\ftent{1}$ has an increasing $p$-cycle $C_p$ for every $p \in \N$ with
    \[C_p = \paren{\frac{2}{1 + 2^p}, \frac{2^2}{1 + 2^p}, \dots, \frac{2^p}{1 + 2^p}}.\]
    Thus Theorem~\ref{thm:general-lb-cls} and Fact~\ref{fact:root-lb} retrieve the fact used by Telgarsky that $M(\ftent{1}) = \Omega(2^k)$.
\end{example}

\subsection{Orderings of Itineraries}\label{assec:order}
As has been mentioned before, the existence of some cycles can be shown to imply the existence of other cycles. 
Sharkovsky's Theorem famously does this by showing that if $p \triangleright p'$, then the existence of a $p$-cycle implies the existence of a $p'$-cycle.
Proposition~\ref{prop:half-inc-cycle} can be used to imply that the existence of a chaotic $p$-cycle implies the existence of a chaotic $(p-1)$-cycle.
These pose a broader question: Is there a complete ordering on all cycle itineraries that can appear in unimodal mappings? 
And does this ordering coincide with the amount of ``chaos'' induced by a cycle?

Researchers of discrete dynamical systems have thoroughly investigated these questions; we refer interested readers to~\cite{mss73, alseda2000} for a more comprehensive survey.
We introduce the basics of this theory as it relates to our results.

\cite{mss73} present a partial ordering over cyclic itineraries present in unimodal mappings, which serves as a measurement of the complexity of the function.
That is, two itineraries $\mathbf{a}$ and $\mathbf{a}'$ may be related analogously to Sharkovsky's Theorem with $\mathbf{a} \triangleright \mathbf{a}'$, if $f$ having itinerary $\mathbf{a}$ implies that $f$ has itinerary $\mathbf{a}'$.
% By Sharkovsky's theorem, for all $p \triangleright p'$, there exist itineraries $\mathbf{a}_p$ and $\mathbf{a}_{p'}$ of lengths $p$ and $p'$ respectively such that $\mathbf{a}_p \triangleright \mathbf{a}_{p'}$.
% However, this does not rule out the possibility that there \textit{also} exist $\mathbf{a}_p'$ and $\mathbf{a}_{p'}'$ of lengths $p$ and $p'$ with $\mathbf{a}_{p'}' \triangleright \mathbf{a}_{p}'$ instead.
% \cite{mss73} shows that there is such an ordering over itineraries on all unimodal functions.
This ordering for all cycles of length at most 6 is illustrated in Table~\ref{table:itineraries}.
For instance, if a unimodal map has a cycle with itinerary 12435, then it also has a cycle with itinerary 135246.

\begin{table}[]
    \centering
        \caption{For any unimodal function $f$, let $f_r(x) := rf(x)$ for $r > 0$. As $r$ increases, any such family obtains new cycles in the same order, and those cycles are super-stable in the same order. This translates Table~1 of \cite{mss73} to our notation and shows at what values of $r$, $\flog{r}$ has various super-stable cycles of length at most 6.\\}
    \begin{tabular}{|l|l|l|l|l|} \hline
        Cycle length $p$ & Itinerary  & Regime & $r$ s.t. super-stable for $\flog{r}$ & Cycle Type \\\hline\hline
        2 & 12 & Doubling & $0.8090$ & Primary \\ \hline
        4 & 1324 & Doubling & $0.8671$ & Primary \\ \hline
        6 & 143526 & Chaotic & $0.9069$ &  Primary \\ \hline
        5 & 13425 & Chaotic & $0.9347$ & Stefan, Primary \\ \hline
        3 & 123 & Chaotic & $0.9580$ & Stefan, Increasing, Primary \\ \hline
        6 & 135246 & Chaotic & $0.9611$ & \\ \hline
        5 & 12435 & Chaotic & $0.9764$ & \\ \hline
        6 & 124536 & Chaotic & $0.9844$ & \\ \hline
        4 & 1234 & Chaotic & $0.9901$ & Increasing \\ \hline
        6 & 123546 & Chaotic & $0.9944$ & \\ \hline
        5 & 12345 & Chaotic & $0.9976$ & Increasing \\ \hline
        6 & 123456 & Chaotic & $0.9994$ & Increasing \\ \hline
    \end{tabular}
    \label{table:itineraries}
\end{table}

We make several observations about the table and make connections to the itineraries discussed elsewhere in the paper.
\begin{itemize}
    \item The table does not contradict Sharkovsky's Theorem. 
    Note that $3 \triangleright 5 \triangleright 6 \triangleright 4 \triangleright 2$, and order in which the first itinerary occurs of a  period is the same as the Sharkovsky ordering:
    \[12 \triangleleft 1324 \triangleleft 143526 \triangleleft 13425 \triangleleft 123 .\] 
    \item The last cycle to occur for a given period is its increasing cycle and it occurs as $p$ increases (not with the Sharkovsky ordering of $p$):
    \[12 \triangleleft 123 \triangleleft 1234 \triangleleft 12345 \triangleleft 123456.\]
    \item The first cycle to appear for every odd period is its \textit{Stefan cycle} (123, 13425). 
    This is proved by~\cite{alseda2000} and justifies why Theorem~\ref{thm:odd-linf} relies on the existence of a Stefan cycle whenever there is an odd period.
    \item There exist cycles of power-of-two length (e.g. 1234) that induce non-power-of-two cycles (e.g. 123).
\end{itemize}

Following the last bullet point, we distinguish between the $2^q$-cycles that only induce cycles of length $2^{i}$ for $i < q$ and those that induce non-power-of-two cycles.
To do so, we say that the itinerary of a $p$-cycle is \textit{primary} if it induces no other $p$-cycle with a different itinerary.

We say that an itinerary $\ba'=a_1'\dots a_{2p}'$ of a $2p$-cycle is a \textit{2-extension} of itinerary $\ba = a_1\dots a_p$ of a $p$-cycle if \[a_i = \ceil{\frac{a_i'}{2}} = \ceil{\frac{a_{i+p}'}{2}}\] for all $i$.
For instance, $12$ is a 2-extension of $1$, $1324$ is of $12$, $15472638$ is of $1324$, and $135246$ is of $123$. 

Theorem 2.11.1 of \cite{alseda2000} characterizes which itineraries are primary.
It critically shows that a power-of-two cycle is primary if and only if it is composed of iterated 2-extensions of the trivial fixed-point itinerary 1. 
As a result, 1324 is a primary itinerary and 1234 is not.
This sheds further light on the warmup example given in Section~\ref{ssec:warmup} and expanded upon in Appendix~\ref{asec:warmup}, where $f_{1324}^k$ has a polynomial number of oscillations, while $f_{1234}^k$ has an exponential number.

According to Theorem~2.12.4 of \cite{alseda2000}, the existence a non-primary itinerary of any period implies the existence of some cycle with period not a power of two. 
Hence, $f$ can \textit{only} be in the doubling regime (where all periods are powers of two) if all of those power-of-two periods are primary.
The existence of any non-primary power-of-two period (such as 1234 or 13726548) implies that the $f$ is in the chaotic regime.


This ordering can also be visualized using the bifurcation diagrams in Figure~\ref{fig:bifurcation}.
The diagram plots the convergent behavior of $f^k_r(x)$ for large $k$, where $r$ is some parameter and reflects the complexity of the unimodal function $f_r$. 
(When $r = 0$, $f_r = 0$; when $r = 1$, $\xmax = 1$, and $\osci{0,1}(f^k) = 2^k$.)
As $r$ increases, the number of oscillations of $f_r^k$ increases and with it, new cycles are introduced.
Each new cycle has a \textit{stable} region over parameters $r$ where $f_r^k(x)$ converges to the cycle, and the bifurcation diagram visualizes when each of these stable regions occurs.
While the three functions families $f_r$ have different underlying unimodal functions, they produce qualitatively identical bifurcation diagrams that feature the same ordering of itineraries.

\begin{figure}
    \centering
    \includegraphics[width=0.32\textwidth]{fig/fig-bifurcation-logistic.png}
    \includegraphics[width=0.32\textwidth]{fig/fig-bifurcation-flat-tent.png}
    \includegraphics[width=0.32\textwidth]{fig/fig-bifurcation-sine.png}
    \caption{Bifurcation diagrams---which display the qualitative behavior of a family of functions $f_r$ as the parameter $r\in[0,1]$ changes---showing the convergence behavior for iterates $f_r^k(x)$ for large $k$. For fixed $r$ on the horizontal axis, the points plotted correspond to $f^k(x_0)$ for very large $k$. Regions of $r$ where a vertical slice contains $p$ discrete points indicates the existence of a \textit{stable} $p$-cycle, since $f^k(x_0)$ converges exclusively to those points. 
    Regions where the slice has a dispersed mass of points exhibit chaos. As $r$ increases, cycles of different itineraries appear and experience stability in the same order indicated by Table~\ref{table:itineraries}. In the first plot, $f_r$ is the logistic map $f_r(x) = \flog{r}(x) = 4rx(1-x)$. The second $f_r$ is the``flat tent map,'' $f_r(x) = \min\{\frac{5rx}{2}, r, \frac{5rx}{2}(1-x)\}$, and the third is the sine map, $f_r(x) = r \sin(\pi x)$.
    The three are qualitatively identical and exhibit self-similarity.}
    \label{fig:bifurcation}
\end{figure}

Our discussions of the \textit{doubling} and \textit{chaotic} regimes in Section~\ref{sec:phase} are inspired by these bifurcation diagrams.
Parameter values $r$ are naturally partitioned into two categories: those on the left side of the diagram where the plot is characterized by a branching of cycles (the doubling regime) and those on the right side where there are extended regions of chaos, interrupted by small stable regions (the chaotic regime).


\subsection{Identifying Increasing Cycles in Unimodal Maps}\label{assec:identifying}
It is straightforward to determine whether a symmetric and unimodal $f$ has an increasing $p$-cycle.
Algorithmically, one can do so by verifying that $f(\frac{1}{2}) > \frac{1}{2}$ and counting how many consecutive values of $k \geq 2$ satisfy $f^k(x_0) < \frac{1}{2}$.
\begin{proposition}\label{prop:half-inc-cycle}
    Consider some $p \geq 2$ and a symmetric unimodal mapping $f$.
    $f$ has an increasing $p$-cycle if \[f^2\paren{\frac{1}{2}} < \dots < f^p\paren{\frac{1}{2}} \leq \frac{1}{2} < f\paren{\frac12},\] then $f$ has an increasing $p$-cycle.
\end{proposition}


\begin{proof}
    % First, we show that the existence of increasing $p$-cycle implies chain of inequalities.
    % Let $x_1 < \dots < x_p$ be that cycle.
    % Because $\frac12$ maximizes $f$, $f(\frac12) \geq x_p > \frac12$. 
    % (If $x_p \leq \frac12$, then the existence of the cycle would be contradicted, because $f$ would be monotonically increasing on $[x_1, x_p]$.)
    % Because $f$ is monotonically decreasing on $[\frac12, 1]$, $f^2(\frac12) \leq f(x_p) = x_1$.
    % By $f$'s monotonicity on $[0, \frac12]$, we can inductively show that $f^{j+1}(\frac12) \leq x_j$.
    
    % Now, we prove the existence of a an increasing $p$-cycle given the assumptions about $f^j(\frac12)$.
    Refer to Figure~\ref{fig:inc-cycle} for a visualization of the variables and inequalities defined.

    Let $x' = f(\frac{1}{2})$.
    By the unimodality of $f$ and the fact that $x' > \frac{1}{2}$, there exists some $x'' > \frac{1}{2}$ such that \[f(x'') < f^2(x'') < \dots < f^{p-1}(x'') = \frac{1}{2}.\]
    
    Because $f$ is monotonically increasing on $[0, \frac{1}{2}]$, the following string of inequalities hold.
    \begin{equation}\label{eq:interleave}
        f(x') \leq f(x'') < f^2(x') \leq f^2(x'') <
        \dots < f^{p-1}(x') \leq f^{p-1}(x'') = \frac{1}{2}
    \end{equation}
    It then must hold that $x' \geq x''$.
    
    Let $g(x) = f^p(x) - x$ and note that $g$ is continuous. 
    Because $\frac{1}{2}$ maximizes $f$, it must be the case that $f^p(x') \leq x'$ and $g(x') \leq 0$.
    Because $f^{p}(x'') = x'$ and $x'' \leq x'$, $g(x'') \geq 0$.
    Hence, there exists $x^* \in [x'', x']$ such that $g(x^*) = 0$ and $f^p(x^*) = x^*$.
    
    Since $x^* \in [x'', x']$, it must also be the case that $f^j(x^*) \in [f^j(x'), f^j(x'')]$ for $j \in [p-1]$.
    By Equation~\eqref{eq:interleave}, it follows that
    \[f(x^*) < f^2(x^*) < \dots < f^{p-1}(x^*) < f^p(x^*) = x^*.\]
    Hence, there exists an increasing $p$-cycle.
\end{proof}

\begin{figure}
    \centering
    \input{fig/fig-inc-cycle}
    \caption{Visualizes the proof of Proposition~\ref{prop:half-inc-cycle}.}
    \label{fig:inc-cycle}
\end{figure}


==> Beyond Sharkovsky Paper/supp_lb.tex <==
\section{Additional Proofs for Section~\ref{sec:lb}}

\subsection{Proof of Lemma~\ref{lemma:increasing-constant-osc}}\label{assec:inc-constant-osc-proof}
We restate and prove the lemma. This is the main technical lemma that we use to get the sharper depth-width tradeoffs and the improved notion of \textit{constant} approximation.

\lemmaincreasingconstantosc*
%\label{lem:main}
\begin{proof}
We first lower-bound the total number of oscillations that will appear an increasing $p$-cycle is present. 
Later, we show that the size of the oscillations is large as well.

Because we have an increasing cycle of itinerary $12\dots p$, we assume (wlog) that the cycle is $(x_1, \dots, x_p)$ with $x_1 < x_2 < \dots < x_p$. 
Define intervals $I_j \vcentcolon= [x_j, x_{j+1}]$ for $j \in \{1, \dots, p-1\}$. Because $f$ is continuous, we conclude that $I_{j+1} \subset f(I_{j})$ for all $j < p$ and $I_{j} \subset f(I_{p-1})$ for all $j$.
Figure~\ref{fig:inc-intervals} visualizes these relationships.

\begin{figure}
    \centering
    \input{fig/fig-inc-intervals}
    \caption{Visualizes the intervals $I_1,\dots, I_{p-1}$ defined in the proof of Lemma~\ref{lemma:increasing-constant-osc} and which intervals $f$ maps to one another when $f$ has an increasing $p$-cycle.}
    \label{fig:inc-intervals}
\end{figure}

Using the methods of \cite{cnpw19}, we define $y^{(k)} \in \N^{p-1}$ such that $y^{(k)}_j$ is a lower bound on the number of times $f^k$ passes through interval $I_j$, or \[\osci{x_{j}, x_{j+1}}(f^k) \geq y^{(k)}_j.\] We can then encode the interval relationships above with $y^{(k+1)} = A_p y^{(k)}$ where $y^{({0})}$ is a vector of all ones and and $A_p \in \bit^{(p-1) \times (p-1)}$ with $(A_p)_{i, j} = \indicator{j = p-1 \text{ or } i = j + 1}$. We get the following adjacency matrix for the intervals, capturing the mapping relationships (under $f$) between them:
\[A_p = 
\begin{bmatrix}
    0 & 0 & 0 & \cdots & 0 & 1 \\
    1 & 0 & 0 & \cdots & 0 & 1 \\
    0 & 1 & 0 & \cdots & 0 & 1 \\
    0 & 0 & 1 & \cdots & 0 & 1 \\
    \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
    0 & 0 & 0 & \cdots & 1 & 1
\end{bmatrix}.\]

We find the characteristic polynomial of $A_p$ and lower-bound $y^{(k+1)}$ with the spectral radius of $A_p$. 
We show by induction on $p \geq 3$ that
\[\det(A_p - \lambda I) = (-1)^{p-1} \paren{\lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i}.\]

For the base case $p = 3$, we have:
\begin{align*}
    \det(A_3 - \lambda I)
    &= \begin{vmatrix}
        -\lambda & 1 \\
        1 & 1 -\lambda
    \end{vmatrix}
    = \lambda^2 - \lambda - 1,
\end{align*}
which satisfies the desired form.

Now, we show the inductive step by expanding the determinant of $A_p - \lambda I$.

{\small
\begin{align*}
    \det(A_p - \lambda I)
    &= 
    \begin{vmatrix}
        -\lambda & 0 & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & 0 & \cdots & 0 & 1 \\
        0 & 1 & -\lambda & \cdots & 0 & 1 \\
        0 & 0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix}
    = -\lambda 
    \begin{vmatrix}
        -\lambda & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & \cdots & 0 & 1 \\
        0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix} - 
    \begin{vmatrix}
        0 & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & \cdots & 0 & 1 \\
        0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix}.
\end{align*}}

The left determinant exactly equals $\det(A_{p-1} - \lambda I)$, which we can expand using the inductive hypothesis.
The second equals $(-1)^{p-2}$, because $p-2$ row swaps (which are elementary row operations) can be used to move the first row to the bottom and make the matrix upper-triangular with diagonals of one. 
We conclude the inductive step below.

\begin{align*}
        \det(A_p - \lambda I)
        &= -\lambda \det(A_{p-1} - \lambda I) - (-1)^{p-2} \\ 
    &= -\lambda (-1)^{p-2} \left(\lambda^{p-2} - \sum_{i=0}^{p-3} \lambda^i \right) + (-1)^{p-1}
    = (-1)^{p-1} \left(\lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i\right).
\end{align*}

We find the eigenvalues of $A_p$ by finding the roots of the polynomial
\[P(x) = \lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i = 0.\] 
Observe that there must be a root greater than $1$ because $P(1) = 2 - p < 0$ and $P(2) = 1 > 0$. Equivalently, if $\lambda \neq 1$,
\[P(x) = \lambda^{p-1} - \frac{1 - \lambda^{p-1}}{1 - \lambda} = \frac{\lambda^p - 2\lambda^{p-1} + 1}{\lambda - 1} =  0.\]

Hence, finding the largest root of $P$ is equivalent to finding the largest root of $\lambda^p - 2\lambda^{p-1} + 1$, which is $\rhoinc{p}$ by definition.


This implies that the spectral radius of $A_p$, sp$(A_p)=\rhoinc{p}>1$, and hence, we also have sp$(A_p^k)=$ sp$(A_p)^k=\rhoinc{p}^k$. Since all the elements in $A_p$ and in $A_p^k$ are non-negative, then the infinity norm of $A_p^k$ is by definition the maximum among its row sums. Since the last column of $A_p$ is the all 1's vector, the largest row sum in $A_p^k$ appears at its last row:

\[
||A_p^k||_{\infty} = \sum_{j=1}^{p-1}(A_{p}^k)_{p-1,j}
\]



We can now use the fact that the infinity norm of a matrix is larger than its spectral norm:
\[
||A_p^k||_{\infty} \ge  \rhoinc{p}^k
\]
%Therefore, there exists at least one interval $I_{j^*}$ which is crossed at least $\rho^k$ times by $f^k$, so $\osci{x_{j^*}, x_{j^*+1}}(f^k) \geq \rho^k$.
We conclude that there exists at least one interval $I_{j^*}$ (e.g., the interval $I_{p-1}$) which is crossed at least $\rhoinc{p}^k$ times by $f^k$, so $\osci{x_{j^*}, x_{j^*+1}}(f^k) \geq \rhoinc{p}^k$.

Thus, for some $a',b'$ we get $\osci{a', b'}(f^k) \geq \rhoinc{p}^k$. But can we find $a',b'$ with large difference $b'-a'$?

Now, we show that the intervals traversed are sufficiently large, in order to lower-bound $\osci{a,b}(f^k)$ with $b-a \geq \frac{1}{18}$.
By Lemma~\ref{lemma:interval-inc-cycle}, there exists some $j$ with $x_{j+1} - x_{j} \geq \frac{1}{18}$.
It suffices to show that $f^k$ traverses the interval $I_j$ sufficiently many times.

From earlier in the proof, there exists some $j^*$ such that $f$ crosses $I_{j^*}$ at least $N\vcentcolon=\rhoinc{p}^{k}$ times. 
We conclude by showing that every other interval is traversed at least half as often as this most popular interval, which suggests that $\osci{x_{j}, x_{j+1}}(f) \geq \frac{N}{2}$.
    

    
For $A \in \mathbb{R}^{(p-1)\times (p-1)}$ as defined earlier in the section and for $y^{(k)} \vcentcolon= A^{k} \vec{1}$, we argue inductively that the elements of $y^{(k)}$ are non-decreasing and that $y^{(k)}_{p-1} \leq 2 y^{(k)}_1$. For the base case, this is trivially true for $k = 0$.

Suppose it holds for $k$.
    By construction, we have $y^{(k+1)}_1 = y^{(k)}_{p-1}$ and $y^{(k+1)}_j = y^{(k)}_{j-1} + y^{(k)}_{p-1}$ for all $j > 1$.
    By the inductive hypotheses,
    \[y^{(k+1)}_1 \leq y^{(k+1)}_2 \leq \dots \leq y^{(k+1)}_{p-1} \leq 2y^{(k+1)}_1.\]
    
Therefore, $f^k$ crosses interval $I_{j}$ at least $\frac{N}{2}$ times, and $I_j$ has width at least $\frac{1}{18}$. The claim immediately follows.
\end{proof}
    
\begin{lemma}\label{lemma:interval-inc-cycle}
    For some $p \geq 3$, consider a symmetric concave unimodal function $f$ with an increasing $p$-cycle of $x_1 < \dots < x_p$. Then, there exists $j \in [p-1]$ such that $x_{j+1} - x_j \geq \frac{1}{18}$.
\end{lemma}

\begin{proof}
By the continuity of $f$, note that $[x_1, x_p] \subset f^3([x_{p-3}, x_{p-2}])$. 
There then exists some $y_1 \in [x_{p-3}, x_{p-2}]$ such that $f^3(y_1) = y_1$, $y_2\vcentcolon= f(y_1) \in [x_{p-2}, x_{p-1}]$, and $y_3\vcentcolon= f(y_2) \in [x_{p-1}, x_p]$.
Thus, if $f$ has a maximal $p$-cycle, then $f$ also has a 3-cycle corresponding to $x_{p-3} < y_1 < y_2 < y_3 < x_p$.

We now show that $y_3 - y_1$ must be sufficiently large by concavity.
For $f$ to be concave, the following inequality must hold:
\begin{align*}
    \frac{f(y_1) - f(0)}{y_1 - 0} \geq \frac{f(y_2) - f(y_1)}{y_2 - y_1} > 0  > \frac{f(y_3) - f(y_2)}{y_3 - y_2} \geq \frac{f(1) - f(y_3)}{1 - y_3},
\end{align*}
or equivalently,
 \[\frac{y_2}{y_1} \geq \frac{y_3 - y_2}{y_2 - y_1} > 0 > -\frac{y_3 - x_1}{y_3 - y_2} \geq -\frac{y_1}{1 - y_3}.\]
 
In addition, note that $y_1 < \frac{1}{2}$ and $y_3 > \frac{1}{2}$. 
If the former were false, then $f(y_2) \leq f(y_1)$ (by unimodality), which contradicts $y_3 > y_2$. If the latter were false, then $f(y_3) > f(y_2)$, which contradicts $y_1 < y_3$.

We consider two cases and show that either way, the interval must have width at least $\frac{1}{6}$.
\begin{itemize}
    \item If $y_2 - y_1 \leq \frac{2}{5}(y_3 - y_1)$, then $\frac{y_3 - y_2}{y_2 - y_1} \geq \frac{3}{2},$
    which mandates that $y_1 \leq \frac{2y_2}{3}$ to ensure concavity. Thus,
    \[y_3 - y_1 \geq y_3 - \frac{2y_2}{3} \geq \frac{y_3}{3} \geq \frac{1}{6}.\]
    \item If $y_2 - y_1 \geq \frac{2}{5}(y_3 - y_1)$, then $\frac{y_3 - y_1}{y_3 - y_2} \geq \frac{5}{3},$ and thus $y_1 \geq \frac{5}{3}(1 - y_3)$ and $y_3 \geq 1 - \frac{3y_1}{5}$. Then,
    \[y_3 - y_1 \geq 1 - \frac{3y_1}{5} - y_1 = 1 - \frac{8y_1}{5} \geq \frac{1}{5}.\]
\end{itemize}

Thus, we must have \[\max\{x_{p-2} - x_{p-3}, x_{p-2} - x_{p-1}, x_p - x_{p-1}\} \geq \frac{1}{18}.\qedhere\]

\end{proof}

\subsection{Proof of Fact~\ref{fact:root-lb}}\label{assec:fact}
\factrootlb*
\begin{proof}

Let $P_{\mathrm{inc}, p}(\lambda) = \lambda^{p} - 2\lambda^{p-1} + 1$.

First, observe that $\rhoinc{p} < 2$, because $P_{\mathrm{inc}, p}(\lambda) > 0$ whenever $\lambda \geq 2$. 
We lower-bound $\rhoinc{p}$ by finding some $\lambda$ for each $p$ such that $P_{\mathrm{inc}, p}(\lambda) \leq 0$ or equivalently $\lambda^{p-1}(2 - \lambda) \geq 1$ for all $p\geq3$, which bounds $\rhoinc{p}$ by the Intermediate Value Theorem. 

Consider $\lambda = 2 - \frac{4}{2^p}$. Then,
\begin{align*}
    \lambda^{p-1}(2 - \lambda)
    &= \paren{2 - \frac{4}{2^p}}^{p-1} \cdot \frac{4}{2^p}
    = 2 \paren{1 - \frac{2}{2^p}}^{p-1} \\
    &\geq 2 \paren{1 - \frac{2(p-1)}{2^p}}
    = 2 - 2 \cdot \frac{p-1}{2^{p-1}} \\
    &\geq 2 - 2 \cdot \frac{1}{2} = 1.\qedhere
\end{align*}
\end{proof}

\subsection{Previous Results about Hardness of Approximating Oscillatory Functions}

We rely on prior results from~\cite{cnpw19, cnp20} to show that an iterated function $f^k$ is inapproximable by neural networks.
These results hold if $f^k$ has sufficiently many crossings of some interval.
We apply these results later with improved bounds on both the number and the size of crossings.

\cite{cnpw19} show that the classification error of $f^k$ can be bounded if there are enough oscillations.

\begin{theorem}[\citep{cnpw19}, Section 4]\label{thm:general-lb-cls}
    Consider any continuous $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a, b}(f) = \Omega(\rho^t)$ and suppose $u \leq \frac{1}{8}\rho^{k/\ell}$.
    Then, for $t = \frac{a+b}{2}$, there exists $S$ with $\abs{S} =  \frac{1}{2} \floor{\rho^k}$ samples such that 
    \[\errcls{S,t}{f^k, g}  \geq \frac{1}{2} - \frac{(2u)^\ell}{n}.\]
\end{theorem}

We adapt that claim to lower-bound the $L_\infty$ approximation of $f^k$ by $g$.

\begin{corollary}\label{cor:general-lb-linf}
    Consider any continuous $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a, b}(f) = \Omega(\rho^t)$ and suppose $u \leq \frac{1}{8}\rho^{k/\ell}$.
    Then, 
    \[\norm[\infty]{f^k - g} \geq \frac{b-a}{2}.\]
\end{corollary}
\begin{proof}
    By Theorem~\ref{thm:general-lb-cls}, there exists some $x \in [0,1]$ such that (wlog) $f^k(x) \leq a$ and $g(x) \geq \frac{a + b}{2}$.
    The conclusion for the $L_\infty$ error is immediate by definition.
\end{proof}

\cite{cnp20} give a lower-bound on the ability of a neural network $g$ to $L_1$-approximate $f^k$, provided a correspondence between the Lipschitz constant of $f$ and the rate of oscillations $\rho$.

\begin{theorem}[\cite{cnp20} Theorem 3.2]\label{thm:general-lb-l1}
    Consider any $L$-Lipschitz $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a,b}(f) = \Omega(\rho^t)$. If $L \leq \rho$ and $u \leq \frac{1}{16} \rho^{k/\ell}$, then 
    \[\norm[1]{f^k - g} = \Omega((b-a)^2).\]
\end{theorem}

The Lipschitzness assumption is extremely strict, especially because they show in their Lemma~3.1 that $L \geq \rho$ whenever $f$ has a period of odd length.

\subsection{Proof of Corollary~\ref{cor:main-l1}}\label{assec:cor-main-proof}
\cormainl*
\begin{proof}
    This theorem follows from Theorem~\ref{thm:main-l1} and Lemma~\ref{lemma:increasing-constant-osc}.
    Because $\ftent{\rho_p/2}$ is $\rho_p$-Lipschitz, it remains only to prove that there exists an increasing $p$-cycle.
    We show that 
    \[\frac{1}{2}, f\paren{\frac12},\dots, f^{p-1}\paren{\frac12}\]
    is such a cycle.
    
    By definition of the tent map, $f(\frac12) = \frac{\rhoinc{p}}2$ and $f^2(\frac12) = \rhoinc{p} (1 - \frac{\rhoinc{p}}{2})$.
    If we assume for now that $f^j(\frac12) \leq \frac12$ for all $j \in \{2, \dots, p-1\}$,
    then
    \[f^p\paren{\frac12} = \rhoinc{p}^{p-1}\paren{1 - \frac{\rhoinc{p}}2} = -\frac{1}{2}\paren{\rhoinc{p}^p - 2\rhoinc{p}^{p-1} + 1} + \frac{1}{2} = 0 + \frac{1}{2}.\]
    
    Because $f^p(\frac12) = \frac12$ and we assumed that $f^{j+1}(\frac12) = \rhoinc{p} f^{j}(\frac12)$ for $j \geq 2$ and $\rho > 1$, it must be the case that $f^j(\frac12) \leq \frac12$ for all $j \in \{2, \dots, p-1\}$.
    
    Lemma~\ref{lemma:increasing-constant-osc} thus implies that $f^k$ has $\Omega(\rhoinc{p}^k)$ crossings, which enables us to complete the proof by invoking Theorem~\ref{thm:main-l1}, since the Lipschitzness condition is met.
    % To apply them, it remains only to prove that the Lipschitz constant of $\ftent{r}$ is $\rho$, or equivalently, $r = \frac{\rho}{2}$.
    % Given $\ftent{r}^p(\frac12) = \frac12$, we show that $\frac12$ must be contained in an increasing $p$-cycle.
    % Suppose not.
    % There exists some increasing $p$-cycle $x_1 < \dots < x_p$ and we assume that it does not contain $\frac12$.
    % It must be the case that $x_{p-2} < \frac12$; assuming otherwise would cause $f(x_{p-2}) \geq f(x_{p-1})$, a contradiction.
    % Because $\frac12$ maximizes $f$, $x_p \leq f(\frac12)$.
    % Since $f$ decreases on $[\frac12, 1]$, it follows that $f^2(\frac12) \leq x_1$.
    % $f$ increasing on $[0, \frac12]$ implies that $f^{j+1}(\frac12) \leq x_{j}$ for all $j \in [p-1]$.
    % Therefore, $f^{j}(\frac12) \neq \frac12$ for all $j \in [p]$ and $f^2(\frac12) <  \dots < f^{p}(\frac12) = \frac12$.
    % We conclude that $\frac12$ is contained in an increasing $p$-cycle, which has a $123\dots p$ itinerary; call that cycle $x_1', \dots, x_{p-1}'= \frac12, x_p'$
    % % For $\ftent{r}$ to have a super-stable $p$-cycle, it must pass through $\frac{1}{2}$. Because $\ftent{r}$ only has zero-slope at $x = \frac{1}{2}$, a fixed point $x_1$ for $\ftent{p}$ will only be super-stable if $f^j(x_1) = \frac{1}{2}$ for some $j \in [p]$. (Otherwise $\frac{d}{dx} f^j(x_1) \neq 0$, and $x_1$ cannot be part of a super-stable cycle.)
    % % Therefore, there must exist a cycle of the form
    % % \[x_1 < \dots < x_{p-2} < x_{p-1} = \frac{1}{2} < x_{p} = r,\]
    % % which signals an $12\dots p$ itinerary.
    % % Note that $x_{p-1} = \frac{1}{2}$ because any assignment would contradict the cycle being increasing.
    % % If $x_p = \frac{1}{2}$, then $x_1 = f(x_p) = r > x_p > x_1$.
    % % If $x_j = \frac{1}{2}$ for $j < p-1$, then $x_p = f(x_{p-1}) < f(x_{j}) = x_{j+1} < x_p$, both contradictions.
    % We apply the definition of the tent map to note that $x_{j}' = 2rx_{j-1}'$ for $j \in \{2, \dots, p\}$ and $x_1' = 2r(1 - x_p')$.
    % Thus, 
    % \[\frac{1}{2} = (2r)^{p-2} x_1' = (2r)^{p-1}(1 - x_p') = (2r)^{p-1}(1 - r).\]
    % Equivalently, 
    % \[(2r)^p - 2 (2r)^{1-p} + 1 = 0,\]
    % which has $\rho = 2r$ as its largest root.
    % Hence, $\ftent{r}$ has Lipschitz constant $\rho$ and we can apply Theorem~\ref{thm:main-l1}.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:odd-constant-osc}}\label{assec:lemma-odd-proof}

\lemmaoddconstantosc*

\begin{proof}
    By Theorems~2.94 and 3.11.1 of~\cite{alseda2000}, there exists a $p$-cycle of the form \[x_p < x_{p-2} < \dots < x_3 < x_1 < x_2 < x_4 < \dots < x_{p-1},\]
    which is known as a \textit{Stefan cycle}.
    The analysis of Section~3.2 of~\cite{cnp20} shows that $\osci{[x_1, x_2]}(f^{k}) \geq \rhoodd{p}^{k}$.
    Their exploitation of the relationships between intervals is visualized in Figure~\ref{fig:stefan-intervals}.
    By the continuity of $f$, applying $f$ an additional $p-1$ times gives $\osci{[x_p, x_1]}(f^{k+p-1}) \geq \rhoodd{p}^{k}$.
    Because $[x_{p-2}, x_1] \subset [x_p, x_1]$, applying $f$ one more time gives $\osci{[x_2, x_{p-1}]}(f^{k+p}) \geq \rhoodd{p}^k$.
    
    
    \begin{figure}
        \centering
        \input{fig/fig-stefan-intervals}
        \caption{Gives an example of a Stefan $p$-cycle (which is relied upon in Lemma~\ref{lemma:odd-constant-osc} and demonstrates the interval relationships). Analogous to Figure~\ref{fig:inc-intervals}.}
        \label{fig:stefan-intervals}
    \end{figure}
    
    Hence, by redefining $k$, we have 
    \[\max\{ \osci{[x_1, x_2]}(f^{k}), \osci{[x_2, x_{p-1}]}(f^{k}), \osci{[x_p, x_1]}(f^{k})\} \geq \rhoodd{p}^{k-p}.\]
    
    Since $[x_p, x_{p-1}]$ is the disjoint union of $[x_1, x_2]$, $[x_2, x_{p-1}]$, and $[x_p, x_1]$, there exists $[a, b] \subset [x_p, x_{p-1}]$ with $b- a \geq \frac{1}{3}(x_{p-1} - x_p)$ such that $\osci{[a,b]}(f^{k}) \geq \\rhoodd{p}^{k-p}$.
    
    The problem reduces to placing a lower bound on $x_{p-1} - x_p$.
    To do so, we derive contradictions on the concavity and symmetry of $f$. 
    Let $r = f(\frac12) \in (x_p, 1)$ be the the largest outcome of $f$, and
    let \[a= \sup_{x, x' \in [1-r, r]} \abs{\frac{f(x) - f(x')}{x - x'}}\] be the maximum absolute slope of $f$ on $[1-r,r]$. $a$ must be finite by the concavity and continuity of $f$, and if $f$ is differentiable, $a = f'(1-r) = -f'(r)$.
    Thus, $f$ is $a$-Lipschitz on that interval.
    
    Because $f([x_p, x_{p-1}]) \subseteq [x_p, r] \subset [1-r, r]$, it follows that $\abs{f^2(x) - f^2(x')} \leq a^2 \abs{x - x'}$.
    Thus, $x_2 - x_p \leq a^2(x_{p-2} - x_{p})$ and $x_2 - x_p \leq x_4 - x_p \leq a^2(x_2 - x_{p-2})$.
    Averaging the two together, we have $x_2 - x_p \leq \frac{a^2}{2}(x_2 - x_{p})$, which means $a \geq \sqrt{2}$.
    
    To satisfy concavity, the following must be true:
    \[\frac{f(1-r) - f(0)}{1-r - 0} = \frac{f(r)}{1-r} \geq a \geq \sqrt{2}.\]
    
    We rearrange the inequality and apply properties of monotonicity to lower-bound $r$ away from $\frac12$:
    \[r 
    \geq 1 - \frac{f(r)}{\sqrt{2}}  
    \geq 1 - \frac{f(x_{p-1})}{\sqrt{2}}
    = 1 - \frac{x_p}{\sqrt{2}}
    > 1 - \frac1{2\sqrt2}.\]
    
    It also must be the case for any $x \in [\frac12, 1]$, that:
    \[\abs{\frac{f(x) - f\paren{\frac12}}{x - \frac12}} \leq 2.\]
    Otherwise, the concavity of $f$ would force $f(\frac12) > 1$.
    
    We finally assemble the pieces to lower-bound the gap between $x_{p-1}$ and $x_p$:
    \begin{align*}
        x_{p-1} - x_p
        &\geq x_{p-1} - \frac12 
        \geq -\frac{1}{2} \paren{f(x_{p-1}) - f\paren{\frac12}}
        = \frac{r}{2} - \frac{x_p}{2} \\
        &> \frac{1}{2} - \frac1{4\sqrt{2}} - \frac14 
        = \frac14 - \frac1{4\sqrt{2}}
        > 0.07.\qedhere
    \end{align*}
    
    
    
    % Under the assumption, it must be the case that $r \leq 0.54$. If not, then 
    % \[\frac{f(x_p) - f(\frac12)}{x_p - \frac12} > \frac{0.04}{0.02} = 2.\]
    % By concavity, this would imply that $f(\frac12) > 1$, which is a contradiction. Hence, we continue with $r \leq 0.54$.
    
    % By the monotonicity of $f$ on $[\frac12, 1]$ and the fact that $r > x_{p-1}$, it follows that $f(r) < x_{p} < \frac12$.
    
    % By symmetry and unimodality of $f$, $1-x_{p-1} \leq x_p$, since $f(x_{p-1}) < f(x_p)$.
    % The concavity of $f$ implies the following:
    % \begin{align*}
    %     -\frac{x_p}{1 - x_{p-1}} 
    %     &= \frac{f(1) - f(x_{p-1})}{1 - x_{p-1}}
    %     \leq \sup_{x, x' \in [1/2, x_{p-1}]} \frac{f(x) - f(x')}{x - x'} \\
    %     &= \sup_{x, x' \in [1-x_{p-1}, x_{p-1}]} -\abs{\frac{f(x) - f(x')}{x - x'}} 
    %     \leq \sup_{x, x' \in [x_p, x_{p-1}]} -\abs{\frac{f(x) - f(x')}{x - x'}}\\
    %     &= -a \leq -\sqrt{2}.
    % \end{align*}
    
    % Thus, $\abs{f'(x)}$ is maximized on the interval $[x_p, x_{p-1}]$ at $x_{p-1}$.
    % By concavity, it must be the case that $f'(x)\leq -\sqrt{2}$ whenever $x \in [x_{p-1}, 1]$ and thus, 
    % \[\frac{f(1) - f(x_{p-1})}{1 - x_{p-1}} = -\frac{x_p}{1 - x_{p-1}} \leq -\sqrt{2}.\]
    % Equivalently,
    % \[x_{p-1} \geq 1 - \frac{x_p}{\sqrt{2}}.\]
    
    % We conclude with the lower bound on $x_{p-1} - x_p$. Note that $x_p < \frac{1}{2}$ by symmetry and the fact that $f(x_p) \leq f(x_{p-2})$.
    % \begin{align*}
    %     x_{p-1} - x_p
    %     &\geq 1 - \frac{x_p}{\sqrt{2}} - x_p 
    %     = 1 - \frac{2 + \sqrt{2}}{2} x_p \\
    %     &\geq 1 - \frac{2 + \sqrt{2}}{4} > 0.12.\qedhere
    % \end{align*}
\end{proof}

\subsection{Necessity of Symmetry and Concavity Assumptions in Theorems~\ref{thm:main-linf} and \ref{thm:main-l1}}\label{assec:sym-conc}

We demonstrate the weakness of the bounds promised by \cite{cnpw19, cnp20, bzl20} and argue that our assumptions of symmetry and concavity are necessary in order to avoid such non-vacuous bounds.
To do so, we exhibit two families of functions in Propositions~\ref{prop:need-symmetry} and ~\ref{prop:need-concavity} which contain functions with increasing $p$-cycles for every $p$ that produce large numbers of oscillations, yet are trivial to approximate because their oscillations can be made arbitrarily small.
The functions considered in both cases are unimodal and lack symmetry and concavity respectively.

These expose a fundamental shortcoming of other approaches to the hardness of neural network approximation in the aforementioned works because they all rely on showing that for every mapping $f$ meeting some condition (e.g. odd period, positive topological entropy), there exists some $[a,b] \in [0,1]$ where $\osci{a,b}$ is exponentially large, and hence no poly-size shallow neural network $g$ can obtain $L_{\infty}(f^k, g) \leq P(b-a)$ for some polynomial $P$.
However, because $[a,b]$ depends on $f$, their difference can potentially be arbitrarily small. 
The propositions show that this concern is significant and that $[a,b]$ indeed becomes arbitrarily narrow for simple 3-periodic functions. 
While \cite{cnpw19} avoid addressing this issue head-on by focusing on classification error over $L_\infty $ error, their classification lower-bounds rely on misclassification of points whose actual distance can be shrinking (see for example Figure~\ref{fig:asymmetric}).
%microscopically small degrees of inapproximation on a small number of points.


The implications of these propositions contrast with the more robust hardness results we present in Theorems~\ref{thm:main-linf}, \ref{thm:main-l1}, \ref{thm:odd-linf}, and \ref{thm:odd-l1}, which leverage unimodality, symmetry, and concavity to ensure that the accuracy of approximation can be no better than some constant (independent on $f,p$) when the neural network $g$ is too small.
% In order for the accuracy of the neural network approximation to be lower-bounded by a constant value, Theorems~\ref{thm:main-linf} and \ref{thm:main-l1} assume that the unimodal function $f$ is additionally concave and symmetric. 
We show here that those assumptions are necessary by exhibiting functions that satisfy all but one, and become easy to $L_\infty$-approximate with small depth-2 ReLU networks.

% \todo{Show that ICML and ICLR fail}

% \todo{Note that prior analysis doesn't give us anything about setting for why large L fails; we show why that's the case}

% \todo{mention that oscillation LBs for increasing cycle still give large number of oscillations even if not unimodal (just small oscillations)}

% \todo{Or, just directly attack previous constructions... Show that oscillation size becomes arbitrarily small}

% \vaggos{forward pointer in section where we dwell on cosntant error rates.}


\begin{proposition}\label{prop:need-symmetry}
For $p \geq 3$ and for sufficiently small $\eps > 0$, there exists a concave unimodal mapping $f$ with a chaotic $p$-cycle such that for any $k$, there exists $g \in \mathcal{N}(3,2)$ with
\[L_\infty(f^k, g) \leq \eps.\]
\end{proposition}

\begin{proof}
    For all $j \in [p]$, let $x_j = 1 - \frac{p-j+1}{p} \eps$.
    Define $f$ to be a piecewise-linear function with $p+1$ pieces chosen with boundaries that satisfy 
    \[f(0) = 0, f(x_1) = x_2, f(x_2) = x_3, \dots, f(x_{p-1}) = x_p, f(x_p) = x_1, f(1) = 0.\]
    
    We visualize $f$ for $p=3$ in Figure~\ref{fig:asymmetric}. $f$ is unimodal because it increases on $[0, x_{p-1}]$ and decreases on $[x_{p-1}, 1]$.
    It is concave because $f'(x)$ does not increase as $x$ grows, since 
    \[f'(x) = \begin{cases}
        \frac{1-\frac{p-1}{p}\eps}{1 - \eps} > 1 & x \in [0, x_1) \\
        1 & x \in (x_1, x_{p-1}) \\
        - p + 1 & x \in (x_{p-1}, x_p) \\
        - \frac{1 - \eps}{\eps} & x \in (x_p, 1],
    \end{cases}\]
    as long as $\frac{1 - \eps}{\eps} > p - 1$.
    
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/fig-asymmetric1.png}
        \includegraphics[width=0.45\textwidth]{fig/fig-asymmetric10.png}
        \caption{Plots the asymmetric function with a $p$-cycle referenced in Proposition~\ref{prop:need-symmetry} for $p=3$ and $\eps = 0.1$. While $f$ oscillates frequently, $f$ can be trivially $0.1$-approximated by three ReLUs. As $\eps \to 0$, the $L_\infty$ approximation hardness guarantees implied by \cite{cnpw19} become vacuous because the oscillations, even though they are exponentially many, they shrink in size.}
        \label{fig:asymmetric}
    \end{figure}

    
    We show inductively that for all $k$, there exists $a_k < b_k$ such that $f^k(a_k) = f^k(b_k) = 1 - \eps$, $f^k([a_k, b_k]) \in [1 - \eps, 1]$, and $f^k$ has exactly one linear piece for each of the intervals $[0, a_k]$ and $[b_k, 1]$.
    
    These are true for the base case $k = 1$ for $a_1 \in (0, x_1)$ and $b_1 = x_p$.
    
    If the claim holds for $k$, then there is some $a_{k+1} \in (0, a_k)$ and $b_{k+1}\in (b_k, 1)$ such that $f(a_{k+1}) = f(b_{k+1}) = a_k$.
    Then, $f^{k+1}(a_{k+1}) = f^{k+1}(b_{k+1}) = 1-\eps$ and $f^{k+1}([0, a_{k+1}]) = f^{k+1}([b_{k+1},1]) = [0, 1 - \eps]$.
    For all $x \in [0, a_{k+1}]$, $f^j(x) \leq 1 - \eps$ for all $j \leq k+1$. Hence, $f^{k+1}$ is linear on $[0, a_{k+1}]$ (and also $[b_{k+1}, 1]$.
    Because $f([x_1, x_p]) = [x_1, x_p]$, $f^{k+1}([a_{k+1}, b_{k+1}]) \subseteq [x_1, x_p] \subseteq [1 - \eps, 1]$.
    The claim then holds for $k+1$.
    
    Thus, the piecewise linear mapping $g$ with boundaries $g(0)=0$, $g(a_k) = 1-\eps$, $g(b_k) = 1-\eps$, and $g(1) = 0$ is an $\eps$-approximation of $f$.
    Because $g$ has three pieces and contains the origin, it can be exactly represented by a linear combination of four ReLUs, and hence as a depth-2 neural network of width 3.
\end{proof}

\begin{proposition}\label{prop:need-concavity}
% For sufficiently small $\eps > 0$ and $p \geq 3$, there exists a symmetric unimodal mapping $f$ that is \textit{not concave} such that there exists a 2-layer ReLU network of width 3 such that
% \[\max_{x \in [0,1]} \abs{f(x) - g(x)} \leq \eps.\]
For $p \geq 3$ and for sufficiently small $\eps > 0$, there exists a symmetric unimodal mapping $f$ with a chaotic $p$-cycle such that for any $k$, there exists $g \in \mathcal{N}(3,2)$ with
\[L_\infty(f^k, g) \leq \eps.\]
\end{proposition}
\begin{proof}
    Let $x_j = \frac{1}{2} - \frac{p-1-j}{2(p-1)}\eps$ for all $j \in [p-1]$ and $x_p = \frac{1}{2} + \frac{\eps}{2}$.
    Let $f$ be a piecewise-linear function with boundaries
    \begin{align*}
        f(0) = 0, \
        f\paren{\frac{1}{2} - \frac{\eps}{2}} = \frac{1}{2}-\frac{p-2}{p-1} \cdot \frac{\eps}{2}, \
        f\paren{\frac{1}{2} - \frac{\eps}{2(p-1)}} = \frac{1}{2}, \ f\paren{\frac{1}{2}} = \frac{1}{2} + \frac{\eps}{2}, \\
        f\paren{\frac{1}{2} + \frac{\eps}{2(p-1)}} = \frac{1}{2},  \ 
        f\paren{\frac{1}{2} + \frac{\eps}{2}} = \frac{1}{2}-\frac{p-2}{p-1} \cdot \frac{\eps}{2},\
        f(1) = 0.
    \end{align*}
    
    We visualize $f$ for $p=3$ in Figure~\ref{fig:non-concave}. Note that $f$ is symmetric and unimodal and has an increasing $p$-cycle $x_1 < \dots < x_p$. 
    It is \textit{not} concave because $f'(x) = 1$ for $x \in [x_1, x_{p-2}]$ and $f'(x) = 2(p-1)$ for $x \in [x_{p-2}, x_{p-1}]$.
    
    Using a very similar argument to argument from the proof of Proposition~\ref{prop:need-symmetry}, for all $k$, there exists $a_k < b_k$ such that $f^k$ is linear on $[0, a_k]$ and $[b_k, 1]$ and $f^k([a_k, b_k]) \in [\frac{1}{2} - \eps, \frac{1}{2} + \eps]$.
    As before, there exists a piecewise linear function with three pieces (which can be thought of as a depth-2 neural network of width 3) that $\eps$-approximates $f$.
\end{proof}

==> Beyond Sharkovsky Paper/supp_lb_arxiv.tex <==
\section{Additional Proofs for Section~\ref{sec:lb}}

\subsection{Proof of Lemma~\ref{lemma:increasing-constant-osc}}\label{assec:inc-constant-osc-proof}
We restate and prove the lemma. This is the main technical lemma that we use to get the sharper depth-width tradeoffs and the improved notion of \textit{constant} approximation.

\lemmaincreasingconstantosc*
%\label{lem:main}
\begin{proof}
We first lower-bound the total number of oscillations that will appear an increasing $p$-cycle is present. 
Later, we show that the size of the oscillations is large as well.

Because we have an increasing cycle of itinerary $12\dots p$, we assume (wlog) that the cycle is $(x_1, \dots, x_p)$ with $x_1 < x_2 < \dots < x_p$. 
Define intervals $I_j \vcentcolon= [x_j, x_{j+1}]$ for $j \in \{1, \dots, p-1\}$. Because $f$ is continuous, we conclude that $I_{j+1} \subset f(I_{j})$ for all $j < p$ and $I_{j} \subset f(I_{p-1})$ for all $j$.
Figure~\ref{fig:inc-intervals} visualizes these relationships.

\begin{figure}
    \centering
    \input{fig/fig-inc-intervals}
    \caption{Visualizes the intervals $I_1,\dots, I_{p-1}$ defined in the proof of Lemma~\ref{lemma:increasing-constant-osc} and which intervals $f$ maps to one another when $f$ has an increasing $p$-cycle.}
    \label{fig:inc-intervals}
\end{figure}

Using the methods of \cite{cnpw19}, we define $y^{(k)} \in \N^{p-1}$ such that $y^{(k)}_j$ is a lower bound on the number of times $f^k$ passes through interval $I_j$, or \[\osci{x_{j}, x_{j+1}}(f^k) \geq y^{(k)}_j.\] We can then encode the interval relationships above with $y^{(k+1)} = A_p y^{(k)}$ where $y^{({0})}$ is a vector of all ones and and $A_p \in \bit^{(p-1) \times (p-1)}$ with $(A_p)_{i, j} = \indicator{j = p-1 \text{ or } i = j + 1}$. We get the following adjacency matrix for the intervals, capturing the mapping relationships (under $f$) between them:
\[A_p = 
\begin{bmatrix}
    0 & 0 & 0 & \cdots & 0 & 1 \\
    1 & 0 & 0 & \cdots & 0 & 1 \\
    0 & 1 & 0 & \cdots & 0 & 1 \\
    0 & 0 & 1 & \cdots & 0 & 1 \\
    \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
    0 & 0 & 0 & \cdots & 1 & 1
\end{bmatrix}.\]

We find the characteristic polynomial of $A_p$ and lower-bound $y^{(k+1)}$ with the spectral radius of $A_p$. 
We show by induction on $p \geq 3$ that
\[\det(A_p - \lambda I) = (-1)^{p-1} \paren{\lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i}.\]

For the base case $p = 3$, we have:
\begin{align*}
    \det(A_3 - \lambda I)
    &= \begin{vmatrix}
        -\lambda & 1 \\
        1 & 1 -\lambda
    \end{vmatrix}
    = \lambda^2 - \lambda - 1,
\end{align*}
which satisfies the desired form.

Now, we show the inductive step by expanding the determinant of $A_p - \lambda I$.

{\small
\begin{align*}
    \det(A_p - \lambda I)
    &= 
    \begin{vmatrix}
        -\lambda & 0 & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & 0 & \cdots & 0 & 1 \\
        0 & 1 & -\lambda & \cdots & 0 & 1 \\
        0 & 0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix}
    = -\lambda 
    \begin{vmatrix}
        -\lambda & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & \cdots & 0 & 1 \\
        0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix} - 
    \begin{vmatrix}
        0 & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & \cdots & 0 & 1 \\
        0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix}.
\end{align*}}

The left determinant exactly equals $\det(A_{p-1} - \lambda I)$, which we can expand using the inductive hypothesis.
The second equals $(-1)^{p-2}$, because $p-2$ row swaps (which are elementary row operations) can be used to move the first row to the bottom and make the matrix upper-triangular with diagonals of one. 
We conclude the inductive step below.

\begin{align*}
        \det(A_p - \lambda I)
        &= -\lambda \det(A_{p-1} - \lambda I) - (-1)^{p-2} \\ 
    &= -\lambda (-1)^{p-2} \left(\lambda^{p-2} - \sum_{i=0}^{p-3} \lambda^i \right) + (-1)^{p-1}
    = (-1)^{p-1} \left(\lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i\right).
\end{align*}

We find the eigenvalues of $A_p$ by finding the roots of the polynomial
\[P(x) = \lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i = 0.\] 
Observe that there must be a root greater than $1$ because $P(1) = 2 - p < 0$ and $P(2) = 1 > 0$. Equivalently, if $\lambda \neq 1$,
\[P(x) = \lambda^{p-1} - \frac{1 - \lambda^{p-1}}{1 - \lambda} = \frac{\lambda^p - 2\lambda^{p-1} + 1}{\lambda - 1} =  0.\]

Hence, finding the largest root of $P$ is equivalent to finding the largest root of $\lambda^p - 2\lambda^{p-1} + 1$, which is $\rhoinc{p}$ by definition.


This implies that the spectral radius of $A_p$, sp$(A_p)=\rhoinc{p}>1$, and hence, we also have sp$(A_p^k)=$ sp$(A_p)^k=\rhoinc{p}^k$. Since all the elements in $A_p$ and in $A_p^k$ are non-negative, then the infinity norm of $A_p^k$ is by definition the maximum among its row sums. Since the last column of $A_p$ is the all 1's vector, the largest row sum in $A_p^k$ appears at its last row:

\[
||A_p^k||_{\infty} = \sum_{j=1}^{p-1}(A_{p}^k)_{p-1,j}
\]



We can now use the fact that the infinity norm of a matrix is larger than its spectral norm:
\[
||A_p^k||_{\infty} \ge  \rhoinc{p}^k
\]
%Therefore, there exists at least one interval $I_{j^*}$ which is crossed at least $\rho^k$ times by $f^k$, so $\osci{x_{j^*}, x_{j^*+1}}(f^k) \geq \rho^k$.
We conclude that there exists at least one interval $I_{j^*}$ (e.g., the interval $I_{p-1}$) which is crossed at least $\rhoinc{p}^k$ times by $f^k$, so $\osci{x_{j^*}, x_{j^*+1}}(f^k) \geq \rhoinc{p}^k$.

Thus, for some $a',b'$ we get $\osci{a', b'}(f^k) \geq \rhoinc{p}^k$. But can we find $a',b'$ with large difference $b'-a'$?

Now, we show that the intervals traversed are sufficiently large, in order to lower-bound $\osci{a,b}(f^k)$ with $b-a \geq \frac{1}{18}$.
By Lemma~\ref{lemma:interval-inc-cycle}, there exists some $j$ with $x_{j+1} - x_{j} \geq \frac{1}{18}$.
It suffices to show that $f^k$ traverses the interval $I_j$ sufficiently many times.

From earlier in the proof, there exists some $j^*$ such that $f$ crosses $I_{j^*}$ at least $N\vcentcolon=\rhoinc{p}^{k}$ times. 
We conclude by showing that every other interval is traversed at least half as often as this most popular interval, which suggests that $\osci{x_{j}, x_{j+1}}(f) \geq \frac{N}{2}$.
    

    
For $A \in \mathbb{R}^{(p-1)\times (p-1)}$ as defined earlier in the section and for $y^{(k)} \vcentcolon= A^{k} \vec{1}$, we argue inductively that the elements of $y^{(k)}$ are non-decreasing and that $y^{(k)}_{p-1} \leq 2 y^{(k)}_1$. For the base case, this is trivially true for $k = 0$.

Suppose it holds for $k$.
    By construction, we have $y^{(k+1)}_1 = y^{(k)}_{p-1}$ and $y^{(k+1)}_j = y^{(k)}_{j-1} + y^{(k)}_{p-1}$ for all $j > 1$.
    By the inductive hypotheses,
    \[y^{(k+1)}_1 \leq y^{(k+1)}_2 \leq \dots \leq y^{(k+1)}_{p-1} \leq 2y^{(k+1)}_1.\]
    
Therefore, $f^k$ crosses interval $I_{j}$ at least $\frac{N}{2}$ times, and $I_j$ has width at least $\frac{1}{18}$. The claim immediately follows.
\end{proof}
    
\begin{lemma}\label{lemma:interval-inc-cycle}
    For some $p \geq 3$, consider a symmetric concave unimodal function $f$ with an increasing $p$-cycle of $x_1 < \dots < x_p$. Then, there exists $j \in [p-1]$ such that $x_{j+1} - x_j \geq \frac{1}{18}$.
\end{lemma}

\begin{proof}
By the continuity of $f$, note that $[x_1, x_p] \subset f^3([x_{p-3}, x_{p-2}])$. 
There then exists some $y_1 \in [x_{p-3}, x_{p-2}]$ such that $f^3(y_1) = y_1$, $y_2\vcentcolon= f(y_1) \in [x_{p-2}, x_{p-1}]$, and $y_3\vcentcolon= f(y_2) \in [x_{p-1}, x_p]$.
Thus, if $f$ has a maximal $p$-cycle, then $f$ also has a 3-cycle corresponding to $x_{p-3} < y_1 < y_2 < y_3 < x_p$.

We now show that $y_3 - y_1$ must be sufficiently large by concavity.
For $f$ to be concave, the following inequality must hold:
\begin{align*}
    \frac{f(y_1) - f(0)}{y_1 - 0} \geq \frac{f(y_2) - f(y_1)}{y_2 - y_1} > 0  > \frac{f(y_3) - f(y_2)}{y_3 - y_2} \geq \frac{f(1) - f(y_3)}{1 - y_3},
\end{align*}
or equivalently,
 \[\frac{y_2}{y_1} \geq \frac{y_3 - y_2}{y_2 - y_1} > 0 > -\frac{y_3 - x_1}{y_3 - y_2} \geq -\frac{y_1}{1 - y_3}.\]
 
In addition, note that $y_1 < \frac{1}{2}$ and $y_3 > \frac{1}{2}$. 
If the former were false, then $f(y_2) \leq f(y_1)$ (by unimodality), which contradicts $y_3 > y_2$. If the latter were false, then $f(y_3) > f(y_2)$, which contradicts $y_1 < y_3$.

We consider two cases and show that either way, the interval must have width at least $\frac{1}{6}$.
\begin{itemize}
    \item If $y_2 - y_1 \leq \frac{2}{5}(y_3 - y_1)$, then $\frac{y_3 - y_2}{y_2 - y_1} \geq \frac{3}{2},$
    which mandates that $y_1 \leq \frac{2y_2}{3}$ to ensure concavity. Thus,
    \[y_3 - y_1 \geq y_3 - \frac{2y_2}{3} \geq \frac{y_3}{3} \geq \frac{1}{6}.\]
    \item If $y_2 - y_1 \geq \frac{2}{5}(y_3 - y_1)$, then $\frac{y_3 - y_1}{y_3 - y_2} \geq \frac{5}{3},$ and thus $y_1 \geq \frac{5}{3}(1 - y_3)$ and $y_3 \geq 1 - \frac{3y_1}{5}$. Then,
    \[y_3 - y_1 \geq 1 - \frac{3y_1}{5} - y_1 = 1 - \frac{8y_1}{5} \geq \frac{1}{5}.\]
\end{itemize}

Thus, we must have \[\max\{x_{p-2} - x_{p-3}, x_{p-2} - x_{p-1}, x_p - x_{p-1}\} \geq \frac{1}{18}.\qedhere\]

\end{proof}

\subsection{Proof of Fact~\ref{fact:root-lb}}\label{assec:fact}
\factrootlb*
\begin{proof}

Let $P_{\mathrm{inc}, p}(\lambda) = \lambda^{p} - 2\lambda^{p-1} + 1$.

First, observe that $\rhoinc{p} < 2$, because $P_{\mathrm{inc}, p}(\lambda) > 0$ whenever $\lambda \geq 2$. 
We lower-bound $\rhoinc{p}$ by finding some $\lambda$ for each $p$ such that $P_{\mathrm{inc}, p}(\lambda) \leq 0$ or equivalently $\lambda^{p-1}(2 - \lambda) \geq 1$ for all $p\geq3$, which bounds $\rhoinc{p}$ by the Intermediate Value Theorem. 

Consider $\lambda = 2 - \frac{4}{2^p}$. Then,
\begin{align*}
    \lambda^{p-1}(2 - \lambda)
    &= \paren{2 - \frac{4}{2^p}}^{p-1} \cdot \frac{4}{2^p}
    = 2 \paren{1 - \frac{2}{2^p}}^{p-1} \\
    &\geq 2 \paren{1 - \frac{2(p-1)}{2^p}}
    = 2 - 2 \cdot \frac{p-1}{2^{p-1}} \\
    &\geq 2 - 2 \cdot \frac{1}{2} = 1.\qedhere
\end{align*}
\end{proof}

\subsection{Previous Results about Hardness of Approximating Oscillatory Functions}

We rely on prior results from~\cite{cnpw19, cnp20} to show that an iterated function $f^k$ is inapproximable by neural networks.
These results hold if $f^k$ has sufficiently many crossings of some interval.
We apply these results later with improved bounds on both the number and the size of crossings.

\cite{cnpw19} show that the classification error of $f^k$ can be bounded if there are enough oscillations.

\begin{theorem}[\citep{cnpw19}, Section 4]\label{thm:general-lb-cls}
    Consider any continuous $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a, b}(f) = \Omega(\rho^t)$ and suppose $u \leq \frac{1}{8}\rho^{k/\ell}$.
    Then, for $t = \frac{a+b}{2}$, there exists $S$ with $\abs{S} =  \frac{1}{2} \floor{\rho^k}$ samples such that 
    \[\errcls{S,t}{f^k, g}  \geq \frac{1}{2} - \frac{(2u)^\ell}{n}.\]
\end{theorem}

We adapt that claim to lower-bound the $L_\infty$ approximation of $f^k$ by $g$.

\begin{corollary}\label{cor:general-lb-linf}
    Consider any continuous $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a, b}(f) = \Omega(\rho^t)$ and suppose $u \leq \frac{1}{8}\rho^{k/\ell}$.
    Then, 
    \[\norm[\infty]{f^k - g} \geq \frac{b-a}{2}.\]
\end{corollary}
\begin{proof}
    By Theorem~\ref{thm:general-lb-cls}, there exists some $x \in [0,1]$ such that (wlog) $f^k(x) \leq a$ and $g(x) \geq \frac{a + b}{2}$.
    The conclusion for the $L_\infty$ error is immediate by definition.
\end{proof}

\cite{cnp20} give a lower-bound on the ability of a neural network $g$ to $L_1$-approximate $f^k$, provided a correspondence between the Lipschitz constant of $f$ and the rate of oscillations $\rho$.

\begin{theorem}[\cite{cnp20} Theorem 3.2]\label{thm:general-lb-l1}
    Consider any $L$-Lipschitz $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a,b}(f) = \Omega(\rho^t)$. If $L \leq \rho$ and $u \leq \frac{1}{16} \rho^{k/\ell}$, then 
    \[\norm[1]{f^k - g} = \Omega((b-a)^2).\]
\end{theorem}

The Lipschitzness assumption is extremely strict, especially because they show in their Lemma~3.1 that $L \geq \rho$ whenever $f$ has a period of odd length.

\subsection{Proof of Corollary~\ref{cor:main-l1}}\label{assec:cor-main-proof}
\cormainl*
\begin{proof}
    This theorem follows from Theorem~\ref{thm:main-l1} and Lemma~\ref{lemma:increasing-constant-osc}.
    Because $\ftent{\rho_p/2}$ is $\rho_p$-Lipschitz, it remains only to prove that there exists an increasing $p$-cycle.
    We show that 
    \[\frac{1}{2}, f\paren{\frac12},\dots, f^{p-1}\paren{\frac12}\]
    is such a cycle.
    
    By definition of the tent map, $f(\frac12) = \frac{\rhoinc{p}}2$ and $f^2(\frac12) = \rhoinc{p} (1 - \frac{\rhoinc{p}}{2})$.
    If we assume for now that $f^j(\frac12) \leq \frac12$ for all $j \in \{2, \dots, p-1\}$,
    then
    \[f^p\paren{\frac12} = \rhoinc{p}^{p-1}\paren{1 - \frac{\rhoinc{p}}2} = -\frac{1}{2}\paren{\rhoinc{p}^p - 2\rhoinc{p}^{p-1} + 1} + \frac{1}{2} = 0 + \frac{1}{2}.\]
    
    Because $f^p(\frac12) = \frac12$ and we assumed that $f^{j+1}(\frac12) = \rhoinc{p} f^{j}(\frac12)$ for $j \geq 2$ and $\rho > 1$, it must be the case that $f^j(\frac12) \leq \frac12$ for all $j \in \{2, \dots, p-1\}$.
    
    Lemma~\ref{lemma:increasing-constant-osc} thus implies that $f^k$ has $\Omega(\rhoinc{p}^k)$ crossings, which enables us to complete the proof by invoking Theorem~\ref{thm:main-l1}, since the Lipschitzness condition is met.
    % To apply them, it remains only to prove that the Lipschitz constant of $\ftent{r}$ is $\rho$, or equivalently, $r = \frac{\rho}{2}$.
    % Given $\ftent{r}^p(\frac12) = \frac12$, we show that $\frac12$ must be contained in an increasing $p$-cycle.
    % Suppose not.
    % There exists some increasing $p$-cycle $x_1 < \dots < x_p$ and we assume that it does not contain $\frac12$.
    % It must be the case that $x_{p-2} < \frac12$; assuming otherwise would cause $f(x_{p-2}) \geq f(x_{p-1})$, a contradiction.
    % Because $\frac12$ maximizes $f$, $x_p \leq f(\frac12)$.
    % Since $f$ decreases on $[\frac12, 1]$, it follows that $f^2(\frac12) \leq x_1$.
    % $f$ increasing on $[0, \frac12]$ implies that $f^{j+1}(\frac12) \leq x_{j}$ for all $j \in [p-1]$.
    % Therefore, $f^{j}(\frac12) \neq \frac12$ for all $j \in [p]$ and $f^2(\frac12) <  \dots < f^{p}(\frac12) = \frac12$.
    % We conclude that $\frac12$ is contained in an increasing $p$-cycle, which has a $123\dots p$ itinerary; call that cycle $x_1', \dots, x_{p-1}'= \frac12, x_p'$
    % % For $\ftent{r}$ to have a super-stable $p$-cycle, it must pass through $\frac{1}{2}$. Because $\ftent{r}$ only has zero-slope at $x = \frac{1}{2}$, a fixed point $x_1$ for $\ftent{p}$ will only be super-stable if $f^j(x_1) = \frac{1}{2}$ for some $j \in [p]$. (Otherwise $\frac{d}{dx} f^j(x_1) \neq 0$, and $x_1$ cannot be part of a super-stable cycle.)
    % % Therefore, there must exist a cycle of the form
    % % \[x_1 < \dots < x_{p-2} < x_{p-1} = \frac{1}{2} < x_{p} = r,\]
    % % which signals an $12\dots p$ itinerary.
    % % Note that $x_{p-1} = \frac{1}{2}$ because any assignment would contradict the cycle being increasing.
    % % If $x_p = \frac{1}{2}$, then $x_1 = f(x_p) = r > x_p > x_1$.
    % % If $x_j = \frac{1}{2}$ for $j < p-1$, then $x_p = f(x_{p-1}) < f(x_{j}) = x_{j+1} < x_p$, both contradictions.
    % We apply the definition of the tent map to note that $x_{j}' = 2rx_{j-1}'$ for $j \in \{2, \dots, p\}$ and $x_1' = 2r(1 - x_p')$.
    % Thus, 
    % \[\frac{1}{2} = (2r)^{p-2} x_1' = (2r)^{p-1}(1 - x_p') = (2r)^{p-1}(1 - r).\]
    % Equivalently, 
    % \[(2r)^p - 2 (2r)^{1-p} + 1 = 0,\]
    % which has $\rho = 2r$ as its largest root.
    % Hence, $\ftent{r}$ has Lipschitz constant $\rho$ and we can apply Theorem~\ref{thm:main-l1}.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:odd-constant-osc}}\label{assec:lemma-odd-proof}

\lemmaoddconstantosc*

\begin{proof}
    By Theorems~2.94 and 3.11.1 of~\cite{alseda2000}, there exists a $p$-cycle of the form \[x_p < x_{p-2} < \dots < x_3 < x_1 < x_2 < x_4 < \dots < x_{p-1},\]
    which is known as a \textit{Stefan cycle}.
    The analysis of Section~3.2 of~\cite{cnp20} shows that $\osci{[x_1, x_2]}(f^{k}) \geq \rhoodd{p}^{k}$.
    Their exploitation of the relationships between intervals is visualized in Figure~\ref{fig:stefan-intervals}.
    By the continuity of $f$, applying $f$ an additional $p-1$ times gives $\osci{[x_p, x_1]}(f^{k+p-1}) \geq \rhoodd{p}^{k}$.
    Because $[x_{p-2}, x_1] \subset [x_p, x_1]$, applying $f$ one more time gives $\osci{[x_2, x_{p-1}]}(f^{k+p}) \geq \rhoodd{p}^k$.
    
    
    \begin{figure}
        \centering
        \input{fig/fig-stefan-intervals}
        \caption{Gives an example of a Stefan $p$-cycle (which is relied upon in Lemma~\ref{lemma:odd-constant-osc} and demonstrates the interval relationships). Analogous to Figure~\ref{fig:inc-intervals}.}
        \label{fig:stefan-intervals}
    \end{figure}
    
    Hence, by redefining $k$, we have 
    \[\max\{ \osci{[x_1, x_2]}(f^{k}), \osci{[x_2, x_{p-1}]}(f^{k}), \osci{[x_p, x_1]}(f^{k})\} \geq \rhoodd{p}^{k-p}.\]
    
    Since $[x_p, x_{p-1}]$ is the disjoint union of $[x_1, x_2]$, $[x_2, x_{p-1}]$, and $[x_p, x_1]$, there exists $[a, b] \subset [x_p, x_{p-1}]$ with $b- a \geq \frac{1}{3}(x_{p-1} - x_p)$ such that $\osci{[a,b]}(f^{k}) \geq \\rhoodd{p}^{k-p}$.
    
    The problem reduces to placing a lower bound on $x_{p-1} - x_p$.
    To do so, we derive contradictions on the concavity and symmetry of $f$. 
    Let $r = f(\frac12) \in (x_p, 1)$ be the the largest outcome of $f$, and
    let \[a= \sup_{x, x' \in [1-r, r]} \abs{\frac{f(x) - f(x')}{x - x'}}\] be the maximum absolute slope of $f$ on $[1-r,r]$. $a$ must be finite by the concavity and continuity of $f$, and if $f$ is differentiable, $a = f'(1-r) = -f'(r)$.
    Thus, $f$ is $a$-Lipschitz on that interval.
    
    Because $f([x_p, x_{p-1}]) \subseteq [x_p, r] \subset [1-r, r]$, it follows that $\abs{f^2(x) - f^2(x')} \leq a^2 \abs{x - x'}$.
    Thus, $x_2 - x_p \leq a^2(x_{p-2} - x_{p})$ and $x_2 - x_p \leq x_4 - x_p \leq a^2(x_2 - x_{p-2})$.
    Averaging the two together, we have $x_2 - x_p \leq \frac{a^2}{2}(x_2 - x_{p})$, which means $a \geq \sqrt{2}$.
    
    To satisfy concavity, the following must be true:
    \[\frac{f(1-r) - f(0)}{1-r - 0} = \frac{f(r)}{1-r} \geq a \geq \sqrt{2}.\]
    
    We rearrange the inequality and apply properties of monotonicity to lower-bound $r$ away from $\frac12$:
    \[r 
    \geq 1 - \frac{f(r)}{\sqrt{2}}  
    \geq 1 - \frac{f(x_{p-1})}{\sqrt{2}}
    = 1 - \frac{x_p}{\sqrt{2}}
    > 1 - \frac1{2\sqrt2}.\]
    
    It also must be the case for any $x \in [\frac12, 1]$, that:
    \[\abs{\frac{f(x) - f\paren{\frac12}}{x - \frac12}} \leq 2.\]
    Otherwise, the concavity of $f$ would force $f(\frac12) > 1$.
    
    We finally assemble the pieces to lower-bound the gap between $x_{p-1}$ and $x_p$:
    \begin{align*}
        x_{p-1} - x_p
        &\geq x_{p-1} - \frac12 
        \geq -\frac{1}{2} \paren{f(x_{p-1}) - f\paren{\frac12}}
        = \frac{r}{2} - \frac{x_p}{2} \\
        &> \frac{1}{2} - \frac1{4\sqrt{2}} - \frac14 
        = \frac14 - \frac1{4\sqrt{2}}
        > 0.07.\qedhere
    \end{align*}
    
    
    
    % Under the assumption, it must be the case that $r \leq 0.54$. If not, then 
    % \[\frac{f(x_p) - f(\frac12)}{x_p - \frac12} > \frac{0.04}{0.02} = 2.\]
    % By concavity, this would imply that $f(\frac12) > 1$, which is a contradiction. Hence, we continue with $r \leq 0.54$.
    
    % By the monotonicity of $f$ on $[\frac12, 1]$ and the fact that $r > x_{p-1}$, it follows that $f(r) < x_{p} < \frac12$.
    
    % By symmetry and unimodality of $f$, $1-x_{p-1} \leq x_p$, since $f(x_{p-1}) < f(x_p)$.
    % The concavity of $f$ implies the following:
    % \begin{align*}
    %     -\frac{x_p}{1 - x_{p-1}} 
    %     &= \frac{f(1) - f(x_{p-1})}{1 - x_{p-1}}
    %     \leq \sup_{x, x' \in [1/2, x_{p-1}]} \frac{f(x) - f(x')}{x - x'} \\
    %     &= \sup_{x, x' \in [1-x_{p-1}, x_{p-1}]} -\abs{\frac{f(x) - f(x')}{x - x'}} 
    %     \leq \sup_{x, x' \in [x_p, x_{p-1}]} -\abs{\frac{f(x) - f(x')}{x - x'}}\\
    %     &= -a \leq -\sqrt{2}.
    % \end{align*}
    
    % Thus, $\abs{f'(x)}$ is maximized on the interval $[x_p, x_{p-1}]$ at $x_{p-1}$.
    % By concavity, it must be the case that $f'(x)\leq -\sqrt{2}$ whenever $x \in [x_{p-1}, 1]$ and thus, 
    % \[\frac{f(1) - f(x_{p-1})}{1 - x_{p-1}} = -\frac{x_p}{1 - x_{p-1}} \leq -\sqrt{2}.\]
    % Equivalently,
    % \[x_{p-1} \geq 1 - \frac{x_p}{\sqrt{2}}.\]
    
    % We conclude with the lower bound on $x_{p-1} - x_p$. Note that $x_p < \frac{1}{2}$ by symmetry and the fact that $f(x_p) \leq f(x_{p-2})$.
    % \begin{align*}
    %     x_{p-1} - x_p
    %     &\geq 1 - \frac{x_p}{\sqrt{2}} - x_p 
    %     = 1 - \frac{2 + \sqrt{2}}{2} x_p \\
    %     &\geq 1 - \frac{2 + \sqrt{2}}{4} > 0.12.\qedhere
    % \end{align*}
\end{proof}

\subsection{Necessity of Symmetry and Concavity Assumptions in Theorems~\ref{thm:main-linf} and \ref{thm:main-l1}}\label{assec:sym-conc}

We demonstrate the weakness of the bounds promised by \cite{cnpw19, cnp20, bzl20} and argue that our assumptions of symmetry and concavity are necessary in order to avoid such non-vacuous bounds.
To do so, we exhibit two families of functions in Propositions~\ref{prop:need-symmetry} and ~\ref{prop:need-concavity} which contain functions with increasing $p$-cycles for every $p$ that produce large numbers of oscillations, yet are trivial to approximate because their oscillations can be made arbitrarily small.
The functions considered in both cases are unimodal and lack symmetry and concavity respectively.

These expose a fundamental shortcoming of other approaches to the hardness of neural network approximation in the aforementioned works because they all rely on showing that for every mapping $f$ meeting some condition (e.g. odd period, positive topological entropy), there exists some $[a,b] \in [0,1]$ where $\osci{a,b}$ is exponentially large, and hence no poly-size shallow neural network $g$ can obtain $L_{\infty}(f^k, g) \leq P(b-a)$ for some polynomial $P$.
However, because $[a,b]$ depends on $f$, their difference can potentially be arbitrarily small. 
The propositions show that this concern is significant and that $[a,b]$ indeed becomes arbitrarily narrow for simple 3-periodic functions. 
While \cite{cnpw19} avoid addressing this issue head-on by focusing on classification error over $L_\infty $ error, their classification lower-bounds rely on misclassification of points whose actual distance can be shrinking (see for example Figure~\ref{fig:asymmetric}).
%microscopically small degrees of inapproximation on a small number of points.


The implications of these propositions contrast with the more robust hardness results we present in Theorems~\ref{thm:main-linf}, \ref{thm:main-l1}, \ref{thm:odd-linf}, and \ref{thm:odd-l1}, which leverage unimodality, symmetry, and concavity to ensure that the accuracy of approximation can be no better than some constant (independent on $f,p$) when the neural network $g$ is too small.
% In order for the accuracy of the neural network approximation to be lower-bounded by a constant value, Theorems~\ref{thm:main-linf} and \ref{thm:main-l1} assume that the unimodal function $f$ is additionally concave and symmetric. 
We show here that those assumptions are necessary by exhibiting functions that satisfy all but one, and become easy to $L_\infty$-approximate with small depth-2 ReLU networks.

% \todo{Show that ICML and ICLR fail}

% \todo{Note that prior analysis doesn't give us anything about setting for why large L fails; we show why that's the case}

% \todo{mention that oscillation LBs for increasing cycle still give large number of oscillations even if not unimodal (just small oscillations)}

% \todo{Or, just directly attack previous constructions... Show that oscillation size becomes arbitrarily small}

% \vaggos{forward pointer in section where we dwell on cosntant error rates.}


\begin{proposition}\label{prop:need-symmetry}
For $p \geq 3$ and for sufficiently small $\eps > 0$, there exists a concave unimodal mapping $f$ with a chaotic $p$-cycle such that for any $k$, there exists $g \in \mathcal{N}(3,2)$ with
\[L_\infty(f^k, g) \leq \eps.\]
\end{proposition}

\begin{proof}
    For all $j \in [p]$, let $x_j = 1 - \frac{p-j+1}{p} \eps$.
    Define $f$ to be a piecewise-linear function with $p+1$ pieces chosen with boundaries that satisfy 
    \[f(0) = 0, f(x_1) = x_2, f(x_2) = x_3, \dots, f(x_{p-1}) = x_p, f(x_p) = x_1, f(1) = 0.\]
    
    We visualize $f$ for $p=3$ in Figure~\ref{fig:asymmetric}. $f$ is unimodal because it increases on $[0, x_{p-1}]$ and decreases on $[x_{p-1}, 1]$.
    It is concave because $f'(x)$ does not increase as $x$ grows, since 
    \[f'(x) = \begin{cases}
        \frac{1-\frac{p-1}{p}\eps}{1 - \eps} > 1 & x \in [0, x_1) \\
        1 & x \in (x_1, x_{p-1}) \\
        - p + 1 & x \in (x_{p-1}, x_p) \\
        - \frac{1 - \eps}{\eps} & x \in (x_p, 1],
    \end{cases}\]
    as long as $\frac{1 - \eps}{\eps} > p - 1$.
    
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/fig-asymmetric1.png}
        \includegraphics[width=0.45\textwidth]{fig/fig-asymmetric10.png}
        \caption{Plots the asymmetric function with a $p$-cycle referenced in Proposition~\ref{prop:need-symmetry} for $p=3$ and $\eps = 0.1$. While $f$ oscillates frequently, $f$ can be trivially $0.1$-approximated by three ReLUs. As $\eps \to 0$, the $L_\infty$ approximation hardness guarantees implied by \cite{cnpw19} become vacuous because the oscillations, even though they are exponentially many, they shrink in size.}
        \label{fig:asymmetric}
    \end{figure}

    
    We show inductively that for all $k$, there exists $a_k < b_k$ such that $f^k(a_k) = f^k(b_k) = 1 - \eps$, $f^k([a_k, b_k]) \in [1 - \eps, 1]$, and $f^k$ has exactly one linear piece for each of the intervals $[0, a_k]$ and $[b_k, 1]$.
    
    These are true for the base case $k = 1$ for $a_1 \in (0, x_1)$ and $b_1 = x_p$.
    
    If the claim holds for $k$, then there is some $a_{k+1} \in (0, a_k)$ and $b_{k+1}\in (b_k, 1)$ such that $f(a_{k+1}) = f(b_{k+1}) = a_k$.
    Then, $f^{k+1}(a_{k+1}) = f^{k+1}(b_{k+1}) = 1-\eps$ and $f^{k+1}([0, a_{k+1}]) = f^{k+1}([b_{k+1},1]) = [0, 1 - \eps]$.
    For all $x \in [0, a_{k+1}]$, $f^j(x) \leq 1 - \eps$ for all $j \leq k+1$. Hence, $f^{k+1}$ is linear on $[0, a_{k+1}]$ (and also $[b_{k+1}, 1]$.
    Because $f([x_1, x_p]) = [x_1, x_p]$, $f^{k+1}([a_{k+1}, b_{k+1}]) \subseteq [x_1, x_p] \subseteq [1 - \eps, 1]$.
    The claim then holds for $k+1$.
    
    Thus, the piecewise linear mapping $g$ with boundaries $g(0)=0$, $g(a_k) = 1-\eps$, $g(b_k) = 1-\eps$, and $g(1) = 0$ is an $\eps$-approximation of $f$.
    Because $g$ has three pieces and contains the origin, it can be exactly represented by a linear combination of four ReLUs, and hence as a depth-2 neural network of width 3.
\end{proof}

\begin{proposition}\label{prop:need-concavity}
% For sufficiently small $\eps > 0$ and $p \geq 3$, there exists a symmetric unimodal mapping $f$ that is \textit{not concave} such that there exists a 2-layer ReLU network of width 3 such that
% \[\max_{x \in [0,1]} \abs{f(x) - g(x)} \leq \eps.\]
For $p \geq 3$ and for sufficiently small $\eps > 0$, there exists a symmetric unimodal mapping $f$ with a chaotic $p$-cycle such that for any $k$, there exists $g \in \mathcal{N}(3,2)$ with
\[L_\infty(f^k, g) \leq \eps.\]
\end{proposition}
\begin{proof}
    Let $x_j = \frac{1}{2} - \frac{p-1-j}{2(p-1)}\eps$ for all $j \in [p-1]$ and $x_p = \frac{1}{2} + \frac{\eps}{2}$.
    Let $f$ be a piecewise-linear function with boundaries
    \begin{align*}
        f(0) = 0, \
        f\paren{\frac{1}{2} - \frac{\eps}{2}} = \frac{1}{2}-\frac{p-2}{p-1} \cdot \frac{\eps}{2}, \
        f\paren{\frac{1}{2} - \frac{\eps}{2(p-1)}} = \frac{1}{2}, \ f\paren{\frac{1}{2}} = \frac{1}{2} + \frac{\eps}{2}, \\
        f\paren{\frac{1}{2} + \frac{\eps}{2(p-1)}} = \frac{1}{2},  \ 
        f\paren{\frac{1}{2} + \frac{\eps}{2}} = \frac{1}{2}-\frac{p-2}{p-1} \cdot \frac{\eps}{2},\
        f(1) = 0.
    \end{align*}
    
    We visualize $f$ for $p=3$ in Figure~\ref{fig:non-concave}. Note that $f$ is symmetric and unimodal and has an increasing $p$-cycle $x_1 < \dots < x_p$. 
    It is \textit{not} concave because $f'(x) = 1$ for $x \in [x_1, x_{p-2}]$ and $f'(x) = 2(p-1)$ for $x \in [x_{p-2}, x_{p-1}]$.
    
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/fig-non-concave1.png}
         \includegraphics[width=0.45\textwidth]{fig/fig-non-concave10.png}
        \caption{Another example of a function with a 3-cycle that can be $\eps$-approximated for arbitrarily small $\eps$. (Here, $\eps = 0.1$.) This function corresponds to the one in Proposition~\ref{prop:need-concavity} and the \cite{cnpw19} bounds are again vacuous for small $\eps$. Unlike Figure~\ref{fig:asymmetric}, this function is symmetric, but not concave.}
        \label{fig:non-concave}
    \end{figure}
    
    Using a very similar argument to argument from the proof of Proposition~\ref{prop:need-symmetry}, for all $k$, there exists $a_k < b_k$ such that $f^k$ is linear on $[0, a_k]$ and $[b_k, 1]$ and $f^k([a_k, b_k]) \in [\frac{1}{2} - \eps, \frac{1}{2} + \eps]$.
    As before, there exists a piecewise linear function with three pieces (which can be thought of as a depth-2 neural network of width 3) that $\eps$-approximates $f$.
\end{proof}

==> Beyond Sharkovsky Paper/supp_toy.tex <==
\section{Supplement for Section~\ref{ssec:warmup}}\label{asec:warmup}

Figures~\ref{fig:toy-ex} and \ref{fig:toy-ex-logistic} demonstrate two emblematic cases where the differences in function complexity of $f_{123}$, $f_{1234}$, and $f_{1324}$ are most evident.
Both figures provide a function for each $f_{\mathbf{a}}$ that has a maximal itinerary of $\mathbf{a}$. (That is, there is no ``higher-ranked'' itinerary from Table~\ref{table:itineraries} present in $f_{\mathbf{a}}$; all other cycles are induced by the existence of a cycle with itinerary $\mathbf{a}$.)

Figures~\ref{fig:toy-ex} and \ref{fig:toy-ex-monotone} provide a simple case where the elements of the cycles are evenly spaced ($\frac14,\frac12, \frac34$ for $f_{123}$; $\frac15, \frac25, \frac35, \frac45$ for $f_{1234}, f_{1324}$).
Despite the fact that $f_{1234}$ and $f_{1324}$ have the same maximum value, they exhibit substantially different fractal-like patterns, which produce exponentially more oscillations for $f_{1234}$.

Figure~\ref{fig:toy-ex-logistic} and \ref{fig:toy-ex-logistic-monotone} instead considers logistic maps of the form $\flog{r}(x) = 4rx(1-x)$ for the values of $r$ where itinerary $\mathbf{a}$ is \emph{super-stable}, or when nearby iterates converge to the cycle exponentially fast.
These functions are concave, symmetric, and unimodal.
Here, complexity strictly increases with the maximum value of $\flog{r}$. Indeed, $f_{1234}, f_{123}$ and $f_{1324}$ ordered by height is the order by which they exhibit most to least chaotic behavior.

\begin{figure}[h]
    \centering
    % \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-1234.png}
    % \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-1324.png}\\
    % \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-123.png}
    % \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-osc.png}
    \includegraphics[width=0.32\textwidth]{fig/fig-toy-ex-1234-thin.png}
    \includegraphics[width=0.32\textwidth]{fig/fig-toy-ex-1324-thin.png}
    \includegraphics[width=0.32\textwidth]{fig/fig-toy-ex-123-thin.png}
    % \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-osc.png}
    \caption{A comparison of the function complexity (as measured by the number of monotone pieces) of $f^k$ for unimodal mappings $f$ having cycles with different itineraries. The left shows $f$, $f^2$, $f^5$, and $f^{10}$ for a function with a 1234 4-cycle. The center has a 1324 4-cycle. The bottom has a 123 3-cycle. 
    Figure~\ref{fig:toy-ex-monotone} shows how the number of monotone pieces of $f^k$ increases with $k$ for each mapping.}
    \label{fig:toy-ex}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-osc.png}
    \caption{Visualizes the number of monotone pieces of $f^k$ which increases with $k$ for each mapping along with $2^k$ (the maximum number of monotone pieces of any unimodal $f$).
    Note that the 1234 itinerary produces a more ``complex'' function with more monotone pieces than 123, despite the Sharkovsky analysis from \cite{cnpw19} arguing that 3-cycles are the most powerful when determining iteration counts.
    Moreover, the number of monotone pieces of the  1234 and 123 itineraries increases exponentially, while that of the 1324 itineraries does not. (Identical to Figure~\ref{fig:toy-intro}.)}
    \label{fig:toy-ex-monotone}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.32\textwidth]{fig/fig-toy-ex-logistic-1234-thin.png}
    \includegraphics[width=0.32\textwidth]{fig/fig-toy-ex-logistic-1324-thin.png}
    \includegraphics[width=0.32\textwidth]{fig/fig-toy-ex-logistic-123-thin.png}
    \caption{Demonstrates the same ideas as Figure~\ref{fig:toy-ex}, except instead of using asymmetric and non-concave piecewise functions, we use the scaled logistic map, $\flog{r}$.
    Using Table~1 of \cite{mss73}, we set the parameter $r$ to $3.96$, $3.50$, and $3.83$ respectively to ensure that a super-stable 1234, 1324, and 123 cycle exists.}
    \label{fig:toy-ex-logistic}
\end{figure}

\begin{figure}
    \centering
        \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-logistic-osc.png}

    \caption{Like Figure~\ref{fig:toy-ex-monotone}, vizualizes the differences in number of monotone pieces for the logistic mappings described in Figure~\ref{fig:toy-ex-logistic}.}
    \label{fig:toy-ex-logistic-monotone}
\end{figure}

==> Beyond Sharkovsky Paper/trash.tex <==
% \section{TRASH}

% %% This is a holding place for anything that we want to axe from the paper before making the cut

% \subsection{Stability}
% It is also occasionally useful to consider the \textit{stability} of a cycle.
% This governs the attractiveness of a cycle.
% A stable cycle will attract nearby iterates, while an unstable cycle repels them.
% Super-stable cycles have exponentially fast rates of convergence.
% shows the connection between these properties and the derivative of the mapping.
% For the definition, we assume that $f$ is differentiable, which can be done by infinitesimally smoothing any maps with discontinuities in slope.

% \begin{definition}
%     A fixed point $x^*$ of $f$ is:
%     \begin{itemize}
%         \item \emph{unstable} if $\abs{\deriv{f(x^*)}{x}} > 1$.
%         \item \emph{stable} if $\abs{\deriv{f(x^*)}{x}} < 1$.
%         \item \emph{super-stable} if $\abs{\deriv{f(x^*)}{x}} = 0$.
%     \end{itemize}
%     A $p$-cycle is said to belong to one of above if the criterion holds for every element of the cycle for $f^p$.
% \end{definition}

% We refer back to a simple correspondence between super-stable cycles and symmetric functions.

% \begin{fact}
%     If $f$ is a symmetric unimodal mapping with a $p$-cycle containing $\frac{1}{2}$, then the cycle is super-stable.
% \end{fact}
% \begin{proof}
%     If we assume that $f$ is symmetric and differentiable everywhere, then $f'(\frac{1}{2}) = 0$.
%     By the chain rule,
%     \[\frac{d}{dx} f^{p}(x) = f'(f^{p-1}(x)) f'(f^{p-2}(x)) \dots f'(f(x)) f'(x).\]
%     Therefore, if the $p$-cycle is $x_1, \dots, x_p$,  WLOG $x_1 = \frac{1}{2}$, then the derivative at any $x_i$ is
%     \[\frac{d}{dx} f^{p}(x_i) = \prod_{j=1}^p f'(x_j) = 0.\qedhere\]
% \end{proof}

% \subsection{Positive Results on Approximation with Deep Neural Networks}

% \begin{proposition}\label{prop:dnn-approx}
%     Suppose $f$ is a continuous piece-wise linear function with $m$ pieces and $f(0)$. For any $k$, $f^k$ can be exactly represented by a ReLU neural network of depth $2k$ and width $m$.
% \end{proposition}
% \begin{proof}
%     $f$ can be exactly represented as a linear combination of $m$ ReLUs, which is a 2-layer neural network of width $m$.
%     Thus, $f^k$ can be represented as the composition of $k$ of those networks, which is of depth $2k.$
% \end{proof}

% \begin{proposition}\label{prop:cycle-chaotic-domination}
%     Suppose $f$ and $g$ are symmetric unimodal functions with $f(x) \geq g(x)$ for all $x \in [0,1]$ and $f(\frac{1}{2}) = g(\frac{1}{2})$.
%     Then, if $f$ has an increasing $p$-cycle, $g$ also has an increasing $(p-1)$-cycle.
% \end{proposition}
% \begin{proof}
%     Let $f$ have the $p$-cycle $x_1 < \dots < x_p$.
%     Because $\frac{1}{2}$ maximizes $f$, it follows that $f(\frac{1}{2}) \geq x_p$ and for any $j \in [p-1]$, $f^{j+1}(\frac{1}{2}) \leq x_j$.
%     Similarly, $g(\frac{1}{2}) = f(\frac{1}{2})$ and $g^{j+1}(\frac{1}{2}) \leq f^{j+1}(\frac{1}{2}) \leq x_j$ by induction.
    
%     It must be the case that $x_{p-2} < \frac{1}{2}$. 
%     If not, then $f(x_{p-2}) =x_{p-1} > f(x_{p-1}) = x_p$, which contradicts $x_p > x_{p-1}$.
%     Thus, $g^{p-1}(\frac{1}{2}) < \frac{1}{2}$, so by Proposition~\ref{prop:half-inc-cycle}, $g$ has an increasing $(p-1)$-cycle.
% \end{proof}

% \begin{remark}
%     By putting Propositions~\ref{prop:dnn-approx} and \ref{prop:cycle-chaotic-domination} together with Theorem~\ref{thm:general-lb-cls}, if there exists some symmetric concave unimodal $f$ with an increasing $p$-cycle for $p \geq 4$, the tent map $\ftent{f(1/2)}$ has an increasing $(p-1)$-cycle.
    
%     Thus, $\ftent{f(1/2)}$ can be exactly represented by a neural network of depth $2k$ and width $2$, but there is no neural network $g$ of depth $\sqrt{k}$ and width $\frac{1}{8}(2 - (2/3)^{p-1})^{\sqrt{k}}$ such that 
%     \[\norm[\infty]{\ftent{f(1/2)}^k - g} < \frac{1}{36}.\]
% \end{remark}

% % The proof relies on several facts about increasing cycles.

% % \begin{lemma}\label{lemma:inc-p-to-inc-p-1}
% %     Suppose for $p \geq 3$ symmetric unimodal mapping $f$ has an increasing $p$-cycle $x_1< \dots < x_p$.
% %     Then, $f$ also has an increasing $(p-1)$-cycle $x_1', \dots, x_{p-1}'$ satisfying
% %     \[x_1 < x_1' < x_2 < x_2' < \dots < x_{p-1} < x_{p-1}' < x_p.\]
% % \end{lemma}
% % \begin{proof}
% %     Because $f$ is continuous, $f^{p-1}(x_1) - x_1 = x_p - x_1 > 0$, and $f^{p-1}(x_2) - x_2 = x_1 - x_2 < 0$, there exists some $x_1' \in (x_1, x_2)$ such that $f^{p-1}(x_1') = 0$.
% %     It remains to show that $x_1'$ cannot be a $p'$ cycle for $p' < p-1$.
    
% %     It must be the case that $x_1 < \dots < x_{p-2} < \frac{1}{2}$.
% %     If not, $f$ would be decreasing on the interval $[x_{p-2}, x_{p-1}]$, which would contradict the fact that $f(x_{p-2}) = x_{p-1} < f(x_{p-1}) = x_p$.
% %     Thus, $f$ is monotonically increasing along $[x_1, x_{p-2}]$, which means that $f$ maps $(x_j, x_{j+1})$ onto $(x_{j+1}, x_{j+2})$ for all $j \in [p-3]$ and $f((x_{p-2}, x_{p-1})) \subset (x_{p-1}, 1)$.
    
% %     As a result, $x_{j+1}' := f^j(x_1') \in (x_{j+1}, x_{j+2})$ for all $j \in [p-3]$ and $x_{p-1} \in (x_{p-1}, 1)$, so the $(p-1)$-cycle $x_1', \dots, x_{p-1}'$ is increasing and does contain duplicates.
% % \end{proof}

% % \begin{lemma}\label{lemma:inc-p-below-half}
% %     Suppose symmetric unimodal mapping $f$ has an increasing $p$-cycle for $p \geq 3$. Then, there exists an increasing $p$-cycle \[x_1' < \dots < x_{p-1}' \leq \frac{1}{2} < x_p'.\]
% % \end{lemma}
% % \begin{proof}
% %     Let $x_1 < \dots < x_p$ be the existing $p$-cycle, and assume that it does not satisfy the desired inequalities.
% %     (Otherwise, the claim is trivial.)
% %     It must be the case that 
% %     \[x_1 < \dots < x_{p-2} < \frac{1}{2} < x_{p-1} < x_p.\]
% %     As discussed in the proof of Lemma~\ref{lemma:inc-p-to-inc-p-1}, having $x_{p-2} \geq \frac{1}{2}$ contradicts $x_{p} > x_{p-1}$.
% %     Having $x_p < \frac{1}{2}$ forces the contradiction $x_1 = f(x_p) > f(x_{p-1}) = x_p$.
    
% %     We consider three cases. Let $g(x) = f^p(x) - x$ and note that $g$ is continuous.
% %     \begin{enumerate}
% %         \item Suppose for some $\eps > 0$, for all $y \in (x_1 -\eps, x_1)$, $g(y) < 0$. Fix some such $y$.
% %         Because $f(0) = 0$ is increasing along $[0, x_1]$, there exists some $y' \in (0, x_1 - \eps)$ with $f^p(y') = x_1 > y'$ and $g(y) > 0$. 
% %         Thus, there exists $x_1' \in (y', y)$ with $g(y) = 0$. Due to a similar argument to the one in the proof of Lemma~\ref{lemma:inc-p-to-inc-p-1}, $x_1'$ must be the first element of a $p$-cycle.
% %     \end{enumerate}
% % \end{proof}

% % \begin{proof}[Proof of Proposition~\ref{prop:cycle-chaotic-domination}]
% %     If $f$ has an increasing $p$-cycle, there exists $1 < x_1 < \dots, x_p < 1$ such that $f(x_j) = x_{j+1}$ and $f(x_p) = x_1$.
% %     Because $\frac{1}{2}$ maximizes $f$, $f(\frac{1}{2}) > x_p$.
% %     Thus, $f^2(\frac{1}{2}) < x_1$ and inductively, $f^{j}(\frac{1}{2}) < x_{j-1}$.
% % \end{proof}

==> abstract.tex <==
\begin{abstract}
    

%Given a target function $f$, how large does a neural network have to be before it can output $f$ approximately? This basic question in neural networks expressivity was recently examined from the lens of dynamical systems leading to novel ``depth vs width'' tradeoffs for a large family of functions $f$. %characterized by an oscillatory behavior.
%A key notion that was shown to govern such tradeoffs was the existence of higher-order fixed points in $f$'s trajectories (called \textit{periodic} points). In this paper, we further deploy dynamical systems ideas in the context of neural networks, proving that periodic points alone lead to far looser bounds on the depth-width tradeoffs; we improve upon them by analyzing stable and super-stable trajectories of $f$, demonstrating that certain ``chaotic itineraries'' can give stronger exponential tradeoffs, even in regimes where previous analyses would only imply polynomial gaps. Furthermore, our bounds are nearly-optimal and, contrary to prior works, they become tighter as the period increases, leading to a more refined understanding for why certain functions $f$ are hard-to-represent with low-depth networks. %As a byproduct, should we include RNN VC sentence?

Given a target function $f$, how large must a neural network be in order to approximate $f$?\\ 
Recent works examine this basic question on neural network \textit{expressivity} from the lens of dynamical systems and provide novel ``depth-vs-width'' tradeoffs for a large family of functions $f$. 
They suggest that such tradeoffs are governed by the existence of  \textit{periodic} points or \emph{cycles} in $f$. 
Our work, by further deploying dynamical systems concepts, illuminates a more subtle connection between periodicity and expressivity: we prove that periodic points alone lead to suboptimal depth-width tradeoffs and we improve upon them by demonstrating that certain ``chaotic itineraries'' give stronger exponential tradeoffs, even in regimes where previous analyses only imply polynomial gaps. 
Contrary to prior works, our bounds are nearly-optimal, tighten as the period increases, and handle strong notions of inapproximability (e.g., constant $L_1$ error). 
More broadly, we identify a phase transition to the \textit{chaotic regime} that exactly coincides with an abrupt shift in other notions of function complexity, including VC-dimension and topological entropy. 

%Finally, we develop strong relationships between periodicity in discrete dynamical systems and other notions of function complexity, 



%further dynamical systems ideas, stable and super-stable cycles analyzing specific chaotic itineraries that give sharper bounds on tradeoffs whereas just relying on periods we would get far looser bounds.



%byproduct VC dimension bounds based on our construction for iterated maps akin to recurrent neural networks.

%Whether a neural network will succeed or fail in representing (or even approximating) a given target function $f$ in its output depends on its depth and width. However, 

%Recent works have established such depth-width tradeoffs by relying on the oscillatory behavior of

%functions as depth-width property
%recent works
%dynamical systems deeper, twist
%1 technical sentence: stronger bounds, L1?, tradeoffs, existence of chaotic itineraries can lead to many more oscillations than what we would expect from Sharkovsky's theorem. 
%overall message
%  \todo{abstract here!}
  \end{abstract}


==> intro.tex <==
\section{Introduction}

%depth inflation, architecture leads to expressivity, analogous to circuit for boolean functions
%simple XOR gate couldn't be represented and this was taken as evidence of weakness of neural networks leading the first AI winter.

%whether we want to deply a NN for image analysis or text or speech one of the first crucial decisions that will determine its success or failure is the architecture of the network

%bounded resources?
Whether a neural network (NN) succeeds or fails at a given task crucially depends on whether or not its architecture (depth, width, types of activation units etc.) is suitable for the task at hand. 
For example, a ``size-inflation'' phenomenon has occurred in recent years, in which NNs tend to be deeper and/or larger. 
Recall that in 2012, AlexNet had 8 layers.
In 2015, ResNet won the ImageNet competition with 152 layers~\citep{krizhevsky2012imagenet,he2016deep},
This trend still continues to date, with modern models using billions of parameters~\citep{brown2020language}. 
The empirical success of deep neural networks motivates researchers to ask: What are the theoretical benefits of depth, and what are the depth-vs-width tradeoffs?

This question gives rise to the study of neural network \textit{expressivity}, which characterizes the class of functions that are representable (or approximately representable) by a NN of certain depth, width, and activation. 
For instance, \cite{eldan2016COLT} propose a family of ``radial'' functions in $\mathbb{R}^d$ that are easily expressible with 3-layered feedforward neural nets of small width, but require any approximating 2-layer network to have exponentially (in $d$) many neurons. In other words, they formally show that depth---even if increased by 1---can be exponentially more valuable than width. 
%add Telgarsky, Schmitt here to illustrate and give a taste of the type of statements...some results: triagnle wave, polynomials. schmitt uses VC to give lower bounds for size of NN for polynomials of degree k, we deploy sharkovsky and get lower bounds for a wider array of periodic cycles...We illuminate the problem from different perspectives


Not surprisingly, understanding the expressivity of NNs was an early question asked in 1969, when Minsky and Papert showed that the Perceptron can only learn linearly separable data and fails on simple XOR functions~\citep{minsky2017perceptrons}. 
The natural question of which functions can multiple such Perceptrons (i.e., multilayer feedforward NN) express was addressed later by \cite{cybenko1989approximation,hornik1989multilayer} proving the so-called \textit{universal approximation} theorem. 
This states, roughly, that just one hidden layer of standard activation units (e.g., sigmoids, ReLUs etc.) suffices to approximate any continuous function arbitrarily well. 
Taken at face value, any continuous function is a 2-layer (i.e., 1-hidden-layer) network in disguise, and hence, there is no reason to consider deeper networks. 
However, the width required can grow arbitrarily, and many works in the following decades quantify those depth-vs-width tradeoffs.


%Numerous results in the literature have established variants of
%this universal approximation property by considering distinct function classes to be
%approximated by network archhitectures using different types of neural activation
%functions with respect to various approximation criteria, see for instance [1, 2, 3, 5,
%6, 11, 12, 14, 15]. (
%All these results and many others not referenced here, some of them being constructive, some being merely existence proofs, provide upper bounds for the network size
%asserting that good approximation is possible if there are sufficiently many network nodes available. This, however, is only a partial answer to the question that
%mainly arises in practical applications: "Given some function, how many network
%nodes are needed to approximate it?" Not much attention has been focused on
%establishing lower bounds on the network size and, in particular, for the approximation of functions over the reals. As far as the computation of binary-valued: GIVE CITATIONS FOR BOOLEAN FUNCTIONS AS WELL Koiran, Maass etc.....


Towards this direction, one typically identifies a function together with a ``measure of complexity'' to demonstrate benefits of depth. 
For example, the seminal work by \cite{telgarsky15,telgarsky16} relies on the number of oscillations of a simple triangular wave function. 
Other relevant notions of complexity to the expressivity of NNs include the VC dimension~\citep{warren1968lower,anthony1999neural,schmitt2000lower}, the number of linear regions~\citep{montufar2014number,arora2016understanding} or activation patterns~\citep{hanin2019deep}, the dimension of algebraic varieties~\citep{kileel2019expressive}, the Fourier spectrum~\citep{barron1993universal,eldan2016COLT,daniely2017depth,lee2017ability, bresler2020sharp}, fractals~\citep{malach2019deeper}, topological entropy~\citep{bzl20}, Lipschitzness~\citep{safran2019depth,hsu2021approximation}, global curvature and trajectory length~\citep{poole2016NIPS,raghu2017ICML} just to name a few. 



%should I put BZL here or above?
This work builds upon recent papers~\citep{cnpw19,cnp20}, which study expressivity from the lens of discrete-time dynamical systems and extend Telgarsky's results beyond triangle (tent) maps. 
At a high-level, their idea is the following: if the initial layers of a NN output a real-valued %\footnote{Lower bounds were proved for dimension 1. However similar statements hold in higher dimension.} 
function $f$, then concatenating the \textit{same} layers $k$ times one after the other outputs $ f^k  \vcentcolon = f\circ f\circ \ldots\circ f$, i.e., the composition of $f$ with itself $k$ times. 
By associating each discrete timestep $k$ to the output of the corresponding layer in the network, one can study expressivity via the underlying properties of $f$'s trajectories. 
Indeed, if $f$ contains higher-order fixed points, called \textit{periodic} points, then deeper NNs can efficiently approximate $f^k$, but shallower nets would require exponential width, governed by $f$'s periodicity.

Inspired by these novel connections to discrete dynamical systems, we pose the following natural question:
\begin{center}
\textit{Apart from periodicity, are there other properties of $f$'s trajectories governing the expressivity tradeoffs?}
\end{center}
%trajectory, periodicity, other properties, augment expressivity, tight bounds from periodicity, can we improve?

We indeed prove that $f$'s periodicity alone is not the end of the story, and we improve on the known depth-width tradeoffs from several perspectives. 
We exhibit functions of the same period with very different behaviors (see Sec.~\ref{ssec:warmup}) that can be distinguished by the concept of ``chaotic itineraries.'' 
We analyze these here in order to achieve nearly-optimal tradeoffs for NNs. 
Our work highlights why previous works that examine periodicity alone only obtain loose bounds. 
More specifically:
%SHOULD WE ADD BULLET POINTS? AND ROUGHLY STATE IN SIMPLE WORDS THE RESULTS?

\begin{itemize} 
\item We accurately quantify the oscillatory behavior of a large family of functions $f$. This leads to sharper and nearly-optimal lower bounds for the width of NNs that approximate $f^k$.
\item Our lower bounds cover a stronger notion of approximation error, i.e., \textit{constant} separations between NNs, instead of bounds that become small depending heavily on $f$ and its periodicity.
\item At a conceptual level, we introduce and study certain chaotic itineraries, which supersede Sharkovsky's theorem~(see Sec.~\ref{subsec:dds}). 
% Our contributions are powered by technical lower bounds on the eigenvalues of a discrete dynamical system arising from such itineraries and show how the resulting oscillations cannot shrink significantly.
\item We elucidate connections between periodicity and other function complexity measures like the VC-dimension and the topological entropy~\citep{alseda2000}. %, and the ease of neural network approximation.
We show that all of these measures undergo a phase transition that exactly coincides with the emergence of the chaotic regime based on periods.
\end{itemize}
%on a conceptual level: we identify that the itineraries are actually important and not only the length of the periodic cycles as prior works on the topic seems to suggest. this allows us to get more refined bounds.


To the best of our knowledge, we are the first to incorporate the notion of chaotic itineraries from discrete dynamical systems into the study of NN expressivity. Before stating and interpreting our results, we provide some basic definitions.


\subsection{Function Approximation and NNs}
%constant errors vs yx errors, L1 L\infty, classification, and history of increasingly better and better results in the litearture
This paper employs three notions of approximation to compare functions $f, g: [0,1] \to [0,1]$.
\begin{itemize}
    \item $L_1(f,g)= \norm[1]{f - g} = \int_{0}^1 \abs{f(x) - g(x)} dx.$
    \item $L_\infty(f,g)=\norm[\infty]{f - g} = \sup_{x \in [0, 1]} \abs{f(x) - g(x)}.$
    \item Classification error $\mathcal{R}_{S,t}$: For $t \in [0,1]$, let $\thres{t}{x} = \indicator{x \geq t}$. Let $S = \{x_1, \dots, x_n\} \subseteq [0,1]$. Then,
    $\errcls{S,t}{f,g}= \frac{1}{n} \sum_{i=1}^n \indicator{\thres{t}{f(x_i)} \neq \thres{t}{g(x_i)}}.$ 
\end{itemize}
For what follows, let $\mathcal{N}(u,\ell)$ be the family of feedforward NNs of depth $\ell$ and width at most $u$ per layer with ReLU activation functions.\footnote{Recall ReLU$(x)=\max(x,0)$.} All our results also hold for the more general family of semialgebraic activations~\citep{telgarsky16}.

%\clayton{Add a note that $L_1 > Cls, L_\infty$ in terms of LBs? I think it's ok to skip, since we will not only derive L_1 bounds. Maybe we can mention in the main body?}

%say about error f,g in classifictation: you choose y_i to be f(x_i) for example of g etc...  then say about comparing these types of errors... What is the best to approximate? and give historical progression with Schmitt

%ntioning that the telgarsky triangle has an increasing cycle of any length
% THIS MEANS WE IDENTIFY NOT ONLY PERIODS AS THE CULPRIT FOR NECESSITY OF DEPTH, BUT RATHER CHAOTIC ITINERARIES THAT GIVE MORE OSCILLATIONS AND SHARPER BOUNDS... so we still abstract away details from triangle wave, but give general certificates for functions that give us bounds...

%It is important to understand that when we prove lower bounds for the difference of two functions, then the most desirable result is to obtain an $L_1$ bound
%not sure if we should phrase classification error wrt to f,g not just f. but that's fine...

%, and in the context of depth-width tradeoffs, we have managed to obtain increasingly better and better separations.

 %and $\round(z) = \round_{1/2}(z)$.

%For some threshold $t \in [0,1]$, , and , we let the \textit{classification error} of $f$ be







\subsection{Discrete Dynamical Systems}
\label{subsec:dds}
%period, sharkovsky, hint that sharkovsky is not the whole story
%chaotic itinerary
To construct families of functions that yield depth-separation results, we rely on a standard notion of \textit{unimodal} functions from dynamical systems~\citep{mss73}.

\begin{definition}
     Let $f: [0,1]\to[0,1]$ be a continuous and piece-wise differentiable function. We say $f$ is a \emph{unimodal mapping} if:
    \begin{enumerate}
        \item $f(0) = f(1) = 0$, and $f(x) > 0$ for all $x \in (0,1)$.
        \item There exists a unique maximizer $x'\in (0,1)$ of $f$, i.e., $f$ is strictly increasing on the interval $[0, x')$ and strictly decreasing on $(x',1]$.
    \end{enumerate}
\end{definition}

Our constructions rely on unimodal functions that are concave and also symmetric (i.e., $f(x) = f(1-x)$ for all $x \in [0, 1]$). 
We note that the resulting function family is fairly general, already capturing the triangle waves of \cite{telgarsky15,telgarsky16} and the logistic map used in previous depth-separation results~\citep{schmitt2000lower}.
Moreover, the study of one-dimensional discrete dynamical systems by applied mathematicians explicitly identifies unimodal mappings as important objects of study~\citep{mss73, alseda2000}.

Recall that a fixed point $x^*$ of $f$ is a point where $f(x^*)=x^*$. A more general notion of higher-order fixed points is that of \textit{periodicity}.

% \begin{definition}
% Let $p\in \mathbb{N}$ with $p\ge1$. We say $f$ has \emph{periodicity} $p$ (or  has a point of period $p$), if there exists a point $x^* \in [0,1]$ such that:\footnote{Throughout the paper, $f^{p}$ means composition of $f$ with itself $p$ times.}
% $$
% 	f^{p}(x^*)=x^* {\text{ \ \ and\ \ \ }} f^{k}(x^*)\neq x^*, \ \forall k \in [p-1].
% $$
% The set $C \vcentcolon= \{x^*,f(x^*), f(f(x^*)),\dots, f^{p-1}(x^*)\}$ contains $p$ distinct elements and is called a \emph{$p$-cycle}. Fixed points correspond to $p=1$.
% %\clayton{Can we make $p$ a an ordered $p$-tuple rather than a set, since order matters? - I think for now this is simpler to grasp.}
 
% \end{definition}
\begin{definition}
For some $p \in \N$, we say that $x_1,\dots, x_p\in [0,1]$ is a \emph{$p$-cycle} if $f(x_j) = x_{j+1}$ for all $j \in [p-1]$ and $f(x_p) = x_1$.
We say that $f$ has \emph{periodicity} $p$ if such a cycle exists and that $x_1$ is a \emph{point of period $p$} if $x_1$ belongs to a $p$-cycle. 
Equivalently, $x_1$ is a point of period $p$ if $f^p(x_1) = x_1$ and $f^{k}(x_1) \neq x_1$\footnote{Throughout the paper, $f^{k}$ means composition of $f$ with itself $k$ times.} for all $k \in [p-1]$.\footnote{As is common, $[m] = \{1, 2, \dots, m\}$.}
\end{definition}

%chaos theory, period 3 implies chaos, 
Does the existence of some $p$-cycle in $f$ have any implications about the existence of other cycles?
% Are there constraints between the types of periods a mapping $f$ can possess? 
These relations between the periods of $f$ are of fundamental importance to the study of dynamical systems. 
In particular, \cite{li1975period} proved in 1975 that ``period 3 implies chaos'' in their celebrated work, which also introduced the term ``chaos'' to mathematics and later spurred the development of chaos theory. 
Interestingly, an even more general result was already obtained a decade earlier in Eastern Europe, by~\cite{sharkovsky1964coexistence,sharkovsky1965cycles}:


\begin{theorem}[Sharkovsky's Theorem]
\label{thm:sharkovsky}
Let $f: [0,1]\to[0,1]$ be continuous. If $f$ contains period $p$ and $p \triangleright p'$, then $f$ also contains period $p'$, where the symbol `` $\triangleright$'' is defined based on the following (decreasing) ordering: 
\[
3 \triangleright 5 \triangleright 7\triangleright \ldots \triangleright2\cdot3 \triangleright 2\cdot5 \triangleright 2\cdot7\triangleright\ldots
\]
\[
\ldots \triangleright 2^2\cdot3 \triangleright 2^2\cdot5 \triangleright 2^2\cdot7\triangleright\ldots\triangleright2^3\triangleright2^2\triangleright2\triangleright1.
\]
\end{theorem}

This ordering, called \textit{Sharkovsky's ordering}, is a total ordering on the natural numbers, where $l\triangleright r$ whenever $l$ is to the left of $r$. The maximum number in this ordering is 3; if $f$ contains period 3, then it also has all other periods, which is also known as \emph{Li-Yorke chaos}. 
\cite{cnpw19,cnp20} apply this theorem to obtain depth-width tradeoffs based on periods and obtain their most powerful results when $p = 3$. 
We go beyond Sharkovsky's theorem and prove that tradeoffs are determined by the ``itineraries'' of periods.\footnote{These are called ``patterns'' in~\cite{alseda2000}.}

%\begin{definition}[Chaotic Itineraries]
%    Let $C$ be some $p$-cycle $x_1, \dots, x_p$ of a unimodal $f$. 
%    The \emph{itinerary} of $C$ is a string $\textbf{a}=a_1a_2\ldots a_p \in \{L, C, R\}^p$ of length $p$, with:
%    \[a_i \vcentcolon = \begin{cases}
%        L & x_i < x_{\max} \\
%        C & x_i = x_{\max} \\
%        R & x_i > x_{\max}.
%    \end{cases}\]
%Furthermore, any itinerary consisting of $(p-1)$ consecutive $L$'s followed by a single $R$, i.e., $\textbf{a}= L^{p-1}R = LL\ldots LR$ is called a \emph{chaotic} itinerary.
%\end{definition}

\begin{definition}[Itineraries]
    For a $p$-cycle $x_1, \dots, x_p$, suppose that $x_{a_1} < \dots < x_{a_p}$ for $a_j \in [p]$.
    The \emph{itinerary} of the cycle is the cyclic permutation of $x_{a_1}, \dots, x_{a_p}$ induced by $f$, which we represent by the string $\ba= a_1\dots a_p$.
    Because cyclic permutations are invariant to rotation, we assume (wlog) that $a_1 = 1$.


    % The \textit{itinerary} of a $p$-cycle is a cyclic permutation of the $p$ sorted elements $x_1 < \dots < x_p$ that indicates in what order they are traversed.
    % We represent the permutation with a string $\ba=a_1a_2\ldots a_p \in [p]^p$ that encodes this ordering and implies that $f(x_{a_i}) = f(x_{a_{i+1}})$ for all $i \in [p-1]$ and $f(x_{a_p}) = f(x_{a_1})$.
    % Itineraries are invariant to rotation, so we can assume (wlog) $x_1$ to be the smallest element of $C$, i.e., $a_1 = 1$.
    
    % Let $C$ be a $p$-cycle $x_1, \dots, x_p$ of a mapping $f$. 
    % The \emph{itinerary} of $C$ is a string $\ba=a_1a_2\ldots a_p \in [p]^p$ of length $p$ representing a permutation of the points in $C$. That is, $a_ia_j$ is a substring of $\ba$ if $f(x_i) = x_j$. 
    % Itineraries are invariant to rotation, so we can assume (wlog) $x_1$ to be the smallest element of $C$, i.e., $a_1 = 1$.
\end{definition}  

\begin{definition} [Chaotic Itineraries]
%   Any itinerary whose cycle has $x_1 < x_2 < \dots < x_p$ is called a \emph{chaotic} itinerary and is identifiable by $12\dots p$. (Because of its form, it is often called an \emph{increasing} $p$-cycle as well.) 
    A $p$-cycle is a \emph{chaotic itinerary} or an \emph{increasing cycle} if its itinerary is $12\dots p$. That is, $x_1 < \dots < x_p$. 
\end{definition}
Examining chaotic itineraries circumvents the limitations of prior works based on periods and yields sharper exponential depth-width tradeoffs. 
Unlike other function complexity properties, the existence of a chaotic itinerary is easily verifiable (see App.~\ref{assec:identifying}).
To grasp clean examples of itineraries, see App.~\ref{assec:it-exs}.




%Observe that the number 3 is the largest according to this ordering. Sharkovsky showed a surprising and elegant result about his ordering: it describes which numbers can be periods for a
%continuous map on an interval; allowed periods must be a suffix of his ordering:


%According to Sharkovsky's Theorem, 3 is the maximum period, so one important and easy-to-remember corollary is that period 3 implies \textit{all} periods.\footnote{On a historical plot twist, this special case was proved a decade later by James Yorke and Tien-Yien Li, in their seminal paper called ``Period Three Implies Chaos''~\cite{li1975period}; this is a celebrated result that actually introduced the term ``chaos'' as used in Mathematics (chaos theory).}



% $x^*$ is a \textit{fixed point} if $f(x^*) = x^*$.
%    For any $p > 1$, $x^*$ is a \textit{$p$-cyclic} point if $f^p(x^*) = x^*$ and $f^q(x^*) \neq x^*$ for all $q < p$.
%    We say that $f$ has a \textit{$p$-cycle} if there exists $p$ points $x_1, \dots, x_p$ such that $f(x_i) = x_{i+1}$ for $i \in [p-1]$ and $f(x_p) = x_1$.


\subsection{Our Main Contributions}

Our principal goal is to use knowledge about $f$'s itineraries to more accurately quantify the ``oscillations'' of $f^k$ as a measure of complexity and draw connections to other complexity measures. 
Section~\ref{sec:lb} produces sharper and more robust NN approximability tradeoffs than prior works by leveraging chaotic itineraries and unimodality.
Section~\ref{sec:phase} shows how a phase transition in VC-dimension and topological entropy of $f$ occurs exactly when the growth rate of oscillations shifts from polynomial to exponential. 


While previous works count oscillations too, they either construct too narrow a range of functions\footnote{e.g.,~\cite{telgarsky15,telgarsky16} only analyzes triangles.}, obtain loose depth-width tradeoffs\footnote{e.g.,~\cite{cnpw19,cnp20} have a suboptimal dependence on $p$ under stringent Lipschitz assumptions.}, or have unsatisfactory approximation error. \footnote{e.g.,~\cite{cnpw19,cnp20,bzl20} do not obtain constant error rates.} 
In Section~\ref{sec:lb}, we improve along these three directions by taking advantage of the unimodality and itineraries of $f$. 
% Roughly speaking, we compose $k$ times a unimodal function $f$ with itself to obtain $f^k$. 
The \textit{unimodality} of $f$ allows us to quantify both the number of piecewise monotone pieces of $f^k$ (i.e., oscillations) and the corresponding height between the highest and lowest values of $f^k$'s oscillations. 
This improvement on the height enables stronger notions of function approximation (e.g., constant error rates with no dependence on $f$ or its period $p$). 
\textit{Chaotic itineraries} allow an improved analysis of the number of oscillations in $f^k$ and grant sharper exponential lower bounds on the width of any shallow net $g$ approximating $f^k$. 

We say that our results are \textit{nearly-optimal} because we exhibit a broad family of functions $f$ that are inapproximable by shallow networks of width $O(\rho^k)$ for $\rho$ arbitrarily close to 2.
Because no unimodal function $f$ can induce more than $2^k$ oscillations in $f^k$, we cannot aspire to tighter exponent bases in this setting.\footnote{Our results also transfer to non-unimodal functions via the observation that for bimodal $g$, there is some unimodal $f$ such that the number of oscillations of $g$ is at most twice those of $f$.}
On the other hand, none of the bounds from previous works (except the narrow bounds of Telgarsky) produce width bounds of more than $\Omega(\phi^k)$, where $\phi \approx 1.618$ is the Golden Ratio.
To demonstrate our sharper tradeoffs, we state a special case of our results for the $L_\infty$ error.

\begin{theorem}\label{thm:motivation-lb-inc} 
% Let $g\in \mathcal{N}(u,\ell)$. For $p\ge 3$, let $\rho$ be the largest root of the polynomial equation $\lambda^{p} - 2\lambda^{p-1} + 1 = 0$.\footnote{Notice that $\rho \geq \max({2 - \frac4{2^{p}},{\tfrac{1+\sqrt 5}{2}}})$~(see Fact~\ref{fact:root-lb}) and is much stronger than previous bounds~\citep{cnpw19,cnp20}.} Moreover, let $f$ be any symmetric, concave unimodal mapping with a increasing $p$-cycle. For all $k\in\N$, if $g$ has $L_\infty(f^k,g) \le \tfrac{1}{36}$, then it must have large width:\todo{swap polynomial with bound}
% \[
% u  > \frac{1}{8} \rho^{k/\ell}
% \]
For $p \geq 3$ and $k \in \N$, consider any symmetric, concave unimodal mapping $f$ with an increasing $p$-cycle and any $g \in \mathcal{N}(u, \ell)$ with width \[u \leq \frac18 \left(\max\paren{2-\frac4{2^p}, \phi}\right)^{k/\ell}\]
Then, $L_\infty(f^k, g) = \Omega(1)$, independent of $f,p,k$.
\end{theorem}  
%\clayton{How about we instead say ``there exists a $\rho \geq 2 - \frac4{2^{\rho}}$'' to avoid introducing the polynomial? I like this polynomial to be there just so that they wonder how did it appear ? :P}
    
\begin{remark} When $g$ is shallow with depth $\ell=O(k^{1-\eps})$ (e.g., $\ell=k^{0.99}$), then its width must be exponentially large in order to well-approximate $f^k$.
% This shows how depth can be exponentially more valuable than width. 
% Moreover, $\rho \geq \max({2 - \frac4{2^{p}},{\tfrac{1+\sqrt 5}{2}}})$~(see Fact~\ref{fact:root-lb}). 
This exponential separation is sharper than prior works~\citep{cnpw19,cnp20}, and quickly becomes even sharper (tending to 2) with larger values of $p$. 
This is counterintuitive as Sharkovsky's ordering implies that period 3 is the most chaotic and prior works recover a suboptimal rate of at most $\phi\approx 1.618$ (see Table~\ref{table:rho_inc}). 
% Since $\rho\le 2$ for unimodal $f$, our bound quickly converges to the optimal tradeoff (see Fig.~\ref{fig:toy-intro}). 
\end{remark}
\begin{remark}
Our approximation error is constant independent of all other parameters $f, k, p$. 
Previous results~\citep{cnpw19,cnp20,bzl20} obtain a gap that depends on $f,p$ and may be arbitrarily small.
Moreover, we have required nothing of the Lipschitz constant of $f$, unlike the strict assumptions on the Lipschitz constant $L$ of $f$ by~\cite{cnp20} (e.g., they require $L=\phi$ for period $p=3$).
Indeed, Propositions~\ref{prop:need-symmetry} and \ref{prop:need-concavity} in the Appendix~\ref{assec:sym-conc} illustrate how their lower bounds break down for large $L$ and how their $L_\infty$ bounds can shrink, becoming arbitrarily weak for certain 3-periodic $f$.
\end{remark}

We also present analogous results for the classification error and the $L_1$ errors. Please see the full statements in Theorems~\ref{thm:main-linf} and \ref{thm:main-l1}. Furthermore, Theorems~\ref{thm:odd-linf} and \ref{thm:odd-l1} offer an improvement on the results of \cite{cnp20} by giving constant-accuracy $L_\infty$ lower bounds without needing a chaotic itinerary.

In addition, Section~\ref{sec:phase} relates our chaotic itineraries to standard notions of function complexity like the VC dimension and the topological entropy (for precise definitions, see Sec.~\ref{sec:phase}). The types of periodic itineraries of $f$ give rise to two regimes: the \textit{doubling} regime and the \textit{chaotic} regime. In the former, we have a polynomial number of oscillations, while the latter is characterized by an exponential number of oscillations. Here we show the following correspondence:

\begin{theorem}[Informal]\label{thm:informal-phase}
The transition between these two regimes exactly coincides with a sharp transition in the VC-dimension of the iterated mappings $f^k$ for fixed $f$ (from bounded to infinite) and in the topological entropy (from zero to positive).
\end{theorem}


%challenge? technical side? more broadly VC...
\paragraph{Our Techniques} To quantify the oscillations of $f^k$, we use its chaotic itineraries to decompose the $[0,1]$ interval into several subintervals $\{I_j\}_{j=1}^{j=p-1}$. We count the number of times $f^k$ ``visits'' each $I_j$, by identifying a suitable matrix $A$ whose spectral radius is a lower bound on the growth rate of oscillations. The associated characteristic polynomial of $A$ is $\lambda^{p} - 2\lambda^{p-1} + 1$ and has larger spectral radius that that of prior works for \textit{all} periods. 
Moreover, the corresponding oscillations of at least one of the subintervals $I_j$ do not shrink in size, giving a bound on the total number of oscillations of a \textit{sufficient} size. 
This provides a lower bound on the height between the peak and the bottom of these oscillations that later provides \textit{constant} approximation errors for small shallow NNs.

More broadly, our work builds on the efforts to characterize large families of functions that give depth separations and addresses questions raised by~\cite{eldan2016COLT,telgarsky16,poole2016NIPS, malach2019deeper} about the properties of hard-to-represent functions. Similar to periods, the concept of chaotic itineraries can serve as a certificate of complexity, which is also easy to verify for unimodal $f$ (see Proposition~\ref{prop:half-inc-cycle} in Appendix).

%and relying on shallow nets few oscillations, 




%high-level: shallow nets few oscillations, deep nets large number of oscillations, following prior works we use oscillations as notion of complexity. We present refined bounds based on our unimodal funtions and f^k. This boosted oscillations numbers allow to get our improved bounds alongside the VC and topological entropy phase shift.



%on a technical level: eigenvalue analysis based on chaotic itineraries provide us with more oscillations. Furthermore, they provide us with constat-separated oscillations sth which was not known if it can be done before where the gap was shrinking based on y-x which we could not control. Now we change the quantifiers saying that for there is a gap such that for any period p .... whereas before they said for every period p function there is a constant that depends on f and p and y-x such that... this boosting on the number of oscillations allow us to get sharper tradeoffs that become sharper and sharper as p increases, sth that was not known before and are nearly optimal approaching the best 2^n dependence of unimodal functions.

%more broadly, we also provide evidence that the shift in regimes from doubling to chaotic coincides exactly with VC bounds change and also topological entropy of related function family based on iterated maps.

%say that throughout the paper we provide experiments or simulations to demonstrate our resutls.

%briefly we summarize our contributions bellow: give 3 bullet points: 1) sharkovsky and periods not the end of story. using chaotic itineraries we get boosted number of oscillations. 2) these translate to larger and constant gaps in errors, better dependence on p, more subtle connection with expressivity and depth-width tradeoffs. Informally, state two main theorems. 3) state informally results for VC and topological entropy.


%some of our results are incomparable to prior works: on the one hand, in ICML they have very stringent assumptions on the lipschitz constant in order to prove bounds which we destroy by the two counterexamples. On the other hand, we do require symmetry and concavity and altough natural these can't compare with the lipschitz assumption. We get stronger separations compared to ICLR, we completely generalize Telgarsky, and we get better bounds than Harvard paper.


\section{Warm-up Examples}\label{ssec:warmup}

This section presents illustrative examples and instantiates our results for some simple cases. 
These highlight the limitations of exclusively considering periodicity of cycles alone---and not itineraries---when developing accurate oscillation/crossing bounds~(see also Def.~\ref{def:osc},~\ref{def:cross}) and sharp expressivity tradeoffs.

%To demonstrate the strength of our bounds and the centrality of itineraries to the connections between dynamical systems and neural network expressivity, we consider a simple case where itineraries supersede periodicity in number of oscillations and hardness of approximation.

Consider the three unimodal mappings in Figure~\ref{fig:toy-ex-compare-map}, $f_{\ba}$ with itineraries $\ba \in \{1324, 1234, 123\}$. 
Observe that $f_{1234}$ has the cycle $(\frac{1}{5}, \frac{2}{5}, \frac{3}{5}, \frac{4}{5})$, $f_{1324}$ has $(\frac{1}{5}, \frac{3}{5}, \frac{2}{5}, \frac{4}{5})$, and $f_{123}$ has $(\frac{1}{4}, \frac{1}{2}, \frac{3}{4})$. Despite their similarities, they give rise to significantly different behaviours in $f_{\ba}^k$.

What do prior works based on NN approximation with respect to periods and Sharkovsky's theorem alone tell us?  
\cite{cnpw19,cnp20} show that the 3-cycle of $f_{123}$ ensures that $f^k$ has $\Omega(\phi^k)$ oscillations, where $\phi \approx 1.618$ is the golden ratio. However, their theorems do not imply anything for $f_{1324}$ and $f_{1234}$, since 4 is a power of 2, and they require odd periods.  
%One might expect a ``chaos hierarchy'' that ranks $f_{123}$ above $f_{1324}$ and %$f_{1234}$.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-compare_map.png}
    \caption{Plots of unimodal mappings with different itineraries $f_{1234}$, $f_{1324}$, and $f_{123}$. Despite their similarities, $f_{1234}$ leads to the most oscillations and sharpest depth-width tradeoffs (see Fig.~\ref{fig:toy-intro}).}
    \label{fig:toy-ex-compare-map}
\end{figure}
As it turns out, $f_{1234}$ leads to exponential oscillations and $f_{1324}$ leads only to polynomial oscillations:
\begin{itemize}
    \item A mapping with a 1324-itinerary is guaranteed no other cycles except the 2-cycle and a fixed point~\citep{mss73}. 
    Sharkovsky's theorem and \cite{cnpw19} predict this outcome, since 4 is the third-right-most element of the Sharkovsky ordering, and its existence alone promises nothing more.
    The ordering of itineraries introduced by~\citep{mss73} (see Table~\ref{table:itineraries} in Appendix) indicates that the particular 1324-itinerary only implies the periods 2 and 1, and confirms this intuition.
    % \vaggos{what is 12 itinerary?}
    We classify this itinerary as part of the \emph{doubling regime} and prove in Theorem~\ref{thm:properties-doubling} that any $f^k$ with a \textit{maximal} 1324-itinerary (that is, there is no 8-cycle) cannot exhibit sharp depth-width tradeoffs: for any $\eps>0$, there exists a 2-layer ReLU neural network $g$ of width $O(\frac{k^3}{\eps})$ such that 
    $L_\infty(f_{1324}^k, g) \leq \eps.$
    

    \item Going beyond Sharkovsky's theorem, a mapping with a 1234-itinerary---even though it is of period 4---it is guaranteed to contain a 3-cycle as well (see Table~\ref{table:itineraries} in Appendix). Hence, ``itinerary-1234 implies period-3, implies chaos,'' and $f_{1234}^k$ has at least $\Omega(\phi^k)$ oscillations and is hard to approximate by small shallow NNs. Moreover, Theorem~\ref{thm:main-linf} and Table~\ref{table:rho_inc} show that $f_{1234}^k$ actually has $\Omega(\rho^k)$ oscillations for $\rho \approx 1.839 > \phi$. A corollary is that any NN $g$ of depth $\sqrt{k}$ and width $O(1.839^{\sqrt{k}})$ has $L_{\infty}(f_{1234}^k, g) = \Omega(1)$, which is a stronger separation (\textit{constant} error) than the ones given by~\cite{cnpw19, cnp20}.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{fig/fig-toy-ex-osc.png}
    \caption{The chaotic itinerary $f_{1234}$ has more oscillations than $f_{123}$ even though $3 \triangleright 4$ by Sharkovsky's Theorem. Itineraries $f_{1234}$ and $f_{1324}$ (both of period 4) differ dramatically in oscillation count, showing why periodicity alone fails to capture the optimal tradeoffs.}
    \label{fig:toy-intro}
\end{figure}
%\vspace{-0.4cm}
The reverse is not true: Sharkovsky's Theorem guarantees that period-3 implies period-4, but the only 4-cycle guaranteed by the theorem is actually the non-chaotic 1324-itinerary, already shown to lead to minimal function complexity. 


Furthermore, as $p$ increases, the existence of a chaotic itinerary $12\dots p$ on $f$ ensures that $f^k$ has $\Omega(\rho^k)$ oscillations for $\rho \to 2$.\footnote{Similarly to~\cite{telgarsky16}, the optimal achievable rate is $\rho\le 2$ if we start with a unimodal $f$ (e.g., tent map). If one used multimodal functions as a building block (e.g., starting with $f'=f^2$ or $f'=f^3$), we could achieve larger rates (e.g., 4 or 8 respectively).} Figure~\ref{fig:toy-intro} demonstrates these differences in oscillations (by counting the number of monotone pieces of functions $f^k_{\mathbf{a}}$ with a maximal itinerary-$\mathbf{a}$). As indicated theoretically, the number of oscillations of $f_{1324}$ is polynomially-bounded, while the others grow exponentially fast, with $f_{1234}$ being closer to $2^k$. Please see Appendix~\ref{asec:warmup} for more such examples. 

%As a result, the true chaos hierarchy of these functions orders them as $f_{1234} > f_{123} >  f_{1324}$.
Generally, prior constructions where the oscillation count of $f^k$ increase at a rate faster than $\phi^k$ were too narrow (including only the triangle map). 
Because $f_{1234}$ breaks the barrier, we abstract away the details and point to chaotic itineraries as the main source of complexity, leading to sharper depth-width tradeoffs. 

While periodicity tells a compelling story about why $f_{123}^k$ is difficult to approximate, it fails to explain why $f_{1234}^k$ is even more complex.
The exponential-vs-polynomial gap in the function complexity of $f_{1234}$ and $f_{1324}$ depends solely on the order of the elements of the cycle and distinguishes functions that NNs can easily approximate from those they cannot.

The remainder of the paper addresses the question introduced here---when does the itinerary tell us much more than the length of the period---in a general context that explores a ``hierarchy'' of such chaotic itineraries, strengthens a host of NN inapproximability bounds (Sec.~\ref{sec:lb}), and reveals tight connections with other complexity notions, like the VC-dimension and topological entropy~(Sec.~\ref{sec:phase}).




%however in the study of DS it is known that orbits specifically can govern the oscillations rather than just the orbit length. Can we further deploy this idea to give better bounds on the tradeoffs?
\iffalse
\newpage
\vaggos{check two recent papers neurips related? Exact expressibility of functions vs approximate...}

\vaggos{bounded width also limits the NN so benefits of width?}

%cite Minsk Papert Perceptron multilayerThis led to s which state
%unbounded width
%works try to quantify the tradeoffs
%using various techniques all over math
%more broadly, analogous questions are fundamental in complexity, circuit and other models of computation


%a basic, yet challenging question in deep learning theory with rich connections to many other areas of mathematics and computer science. One of the earliest results


%parity function in boolean functions is difficult unless we have logn depth...

%AI Winter due to misunderstanding about XOR and expressivity. so we need to figure out the class of functions representable. 
%2 vs 3 layers 

%Why aren’t AIs running around solving all the world’s problems? In brief, the problem is that neural networks are hard to train. Just because you know there should be a set of parameters that approximates your function well with your given network architecture, doesn’t mean there is any good way of finding those parameters.


\vaggos{our bounds: they tighten as the period increases contrary to prior works.}
\vaggos{important to clarify that we quantify the xy gap. for every function that had odd period there exist xy... exists xy gap such that every function with odd period has gap at least some 0.1 or sth...}

-DNNs remarkable performance last few years, but why do deeper nets perform better than shallow? Expressivity questions studies types of functions that are representable or approximately representable by the output of a NN. e.g. can we find functions that are easily represented as 3 layers but not as two? Cite Eldan/Shamir. What about deeper regimes? However early results show depth 2 suffices. Bounded resources lead to depth vs width separations. An example is Telgarsky's result which gives a specific function that deep nets represent easily but shallow nets need to be exponentially wide. A main question in Telgarsky's and other papers (cite Malach/SSS) is to find larger families or what are the properties of such hard-to-represent functions?

-List of complexity measures to distinguish depth separations. Note that the question of expressivity makes sense in other computational models like boolean circuits where analogous depth separation results are fundamental in complexity theory etc. (cite Hastad).

-Most recently papers rely on dynamical systems ideas eg ICLR ICML and Harvard paper. Nice thing about these is that they point out to exciting new connections with DS literature and be able to prove much stronger bounds and larger families of functions that yield depth separations.

-Crucial connecting thread is higher order notion of fixed points and oscillations that was made explicit in ICLR/ICML via Sharkovsky's theorem.

-Pose 1 main motivating question: Can we go beyond Sharkovsky's theorem and exploit further properties of chaotic maps derive sharper depth separation results further proving benefits of depth for certain classes of functions?

-explain the main surprise, state informal theorem, explain bounds, and how we improve.

-motivating warm-up example: idea of ``chaotic itineraries'' and connection to eigenvalue and characteristic polynomial governing the oscillations.

-show two period 3 functions one with LLLR other with RRRL so we get different bounds. Trajectory matters cause if we only had RRRL then we could even get only prime period 4 and hence polynomially many oscillations.




%expressivity, standard old results, newer approach Telgarsky with dynamical systems, notions of copmlexity

%motivating example: not tent map, not periodic analysis, but LLLR gives tight bounds



\vaggos{chaotic itineraries lead to better characteristic polynomial}

\vaggos{Title: may be good to include somehow the words "chaotic itineraries" or "benefits of depth" or "depth-width tradeoffs" ...}



\vaggos{regarding high level: it's good to formulate 1 or 2 questions in the introduction that are very natural and intuitive. Examples: "Can we characterize benefits of depth in neural networks via larger families of functions?" or "Can we exploit dynamical systems constructions to obtain sharper tradeoffs for the benefits of depth?"...}

\vaggos{It's nice for our story to have a "surprise" element. This can be for example: Based on prior works, from the Sharkovsky ordering one expects fewer and fewer oscillations as the period increases and especially if it's a power of 2. However we show the opposite can happen. The crucial observation is that types of itineraries matter.}

\vaggos{When we phrase our main result, I think the community is more interested in hearing about Neural Networks tradeoffs or NN limitations or NN benefits of depth vs width. We should phrase our result as such I think i.e. the application of all the theory is that shallow nets cannot approximate certain large families of functions.}

\vaggos{Periods serve as certificate of difficulty or of necessity of depth. Here we give another type of certificate that can point to very sharp separations or important benefits of depth"...}

\vaggos{Motivation: we can still include sth about Recurrent Neural Nets since our functions come from iterated applications of the "same network" in some sense. (understanding limitations and types of functions RNNs can represent is important)}

\vaggos{Potential Remarks we should add: what about semialgebraic gates in NN? or we talk only about ReLU? I guess this should be easy since we only use the upper bound on monotone pieces. What about higher dimensions? Telgarsky and in ICLR/ICML dealt with it simply by saying about a projection on a direction that contains lots of oscillations. Can we get away with a simple remark on that?}

\vaggos{Examples: Can we have examples where lipschitz $L >> \rho$ and then ICML fails i.e. L1 error is still 0 instead of >0? Maybe like a convex steep function or sth? Also, we should add maybe pathological example with topological entropy $\pm\infty$ so to point out the weakness in Harvard paper about their notion of separation... (doubly weak since they have potentially shrinking separation)}

\vaggos{For background story: Telgarsky shows triangle (very specific function) but gets sharp $2^t$ separations. Natural question: What if we don't have a triangle exactly? Can we relax tent-map-assumption and give larger families? Telgarsky's result won't tell us anything. ICLR/ICML: Yes even if only odd periods are present we get separations but less sharp e.g. $sqrt{2}^t$ instead of $2^t$. But can we exploit further structure to get sharper bounds? Here: Yes, trajectory or chaotic itineraries are important and give almost $2^t$ separations.}

\vaggos{"We are first to find that periods don't tell the whole story and that types of itineraries matter"
Vaggelis
(e.g., since 4 appears almost last in Sharkovsky's ordering one might expect not strong separations, YET we get very sharp due to itinerary LLLR --> counterintuitive based on prior works)}

\todo{Start off by focusing on motivation of LLLR super-stable tent map cycle. Shows sub-optimality of ICLR, allows us to instantiate ICML bounds, Lipschitz, constant size (chaotic itinerary)\dots motivate extension to longer cycles with more LLLLLLLLLLLR. Increasing period can actually help when you care about making it harder to learn, unlike Sharkovsky!! Give an informal theorem statement.}

\todo{Show limitations of these methods with any curve with LRRR cycle and no 8-cycles that can be polynomially approximated. What's the difference? Number of oscillations. Ask question: is this the end of the cycle? No!}

Motivating question in ML theory: depth separation/powers of depth. Introduced by \cite{telgarsky16} to capture what deep networks can compute but shallow networks cannot. Telgarsky took gave an $L_1$ lower bound by applying iterated triangle maps to show that they create highly oscillatory functions that can't be approximated NNs that aren't sufficiently deep or exponentially wide.

Question was built upon by \cite{cnpw19} (by Sharkovsky, $L_\infty$ depth-separation bounds can be created whenever there's an non-power-of-two cycle), \cite{cnp20} (tighter lower bounds by periodicity, $L_1$ bounds under a Lipschitzness assumption), and \cite{bzl20} (lower bounds tied to topological entropy rather than periodicity).


A broader story about periodicity can be told by incorporating more dynamical systems theory from papers like \cite{mss73}. Namely, it's not just the length of the cycle of $f$ but also the itinerary of the cycle that determines how many oscillations that $f^k$ has and how difficult $f^k$ is to approximate. For instance, a LLLR 4-cycle will produce $\rho^k$ oscillations, while a ``maximal'' LRLR 4-cycle will produce $k^2$ oscillations.


To tell this story, we consider a broad class of scaling concave unimodal maps and examine how their behavior changes as the scaling parameter $r$ increases. We can divide functions in the family into two regimes based on the size of $r$: the \textit{doubling regime} and the \textit{chaos regime}.
Awareness of these regimes can give us more specific and powerful bounds than the preceding papers.
    
In the doubling regime, the largest period is a power of two that strictly increases as $r$ increases. There is always a stable cycle. All PO2 periods have the same kind of itinerary. If the maximal period is $2^q$, then the number of oscillations of $f^k$ is $O(k^q)$, the topological entropy is zero, and the VC dimension is $O(2^q)$. (We're thinking of VC dimension mostly as a general measure of function class complexity rather than in its more specific learning theory context. This is because the hypothesis class of $\{f^k: k \in \mathbb{N}\}$ is not terribly natural for ML.)


In the chaos regime, there are tons of types of cycles of different itineraries. These cycles obey Sharkovsky's theorem, but there's more than that. For instance, the ``maximal'' itinerary $L^{p-1} R$ occurs for every $p$ in increasing order of $p$, and the number of oscillations strictly increases with increasing $r$. We can then show that the number of oscillations gets increasingly close to $2^k$ as $p$ increases (irrespective of Sharkovsky). Thus, you can have exponentially many oscillations even when the stable cycle has length a power of two. The topological entropy is nonzero, and the VC dimension is infinite.

We can also produce stronger bounds than \cite{cnpw19} and \cite{cnp20} because we can show that an interval of width $0.1$ is crossed a large number of times; this gives immediate $L_\infty$ bounds without needing more assumptions.

\vaggos{"Also the aforementioned phase transition is also quantifiable via the VC dimension which is another standard way of characterizing the complexity of functions, and hence also of NN capabilities" -- sth along these lines just to include VC

(e.g., I guess there are NN bounds based on depth, width for their VC dimension, so if the functions we try to represent have infinite VC dimension then we can't approximate them basically.)}


\subsection{Related Work}

\vaggos{search most recent related works: ie Shamir recent paper, Chelsea Finn on Reinforcement Learning, MIT for graph neural nets, Loukas etc.}
\todo{Dynamical systems papers like \cite{mss73}}

\todo{Depth separation results by \cite{telgarsky16}, \cite{cnpw19}, \cite{bzl20}. 
Be clear about their limitations.}
\begin{itemize}
    \item \cite{telgarsky16} considers only a single type of function that is difficult to approximate; unclear from that paper alone whether that's a single hard instance or one of a more general class.
    \item \cite{cnpw19} extends this to a broader family of iterated functions, showing that a function with a non-power-of-two period is hard to approximate in a weaker sense than \cite{telgarsky16} (not $\L_1$ error). Based on Sharkovsky's theorem (period-3 implies any period).
    \item \cite{cnp20} builds on its predecessor by giving tighter bounds based on periods and showing limited conditions where $L_1$ bounds can be obtained. However, these bounds are still not the full story, and they give few settings where the $L_1$ bounds apply and are strong.
    \item \cite{bzl20} connects these concepts to topological entropy and proves bounds related to that. However, those bounds are also weaker than $L_1$.
\end{itemize}


\subsection{Our Results}

\begin{enumerate}
    \item We point out an incompleteness in the past theory. Namely, Sharkovsky's theorem doesn't tell the whole story, and much tighter bounds can be obtained if one assumes that certain ``itineraries'' of cycles exist.
    \item We give stronger $L_\infty$ lower bounds on approximating functions with neural networks. Unlike previous work, these are at least constant-size for large networks whenever there is any non-power-of-two cycle.
    \item We give several instances of strong $L_1$ bounds by applying the methodology of \cite{cnp20} for ``superstable'' cycles of certain itineraries on the tent map.
    \item More from a dynamical systems perspective, we note that these and the preceding results are characterized by a phase transition at between a ``doubling regime'' and a ``chaotic regime.'' We note that these regimes correspond to sharp cutoffs in the periodicity, the number of oscillations, the topological entropy, and the VC dimension of a corresponding function class. Our connections to the VC dimension are novel and demonstrate a sharp change in function complexity.
\end{enumerate}

\vaggos{Definition 1: can we include simple examples where if we didn't have assumption 1 or ass. 2 or ass. 3 then we will fail? Just to point out why we make these fairly natural assumptions. For example condition 2 seems to be there for purely technical reasons; do we mind if f is all 0 in the beginning for some interval?}
\fi

==> prelims.tex <==
% \section{Preliminaries}

% \subsection{Notation}
% For $f, g: [0,1] \to [0,1]$, let
% \[\norm[1]{f - g} = \int_{0}^1 \abs{f(x) - g(x)} dx\]
% and
% \[\norm[\infty]{f - g} = \sup_{x \in [0, 1]} \abs{f(x) - g(x)}.\]

% For $x \in [0,1]$, let $\round_t(z) = \indicator{z \geq t}$ and $\round(z) = \round_{1/2}(z)$.

% For some threshold $t \in [0,1]$, $n \in \N$, and sample $S = \{(x_i, y_i) \in [0,1] \times \bit: i \in [n]\}$, we let the \textit{classification error} of $f$ be
% \[\errcls{S,t}{f} = \frac{1}{n} \sum_{i=1}^n \indicator{y_i = \round_t(f(x))}.\]

% Let $[m] = \{1, 2, \dots, m\}$.

% \subsection{Discrete Dynamical Systems}
% We construct hard functions for neural networks to approximate and investigate the function complexity properties of a family of iterated one-dimensional maps, $f^k$, for some function $f:[0,1]\to[0,1]$.
% Borrowing from the literature on discrete dynamical systems \cite{mss73}, we limit ourselves to a certain class of mappings---which we refer to as \textit{unimodal mappings}---that yield nice dynamical systems properties.

% \begin{definition}
%     $f: [0,1]\to[0,1]$ is a \textit{unimodal mapping} if it fulfills the following characteristics:
%     \begin{enumerate}
%         \item $f$ is continuous and piece-wise differentiable on $[0,1]$.
%         \item $f(x) > 0$ for all $x \in (0,1)$ and $f(0) = f(1) = 0$.
%         \item There exists some $x_{\max}$ that uniquely maximizes $f$. $f$ is strictly increasing on the interval $[0, x_{\max})$ and decreasing on $(x_{\max},1]$.
%     \end{enumerate}
%     Periodically, we will need to make additional assumptions about $f$ for our results to hold. We say that $f$ is a \textit{concave} unimodal mapping if $f$ is also concave on $[0,1]$, and that $f$ is a \textit{symmetric} unimodal mapping if $f(x) = f(1-x)$ for all $x \in [0, 1]$.
% \end{definition}

% Two very standard unimodal mappings that are symmetric and concave are the \textit{logistic mapping} and the \textit{tent mapping} defined respectively as:
%  \[\flog{r}(x) = 4r x(1 - x)\] and  \[\ftent{r}(x) = \begin{cases}2rx & x \leq \frac{1}{2} \\ 2r(1 - x) & x \geq \frac{1}{2} \end{cases},\] 
%  Though trivial, they will serve as guiding examples for building intuition throughout the paper. They are both  parameterized by $r \in (0, 1]$ and studying their phase transitions as the parameter $r$ changes will be illuminating for understanding the chaotic itineraries.


% As shown in recent papers on the intersection of machine learning and discrete dynamical systems \cite{cnpw19, cnp20}, the periodicity of a unimodal mapping corresponds to key properties such as the number of monotone pieces of $f^k$.
% We define those concepts.

% \begin{definition}
%     $x^*$ is a \textit{fixed point} if $f(x^*) = x^*$.
%     For any $p > 1$, $x^*$ is a \textit{$p$-cyclic} point if $f^p(x^*) = x^*$ and $f^q(x^*) \neq x^*$ for all $q < p$.
%     We say that $f$ has a \textit{$p$-cycle} if there exists $p$ points $x_1, \dots, x_p$ such that $f(x_i) = x_{i+1}$ for $i \in [p-1]$ and $f(x_p) = x_1$.
% \end{definition}

% Sharkovsky's Theorem proves a clear relationship between the various periodicities of some mapping $f$. 
% It provides an ordering on the natural numbers such that if $p$ precedes $q$ in the ordering, then the existence of a $q$-cycle implies the existence of a $p$-cycle

% \begin{theorem}
%     \todo{Sharkovksy's goes here!}
%     \vaggos{I will write Sharkovsky and explain in intro.}
% \end{theorem}

% Past results \cite{cnpw19, cnp20} apply Sharkovsky's Theorem to show that the existence of a certain cycle in a mapping $f$ implies that $f^k$ will be difficult to approximate.
% Our key results are to show that more information than just the length of the cycle is relevant to determining the complexity of $f$ (and hence, the hardness of approximation). 
% We define a notion of \textit{cycle itinerary}, which we rely on heavily when proving our bounds.

% \clayton{Let's call these ``patterns'' instead and write them as permutations rather than L/Rs. e.g. $(1,2,3,4,5)$ instead of $L^4R$.}

% \begin{definition}
%     Consider some $p$-cycle $x_1, \dots, x_p$. 
%     The \textit{itinerary} of this cycle is some string of length $a \in \{L, C, R\}^p$, where 
%     \[a_i := \begin{cases}
%         L & x_i < x_{\max} \\
%         C & x_i = x_{\max} \\
%         R & x_i > x_{\max}.
%     \end{cases}\]
% \end{definition}

% \begin{remark}
%     This is slightly different notation than the notion used in Table~1 of \cite{mss73}, which focuses on only the itineraries of cycles that contain a $C$ and represents a $p$-cycle with a string of length $p-1$.
% \end{remark}



% The story of cycles in discrete dynamical systems can be shown to be more complex than just what is indicated in Sharkovsky's theorem.
% The application of Sharkovsky's Theorem in \cite{cnpw19, cnp20} non-power-of-two cycles are in $f$ are key to showing that $f^k$ is hard to approximate by neural networks.
% In this work, we illustrate that this is only a small piece of the puzzle and that the trajectory of the cycles matter too.
% Certain power-of-two cycles are more indicative of $f^k$ being hard to approximate than $f$; for instance, the existence of an $L^3R$ 4-cycle gives more powerful approximation bounds than the existence of a 3-cycle.

% Since cycles of the form $L^{p-1}R$ and $L^{p-2}CR$ will be frequently considered in this work, we give them a name.

% \begin{definition}
%     $f$ has an \textit{increasing $p$-cycle} if it has a $p$-cycle with $x_1 < x_2 < \dots < x_p$.
% \end{definition}
% If $f$ is unimodal, we can show that a cycle is an increasing $p$-cycle if and only if its itinerary is $L^{p-1}R$, $L^{p-2}CR$, or $L^{p-2}R^2$. \todo{prove this/refer to appendix}





% \begin{itemize}
%     \item Cycle itineraries and order from \cite{mss73}. Note that it's first a bunch of PO2 cycles (doubling regime) and then a bunch of others (chaotic regime). First cycles appear in order of Sharkovsky's thoerem. Cycles never go away as scaling parameter increases. Final stable cycle of period $p$ is $L^{p-1}R$. (Lemma 3 of OC, ideally with less notation involved)
% \end{itemize}

% \clayton{Idea: one of the things we'll have trouble with here is that the proofs are more cumbersome than the ideas. For instance, the MSS73 chart implies on inspection that a cycle of the form $RL^{p-1}$ implies the existence of one of the form $RL^{p-2}$. But it's somewhat cumbersome to prove. 

% Maybe we can define a list of heuristic rules in a section that hold and motivate them, which can encapsulate concepts that are a pain to prove but easy to observe via MSS or visuals. When describing the proof we can refer back to these kinds of heuristics to make it easier to understand, while still including all of the rigor in other areas.}

% \subsection{Number and Size of Oscillations}
% Our plan is to use properties of the $p$-cycles of mappings $f$ in order to derive properties of $f^k$ and to establish the difficulty of approximating $f^k$ with neural networks. 
% To measure the function complexity of $f^k$, we primarily rely on the number of times $f^k$ oscillates. To quantify the tendency of $f^k$ to oscillate, we develop ways to accurately count the number of monotone pieces $f^k$ has. 

% %\cite{telgarsky16, cnpw19, cnp20, bzl20} show that counting the number of oscillations of $f^k$ is key to proving that it cannot be approximated by any polynomial-size shallow neural network.

% We employ two notions of oscillation counts.
% The first is a weak notion, which counts every interval on which $f$ is either increasing or decreasing, regardless of how large this interval is.

% \begin{definition}\label{def:osc}
%     Let $f: [0, 1] \to [0, 1]$. We let $\oscm(f)$ represent the \emph{number of monotone pieces} of $f$. That is, it is the minimum $m$ such that there exists $x_0 = 0 < x_1 < \dots < x_{m-1} < x_m = 1$ such that $f$ is monotone on $[x_j, x_{j+1}]$ for all $j\in \{0\}\cup[m-1]$.
% \end{definition}

% The second instead counts the number of times a certain interval of size $b-a$ is crossed:

% \begin{definition}\label{def:cross}
%     Let $f: [0, 1] \to [0, 1]$ and $[a, b] \in [0,1]$. We let $\osci{a,b}(f)$ represent the \emph{number of crossings} of $f$ on the interval $[a,b]$. 
%     That is, it is the maximum $c$ such that there exist \[0 \leq x_1 < x'_1 \leq x_2 < x'_2 \leq \dots \leq x_c < x_c' \leq 1\] such that for all $j \in [c]$, $f([x_j, x'_j]) \subset [a,b]$ and either $f(x_j) = a$ and $f(x'_j) = b$ or vice versa.
% \end{definition}

%\subsection{Neural Networks}

%\todo{brief definition of ReLU neural network of some width and depth}

%\vaggos{We should add a small paragraph to compare L1, classification, $L_\infty$ and constant-gap-$L_\infty$ just to clarify the different regimes. It's nice here to include a "historical" review of how recent papers (Telgarsky's, ours, Harvard, others, current) tried to obtain bounds for these different problems...}



==> supp_lb.tex <==
\section{Additional Proofs for Section~\ref{sec:lb}}

\subsection{Proof of Lemma~\ref{lemma:increasing-constant-osc}}\label{assec:inc-constant-osc-proof}
We restate and prove the lemma. This is the main technical lemma that we use to get the sharper depth-width tradeoffs and the improved notion of \textit{constant} approximation.

\lemmaincreasingconstantosc*
%\label{lem:main}
\begin{proof}
We first lower-bound the total number of oscillations that will appear an increasing $p$-cycle is present. 
Later, we show that the size of the oscillations is large as well.

Because we have an increasing cycle of itinerary $12\dots p$, we assume (wlog) that the cycle is $(x_1, \dots, x_p)$ with $x_1 < x_2 < \dots < x_p$. 
Define intervals $I_j \vcentcolon= [x_j, x_{j+1}]$ for $j \in \{1, \dots, p-1\}$. Because $f$ is continuous, we conclude that $I_{j+1} \subset f(I_{j})$ for all $j < p$ and $I_{j} \subset f(I_{p-1})$ for all $j$.
Figure~\ref{fig:inc-intervals} visualizes these relationships.

\begin{figure}
    \centering
    \input{fig/fig-inc-intervals}
    \caption{Visualizes the intervals $I_1,\dots, I_{p-1}$ defined in the proof of Lemma~\ref{lemma:increasing-constant-osc} and which intervals $f$ maps to one another when $f$ has an increasing $p$-cycle.}
    \label{fig:inc-intervals}
\end{figure}

Using the methods of \cite{cnpw19}, we define $y^{(k)} \in \N^{p-1}$ such that $y^{(k)}_j$ is a lower bound on the number of times $f^k$ passes through interval $I_j$, or \[\osci{x_{j}, x_{j+1}}(f^k) \geq y^{(k)}_j.\] We can then encode the interval relationships above with $y^{(k+1)} = A_p y^{(k)}$ where $y^{({0})}$ is a vector of all ones and and $A_p \in \bit^{(p-1) \times (p-1)}$ with $(A_p)_{i, j} = \indicator{j = p-1 \text{ or } i = j + 1}$. We get the following adjacency matrix for the intervals, capturing the mapping relationships (under $f$) between them:
\[A_p = 
\begin{bmatrix}
    0 & 0 & 0 & \cdots & 0 & 1 \\
    1 & 0 & 0 & \cdots & 0 & 1 \\
    0 & 1 & 0 & \cdots & 0 & 1 \\
    0 & 0 & 1 & \cdots & 0 & 1 \\
    \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
    0 & 0 & 0 & \cdots & 1 & 1
\end{bmatrix}.\]

We find the characteristic polynomial of $A_p$ and lower-bound $y^{(k+1)}$ with the spectral radius of $A_p$. 
We show by induction on $p \geq 3$ that
\[\det(A_p - \lambda I) = (-1)^{p-1} \paren{\lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i}.\]

For the base case $p = 3$, we have:
\begin{align*}
    \det(A_3 - \lambda I)
    &= \begin{vmatrix}
        -\lambda & 1 \\
        1 & 1 -\lambda
    \end{vmatrix}
    = \lambda^2 - \lambda - 1,
\end{align*}
which satisfies the desired form.

Now, we show the inductive step by expanding the determinant of $A_p - \lambda I$.

{\small
\begin{align*}
    \det(A_p - \lambda I)
    &= 
    \begin{vmatrix}
        -\lambda & 0 & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & 0 & \cdots & 0 & 1 \\
        0 & 1 & -\lambda & \cdots & 0 & 1 \\
        0 & 0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix}
    = -\lambda 
    \begin{vmatrix}
        -\lambda & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & \cdots & 0 & 1 \\
        0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix} - 
    \begin{vmatrix}
        0 & 0 & \cdots & 0 & 1 \\
        1 & -\lambda & \cdots & 0 & 1 \\
        0 & 1 & \cdots & 0 & 1 \\
        \vdots & \vdots & \ddots & \vdots & \vdots \\
        0 & 0 & \cdots & -\lambda & 1 \\
        0 & 0 & \cdots & 1 & 1 - \lambda
    \end{vmatrix}.
\end{align*}}

The left determinant exactly equals $\det(A_{p-1} - \lambda I)$, which we can expand using the inductive hypothesis.
The second equals $(-1)^{p-2}$, because $p-2$ row swaps (which are elementary row operations) can be used to move the first row to the bottom and make the matrix upper-triangular with diagonals of one. 
We conclude the inductive step below.

\begin{align*}
        \det(A_p - \lambda I)
        &= -\lambda \det(A_{p-1} - \lambda I) - (-1)^{p-2} \\ 
    &= -\lambda (-1)^{p-2} \left(\lambda^{p-2} - \sum_{i=0}^{p-3} \lambda^i \right) + (-1)^{p-1}
    = (-1)^{p-1} \left(\lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i\right).
\end{align*}

We find the eigenvalues of $A_p$ by finding the roots of the polynomial
\[P(x) = \lambda^{p-1} - \sum_{i=0}^{p-2} \lambda^i = 0.\] 
Observe that there must be a root greater than $1$ because $P(1) = 2 - p < 0$ and $P(2) = 1 > 0$. Equivalently, if $\lambda \neq 1$,
\[P(x) = \lambda^{p-1} - \frac{1 - \lambda^{p-1}}{1 - \lambda} = \frac{\lambda^p - 2\lambda^{p-1} + 1}{\lambda - 1} =  0.\]

Hence, finding the largest root of $P$ is equivalent to finding the largest root of $\lambda^p - 2\lambda^{p-1} + 1$, which is $\rhoinc{p}$ by definition.


This implies that the spectral radius of $A_p$, sp$(A_p)=\rhoinc{p}>1$, and hence, we also have sp$(A_p^k)=$ sp$(A_p)^k=\rhoinc{p}^k$. Since all the elements in $A_p$ and in $A_p^k$ are non-negative, then the infinity norm of $A_p^k$ is by definition the maximum among its row sums. Since the last column of $A_p$ is the all 1's vector, the largest row sum in $A_p^k$ appears at its last row:

\[
||A_p^k||_{\infty} = \sum_{j=1}^{p-1}(A_{p}^k)_{p-1,j}
\]



We can now use the fact that the infinity norm of a matrix is larger than its spectral norm:
\[
||A_p^k||_{\infty} \ge  \rhoinc{p}^k
\]
%Therefore, there exists at least one interval $I_{j^*}$ which is crossed at least $\rho^k$ times by $f^k$, so $\osci{x_{j^*}, x_{j^*+1}}(f^k) \geq \rho^k$.
We conclude that there exists at least one interval $I_{j^*}$ (e.g., the interval $I_{p-1}$) which is crossed at least $\rhoinc{p}^k$ times by $f^k$, so $\osci{x_{j^*}, x_{j^*+1}}(f^k) \geq \rhoinc{p}^k$.

Thus, for some $a',b'$ we get $\osci{a', b'}(f^k) \geq \rhoinc{p}^k$. But can we find $a',b'$ with large difference $b'-a'$?

Now, we show that the intervals traversed are sufficiently large, in order to lower-bound $\osci{a,b}(f^k)$ with $b-a \geq \frac{1}{18}$.
By Lemma~\ref{lemma:interval-inc-cycle}, there exists some $j$ with $x_{j+1} - x_{j} \geq \frac{1}{18}$.
It suffices to show that $f^k$ traverses the interval $I_j$ sufficiently many times.

From earlier in the proof, there exists some $j^*$ such that $f$ crosses $I_{j^*}$ at least $N\vcentcolon=\rhoinc{p}^{k}$ times. 
We conclude by showing that every other interval is traversed at least half as often as this most popular interval, which suggests that $\osci{x_{j}, x_{j+1}}(f) \geq \frac{N}{2}$.
    

    
For $A \in \mathbb{R}^{(p-1)\times (p-1)}$ as defined earlier in the section and for $y^{(k)} \vcentcolon= A^{k} \vec{1}$, we argue inductively that the elements of $y^{(k)}$ are non-decreasing and that $y^{(k)}_{p-1} \leq 2 y^{(k)}_1$. For the base case, this is trivially true for $k = 0$.

Suppose it holds for $k$.
    By construction, we have $y^{(k+1)}_1 = y^{(k)}_{p-1}$ and $y^{(k+1)}_j = y^{(k)}_{j-1} + y^{(k)}_{p-1}$ for all $j > 1$.
    By the inductive hypotheses,
    \[y^{(k+1)}_1 \leq y^{(k+1)}_2 \leq \dots \leq y^{(k+1)}_{p-1} \leq 2y^{(k+1)}_1.\]
    
Therefore, $f^k$ crosses interval $I_{j}$ at least $\frac{N}{2}$ times, and $I_j$ has width at least $\frac{1}{18}$. The claim immediately follows.
\end{proof}
    
\begin{lemma}\label{lemma:interval-inc-cycle}
    For some $p \geq 3$, consider a symmetric concave unimodal function $f$ with an increasing $p$-cycle of $x_1 < \dots < x_p$. Then, there exists $j \in [p-1]$ such that $x_{j+1} - x_j \geq \frac{1}{18}$.
\end{lemma}

\begin{proof}
By the continuity of $f$, note that $[x_1, x_p] \subset f^3([x_{p-3}, x_{p-2}])$. 
There then exists some $y_1 \in [x_{p-3}, x_{p-2}]$ such that $f^3(y_1) = y_1$, $y_2\vcentcolon= f(y_1) \in [x_{p-2}, x_{p-1}]$, and $y_3\vcentcolon= f(y_2) \in [x_{p-1}, x_p]$.
Thus, if $f$ has a maximal $p$-cycle, then $f$ also has a 3-cycle corresponding to $x_{p-3} < y_1 < y_2 < y_3 < x_p$.

We now show that $y_3 - y_1$ must be sufficiently large by concavity.
For $f$ to be concave, the following inequality must hold:
\begin{align*}
    \frac{f(y_1) - f(0)}{y_1 - 0} \geq \frac{f(y_2) - f(y_1)}{y_2 - y_1} > 0  > \frac{f(y_3) - f(y_2)}{y_3 - y_2} \geq \frac{f(1) - f(y_3)}{1 - y_3},
\end{align*}
or equivalently,
 \[\frac{y_2}{y_1} \geq \frac{y_3 - y_2}{y_2 - y_1} > 0 > -\frac{y_3 - x_1}{y_3 - y_2} \geq -\frac{y_1}{1 - y_3}.\]
 
In addition, note that $y_1 < \frac{1}{2}$ and $y_3 > \frac{1}{2}$. 
If the former were false, then $f(y_2) \leq f(y_1)$ (by unimodality), which contradicts $y_3 > y_2$. If the latter were false, then $f(y_3) > f(y_2)$, which contradicts $y_1 < y_3$.

We consider two cases and show that either way, the interval must have width at least $\frac{1}{6}$.
\begin{itemize}
    \item If $y_2 - y_1 \leq \frac{2}{5}(y_3 - y_1)$, then $\frac{y_3 - y_2}{y_2 - y_1} \geq \frac{3}{2},$
    which mandates that $y_1 \leq \frac{2y_2}{3}$ to ensure concavity. Thus,
    \[y_3 - y_1 \geq y_3 - \frac{2y_2}{3} \geq \frac{y_3}{3} \geq \frac{1}{6}.\]
    \item If $y_2 - y_1 \geq \frac{2}{5}(y_3 - y_1)$, then $\frac{y_3 - y_1}{y_3 - y_2} \geq \frac{5}{3},$ and thus $y_1 \geq \frac{5}{3}(1 - y_3)$ and $y_3 \geq 1 - \frac{3y_1}{5}$. Then,
    \[y_3 - y_1 \geq 1 - \frac{3y_1}{5} - y_1 = 1 - \frac{8y_1}{5} \geq \frac{1}{5}.\]
\end{itemize}

Thus, we must have \[\max\{x_{p-2} - x_{p-3}, x_{p-2} - x_{p-1}, x_p - x_{p-1}\} \geq \frac{1}{18}.\qedhere\]

\end{proof}

\subsection{Proof of Fact~\ref{fact:root-lb}}\label{assec:fact}
\factrootlb*
\begin{proof}

Let $P_{\mathrm{inc}, p}(\lambda) = \lambda^{p} - 2\lambda^{p-1} + 1$.

First, observe that $\rhoinc{p} < 2$, because $P_{\mathrm{inc}, p}(\lambda) > 0$ whenever $\lambda \geq 2$. 
We lower-bound $\rhoinc{p}$ by finding some $\lambda$ for each $p$ such that $P_{\mathrm{inc}, p}(\lambda) \leq 0$ or equivalently $\lambda^{p-1}(2 - \lambda) \geq 1$ for all $p\geq3$, which bounds $\rhoinc{p}$ by the Intermediate Value Theorem. 

Consider $\lambda = 2 - \frac{4}{2^p}$. Then,
\begin{align*}
    \lambda^{p-1}(2 - \lambda)
    &= \paren{2 - \frac{4}{2^p}}^{p-1} \cdot \frac{4}{2^p}
    = 2 \paren{1 - \frac{2}{2^p}}^{p-1} \\
    &\geq 2 \paren{1 - \frac{2(p-1)}{2^p}}
    = 2 - 2 \cdot \frac{p-1}{2^{p-1}} \\
    &\geq 2 - 2 \cdot \frac{1}{2} = 1.\qedhere
\end{align*}
\end{proof}

\subsection{Previous Results about Hardness of Approximating Oscillatory Functions}

We rely on prior results from~\cite{cnpw19, cnp20} to show that an iterated function $f^k$ is inapproximable by neural networks.
These results hold if $f^k$ has sufficiently many crossings of some interval.
We apply these results later with improved bounds on both the number and the size of crossings.

\cite{cnpw19} show that the classification error of $f^k$ can be bounded if there are enough oscillations.

\begin{theorem}[\citep{cnpw19}, Section 4]\label{thm:general-lb-cls}
    Consider any continuous $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a, b}(f) = \Omega(\rho^t)$ and suppose $u \leq \frac{1}{8}\rho^{k/\ell}$.
    Then, for $t = \frac{a+b}{2}$, there exists $S$ with $\abs{S} =  \frac{1}{2} \floor{\rho^k}$ samples such that 
    \[\errcls{S,t}{f^k, g}  \geq \frac{1}{2} - \frac{(2u)^\ell}{n}.\]
\end{theorem}

We adapt that claim to lower-bound the $L_\infty$ approximation of $f^k$ by $g$.

\begin{corollary}\label{cor:general-lb-linf}
    Consider any continuous $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a, b}(f) = \Omega(\rho^t)$ and suppose $u \leq \frac{1}{8}\rho^{k/\ell}$.
    Then, 
    \[\norm[\infty]{f^k - g} \geq \frac{b-a}{2}.\]
\end{corollary}
\begin{proof}
    By Theorem~\ref{thm:general-lb-cls}, there exists some $x \in [0,1]$ such that (wlog) $f^k(x) \leq a$ and $g(x) \geq \frac{a + b}{2}$.
    The conclusion for the $L_\infty$ error is immediate by definition.
\end{proof}

\cite{cnp20} give a lower-bound on the ability of a neural network $g$ to $L_1$-approximate $f^k$, provided a correspondence between the Lipschitz constant of $f$ and the rate of oscillations $\rho$.

\begin{theorem}[\cite{cnp20} Theorem 3.2]\label{thm:general-lb-l1}
    Consider any $L$-Lipschitz $f: [0,1] \to [0,1]$ and any $g \in \mathcal{N}(u,\ell)$.
    Suppose there exists $a < b$ such that $\osci{a,b}(f) = \Omega(\rho^t)$. If $L \leq \rho$ and $u \leq \frac{1}{16} \rho^{k/\ell}$, then 
    \[\norm[1]{f^k - g} = \Omega((b-a)^2).\]
\end{theorem}

The Lipschitzness assumption is extremely strict, especially because they show in their Lemma~3.1 that $L \geq \rho$ whenever $f$ has a period of odd length.

\subsection{Proof of Corollary~\ref{cor:main-l1}}\label{assec:cor-main-proof}
\cormainl*
\begin{proof}
    This theorem follows from Theorem~\ref{thm:main-l1} and Lemma~\ref{lemma:increasing-constant-osc}.
    Because $\ftent{\rho_p/2}$ is $\rho_p$-Lipschitz, it remains only to prove that there exists an increasing $p$-cycle.
    We show that 
    \[\frac{1}{2}, f\paren{\frac12},\dots, f^{p-1}\paren{\frac12}\]
    is such a cycle.
    
    By definition of the tent map, $f(\frac12) = \frac{\rhoinc{p}}2$ and $f^2(\frac12) = \rhoinc{p} (1 - \frac{\rhoinc{p}}{2})$.
    If we assume for now that $f^j(\frac12) \leq \frac12$ for all $j \in \{2, \dots, p-1\}$,
    then
    \[f^p\paren{\frac12} = \rhoinc{p}^{p-1}\paren{1 - \frac{\rhoinc{p}}2} = -\frac{1}{2}\paren{\rhoinc{p}^p - 2\rhoinc{p}^{p-1} + 1} + \frac{1}{2} = 0 + \frac{1}{2}.\]
    
    Because $f^p(\frac12) = \frac12$ and we assumed that $f^{j+1}(\frac12) = \rhoinc{p} f^{j}(\frac12)$ for $j \geq 2$ and $\rho > 1$, it must be the case that $f^j(\frac12) \leq \frac12$ for all $j \in \{2, \dots, p-1\}$.
    
    Lemma~\ref{lemma:increasing-constant-osc} thus implies that $f^k$ has $\Omega(\rhoinc{p}^k)$ crossings, which enables us to complete the proof by invoking Theorem~\ref{thm:main-l1}, since the Lipschitzness condition is met.
    % To apply them, it remains only to prove that the Lipschitz constant of $\ftent{r}$ is $\rho$, or equivalently, $r = \frac{\rho}{2}$.
    % Given $\ftent{r}^p(\frac12) = \frac12$, we show that $\frac12$ must be contained in an increasing $p$-cycle.
    % Suppose not.
    % There exists some increasing $p$-cycle $x_1 < \dots < x_p$ and we assume that it does not contain $\frac12$.
    % It must be the case that $x_{p-2} < \frac12$; assuming otherwise would cause $f(x_{p-2}) \geq f(x_{p-1})$, a contradiction.
    % Because $\frac12$ maximizes $f$, $x_p \leq f(\frac12)$.
    % Since $f$ decreases on $[\frac12, 1]$, it follows that $f^2(\frac12) \leq x_1$.
    % $f$ increasing on $[0, \frac12]$ implies that $f^{j+1}(\frac12) \leq x_{j}$ for all $j \in [p-1]$.
    % Therefore, $f^{j}(\frac12) \neq \frac12$ for all $j \in [p]$ and $f^2(\frac12) <  \dots < f^{p}(\frac12) = \frac12$.
    % We conclude that $\frac12$ is contained in an increasing $p$-cycle, which has a $123\dots p$ itinerary; call that cycle $x_1', \dots, x_{p-1}'= \frac12, x_p'$
    % % For $\ftent{r}$ to have a super-stable $p$-cycle, it must pass through $\frac{1}{2}$. Because $\ftent{r}$ only has zero-slope at $x = \frac{1}{2}$, a fixed point $x_1$ for $\ftent{p}$ will only be super-stable if $f^j(x_1) = \frac{1}{2}$ for some $j \in [p]$. (Otherwise $\frac{d}{dx} f^j(x_1) \neq 0$, and $x_1$ cannot be part of a super-stable cycle.)
    % % Therefore, there must exist a cycle of the form
    % % \[x_1 < \dots < x_{p-2} < x_{p-1} = \frac{1}{2} < x_{p} = r,\]
    % % which signals an $12\dots p$ itinerary.
    % % Note that $x_{p-1} = \frac{1}{2}$ because any assignment would contradict the cycle being increasing.
    % % If $x_p = \frac{1}{2}$, then $x_1 = f(x_p) = r > x_p > x_1$.
    % % If $x_j = \frac{1}{2}$ for $j < p-1$, then $x_p = f(x_{p-1}) < f(x_{j}) = x_{j+1} < x_p$, both contradictions.
    % We apply the definition of the tent map to note that $x_{j}' = 2rx_{j-1}'$ for $j \in \{2, \dots, p\}$ and $x_1' = 2r(1 - x_p')$.
    % Thus, 
    % \[\frac{1}{2} = (2r)^{p-2} x_1' = (2r)^{p-1}(1 - x_p') = (2r)^{p-1}(1 - r).\]
    % Equivalently, 
    % \[(2r)^p - 2 (2r)^{1-p} + 1 = 0,\]
    % which has $\rho = 2r$ as its largest root.
    % Hence, $\ftent{r}$ has Lipschitz constant $\rho$ and we can apply Theorem~\ref{thm:main-l1}.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:odd-constant-osc}}\label{assec:lemma-odd-proof}

\lemmaoddconstantosc*

\begin{proof}
    By Theorems~2.94 and 3.11.1 of~\cite{alseda2000}, there exists a $p$-cycle of the form \[x_p < x_{p-2} < \dots < x_3 < x_1 < x_2 < x_4 < \dots < x_{p-1},\]
    which is known as a \textit{Stefan cycle}.
    The analysis of Section~3.2 of~\cite{cnp20} shows that $\osci{[x_1, x_2]}(f^{k}) \geq \rhoodd{p}^{k}$.
    Their exploitation of the relationships between intervals is visualized in Figure~\ref{fig:stefan-intervals}.
    By the continuity of $f$, applying $f$ an additional $p-1$ times gives $\osci{[x_p, x_1]}(f^{k+p-1}) \geq \rhoodd{p}^{k}$.
    Because $[x_{p-2}, x_1] \subset [x_p, x_1]$, applying $f$ one more time gives $\osci{[x_2, x_{p-1}]}(f^{k+p}) \geq \rhoodd{p}^k$.
    
    
    \begin{figure}
        \centering
        \input{fig/fig-stefan-intervals}
        \caption{Gives an example of a Stefan $p$-cycle (which is relied upon in Lemma~\ref{lemma:odd-constant-osc} and demonstrates the interval relationships). Analogous to Figure~\ref{fig:inc-intervals}.}
        \label{fig:stefan-intervals}
    \end{figure}
    
    Hence, by redefining $k$, we have 
    \[\max\{ \osci{[x_1, x_2]}(f^{k}), \osci{[x_2, x_{p-1}]}(f^{k}), \osci{[x_p, x_1]}(f^{k})\} \geq \rhoodd{p}^{k-p}.\]
    
    Since $[x_p, x_{p-1}]$ is the disjoint union of $[x_1, x_2]$, $[x_2, x_{p-1}]$, and $[x_p, x_1]$, there exists $[a, b] \subset [x_p, x_{p-1}]$ with $b- a \geq \frac{1}{3}(x_{p-1} - x_p)$ such that $\osci{[a,b]}(f^{k}) \geq \\rhoodd{p}^{k-p}$.
    
    The problem reduces to placing a lower bound on $x_{p-1} - x_p$.
    To do so, we derive contradictions on the concavity and symmetry of $f$. 
    Let $r = f(\frac12) \in (x_p, 1)$ be the the largest outcome of $f$, and
    let \[a= \sup_{x, x' \in [1-r, r]} \abs{\frac{f(x) - f(x')}{x - x'}}\] be the maximum absolute slope of $f$ on $[1-r,r]$. $a$ must be finite by the concavity and continuity of $f$, and if $f$ is differentiable, $a = f'(1-r) = -f'(r)$.
    Thus, $f$ is $a$-Lipschitz on that interval.
    
    Because $f([x_p, x_{p-1}]) \subseteq [x_p, r] \subset [1-r, r]$, it follows that $\abs{f^2(x) - f^2(x')} \leq a^2 \abs{x - x'}$.
    Thus, $x_2 - x_p \leq a^2(x_{p-2} - x_{p})$ and $x_2 - x_p \leq x_4 - x_p \leq a^2(x_2 - x_{p-2})$.
    Averaging the two together, we have $x_2 - x_p \leq \frac{a^2}{2}(x_2 - x_{p})$, which means $a \geq \sqrt{2}$.
    
    To satisfy concavity, the following must be true:
    \[\frac{f(1-r) - f(0)}{1-r - 0} = \frac{f(r)}{1-r} \geq a \geq \sqrt{2}.\]
    
    We rearrange the inequality and apply properties of monotonicity to lower-bound $r$ away from $\frac12$:
    \[r 
    \geq 1 - \frac{f(r)}{\sqrt{2}}  
    \geq 1 - \frac{f(x_{p-1})}{\sqrt{2}}
    = 1 - \frac{x_p}{\sqrt{2}}
    > 1 - \frac1{2\sqrt2}.\]
    
    It also must be the case for any $x \in [\frac12, 1]$, that:
    \[\abs{\frac{f(x) - f\paren{\frac12}}{x - \frac12}} \leq 2.\]
    Otherwise, the concavity of $f$ would force $f(\frac12) > 1$.
    
    We finally assemble the pieces to lower-bound the gap between $x_{p-1}$ and $x_p$:
    \begin{align*}
        x_{p-1} - x_p
        &\geq x_{p-1} - \frac12 
        \geq -\frac{1}{2} \paren{f(x_{p-1}) - f\paren{\frac12}}
        = \frac{r}{2} - \frac{x_p}{2} \\
        &> \frac{1}{2} - \frac1{4\sqrt{2}} - \frac14 
        = \frac14 - \frac1{4\sqrt{2}}
        > 0.07.\qedhere
    \end{align*}
    
    
    
    % Under the assumption, it must be the case that $r \leq 0.54$. If not, then 
    % \[\frac{f(x_p) - f(\frac12)}{x_p - \frac12} > \frac{0.04}{0.02} = 2.\]
    % By concavity, this would imply that $f(\frac12) > 1$, which is a contradiction. Hence, we continue with $r \leq 0.54$.
    
    % By the monotonicity of $f$ on $[\frac12, 1]$ and the fact that $r > x_{p-1}$, it follows that $f(r) < x_{p} < \frac12$.
    
    % By symmetry and unimodality of $f$, $1-x_{p-1} \leq x_p$, since $f(x_{p-1}) < f(x_p)$.
    % The concavity of $f$ implies the following:
    % \begin{align*}
    %     -\frac{x_p}{1 - x_{p-1}} 
    %     &= \frac{f(1) - f(x_{p-1})}{1 - x_{p-1}}
    %     \leq \sup_{x, x' \in [1/2, x_{p-1}]} \frac{f(x) - f(x')}{x - x'} \\
    %     &= \sup_{x, x' \in [1-x_{p-1}, x_{p-1}]} -\abs{\frac{f(x) - f(x')}{x - x'}} 
    %     \leq \sup_{x, x' \in [x_p, x_{p-1}]} -\abs{\frac{f(x) - f(x')}{x - x'}}\\
    %     &= -a \leq -\sqrt{2}.
    % \end{align*}
    
    % Thus, $\abs{f'(x)}$ is maximized on the interval $[x_p, x_{p-1}]$ at $x_{p-1}$.
    % By concavity, it must be the case that $f'(x)\leq -\sqrt{2}$ whenever $x \in [x_{p-1}, 1]$ and thus, 
    % \[\frac{f(1) - f(x_{p-1})}{1 - x_{p-1}} = -\frac{x_p}{1 - x_{p-1}} \leq -\sqrt{2}.\]
    % Equivalently,
    % \[x_{p-1} \geq 1 - \frac{x_p}{\sqrt{2}}.\]
    
    % We conclude with the lower bound on $x_{p-1} - x_p$. Note that $x_p < \frac{1}{2}$ by symmetry and the fact that $f(x_p) \leq f(x_{p-2})$.
    % \begin{align*}
    %     x_{p-1} - x_p
    %     &\geq 1 - \frac{x_p}{\sqrt{2}} - x_p 
    %     = 1 - \frac{2 + \sqrt{2}}{2} x_p \\
    %     &\geq 1 - \frac{2 + \sqrt{2}}{4} > 0.12.\qedhere
    % \end{align*}
\end{proof}

\subsection{Necessity of Symmetry and Concavity Assumptions in Theorems~\ref{thm:main-linf} and \ref{thm:main-l1}}\label{assec:sym-conc}

We demonstrate the weakness of the bounds promised by \cite{cnpw19, cnp20, bzl20} and argue that our assumptions of symmetry and concavity are necessary in order to avoid such non-vacuous bounds.
To do so, we exhibit two families of functions in Propositions~\ref{prop:need-symmetry} and ~\ref{prop:need-concavity} which contain functions with increasing $p$-cycles for every $p$ that produce large numbers of oscillations, yet are trivial to approximate because their oscillations can be made arbitrarily small.
The functions considered in both cases are unimodal and lack symmetry and concavity respectively.

These expose a fundamental shortcoming of other approaches to the hardness of neural network approximation in the aforementioned works because they all rely on showing that for every mapping $f$ meeting some condition (e.g. odd period, positive topological entropy), there exists some $[a,b] \in [0,1]$ where $\osci{a,b}$ is exponentially large, and hence no poly-size shallow neural network $g$ can obtain $L_{\infty}(f^k, g) \leq P(b-a)$ for some polynomial $P$.
However, because $[a,b]$ depends on $f$, their difference can potentially be arbitrarily small. 
The propositions show that this concern is significant and that $[a,b]$ indeed becomes arbitrarily narrow for simple 3-periodic functions. 
While \cite{cnpw19} avoid addressing this issue head-on by focusing on classification error over $L_\infty $ error, their classification lower-bounds rely on misclassification of points whose actual distance can be shrinking (see for example Figure~\ref{fig:asymmetric}).
%microscopically small degrees of inapproximation on a small number of points.


The implications of these propositions contrast with the more robust hardness results we present in Theorems~\ref{thm:main-linf}, \ref{thm:main-l1}, \ref{thm:odd-linf}, and \ref{thm:odd-l1}, which leverage unimodality, symmetry, and concavity to ensure that the accuracy of approximation can be no better than some constant (independent on $f,p$) when the neural network $g$ is too small.
% In order for the accuracy of the neural network approximation to be lower-bounded by a constant value, Theorems~\ref{thm:main-linf} and \ref{thm:main-l1} assume that the unimodal function $f$ is additionally concave and symmetric. 
We show here that those assumptions are necessary by exhibiting functions that satisfy all but one, and become easy to $L_\infty$-approximate with small depth-2 ReLU networks.

% \todo{Show that ICML and ICLR fail}

% \todo{Note that prior analysis doesn't give us anything about setting for why large L fails; we show why that's the case}

% \todo{mention that oscillation LBs for increasing cycle still give large number of oscillations even if not unimodal (just small oscillations)}

% \todo{Or, just directly attack previous constructions... Show that oscillation size becomes arbitrarily small}

% \vaggos{forward pointer in section where we dwell on cosntant error rates.}


\begin{proposition}\label{prop:need-symmetry}
For $p \geq 3$ and for sufficiently small $\eps > 0$, there exists a concave unimodal mapping $f$ with a chaotic $p$-cycle such that for any $k$, there exists $g \in \mathcal{N}(3,2)$ with
\[L_\infty(f^k, g) \leq \eps.\]
\end{proposition}

\begin{proof}
    For all $j \in [p]$, let $x_j = 1 - \frac{p-j+1}{p} \eps$.
    Define $f$ to be a piecewise-linear function with $p+1$ pieces chosen with boundaries that satisfy 
    \[f(0) = 0, f(x_1) = x_2, f(x_2) = x_3, \dots, f(x_{p-1}) = x_p, f(x_p) = x_1, f(1) = 0.\]
    
    We visualize $f$ for $p=3$ in Figure~\ref{fig:asymmetric}. $f$ is unimodal because it increases on $[0, x_{p-1}]$ and decreases on $[x_{p-1}, 1]$.
    It is concave because $f'(x)$ does not increase as $x$ grows, since 
    \[f'(x) = \begin{cases}
        \frac{1-\frac{p-1}{p}\eps}{1 - \eps} > 1 & x \in [0, x_1) \\
        1 & x \in (x_1, x_{p-1}) \\
        - p + 1 & x \in (x_{p-1}, x_p) \\
        - \frac{1 - \eps}{\eps} & x \in (x_p, 1],
    \end{cases}\]
    as long as $\frac{1 - \eps}{\eps} > p - 1$.
    
    \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{fig/fig-asymmetric1.png}
        \includegraphics[width=0.45\textwidth]{fig/fig-asymmetric10.png}
        \caption{Plots the asymmetric function with a $p$-cycle referenced in Proposition~\ref{prop:need-symmetry} for $p=3$ and $\eps = 0.1$. While $f$ oscillates frequently, $f$ can be trivially $0.1$-approximated by three ReLUs. As $\eps \to 0$, the $L_\infty$ approximation hardness guarantees implied by \cite{cnpw19} become vacuous because the oscillations, even though they are exponentially many, they shrink in size.}
        \label{fig:asymmetric}
    \end{figure}

    
    We show inductively that for all $k$, there exists $a_k < b_k$ such that $f^k(a_k) = f^k(b_k) = 1 - \eps$, $f^k([a_k, b_k]) \in [1 - \eps, 1]$, and $f^k$ has exactly one linear piece for each of the intervals $[0, a_k]$ and $[b_k, 1]$.
    
    These are true for the base case $k = 1$ for $a_1 \in (0, x_1)$ and $b_1 = x_p$.
    
    If the claim holds for $k$, then there is some $a_{k+1} \in (0, a_k)$ and $b_{k+1}\in (b_k, 1)$ such that $f(a_{k+1}) = f(b_{k+1}) = a_k$.
    Then, $f^{k+1}(a_{k+1}) = f^{k+1}(b_{k+1}) = 1-\eps$ and $f^{k+1}([0, a_{k+1}]) = f^{k+1}([b_{k+1},1]) = [0, 1 - \eps]$.
    For all $x \in [0, a_{k+1}]$, $f^j(x) \leq 1 - \eps$ for all $j \leq k+1$. Hence, $f^{k+1}$ is linear on $[0, a_{k+1}]$ (and also $[b_{k+1}, 1]$.
    Because $f([x_1, x_p]) = [x_1, x_p]$, $f^{k+1}([a_{k+1}, b_{k+1}]) \subseteq [x_1, x_p] \subseteq [1 - \eps, 1]$.
    The claim then holds for $k+1$.
    
    Thus, the piecewise linear mapping $g$ with boundaries $g(0)=0$, $g(a_k) = 1-\eps$, $g(b_k) = 1-\eps$, and $g(1) = 0$ is an $\eps$-approximation of $f$.
    Because $g$ has three pieces and contains the origin, it can be exactly represented by a linear combination of four ReLUs, and hence as a depth-2 neural network of width 3.
\end{proof}

\begin{proposition}\label{prop:need-concavity}
% For sufficiently small $\eps > 0$ and $p \geq 3$, there exists a symmetric unimodal mapping $f$ that is \textit{not concave} such that there exists a 2-layer ReLU network of width 3 such that
% \[\max_{x \in [0,1]} \abs{f(x) - g(x)} \leq \eps.\]
For $p \geq 3$ and for sufficiently small $\eps > 0$, there exists a symmetric unimodal mapping $f$ with a chaotic $p$-cycle such that for any $k$, there exists $g \in \mathcal{N}(3,2)$ with
\[L_\infty(f^k, g) \leq \eps.\]
\end{proposition}
\begin{proof}
    Let $x_j = \frac{1}{2} - \frac{p-1-j}{2(p-1)}\eps$ for all $j \in [p-1]$ and $x_p = \frac{1}{2} + \frac{\eps}{2}$.
    Let $f$ be a piecewise-linear function with boundaries
    \begin{align*}
        f(0) = 0, \
        f\paren{\frac{1}{2} - \frac{\eps}{2}} = \frac{1}{2}-\frac{p-2}{p-1} \cdot \frac{\eps}{2}, \
        f\paren{\frac{1}{2} - \frac{\eps}{2(p-1)}} = \frac{1}{2}, \ f\paren{\frac{1}{2}} = \frac{1}{2} + \frac{\eps}{2}, \\
        f\paren{\frac{1}{2} + \frac{\eps}{2(p-1)}} = \frac{1}{2},  \ 
        f\paren{\frac{1}{2} + \frac{\eps}{2}} = \frac{1}{2}-\frac{p-2}{p-1} \cdot \frac{\eps}{2},\
        f(1) = 0.
    \end{align*}
    
    We visualize $f$ for $p=3$ in Figure~\ref{fig:non-concave}. Note that $f$ is symmetric and unimodal and has an increasing $p$-cycle $x_1 < \dots < x_p$. 
    It is \textit{not} concave because $f'(x) = 1$ for $x \in [x_1, x_{p-2}]$ and $f'(x) = 2(p-1)$ for $x \in [x_{p-2}, x_{p-1}]$.
    
    Using a very similar argument to argument from the proof of Proposition~\ref{prop:need-symmetry}, for all $k$, there exists $a_k < b_k$ such that $f^k$ is linear on $[0, a_k]$ and $[b_k, 1]$ and $f^k([a_k, b_k]) \in [\frac{1}{2} - \eps, \frac{1}{2} + \eps]$.
    As before, there exists a piecewise linear function with three pieces (which can be thought of as a depth-2 neural network of width 3) that $\eps$-approximates $f$.
\end{proof}

==> trash.tex <==
% \section{TRASH}

% %% This is a holding place for anything that we want to axe from the paper before making the cut

% \subsection{Stability}
% It is also occasionally useful to consider the \textit{stability} of a cycle.
% This governs the attractiveness of a cycle.
% A stable cycle will attract nearby iterates, while an unstable cycle repels them.
% Super-stable cycles have exponentially fast rates of convergence.
% shows the connection between these properties and the derivative of the mapping.
% For the definition, we assume that $f$ is differentiable, which can be done by infinitesimally smoothing any maps with discontinuities in slope.

% \begin{definition}
%     A fixed point $x^*$ of $f$ is:
%     \begin{itemize}
%         \item \emph{unstable} if $\abs{\deriv{f(x^*)}{x}} > 1$.
%         \item \emph{stable} if $\abs{\deriv{f(x^*)}{x}} < 1$.
%         \item \emph{super-stable} if $\abs{\deriv{f(x^*)}{x}} = 0$.
%     \end{itemize}
%     A $p$-cycle is said to belong to one of above if the criterion holds for every element of the cycle for $f^p$.
% \end{definition}

% We refer back to a simple correspondence between super-stable cycles and symmetric functions.

% \begin{fact}
%     If $f$ is a symmetric unimodal mapping with a $p$-cycle containing $\frac{1}{2}$, then the cycle is super-stable.
% \end{fact}
% \begin{proof}
%     If we assume that $f$ is symmetric and differentiable everywhere, then $f'(\frac{1}{2}) = 0$.
%     By the chain rule,
%     \[\frac{d}{dx} f^{p}(x) = f'(f^{p-1}(x)) f'(f^{p-2}(x)) \dots f'(f(x)) f'(x).\]
%     Therefore, if the $p$-cycle is $x_1, \dots, x_p$,  WLOG $x_1 = \frac{1}{2}$, then the derivative at any $x_i$ is
%     \[\frac{d}{dx} f^{p}(x_i) = \prod_{j=1}^p f'(x_j) = 0.\qedhere\]
% \end{proof}

% \subsection{Positive Results on Approximation with Deep Neural Networks}

% \begin{proposition}\label{prop:dnn-approx}
%     Suppose $f$ is a continuous piece-wise linear function with $m$ pieces and $f(0)$. For any $k$, $f^k$ can be exactly represented by a ReLU neural network of depth $2k$ and width $m$.
% \end{proposition}
% \begin{proof}
%     $f$ can be exactly represented as a linear combination of $m$ ReLUs, which is a 2-layer neural network of width $m$.
%     Thus, $f^k$ can be represented as the composition of $k$ of those networks, which is of depth $2k.$
% \end{proof}

% \begin{proposition}\label{prop:cycle-chaotic-domination}
%     Suppose $f$ and $g$ are symmetric unimodal functions with $f(x) \geq g(x)$ for all $x \in [0,1]$ and $f(\frac{1}{2}) = g(\frac{1}{2})$.
%     Then, if $f$ has an increasing $p$-cycle, $g$ also has an increasing $(p-1)$-cycle.
% \end{proposition}
% \begin{proof}
%     Let $f$ have the $p$-cycle $x_1 < \dots < x_p$.
%     Because $\frac{1}{2}$ maximizes $f$, it follows that $f(\frac{1}{2}) \geq x_p$ and for any $j \in [p-1]$, $f^{j+1}(\frac{1}{2}) \leq x_j$.
%     Similarly, $g(\frac{1}{2}) = f(\frac{1}{2})$ and $g^{j+1}(\frac{1}{2}) \leq f^{j+1}(\frac{1}{2}) \leq x_j$ by induction.
    
%     It must be the case that $x_{p-2} < \frac{1}{2}$. 
%     If not, then $f(x_{p-2}) =x_{p-1} > f(x_{p-1}) = x_p$, which contradicts $x_p > x_{p-1}$.
%     Thus, $g^{p-1}(\frac{1}{2}) < \frac{1}{2}$, so by Proposition~\ref{prop:half-inc-cycle}, $g$ has an increasing $(p-1)$-cycle.
% \end{proof}

% \begin{remark}
%     By putting Propositions~\ref{prop:dnn-approx} and \ref{prop:cycle-chaotic-domination} together with Theorem~\ref{thm:general-lb-cls}, if there exists some symmetric concave unimodal $f$ with an increasing $p$-cycle for $p \geq 4$, the tent map $\ftent{f(1/2)}$ has an increasing $(p-1)$-cycle.
    
%     Thus, $\ftent{f(1/2)}$ can be exactly represented by a neural network of depth $2k$ and width $2$, but there is no neural network $g$ of depth $\sqrt{k}$ and width $\frac{1}{8}(2 - (2/3)^{p-1})^{\sqrt{k}}$ such that 
%     \[\norm[\infty]{\ftent{f(1/2)}^k - g} < \frac{1}{36}.\]
% \end{remark}

% % The proof relies on several facts about increasing cycles.

% % \begin{lemma}\label{lemma:inc-p-to-inc-p-1}
% %     Suppose for $p \geq 3$ symmetric unimodal mapping $f$ has an increasing $p$-cycle $x_1< \dots < x_p$.
% %     Then, $f$ also has an increasing $(p-1)$-cycle $x_1', \dots, x_{p-1}'$ satisfying
% %     \[x_1 < x_1' < x_2 < x_2' < \dots < x_{p-1} < x_{p-1}' < x_p.\]
% % \end{lemma}
% % \begin{proof}
% %     Because $f$ is continuous, $f^{p-1}(x_1) - x_1 = x_p - x_1 > 0$, and $f^{p-1}(x_2) - x_2 = x_1 - x_2 < 0$, there exists some $x_1' \in (x_1, x_2)$ such that $f^{p-1}(x_1') = 0$.
% %     It remains to show that $x_1'$ cannot be a $p'$ cycle for $p' < p-1$.
    
% %     It must be the case that $x_1 < \dots < x_{p-2} < \frac{1}{2}$.
% %     If not, $f$ would be decreasing on the interval $[x_{p-2}, x_{p-1}]$, which would contradict the fact that $f(x_{p-2}) = x_{p-1} < f(x_{p-1}) = x_p$.
% %     Thus, $f$ is monotonically increasing along $[x_1, x_{p-2}]$, which means that $f$ maps $(x_j, x_{j+1})$ onto $(x_{j+1}, x_{j+2})$ for all $j \in [p-3]$ and $f((x_{p-2}, x_{p-1})) \subset (x_{p-1}, 1)$.
    
% %     As a result, $x_{j+1}' := f^j(x_1') \in (x_{j+1}, x_{j+2})$ for all $j \in [p-3]$ and $x_{p-1} \in (x_{p-1}, 1)$, so the $(p-1)$-cycle $x_1', \dots, x_{p-1}'$ is increasing and does contain duplicates.
% % \end{proof}

% % \begin{lemma}\label{lemma:inc-p-below-half}
% %     Suppose symmetric unimodal mapping $f$ has an increasing $p$-cycle for $p \geq 3$. Then, there exists an increasing $p$-cycle \[x_1' < \dots < x_{p-1}' \leq \frac{1}{2} < x_p'.\]
% % \end{lemma}
% % \begin{proof}
% %     Let $x_1 < \dots < x_p$ be the existing $p$-cycle, and assume that it does not satisfy the desired inequalities.
% %     (Otherwise, the claim is trivial.)
% %     It must be the case that 
% %     \[x_1 < \dots < x_{p-2} < \frac{1}{2} < x_{p-1} < x_p.\]
% %     As discussed in the proof of Lemma~\ref{lemma:inc-p-to-inc-p-1}, having $x_{p-2} \geq \frac{1}{2}$ contradicts $x_{p} > x_{p-1}$.
% %     Having $x_p < \frac{1}{2}$ forces the contradiction $x_1 = f(x_p) > f(x_{p-1}) = x_p$.
    
% %     We consider three cases. Let $g(x) = f^p(x) - x$ and note that $g$ is continuous.
% %     \begin{enumerate}
% %         \item Suppose for some $\eps > 0$, for all $y \in (x_1 -\eps, x_1)$, $g(y) < 0$. Fix some such $y$.
% %         Because $f(0) = 0$ is increasing along $[0, x_1]$, there exists some $y' \in (0, x_1 - \eps)$ with $f^p(y') = x_1 > y'$ and $g(y) > 0$. 
% %         Thus, there exists $x_1' \in (y', y)$ with $g(y) = 0$. Due to a similar argument to the one in the proof of Lemma~\ref{lemma:inc-p-to-inc-p-1}, $x_1'$ must be the first element of a $p$-cycle.
% %     \end{enumerate}
% % \end{proof}

% % \begin{proof}[Proof of Proposition~\ref{prop:cycle-chaotic-domination}]
% %     If $f$ has an increasing $p$-cycle, there exists $1 < x_1 < \dots, x_p < 1$ such that $f(x_j) = x_{j+1}$ and $f(x_p) = x_1$.
% %     Because $\frac{1}{2}$ maximizes $f$, $f(\frac{1}{2}) > x_p$.
% %     Thus, $f^2(\frac{1}{2}) < x_1$ and inductively, $f^{j}(\frac{1}{2}) < x_{j-1}$.
% % \end{proof}
